Tapes as Stochastic Matrices of String Diagrams

Tape diagrams provide a graphical notation for categories equipped with two monoidal products, $\otimes$ and $\oplus$, where $\oplus$ is a biproduct. Recently, they have been generalised to handle Kleisli categories of arbitrary monoidal monads. In this work, we show that for the subdistribution monad, tapes are isomorphic to stochastic matrices of subdistributions of string diagrams. We then exploit this result to provide a complete axiomatisation of probabilistic Boolean circuits.

==> oldsections/sections/CD.tex <==


\section{Motivating Example}\label{sec:running} 
To provide a clearer illustration of our approach, we begin with the Kleisli category \(\Cat{Set}_{\subdistr}\) associated with the monad of finitely supported subdistributions \(\subdistr\) on   \(\Cat{Set}\) (see e.g.,~\cite{hasuo2007generic}).
%
%In order to better illustrate our approach, we commence with Kleisli category \(\Cat{Set}_{\subdistr}\) of the monad of finitely supported subdistributions \(\subdistr\) on \(\Cat{Set}\).
Objects are sets; morphisms \(f \colon X \to Y\) are functions \(X \to \subdistr(Y)\) mapping each \(x \in X\) into a finitely supported subdistribution over $Y$.
  We write \(f(y \mid x)\) for \(f(x)(y)\)  as this number represents the probability that \(f\) returns \(y\) given the input \(x\).
  Identities \(\id{X} \colon X \to \subdistr(X)\) map each element \(x \in X\) to \(\delta_{x}\), the Dirac distribution at \(x\).
  For two functions \(f \colon X \to \subdistr(Y)\) and \(g \colon Y \to \subdistr(Z)\), their composition in \(\Cat{Set}_{\subdistr}\) is obtained by summing on the middle variable: \(f ; g (z \mid x) \defeq \sum_{y \in Y} f(y \mid x) \cdot g(z \mid y)\).

The category \(\Cat{Set}_{\subdistr}\) carries two symmetric monoidal structures: $ (\Cat{Set}_{\subdistr}, \per, \uno)$ and $(\Cat{Set}_{\subdistr}, \piu, \zero)$. The monoidal product $\per$ is defined on objects as the cartesian product of sets, hereafter denoted by $\times$, with unit the singleton $\uno \defeq \{\bullet\}$; $\piu$ is the disjoint union of sets with unit the empty set $\zero \defeq \{\}$. Hereafter we denote the disjoint union of two sets $X$ and $Y$ by $X+Y \defeq \{(x,0) \mid x\in X\} \cup \{(y,1) \mid y \in Y\}$ where $0$ and $1$ are tags used to distinguish the set of provenance. For arrows  \(f \colon X \to Y\) and \(g \colon X' \to Y'\), $f\per g\colon X\times X' \to Y \times Y'$ and $f \piu g \colon X+X' \to Y+Y'$ are defined as
\begin{equation}\label{ex:products}
f \per g(y,y' \mid x,x') \defeq f(y \mid x) \cdot g(y' \mid x') \quad  f\piu g(v \mid u) \defeq \begin{cases} f(y \mid x) & \text{if } u=(x,0) \text{ and } v=(y,0)\\ g(y' \mid x') & \text{if } u=(x',1) \text{ and } v=(y',1) \\ 0 & \text{otherwise} \end{cases}
\end{equation}
for all $x\in X$, $x'\in X'$, $y\in Y$, $y'\in Y'$, $u\in X+X'$ and $v\in Y+Y'$. 
%

Within the two monoidal structures, for all objects $X$, there are arrows particularly relevant for us:
%
%$\copier{X}\colon X \to X \times X$ and $\discharger{X}\colon X\to \uno$ and $\codiag{X} \colon X+X \to X$ and $\cobang{X}\colon \zero \to X$
%
%
\begin{equation}\label{ex:comonoids}
\begin{array}{cccc}
\begin{array}{rcl}
\copier{X} \colon  X & \to & X \times X \\
x & \mapsto & \delta_{(x,x)}
\end{array}
&
\begin{array}{rcl}
\discharger{X}  \colon X & \to & \uno\\
x & \mapsto& \delta_{\bullet}
\end{array}
&
\begin{array}{rcl}
\codiag{X}  \colon  X+X & \to & X\\
(x,i) & \mapsto& \delta_{x}
\end{array}
&
\begin{array}{rcl}
\cobang{X}\colon  \zero &\to& X\\
\text{ }
\end{array}
\end{array}
\end{equation}
Indeed $(\copier{X},\discharger{X})$ provide a \emph{comonoid} for the monoidal category  $ (\Cat{Set}_{\subdistr}, \per, \uno)$, while $(\codiag{X},\cobang{X})$ a \emph{monoid} for $(\Cat{Set}_{\subdistr}, \piu, \zero)$. The following arrows, where $p\in (0,1)$, are also crucial:
\begin{equation}\label{ex:op}
 \Br{+_p}_X \colon X \to X+X \qquad \Br{\star}_X \colon X \to 0\end{equation}
The function $\Br{+_p}_X$ maps each $x\in X$ into the distribution that assigns to $(x,0)$ probability $p$ and to $(x,1)$ probability $1-p$. Instead, $\Br{\star}_X$ is the  function mapping each $x$ into the null subdistribution.



The structures above constitute the fundamental linguistic constructs for the language we are about to introduce. Naturally, they are not arbitrary: 
the structures in~\eqref{ex:products} and~\eqref{ex:comonoids} exist in the Kleisli category of any \emph{symmetric monoidal monad}, while those in~\eqref{ex:op} are specific to the monad \(\subdistr\). However, analogous structures can also be found in monads equipped with an \emph{algebraic presentation} \(\mathbb{T}\).

Before introducing our diagrammatic language in Section~\ref{sec:tapediagrams}, we examine how these structures interact: \(\per, \uno,\copier{},\discharger{}\) define a copy-discard category (Definition~\ref{def:cd}); \(\piu, \zero,\codiag{},\cobang{}\) form a finite coproduct category (Definition~\ref{def:fp}). Together, they constitute what we refer to as a \emph{finite coproduct-copy discard rig category} (Definition~\ref{def: distributive gs-monoidal category}). By further incorporating the arrows provided by the algebraic theory \(\mathbb{T}\), we obtain a \emph{\(\mathbb{T}\)-copy discard rig category} (Definition~\ref{def:Trig cat}).



%The structures illustrated above provide the fundamental linguistic constructs for the language that we are going to introduce. Of course they are not arbitrary: 
%the structures in \eqref{ex:products} and \eqref{ex:comonoids} live in the Kleisli category of any \emph{symmetric monoidal monad}; those in \eqref{ex:op} are specific to the monad \(\subdistr\), but analogous structures can similarly be found in monads equipped with an algebraic presentation $\mathbb{T}$.
%
%Before introducing our diagrammatic language in Section \ref{sec:tapediagrams}, we study how these structure interact:  $\per, \uno,\copier{},\discharger{}$ provide a copy discard category (Definition \ref{def:cd}); $\piu, \zero,\codiag{},\cobang{}$  a finite coproduct category (Definition \ref{def:fp});
% together they form what we named a \emph{finite coproduct-copy discard rig category} (Definition \ref{def: distributive gs-monoidal category}). Then, by adding the arrows provided by the algebraic theory $\mathbb{T}$, one obtains a \emph{$\mathbb{T}$-copy discard rig category} (Definition \ref{def:Trig cat}).
%
%
%
%

\section{Copy Discard and Finite (Co)Product Categories}\label{sec:CD}

Fox's theorem \cite{fox1976coalgebras} characterises categories with finite products as symmetric monoidal categories equipped with coherent comonoids which are natural.
It is convenient to split the definition in two:


%
%Recall that, for an object $X$ of a symmetric monoidal category $(\Cat{C}, \perG, \unoG,\sigma^{\perG} )$, a \emph{cocommutative comonoid} on $X$ consists of 
%two arrows $\copier{X}\colon X \to X \perG X$ and $\discharger{X}  \colon X \to \unoG$ such that the equations in Table \ref{tab:axiomsfc}.\eqref{eq:comonoid} hold. A \emph{commutative monoid} in $\Cat{C}$ is a commutative monoid in  $\Cat{C}^{op}$. Hereafter, we will denote the arrows of a monoid by $\codiag{X}\colon X \perG X \to X $ and $\cobang{X} \colon \unoG  \to X$   and, for the sake of brevity, we will always avoid to specify (co)commutative. % and just write (co)monoids.


\begin{table}
{\small
\begin{equation}\label{eq:comonoid}
\copier{X}; (\copier{X} \perG\ \id{X}); \assoc{X}{X}{X} = \mathord{\copier{X}} ; (\id{X}\ \perG \copier{X})\quad
\copier{X}; (\discharger{X} \perG \id{X}) ; \lunit{X} = \id{X} = \mathord{\copier{X}} ; (\id{X} \perG \discharger{X}); \runit{X} \quad
\copier{X}; \sigma_{X,X}^\perG = \mathord{\copier{X}}
\end{equation}
%\hline
\vspace{-0.5cm}
\begin{equation}\label{eq:comonoidcoherence}
\begin{array}{c}\mathord{\copier{X\perG Y}} = (\copier{X}\perG\copier{Y}) ; \assoc{X}{X}{Y\perG Y} ; (\id{X} \perG \assoc{X}{Y}{Y}^-) ; ( \id{X} \perG (\sigma^{\perG}_{X,Y} \perG\id{Y})) ; (\id{X} \perG \assoc{Y}{X}{Y}) ; \assoc{X}{Y}{X\perG Y}^- \\
\discharger{X\perG Y} = \discharger{X} \perG \discharger{Y} ; \lunit{\unoG} \qquad 
\mathord{\copier{\unoG}} = \lunit{\unoG}^- \qquad
\discharger{\unoG} = \id{\unoG}
\end{array}
\end{equation}
%\hline
\vspace{-0.5cm}
\begin{equation}\label{eq:naturality}
f; \mathord{\copier{Y}} = \mathord{\copier{X}}; (f \perG f) \qquad f;\discharger{Y} = \discharger{X} \qquad \qquad \text{for all }f\colon X \to Y
\end{equation}
}
\caption{Axioms of finite product categories. %: \eqref{eq:comonoid} are the axioms of comonoids; \eqref{eq:comonoidcoherence} of coherence axioms \eqref{eq:naturality} those of naturality and . %The arrow $\assoc{X}{Y}{Z}\colon (X \perG Y) \perG Z \to X\perG (Y \perG Z)$, $\lunit{X}\colon \unoG \perG X \to X$ and $\runit{X} \colon X \perG \unoG \to X$ are the usual structural isomorphisms of monoidal categories. 
See also Figure~\ref{fig:comonoidax} and~\ref{fig:fpcoherence} in Appendix~\ref{app:coherence axioms}.}\label{tab:axiomsfc}
\end{table}

\begin{definition}\label{def:cd}
A \emph{copy discard} (cd, for short) \emph{category} is a symmetric monoidal category $(\Cat C, \perG, \unoG)$ and, for all objects $X$, two arrows $\copier{X}\colon X \to X \perG X$ and $\discharger{X}  \colon X \to \unoG$ such that
\begin{itemize}
\item $\copier{X}$ and $\discharger{X}$ form a comonoid, i.e., the laws in Table~\ref{tab:axiomsfc}.\eqref{eq:comonoid} hold;
\item $\copier{X}$ and $\discharger{X}$ satisfy the coherence axioms in Table~\ref{tab:axiomsfc}.\eqref{eq:comonoidcoherence}.
\end{itemize}
A \emph{morphism of cd categories} is a strong symmetric monoidal functor preserving comonoids.
\end{definition}

\begin{definition}\label{def:fp}
A \emph{finite product} (fp, for short) \emph{category} is a copy discard category such that
\begin{itemize}
\item $\copier{}$ and $\discharger{}$  are natural transformations, i.e., for all $f\colon X \to Y$ in $\Cat{C}$ the laws in Table~\ref{tab:axiomsfc}.\eqref{eq:naturality} hold;
\end{itemize}
A \emph{finite coproduct} (fc) \emph{category} is a symmetric monoidal category with natural and coherent monoids $(\codiag{},\cobang{})$, i.e., $\Cat C$ is a finite coproduct category iff $\Cat{C}^{op}$ is a fp category. A morphism of (fp)fc categories is a strong symmetric monoidal functor preserving (co)monoids.
\end{definition}
%
Definition~\ref{def:fp} is equivalent to require the existence of categorical (co)products and (initial) final objects but, differently from the usual definition, it does not rely on universal properties (see Remark~\ref{rem:productcomonoids} in App.~\ref{ssec:fbcat} for more details). 
Moreover, since any monoidal category is equivalent to a \emph{strict} one~\cite{mac_lane_categories_1978}, namely a monoidal category where the structural isomorphism $\assoc{X}{Y}{Z}\colon (X \perG Y) \perG Z \to X\perG (Y \perG Z)$, $\lunit{X}\colon \unoG \perG X \to X$ and $\runit{X} \colon X \perG \unoG \to X$ are identities, the laws in Table~\ref{tab:axiomsfc} can remarkably simplified. In particular, they acquire an intuitive geometrical meaning when drawn as \emph{string diagrams}, formally arrows of a freely generated strict symmetric monoidal category (see App.~\ref{sec:monoidal}).
By depicting, $\copier{X}$ as $\comonoid{X}$, $\discharger{X}$ as $\counit{X}$ and an arbitrary arrow $f\colon X \to Y$ as $\boxTypedCirc{f}{X}{Y}$, the laws in Table~\ref{tab:axiomsfc} appear as follows.
  \[
  \!\!\!\!\begin{array}{c @{} c@{}c@{}c}
  \begin{array}{c@{}c@{}c @{\quad} c@{}c@{}c @{\quad} c@{}c@{}c}
    \tikzfig{fbAx/comonoid/assoc/lhs} & = & \tikzfig{fbAx/comonoid/assoc/rhs}
    &
    \tikzfig{fbAx/comonoid/unit/lhs} & = & \tikzfig{fbAx/comonoid/unit/rhs}
    &
    \tikzfig{fbAx/comonoid/comm/lhs} &=  & \tikzfig{fbAx/comonoid/comm/rhs}
  \end{array}
  &
  \tikzfig{fbAx/comonoid/nat/copy/lhs} &=& \tikzfig{fbAx/comonoid/nat/copy/rhs}
  \\
  \begin{array}{c@{\quad}c@{\quad}c@{\quad}c}
    \CBcopier[][I] = \tikzfig{empty} & \tikzfig{fbAx/coherence/copierLhs} = \tikzfig{fbAx/coherence/copierRhs} & \CBdischarger[][I] = \tikzfig{empty} & \tikzfig{fbAx/coherence/dischargerLhs} = \tikzfig{fbAx/coherence/dischargerRhs}
  \end{array}
  &
  \tikzfig{fbAx/comonoid/nat/discard/lhs} &=& \tikzfig{fbAx/comonoid/nat/discard/rhs}
  \end{array}
  \]



%In our work we will be particularly interested in the \emph{Kleisli category} of a monad $T\colon\Cat{C}\to \Cat{C}$, hereafter denoted by $\Cat{C}_T$. It is well known that, whenever $\Cat{C}$ is a fc category, then $\Cat{C}_T$ is also fc \cite{borceux2}. Instead if $\Cat{C}$ is a fp category, then $\Cat{C}_T$ is \emph{not} necessarily fp, actually not even monoidal. %, unless $T$ is a symmetric monoidal monad.

The archetypical examples of finite product and finite coproduct category are  \((\Cat{Set}, \times, \uno)\) and  \((\Cat{Set}, +, 0)\):  \emph{copy} $\copier{X} \colon X \to X \times X$ is  $\langle \id{X},\id{X}\rangle$;  the \emph{discard} $\discharger{X}\colon X \to \uno$ is the unique function into $\uno$; $\codiag{X}\colon X+X \to X$ is $[\id{X},\id{X}]$ and $\cobang{X}\colon \zero \to X$ is the unique function from $\zero$.  

As anticipated in Section~\ref{sec:running}, also $(\Cat{Set}_{\subdistr}, \piu, \zero)$ is a finite coproduct category. More generally, the \emph{Kleisli category} of a monad $T\colon\Cat{C}\to \Cat{C}$, hereafter denoted by $\Cat{C}_T$, is a fc category whenever $\Cat{C}$ is fc~\cite{borceux2}.  Instead if $\Cat{C}$ is a fp category, then $\Cat{C}_T$ is \emph{not} necessarily fp, actually not even monoidal. %, unless $T$ is a symmetric monoidal monad.

\begin{definition}
Let $(\Cat{C},\perG,\unoG)$ be a symmetric monoidal category. A symmetric monoidal monad  consists of a monad \((T, \eta, \mu)\) over $\Cat{C}$ and a natural transformation \(m_{X,Y} \colon T(X) \perG T(Y) \to T(X \perG Y)\) satisfying the expected laws (see Figure~\ref{fig:monoidalmonads} and also \cite{eilenberg1966closed,kock1972strong,kock1970monads}). 
\end{definition}
\begin{example}\label{ex:monoidal monads}
Any monad on  \((\Cat{Set}, +, 0)\) and, more generally, any monad on a fc category is symmetric monoidal: take $m_{X,Y}=[T(\iota_X),T(\iota_Y)]$. 
Instead, not all monads on \((\Cat{Set}, \times, \uno)\)  are symmetric monoidal: for instance, the monad of convex sets of (sub)distributions (see e.g.~\cite{jacobs2008coalgebraic,goy2020combining}), combining probabilistic and non-deterministic choice. The monad \(\subdistr\) is symmetric monoidal~\cite{jacobs2018probability}: $m_{X,Y}$ is defined for all $d_X\in \subdistr(X)$, $d_Y\in \subdistr(Y)$, $x\in X$ and $y\in Y$ as  $m_{X,Y}(d_X,d_Y)(x,y)=d_X(x)\cdot d_Y(y)$.
%  Objects in its Kleisli category, \(\Cat{Set}_{\subdistr}\), are sets; morphisms \(f \colon X \to Y\) are functions \(X \to \subdistr(Y)\) that associate to each \(x \in X\) and each \(y \in Y\) a number \(f(x)(y) \in [0,1]\).
%  We write \(f(y \mid x)\) for this number as it represents the probability that \(f\) returns \(y\) given the input \(x\).
%  Identities \(\id{X} \colon X \to \subdistr(X)\) map each element \(x \in X\) to \(\delta_{x}\), the Dirac distribution at \(x\).
%  For two functions \(f \colon X \to \subdistr(Y)\) and \(g \colon Y \to \subdistr(Z)\), their composition in \(\Cat{Set}_{\subdistr}\) is obtained by summing on the middle variable: \(f ; g (z \mid x) = \sum_{y \in Y} f(y \mid x) \cdot g(z \mid y)\).
%
\end{example}
When $T$ is a symmetric monoidal monad, then one can define a monoidal product $\perG_T$ on $\Cat{C}_T$: on objects, $\perG_T$ is defined as $\perG$ in $\Cat{C}$; 
for arrows $f\colon X_1 \to X_2$, $g\colon Y_1 \to Y_2$ in $\Cat{C}_T$, $f\perG_T g \defeq (f\perG g) ; m_{X_2,Y_2}$.
%
Moreover, if $\Cat{C}$ has coherent monoids or comonoids, then for all objects $X$, one can define
\begin{equation}\label{eq:copierflat}
\copier{X}^\flat \defeq  \copier{X} ;\eta_{X\perG X} \qquad \discharger{X}^\flat \defeq \discharger{X} ; \eta_{\unoG} \qquad \text{ and } \qquad   \codiag{X}^\flat \defeq  \codiag{X} ;\eta_{X} \qquad  \cobang{X}^\flat \defeq \cobang{X} ; \eta_{X}\text{,}
\end{equation}
forming coherent (co)monoids in $\Cat{C}_T$. If $\Cat{C}$ is fc, then the above monoids are natural in $\Cat{C}_T$. Instead, if $\Cat{C}$ is fp, then the comonoids are \emph{not} necessarily natural. In other words, $\Cat{C}_{T}$ may not have finite products, but it is always a \emph{copy-discard} category (Definition~\ref{def:cd}).

\begin{proposition}[From \cite{cioffogadduccitrotta}]\label{prop: Kleisli gs e cogs}
  %\elena{I feel like this is a known result. It is at least in~\cite[Proposition 3.1]{fritz_2020}.}
  Let $T\colon \Cat{C}\to \Cat{C}$ be a symmetric monoidal monad on a cd category $(\Cat{C},\perG,\unoG, \copier{}, \discharger{})$.
  Then the Kleisli category $(\Cat{C}_T, \perG_T, \unoG, \copier{}^\flat, \discharger{}^\flat)$ is a cd category. % with
   %  $\copier{X}$ and $\discharger{X}$ given for every object $X$ by 
 %   \[\copier{X}^\flat:=(\eta_{X\per X}) \circ \copier{X},\qquad \discharger{X}^\flat:=\eta_I \circ \discharger{X}.\]
    %Similarly, if $\Cat{C}$ is a cogs-monoidal category, then the Kleisli category $\Cat{C}_T$ is a cogs-monoidal category with
    %\[\codiag{X}^\flat:=(\eta_{X}) \circ \codiag{X},\qquad \bang{X}^\flat:=\eta_X \circ \bang{X}.\]
%     \qed
\end{proposition}
%The above proposition justifies our interest in copy discard categories.

In a cd category $(\Cat{C},\perG,\unoG,\copier{},\discharger{})$, an arrow $f\colon X\to Y$ is called \emph{deterministic} if $f;\copier{Y}= \copier{X};(f\perG f)$ and \emph{total} if
$f;\discharger{Y}= \discharger{X}$. The category of total deterministic morphisms is denoted by $\mathrm{Map}(\Cat{C})$ and it is a finite product category.

Since  \((\Cat{Set}, \times, \uno)\) is a finite product category and \(\subdistr\) is a symmetric monoidal monad on  \((\Cat{Set}, \times, \uno)\) (Example~\ref{ex:monoidal monads}) then, by Proposition~\ref{prop: Kleisli gs e cogs}, the Kleisli category $\Cat{Set}_{\subdistr}$ is a copy discard category: monoidal product and comonoids are exactly those defined in \eqref{ex:products} and \eqref{ex:comonoids}. In $\Cat{Set}_{\subdistr}$, deterministic and total morphisms are simply functions.
%deterministic morphisms are partial functions; total morphisms correspond to total stochastic channels. \marginpar{Maybe total stoichatic channel is not too clear?}






\begin{comment}
%
%
%
%
%
%
%
%
%
\section{From finite product to copy discard categories}\label{sec:CD}

Fox's theorem \cite{fox1976coalgebras} characterises finite product categories as symmetric monoidal categories equipped with natural comonoids.
%
Recall that, for an object $X$ of a symmetric monoidal category $(\Cat{C}, \perG, \unoG,\sigma^{\perG} )$, a \emph{cocommutative comonoid} on $X$ consists of 
two arrows $\copier{X}\colon X \to X \perG X$ and $\discharger{X}  \colon X \to \unoG$ such that the equations in Table \ref{tab:axiomsfc}.\eqref{eq:comonoid} hold. A \emph{commutative monoid} in $\Cat{C}$ is a commutative monoid in  $\Cat{C}^{op}$. Hereafter, we will denote the arrows of a monoid by $\codiag{X}\colon X \perG X \to X $ and $\cobang{X} \colon \unoG  \to X$   and, for the sake of brevity, we will always avoid to specify (co)commutative. % and just write (co)monoids.


\begin{table}
{\small
\begin{equation}\label{eq:comonoid}
\copier{X}; (\copier{X} \perG \id{X}); \assoc{X}{X}{X} = \copier{X} ; (\id{X} \perG \copier{X})\quad
\copier{X}; (\discharger{X} \perG \id{X}) ; \lunit{X} = \id{X} = \copier{X} ; (\id{X} \perG \discharger{X}); \runit{X} \quad
\copier{X}; \sigma_{X,X}^\perG = \copier{X}
\end{equation}
%\hline
\begin{equation}\label{eq:naturality}
f; \copier{Y} = \copier{X}; (f \perG f) \qquad f;\discharger{Y} = \discharger{X} \qquad \qquad \text{for all }f\colon X \to Y
\end{equation}
%\hline
\begin{equation}\label{eq:comonoidcoherence}
\begin{array}{c}\copier{X\perG Y} = (\copier{X}\perG\copier{Y}) ; \assoc{X}{X}{Y\perG Y} ; (\id{X} \perG \assoc{X}{Y}{Y}^-) ; ( \id{X} \perG (\sigma^{\perG}_{X,Y} \perG\id{Y})) ; (\id{X} \perG \assoc{Y}{X}{Y}) ; \assoc{X}{Y}{X\perG Y}^- \\
\discharger{X\perG Y} = \discharger{X} \perG \discharger{Y} ; \lunit{\unoG} \qquad 
\copier{\unoG} = \lunit{\unoG}^- \qquad
\discharger{\unoG} = \id{\unoG}
\end{array}
\end{equation}
}
\caption{Axioms of finite product categories: \eqref{eq:comonoid} are the axioms of comonoids; \eqref{eq:naturality} those of naturality and \eqref{eq:comonoidcoherence}. The arrow $\assoc{X}{Y}{Z}\colon (X \perG Y) \perG Z \to X\perG (Y \perG Z)$, $\lunit{X}\colon \unoG \perG X \to X$ and $\runit{X} \colon X \perG \unoG \to X$ are the usual structural isomorphisms of monoidal categories. See also Figure~\ref{fig:comonoidax} in Appendix \ref{}.}\label{tab:axiomsfc}
\end{table}

\begin{definition}\label{def:fp}
A \emph{finite product} (fp, for short) \emph{category} is a symmetric monoidal category $(\Cat C, \perG, \unoG, \sigma^\perG)$ and, for all objects $X$, two arrows $\copier{X}\colon X \to X \perG X$ and $\discharger{X}  \colon X \to \unoG$ such that
\begin{itemize}
\item $(\copier{X},\discharger{X})$ is a comonoid, i.e., the laws in Table \ref{tab:axiomsfc}.\eqref{eq:comonoid} hold;
\item $\copier{}$ and $\discharger{}$  are natural, i.e., for all $f\colon X \to Y$ in $\Cat{C}$ the laws in \eqref{eq:naturality} hold;
\item $\copier{}$ and $\discharger{}$ satisfy the coherence axioms in \eqref{eq:comonoidcoherence}.
\end{itemize}
A \emph{finite coproduct} (fc) \emph{category} is a symmetric monoidal category with natural and coherent monoids $(\codiag{},\cobang{})$, i.e., $\Cat C$ is a finite coproduct category iff $\Cat{C}^{op}$ is a fp category. A morphism of (fp)fc categories is a strong symmetric monoidal functor preserving (co)monoids.
\end{definition}
%
The above definition requires the existence of categorical (co)products but, differently from the usual definitions, it does not rely on universal properties (see Remark \ref{rem:productcomonoids} in App. \ref{ssec:fbcat} for all details). 
Moreover, since any monoidal category is equivalent to a \emph{strict} one \cite{mac_lane_categories_1978}, namely a monoidal category where the structural isomorphism $\assoc{X}{Y}{Z}\colon (X \perG Y) \perG Z \to X\perG (Y \perG Z)$, $\lunit{X}\colon \unoG \perG X \to X$ and $\runit{X} \colon X \perG \unoG \to X$ are identities, the laws in Table \ref{tab:axiomsfc} can remarkably simplified. In particular, they acquire an intuitive geometrical meaning when drawn as \emph{string diagrams} \cite{}, formally arrows of a freely generated strict symmetric monoidal category (see Appendix \ref{sec:monoidal}).
By depicting, $\copier{X}$ as $\comonoid{X}$, $\discharger{X}$ as $\counit{X}$ and an arbitrary arrow $f\colon X \to Y$ as $\boxTypedCirc{f}{X}{Y}$, the laws in Table \ref{tab:axiomsfc} appears as follows.
  \[
  \!\!\!\!\begin{array}{c @{} c@{}c@{}c}
  \begin{array}{c@{}c@{}c @{\quad} c@{}c@{}c @{\quad} c@{}c@{}c}
    \tikzfig{fbAx/comonoid/assoc/lhs} & = & \tikzfig{fbAx/comonoid/assoc/rhs}
    &
    \tikzfig{fbAx/comonoid/unit/lhs} & = & \tikzfig{fbAx/comonoid/unit/rhs}
    &
    \tikzfig{fbAx/comonoid/comm/lhs} &=  & \tikzfig{fbAx/comonoid/comm/rhs}
  \end{array}
  &
  \tikzfig{fbAx/comonoid/nat/copy/lhs} &=& \tikzfig{fbAx/comonoid/nat/copy/rhs}
  \\
  \begin{array}{c@{\quad}c@{\quad}c@{\quad}c}
    \CBcopier[][I] = \tikzfig{empty} & \tikzfig{fbAx/coherence/copierLhs} = \tikzfig{fbAx/coherence/copierRhs} & \CBdischarger[][I] = \tikzfig{empty} & \tikzfig{fbAx/coherence/dischargerLhs} = \tikzfig{fbAx/coherence/dischargerRhs}
  \end{array}
  &
  \tikzfig{fbAx/comonoid/nat/discard/lhs} &=& \tikzfig{fbAx/comonoid/nat/discard/rhs}
  \end{array}
  \]

In our work we will be particularly interested in the \emph{Kleisli category} of a monad $T\colon\Cat{C}\to \Cat{C}$, hereafter denoted by $\Cat{C}_T$. It is well known that, whenever $\Cat{C}$ is a fc category, then $\Cat{C}_T$ is also fc \cite{borceux2}. Instead if $\Cat{C}$ is a fp category, then $\Cat{C}_T$ is \emph{not} necessarily fp, actually not even monoidal. %, unless $T$ is a symmetric monoidal monad.



\begin{definition}
Let $(\Cat{C},\perG,\unoG)$ be a symmetric monoidal category. A symmetric monoidal monad  consists of a monad \((T, \eta, \mu)\) over $\Cat{C}$ and a natural transformation \(m_{X,Y} \colon T(X) \perG T(Y) \to T(X \perG Y)\) satisfying the expected laws (see Figure \ref{fig:monoidalmonads} and also \cite{eilenberg1966closed,kock1972strong,kock1970monads}). 
\end{definition}










\begin{example}
  The monad of finitely supported subdistributions \(\subdistr\) on \(\Cat{Set}\) is a symmetric monoidal monad~\cite{}.
  Objects in its Kleisli category, \(\Cat{Set}_{\subdistr}\), are sets; morphisms \(f \colon X \to Y\) are functions \(X \to \subdistr(Y)\) that associate to each \(x \in X\) and each \(y \in Y\) a number \(f(x)(y) \in [0,1]\).
  We write \(f(y \mid x)\) for this number as it represents the probability that \(f\) returns \(y\) given the input \(x\).
  Identities \(\id{X} \colon X \to \subdistr(X)\) map each element \(x \in X\) to \(\delta_{x}\), the Dirac distribution at \(x\).
  For two functions \(f \colon X \to \subdistr(Y)\) and \(g \colon Y \to \subdistr(Z)\), their composition in \(\Cat{Set}_{\subdistr}\) is obtained by summing on the middle variable: \(f \mathbin{;} g (z \mid x) = \sum_{y \in Y} f(y \mid x) \cdot g(z \mid y)\).

  On the other hand, the monad of convex sets of (sub)distributions, combining probabilistic and non-deterministic choice, is not symmetric monoidal~\cite{}.
\end{example}

When $T$ is symmetric monoidal monads, then one can define a monoidal product on $\Cat{C}_T$ as
\[f\perG_T g \defeq (f\perG g) ; m_{X_2,Y_2} ,\]
for all arrows $f\colon X_1 \to X_2$, $g\colon Y_1 \to Y_2$ in $\Cat{C}_T$.
Moreover, if $\Cat{C}$ is fp, then for all objects $X$, one can define
\begin{equation}\label{eq:copierflat}
  \copier{X}^\flat \defeq  \copier{X} ;\eta_{X\per X} \qquad \text{ and }\qquad \discharger{X}^\flat \defeq \discharger{X} ; \eta_{\unoG}\text{,}
\end{equation}
\elena{have we defined \(\flat\)? Can we use small string diagrams instead of new symbols for copy and discard in the text?}
forming a comonoid. It turns out that comonoids are coherent (Table \eqref{eq:comonoidcoherence}) but, in general, \emph{not} natural. In other words, $\Cat{C}_{T}$ may not have finite products, but it always is a \emph{copy-discard} category.
\elena{Personally, I don't like using acronyms like fp or cd unless strictly necessary. I think they hinder readability more than helping it.}
%Another important consequence of the above definition is that one can relax its constraints, e.g., naturality, and obtains some useful categorical structures.
\begin{definition}\label{def:cd}
A \emph{copy-discard} (cd, for short) \emph{category} is a symmetric monoidal category $(\Cat C, \perG, \unoG, \sigma^\perG)$ and, for all objects $X$, two arrows $\copier{X}\colon X \to X \perG X$ and $\discharger{X}  \colon X \to \unoG$ forming coherent commutative comonoids, namely the laws in  Table \ref{tab:axiomsfc}.\eqref{eq:comonoid} and \eqref{eq:comonoidcoherence} hold.
A \emph{morphism of cd categories} is a strong symmetric monoidal functor preserving comonoids.
\end{definition}


\begin{proposition}[From \cite{cioffogadduccitrotta}]\label{prop: Kleisli gs e cogs}
  Let $T\colon \Cat{C}\to \Cat{C}$ be a symmetric monoidal monad on a cd category $(\Cat{C},\perG,\unoG, \copier{}, \discharger{})$.
  Then the Kleisli category $(\Cat{C}_T, \perG_T, \unoG, \copier{}^\flat and \discharger{}^\flat)$ is a cd category. % with
   %  $\copier{X}$ and $\discharger{X}$ given for every object $X$ by 
 %   \[\copier{X}^\flat:=(\eta_{X\per X}) \circ \copier{X},\qquad \discharger{X}^\flat:=\eta_I \circ \discharger{X}.\]
    %Similarly, if $\Cat{C}$ is a cogs-monoidal category, then the Kleisli category $\Cat{C}_T$ is a cogs-monoidal category with
    %\[\codiag{X}^\flat:=(\eta_{X}) \circ \codiag{X},\qquad \bang{X}^\flat:=\eta_X \circ \bang{X}.\]
%     \qed
\end{proposition}

In a cd category $(\Cat{C},\perG,\unoG,\symmt,\copier{},\discharger{})$ an arrow $f\colon X\to Y$ is called \emph{deterministic} and \emph{total} if respectively:
$f;\copier{Y}= \copier{X};(f\per f)$ { and } $f;\discharger{Y}= \discharger{X}$.
The category of total deterministic morphisms is denoted by $\mathrm{Map}(\Cat{C})$ and it is cartesian monoidal.

Morphisms whose codomain is the monoidal unit are sometimes called \emph{predicates}.
These morphisms in the category of partial functions and in the category of relations are precisely classical predicates: a partial function (or a relation) \(p \colon A \to I\) determines a subset \(A_{p}\) of \(A\) in which the predicate holds, i.e.\ \(\forall a \in A_{p} p(a) = \ast\).
In the Kleisli category of the finitary subdistributions monad, morphisms to the monoidal unit correspond to \emph{fuzzy predicates}.

\begin{example}
  Consider \(\Cat{Set}_{\subdistr}\), the Kleisli category of the finitely supported subdistributions monad on \(\Cat{Set}\).
  Since the monad \(\subdistr\) is symmetric monoidal, its Kleisli category is also symmetric monoidal.
  The monoidal product on objects is the cartesian product of sets: \(X \per Y = X \times Y\); the monoidal product of morphisms \(f \colon X \to Y\) and \(g \colon X' \to Y'\) executes them independently: \((f \per g)(y,y' \mid x,x') = f(y \mid x) \cdot g(y' \mid x')\).
  Since \(\Cat{Set}\) is cartesian, \(\Cat{Set}_{\subdistr}\) inherits the copy-discard structure.
  Deterministic morphisms in \(\Cat{Set}_{\subdistr}\) correspond to partial functions; total morphisms correspond to total stochastic channels.
  Morphisms \(p \colon X \to I\) correspond to fuzzy predicates: they map each \(x \in X\) to a number \(p(x) \in [0,1]\) representing the probability that the predicate \(p\) holds for \(x\).
\end{example}

A monad \(T \colon \Cat{C} \to \Cat{C}\) on a category \(\Cat{C}\) with coproducts is always symmetric monoidal with respect to the coproduct.
This means that the coproducts in \(\Cat{C}\) define a symmetric monoidal product in the Kleisli category \(\Cat{C}_{T}\), which is, moreover, always a coproduct.

\begin{example}
  In the Kleisli category of the finitely supported subdistributions monad, \(\Cat{Set}_{\subdistr}\), coproducts are lifted from \(\Cat{Set}\).
  The coproduct of two objects is their disjoint union as sets.
  For two morphisms \(f \colon X \to Y\) and \(g \colon X' \to Y'\), their coproduct is
  \[(f+g)(y \mid x) = \begin{cases} f(y \mid x) & \text{if } x \in X \text{ and } y \in Y\\ g(y \mid x) & \text{if } x \in X' \text{ and } y \in Y'\\ 0 & \text{otherwise} \end{cases}.\]
\end{example}
\end{comment}


==> oldsections/sections/cb.tex <==
\section{Kleene-Cartesian Tape Diagrams}\label{sec:cb}\marginpar{Qua bisogna togliere un po' di roba}

\begin{figure}[ht!]
    \mylabel{ax:symmtinv}{$\sigma^{\per}$-inv}
    \mylabel{ax:symmtnat}{$\sigma^{\per}$-nat}
    \mylabel{ax:copieras}{$\copier{}$-as}
    \mylabel{ax:copierun}{$\copier{}$-un}
    \mylabel{ax:copierco}{$\copier{}$-co}
    \mylabel{ax:cocopieras}{$\cocopier{}$-as}
    \mylabel{ax:cocopierun}{$\cocopier{}$-un}
    \mylabel{ax:cocopierco}{$\cocopier{}$-co}
    \mylabel{ax:specfrob}{S}
    \mylabel{ax:frob}{F}
    \mylabel{ax:copiernat}{$\copier{}$-nat}
    \mylabel{ax:dischargernat}{$\discharger{}$-nat}
    \mylabel{ax:dischargeradj1}{$\codischarger{}\discharger{}$}
    \mylabel{ax:dischargeradj2}{$\discharger{}\codischarger{}$}
    \mylabel{ax:copieradj1}{$\cocopier{}\copier{}$}
    \mylabel{ax:copieradj2}{$\copier{}\cocopier{}$}
    % \scalebox{0.9}{
	\centering
	\begin{tabular}{c@{}c@{}c @{\qquad} c@{}c@{}c}
		% \tikzfig{cb/symm_inv_left} & $\axeq{\sigma^{\per}\text{-inv}}$ & \tikzfig{cb/symm_inv_right} & \tikzfig{cb/symm_nat_left} & $\axeq{\sigma^{\per}\text{-nat}}$ & \tikzfig{cb/symm_nat_right} \\
        % \hline
        \tikzfig{cb/monoid_assoc_left} & $\axeq{\copier{}\text{-as}}$ & \tikzfig{cb/monoid_assoc_right} & \tikzfig{cb/comonoid_assoc_left} & $\axeq{\cocopier{}\text{-as}}$ & \tikzfig{cb/comonoid_assoc_right} \\
        \tikzfig{cb/monoid_unit_left} & $\axeq{\copier{}\text{-un}}$ & \tikzfig{cb/monoid_unit_right} & \tikzfig{cb/comonoid_unit_left} & $\axeq{\cocopier{}\text{-un}}$ & \tikzfig{cb/comonoid_unit_right} \\
        \tikzfig{cb/monoid_comm_left} & $\axeq{\copier{}\text{-co}}$ & \tikzfig{cb/monoid_comm_right} & \tikzfig{cb/comonoid_comm_left} & $\axeq{\cocopier{}\text{-co}}$ & \tikzfig{cb/comonoid_comm_right} \\
        \hline
        \tikzfig{cb/spec_frob_left} & $\axeq{S}$ & \tikzfig{cb/monoid_unit_right} & \tikzfig{cb/frob_left} & $\axeq{F}$ & \tikzfig{cb/frob_center} \\
        \hline
        \tikzfig{cb/copier_nat_left} & $\axsubeq{\copier{}\text{-nat}}$ & \tikzfig{cb/copier_nat_right} & \tikzfig{cb/discharger_nat_left} & $\axsubeq{\discharger{}\text{-nat}}$ & \tikzfig{cb/discharger_nat_right} \\
        \hline
        \tikzfig{cb/adjoint1_bangs_left} & $\axsubeq{\codischarger{}\discharger{}}$ & \tikzfig{cb/empty} & \tikzfig{cb/monoid_unit_right} & $\axsubeq{\discharger{}\codischarger{}}$ & \tikzfig{cb/adjoint2_bangs_right}\\
        \tikzfig{cb/frob_center} & $\axsubeq{\cocopier{}\copier{}}$ & \tikzfig{cb/adjoint1_diags_right} & \tikzfig{cb/monoid_unit_right} & $\axsubeq{\copier{}\cocopier{}}$ & \tikzfig{cb/spec_frob_left}
	\end{tabular}
    % }
    \caption{Axioms of cartesian bicategories}
    \label{fig:cb axioms}
\end{figure}


In Section \ref{sec:rigcategories}  we recalled from \cite{bonchi2023deconstructing} tape diagrams for rig categories with finite biproducts.
In Section \ref{sec:tapes}, we extended tape diagrams with uniform trace and then, in Section \ref{sec:kleene-tapes}, we imposed to such diagrams the laws of Kleene bicategories.
In this section we illustrate our last step: we illustrate tape diagrams for rig categories where $(\Cat{C}, \piu, \zero)$ is a Kleene bicategory and $(\Cat{C}, \per, \uno)$ is a cartesian bicategory.
More precisely, we are interested in the following structures.

\begin{definition}\label{def:kcbrig}
A \emph{Kleene-Cartesian rig category} (shortly, kc rig) is a poset enriched rig category $\Cat{C}$ such that 
\begin{enumerate}
\item $(\Cat{C}, \piu, \zero)$ is a Kleene bicategory;
\item $(\Cat{C}, \per, \uno)$ is a cartesian bicategory;
\item the (co)monoids of both  $(\Cat{C}, \piu, \zero)$ and $(\Cat{C}, \per, \uno)$ satisfy the following coherence conditions. %\marginpar{Insert Reference}
\end{enumerate}
    \begin{equation}\label{eq:fbcbcoherence}
        \begin{array}{rcl C{0.5cm} rcl}
            \copier{X \piu Y} &=& (\Tcopier{X} \piu  \copier{Y}) ; (\id{XX} \piu \cobang{XY} \piu \cobang{YX} \piu \id{YY}) ; (\Idl{X}{X}{Y} \piu \Idl{Y}{X}{Y}) && \discharger{X \piu Y} &=& (\Tdischarger{X} \piu \discharger{Y}) ; \codiag{\uno} \\
            \cocopier{X \piu Y} &=& (\Tcocopier{X} \piu  \cocopier{Y}) ; (\id{XX} \piu \bang{XY} \piu \bang{YX} \piu \id{YY}) ; (\dl{X}{X}{Y} \piu \dl{Y}{X}{Y}) && \codischarger{X \piu Y} &=& \diag{\uno} ; (\Tcodischarger{X} \piu \codischarger{Y})
        \end{array}
\end{equation}

A \emph{morphism of Kleene-Cartesian rig-categories} is a poset enriched rig functor that is a morphism of both Kleene and cartesian bicategories.
\end{definition}
We have already seen in Section~\ref{sec:2monREL} that $(\Rel,\piu, \zero)$ is an Kleene bicategory and $(\Rel,\per, \uno)$ is a cartesian bicategory. To conclude that $\Rel$ is a kc rig category, it is enough to check the coherence conditions: this is trivial by using the definitions of the two (co)monoids of $\Rel$ in~\eqref{eq:comonoidsREL}.

%\begin{remark}\label{rmk:relsem}
%By exploiting the structure of fb-cb category, one can express finite unions and intersections in $\Rel$. The reader can easily check that for all relations $R,S\colon X \to Y$, it holds that
%\[R\cup S = \diag{X} ; (R \piu S); \codiag{Y} \qquad \{\} = \bang{X}; \cobang{Y} \qquad R\cap S = \copier{X} ; (R \per S) ; \cocopier{Y} \qquad X\per Y = \discharger{X}; \codischarger{Y}\]
%\end{remark}

% MAYBE HERE WE COULD INSERT SOME LAWS... I DO NOT KNOW

\begin{table}
	\[
		\begin{array}{@{}c@{}}
			\toprule
			\begin{array}{@{}c|c@{}}
				\begin{array}{@{}cc@{}}
					\multicolumn{2}{c}{
						\text{Interaction of $\op{(\cdot)}$ with $(\piu, \diag{}, \bang{}, \codiag{}, \cobang{})$}
					}
					\\
					\midrule
					\op{(f \piu g)} = \op{f} \piu \op{g} & \op{(\sigma^{\piu}_{X,Y})} = \sigma^{\piu}_{Y,X}
					\\
					\op{(\diag{X})} = \codiag{X} & \op{(\bang{X})} = \cobang{X}
					\\
					\op{(\codiag{X})} = \diag{X} & \op{(\cobang{X})} = \bang{X}
				\end{array}
				&
				\begin{array}{@{}cc@{}}
					\multicolumn{2}{@{}c@{}}{
						\text{Interaction of $\op{(\cdot)}$ and $\kstar{(\cdot)}$ with $(\sqcap, \top)$ and $(+, \bot)$}
					}
					\\
					\midrule
					% \\[-5pt]
					\begin{array}{@{}cc@{}}
						\op{(f \sqcap g)} = \op{f} \sqcap \op{g} & \op{\top} = \top
						\\
						\op{(f + g)} = \op{f} + \op{g} & \op{\bot} = \bot
					\end{array}
					&
					\begin{array}{@{}cc@{}}
						\kstar{(f \sqcap g)} \leq \kstar{f} \sqcap \kstar{g} & \kstar{\top} = \top
						\\
						 \kstar{f} + \kstar{g} \leq \kstar{(f + g)} & \kstar{\bot} = \id{} 
					\end{array}
					% \\[13pt]
					\\
					\multicolumn{2}{@{}c@{}}{
						\kstar{(\op{f})} = \op{(\kstar{f})}
					}
				\end{array}
			\end{array}
			% \\
			% \midrule
			% \text{Other interaction laws}
			% \\
			% \midrule
			% \begin{array}{@{}c@{\qquad}c@{}}
			% 	\mathfrak{r} \sqcap (\t + \s) = (\, \mathfrak{r} \sqcap \t \, ) + (\, \mathfrak{r} \sqcap \s  \,)
			% 	&
			% 	\kstar{(\op{f})} = \op{(\kstar{f})}
			% \end{array}
			\\
			\midrule
			\text{Interaction of $(\sqcap, \top)$ and $(+, \bot)$}
			\\
			\midrule
			\begin{array}{@{}c @{\qquad} c@{}}
				f \sqcap (g + h) = (\, f \sqcap g \, ) + (\, f \sqcap h  \,)
				&
				f \sqcap \bot = \bot
				\\
				f + (g \sqcap h) = (\, f + g \, ) \sqcap (\, f + h  \,)
				&
				f + \top = \top
			\end{array}
			\\
			\bottomrule
		\end{array}
	\]
	\caption{Derived laws in kc rig categories.}
	\label{table:kc rig derived laws}
\end{table}

\begin{proposition}\label{prop:kc rig laws}
	The laws in \Cref{table:kc rig derived laws} hold in any kc rig category. Moreover, the distributivity of $\op{(\cdot)}$ over $+$, together with the commutativity of $\op{(\cdot)}$ with $\kstar{(\cdot)}$ yield that a kc rig category is also a typed Kleene algebra with converse~\cite{brunet2014kleene}; while the laws at the bottom state that the homsets of a kc rig category are distributive lattices.
\end{proposition}


%
%
%
% COMMENTED FIGURE
%
%
\begin{comment}
\begin{figure}[H]
	\begin{equation}\label{eq:copier coherence}\tag{FBCB1}
		% https://q.uiver.app/?q=WzAsNSxbMCwwLCJYIFxccGl1IFkiXSxbMSwwLCIoWCBcXHBpdSBZKShYIFxccGl1IFkpIl0sWzAsMiwiWFhcXHBpdSBZWSJdLFsxLDIsIlhYIFxccGl1IFhZIFxccGl1IFlYIFxccGl1IFlZIl0sWzEsMSwiWChYIFxccGl1IFkpIFxccGl1IFkoWCBcXHBpdSBZKSJdLFswLDEsIlxcY29waWVye1ggXFxwaXUgWX0iXSxbMCwyLCJcXGNvcGllcntYfSBcXHBpdSBcXGNvcGllcntZfSIsMl0sWzIsMywiXFxpZHtYWH0gXFxwaXUgXFxjb2Jhbmd7WFl9IFxccGl1IFxcY29iYW5ne1lYfSBcXHBpdSBcXGlke1lZfSIsMl0sWzEsNCwiXFxkcntYIFxccGl1IFl9e1h9e1l9Il0sWzMsNCwiXFxJZGx7WH17WH17WX0gXFxwaXUgXFxJZGx7WX17WH17WX0iLDJdXQ==
		\begin{tikzcd}[column sep=80pt]
			{X \piu Y} & {(X \piu Y)(X \piu Y)} \\
			& {X(X \piu Y) \piu Y(X \piu Y)} \\
			{XX\piu YY} & {XX \piu XY \piu YX \piu YY}
			\arrow["{\copier{X \piu Y}}", from=1-1, to=1-2]
			\arrow["{\copier{X} \piu \copier{Y}}"', from=1-1, to=3-1]
			\arrow["{\id{XX} \piu \cobang{XY} \piu \cobang{YX} \piu \id{YY}}"', from=3-1, to=3-2]
			\arrow["{\dr{X}{Y}{X \piu Y}}", from=1-2, to=2-2]
			\arrow["{\Idl{X}{X}{Y} \piu \Idl{Y}{X}{Y}}"', from=3-2, to=2-2]
		\end{tikzcd}
	\end{equation}
	\\[2em]
	\begin{equation}\label{eq:cocopier coherence}\tag{FBCB2}
		% https://q.uiver.app/?q=WzAsNSxbMCwwLCIoWCBcXHBpdSBZKShYIFxccGl1IFkpIl0sWzEsMCwiWCBcXHBpdSBZIl0sWzAsMiwiWFggXFxwaXUgWFkgXFxwaXUgWVggXFxwaXUgWVkiXSxbMCwxLCJYKFggXFxwaXUgWSkgXFxwaXUgWShYIFxccGl1IFkpIl0sWzEsMiwiWFggXFxwaXUgWVkiXSxbMCwxLCJcXGNvY29waWVye1ggXFxwaXUgWX0iXSxbNCwxLCJcXGNvY29waWVyIFggXFxwaXUgXFxjb2NvcGllciBZICIsMl0sWzIsNCwiXFxpZHtYWH0gXFxwaXUgXFxiYW5ne1hZfSBcXHBpdSBcXGJhbmd7WVh9IFxccGl1IFxcaWR7WVl9IiwyXSxbMywyLCJcXGRse1h9e1h9e1l9IFxccGl1IFxcZGx7WX17WH17WX0iLDJdLFswLDMsIlxcZHJ7WH17WX17WCBcXHBpdSBZfSIsMl1d
		\begin{tikzcd}[column sep=80pt]
			{(X \piu Y)(X \piu Y)} & {X \piu Y} \\
			{X(X \piu Y) \piu Y(X \piu Y)} \\
			{XX \piu XY \piu YX \piu YY} & {XX \piu YY}
			\arrow["{\cocopier{X \piu Y}}", from=1-1, to=1-2]
			\arrow["{\cocopier X \piu \cocopier Y }"', from=3-2, to=1-2]
			\arrow["{\id{XX} \piu \bang{XY} \piu \bang{YX} \piu \id{YY}}"', from=3-1, to=3-2]
			\arrow["{\dl{X}{X}{Y} \piu \dl{Y}{X}{Y}}"', from=2-1, to=3-1]
			\arrow["{\dr{X}{Y}{X \piu Y}}"', from=1-1, to=2-1]
		\end{tikzcd}
	\end{equation}
	\\[2em]
	\begin{minipage}[b]{0.45\textwidth}
		\begin{equation}\label{eq:discharger coherence}\tag{FBCB3}
			% https://q.uiver.app/?q=WzAsMyxbMCwwLCJYIFxccGl1IFkiXSxbMSwwLCJcXHVubyJdLFswLDEsIlxcdW5vIFxccGl1IFxcdW5vIl0sWzAsMSwiXFxkaXNjaGFyZ2Vye1ggXFxwaXUgWX0iXSxbMCwyLCJcXGRpc2NoYXJnZXJ7WH0gXFxwaXUgXFxkaXNjaGFyZ2Vye1l9IiwyXSxbMiwxLCJcXGNvZGlhZ3tcXHVub30iLDJdXQ==
			\begin{tikzcd}
				{X \piu Y} & \uno \\
				{\uno \piu \uno}
				\arrow["{\discharger{X \piu Y}}", from=1-1, to=1-2]
				\arrow["{\discharger{X} \piu \discharger{Y}}"', from=1-1, to=2-1]
				\arrow["{\codiag{\uno}}"', from=2-1, to=1-2]
			\end{tikzcd}
		\end{equation}
	\end{minipage}
	\hfill
	\begin{minipage}{0.45\textwidth}
		\begin{equation}\label{eq:codischarger coherence}\tag{FBCB4}
			% https://q.uiver.app/?q=WzAsMyxbMCwwLCJcXHVubyJdLFsxLDAsIlggXFxwaXUgWSJdLFsxLDEsIlxcdW5vIFxccGl1IFxcdW5vIl0sWzAsMSwiXFxjb2Rpc2NoYXJnZXJ7WCBcXHBpdSBZfSJdLFswLDIsIlxcZGlhZ3tcXHVub30iLDJdLFsyLDEsIlxcY29kaXNjaGFyZ2Vye1h9IFxccGl1IFxcY29kaXNjaGFyZ2Vye1l9IiwyXV0=
			\begin{tikzcd}
				\uno & {X \piu Y} \\
				& {\uno \piu \uno}
				\arrow["{\codischarger{X \piu Y}}", from=1-1, to=1-2]
				\arrow["{\diag{\uno}}"', from=1-1, to=2-2]
				\arrow["{\codischarger{X} \piu \codischarger{Y}}"', from=2-2, to=1-2]
			\end{tikzcd}
		\end{equation}
	\end{minipage}
	\caption{Coherence axioms for fb-cb categories}
	\label{fig:fbcbcoherence}
\end{figure}
\end{comment}
%
%
% END COMMENTED FIGURE
%
%



\subsection{From Kleene to Kleene-Cartesian Tapes}
Now we are going to construct the tape diagrams for kc rig categories.

For  a monoidal signature $(\sort, \sign)$, we fix 
\[\Gamma \defeq \{ \cocopier{A} \colon A \perG A \to A, \;\; \codischarger{A} \colon \unoG \to A, \;\; \copier{A} \colon A \to A \perG A, \;\; \discharger{A} \colon A \to \unoG \;\;\mid \;\; A \in \sort \}\]
and consider the signature obtained as the disjoint union of $\sign$ and $\Gamma$, that is $(\sort, \sign + \Gamma)$. Then consider the corresponding category of Kleene tapes: $\CatKTapeC$.
We now define a preorder on this category using the same recipe of $\precongK$ in Section \ref{sec:kleene-tapes}: we take $\basicCB$ to be the set of pairs of tapes containing all and only the pairs in  Figure \ref{fig:cb axioms}.
We fix $\basicKC \defeq \basicCB \cup \basicK$ and define $\leq_{\basicKC}$ according to the rules in \eqref{eq:uniformprecong}. Analogously to Section \ref{sec:kleene-tapes}, $\sim_{\basicKC} \defeq \leq_{\basicKC} \cap \geq_{\basicKC}$.

With these definitions we can construct the category of Kleene cartesian tapes $\KTCB$: objects are the same of $\CatKTapeC$; arrows are $\sim_\basicKC$-equivalence classes of arrows of $\CatKTapeC$; every homset $\KTCB[P,Q]$ is ordered by $\precongKC$. In a nustshell, objects of $\KTCB$ are polynomials in $(\sort^\star)^\star$. Arrows are  $\sim_{\basicKC}$-equivalence classes of the tape generated by the following grammar where $A\in \sort$, $U\in \sort^\star$ and $s \in \sign$.
\begin{equation}\label{kleeneCartesianGrammar}
    \begin{tabular}{rc ccccccccccccccccccccc}\setlength{\tabcolsep}{0.0pt}
        $c$  & ::= & $\id{A}$ & $\!\!\! \mid \!\!\!$ & $ \id{\uno} $ & $\!\!\! \mid \!\!\!$ & $ \gen $ & $\!\!\! \mid \!\!\!$ & $ \sigma_{A,B} $ & $\!\!\! \mid \!\!\!$ & $   c ; c   $ & $\!\!\! \mid \!\!\!$ & $  c \per c$ & $\!\!\! \mid \!\!\!$ & $\discharger{A}$ & $\!\!\! \mid \!\!\!$ & $\copier{A}$ & $\!\!\! \mid \!\!\!$ & $\codischarger{A}$ & $\!\!\! \mid \!\!\!$ & $\cocopier{A} $ \\
        $\t$ & ::= & $\id{U}$ & $\!\!\! \mid \!\!\!$ & $ \id{\zero} $ & $\!\!\! \mid \!\!\!$ & $ \tapeFunct{c} $ & $\!\!\! \mid \!\!\!$ & $ \sigma_{U,V}^{\piu} $ & $\!\!\! \mid \!\!\!$ & $   \t ; \t   $ & $\!\!\! \mid \!\!\!$ & $  \t \piu \t  $ & $\!\!\! \mid \!\!\!$ & $ \bang{U} $ & $\!\!\! \mid \!\!\!$ & $\diag{U}$ & $\!\!\! \mid \!\!\!$ & $\cobang{U}$ & $\!\!\! \mid \!\!\!$ & $\codiag{U}$  &  $\!\!\! \mid \!\!\!$ & $\trace_{U}\t$    
    \end{tabular}
\end{equation}  

%\begin{equation*}\label{tracedTapesDiagGrammar}
%    \setlength{\tabcolsep}{2pt}
%    \begin{tabular}{rc cccccccccccc}
%        $c$  & ::= &  $\wire{A}$ & $\mid$ & $ \tikzfig{empty} $ & $\mid$ & $ \Cgen{\gen}{A}{B}  $ & $\mid$ & $ \Csymm{A}{B} $ & $\mid$ & $ \tikzfig{seq_compC}   $ & $\mid$ & $  \tikzfig{par_compC}$ &  \multicolumn{12}{l}{$\discharger{A} \; \mid \; %\copier{A} \; \mid \; \codischarger{A} \; \mid \; \cocopier{A} $} \\
%        $\t$ & ::= & $\Twire{U}$ & $\mid$ & $ \tikzfig{empty} $ & $\mid$ & $ \Tcirc{c}{U}{V}  $ & $\mid$ & $ \Tsymmp{U}{V} $ & $\mid$ & $ \tikzfig{tapes/seq_comp}  $ & $\mid$ & $  \tikzfig{tapes/par_comp}$ & $\mid$ \\
%             &     & \multicolumn{12}{l}{$\Tcounit{U} \; \mid \; \Tcomonoid{U} \; \mid \; \Tunit{U} \; \mid \; \Tmonoid{U} \; \mid \; \TTraceMon{\t}[U][P][Q]$}
%    \end{tabular}
%\end{equation*} 
Recall from Section \ref{sec:tapes}, that traces and $\piu$-(co)monoids for arbitrary polynomials are defined as in Table \ref{tab:inddefutfb}; the monoidal product $\per$ is defined for arbitrary tapes as in Tables \ref{tab:producttape} and \ref{tab:wisktraces};     left distributors $\delta^l$ and symmetries $\symmt$ as in Table \ref{table:def dl symmt}. In  $\KTCB$,  by means of the coherence conditions in \eqref{eq:fbcbcoherence}, one can inductively define  $\per$-(co)monoids for arbitrary polynomials: see Table \ref{table:defmonoidper}.  For instance, $\copier{A \piu B} \colon A \piu B \to (A \piu B)\per(A \piu B) = AA \piu AB \piu BA \piu BB$ and $\discharger{A \piu B} \colon A \piu B \to \uno$ are
    \[\copier{A \piu B} = \tikzfig{cb/examples/copierApB} \qquad \discharger{A \piu B} = \tikzfig{cb/examples/dischargerApB}\]



\begin{table}
    \begin{equation}\label{eq:copierind}
        \begin{array}{rcl C{0.5cm} rcl}
            \copier{\zero} &\defeq& \id{\zero} && \discharger{\zero} &\defeq& \cobang{\uno}  \\
            \copier{U \piu P'} &\defeq& \Tcopier{U} \piu \cobang{UP'} \piu ((\cobang{P'U} \piu \copier{P'}) ; \Idl{P'}{U}{P'}) && \discharger{U \piu P'} &\defeq& (\Tdischarger{U} \piu \discharger{P'}) ; \codiag{\uno}
        \end{array}
    \end{equation}
    \begin{equation}\label{eq:cocopierind}
        \begin{array}{rcl C{0.5cm} rcl}
            \cocopier{\zero} &\defeq& \id{\zero} && \codischarger{\zero} &\defeq& \bang{\uno}  \\
            \cocopier{U \piu P'} &\defeq& \Tcocopier{U} \piu \bang{UP'} \piu (\dl{P'}{U}{P'} ; (\bang{P'U} \piu \cocopier{P'})) && \codischarger{U \piu P'} &\defeq& \diag{\uno} ; (\Tcodischarger{U} \piu \codischarger{P'})
        \end{array}
    \end{equation}
        \caption{Inductive definitions of $\discharger{P}$, $\copier{P}$, $\codischarger{P}$ and $\cocopier{P}$}
        \label{table:defmonoidper}
\end{table}
These structures make $\KTCB$  a kc rig category.





\begin{theorem}\label{theorem:KTCB is kleene-cartesian}
	$\KTCB$ is a Kleene-Cartesian rig category.
\end{theorem}
\begin{proof}
By construction $\KTCB$ is a Kleene rig category. In order to prove that $(\KTCB, \per, \uno)$ is a cartesian bicategory we widely rely on the proof of \cite[Theorem 7.3]{bonchi2023deconstructing}.
%In such proof $\copier{P} \colon P \to P\per P$, $\discharger{P} \colon P \to \uno$, $\cocopier{P} \colon P \to P \per P$ and  $\codischarger{P} \colon \uno \to P$ are defined for all polynomials $P$ as in Table \ref{able:defmonoidper}.
By \cite[Theorem 7.3]{bonchi2023deconstructing},  $\copier{P}, \discharger{P}, \cocopier{P}$ and $\codischarger{P}$ satisfy the axioms of special Frobenius algebras and the comonoid $(\copier{P}, \discharger{P})$ is left adjoint to the monoid $(\cocopier{P}, \discharger{P})$. Moreover, every trace-free tape diagram $\t \colon P \to Q$ is a lax comonoid homomorphism, i.e. 
	\begin{equation}\label{eq:trace free lax naturality}
		\t ; \copier{Q} \; \leq \; \copier{P} ; (\t \per \t) 	\quad \text{ and } \quad \t ; \discharger{Q} \; \leq \; \discharger{P}.
	\end{equation}
	To conclude, we need to show that the inequalities above hold for \emph{every} tape diagram $\t \colon P \to Q$ in $\KTCB$. 

	By the normal form of traced monoidal categories, there exists a trace-free tape diagram $\t' \colon S \piu P \to S \piu Q$, such that $\trace_{S} \t' = \t$. Now, let $\begin{psmallmatrix} \t'_{SS} & \t'_{SQ} \\ \t'_{PS} & \t'_{PQ} \end{psmallmatrix}$ be the matrix normal form of $\t'$ and observe that the following holds.

	\begingroup
	\allowdisplaybreaks
		\begin{align*}
			\t ; \copier{Q} 
			&= 
			\trace_{S} \t' ; \copier{Q}  
			= 
			\scalebox{0.7}{\tikzfig{laxnaturality/copier/step1}} 
			&&\!\!\!\!\!\!\!\!\!\!\!\!\!\leftstackrel{\eqref{ax:copieradj2}}{=}
			\scalebox{0.7}{\tikzfig{laxnaturality/copier/step2}} \\
			&\leftstackrel{\eqref{ax:trace:sliding}}{=}
			\scalebox{0.7}{\tikzfig{laxnaturality/copier/step3}}
			&&\!\!\!\!\!\!\!\!\!\!\!\!\!\leftstackrel{\eqref{ax:diagnat}, \eqref{ax:codiagnat}}{=}
			\scalebox{0.7}{\tikzfig{laxnaturality/copier/step4}} \\
			&\leftstackrel{\eqref{eq:trace free lax naturality}}{\leq}
			\scalebox{0.7}{\tikzfig{laxnaturality/copier/step5}} 
			&&\!\!\!\!\!\!\!\!\!\!\!\!\!\leftstackrel{\eqref{ax:copieradj1}}{\leq}
			\scalebox{0.7}{\tikzfig{laxnaturality/copier/step6}} \\
			&\leftstackrel{\eqref{ax:diagnat}}{=}
			\scalebox{0.7}{\tikzfig{laxnaturality/copier/step7}}
			&&\!\!\!\!\!\!\!\!\!\!\!\!\!\leftstackrel{\text{(\Cref{prop:trace-per})}}{\leq}
			\copier{P} ; (\trace_{S} \t' \per \trace_{S} \t')
			= 
			\copier{P} ; (\t \per \t)
		\end{align*}
	\endgroup

	To prove the other inequality we exploit again the matrix normal form.

	\begingroup
	\allowdisplaybreaks
		\begin{align*}
			\t ; \discharger{Q} 
			= 
			\trace_{S} \t' ; \discharger{Q}
			&= 
			\scalebox{0.7}{\tikzfig{laxnaturality/discard/step1}}
			\stackrel{\eqref{ax:dischargeradj2}}{\leq}
			\scalebox{0.7}{\tikzfig{laxnaturality/discard/step2}}
			\stackrel{\eqref{ax:trace:sliding}}{=}
			\scalebox{0.7}{\tikzfig{laxnaturality/discard/step3}} \\
			&\leftstackrel{\eqref{ax:diagnat}, \eqref{ax:codiagnat}}{=}
			\scalebox{0.7}{\tikzfig{laxnaturality/discard/step4}} 
			\stackrel{\eqref{eq:trace free lax naturality}}{\leq}
			\scalebox{0.7}{\tikzfig{laxnaturality/discard/step5}}
			\stackrel{\eqref{ax:dischargeradj1}}{\leq}
			\scalebox{0.7}{\tikzfig{laxnaturality/discard/step6}} \\
			&\leftstackrel{\eqref{ax:diagnat}}{=}
			\scalebox{0.7}{\tikzfig{laxnaturality/discard/step7}}
			\stackrel{\eqref{ax:bi}}{=}
			\scalebox{0.7}{\tikzfig{laxnaturality/discard/step8}}
			\stackrel{\eqref{ax:trace:tape:kstar-id}}{=}
			\scalebox{0.7}{\tikzfig{laxnaturality/discard/step9}}
		\end{align*}
	\endgroup

	% \begingroup
	% \allowdisplaybreaks
	% % \begin{minipage}{0.52\textwidth}
	% % 	\begin{align*}
	% % 		\t ; \copier{Q} 
	% % 		&= \trace_{S} \t' ; \copier{Q}  \\
	% % 		&= \scalebox{0.8}{\tikzfig{laxnaturality/copier/step1}} \\
	% % 		&= \scalebox{0.8}{\tikzfig{laxnaturality/copier/step2}} \tag{\ref{ax:specfrob}} \\
	% % 		&= \scalebox{0.8}{\tikzfig{laxnaturality/copier/step3}}  \tag{\ref{ax:trace:sliding}} \\
	% % 		&= \scalebox{0.8}{\tikzfig{laxnaturality/copier/step4}} \tag{\ref{ax:diagnat}, \ref{ax:codiagnat}} \\
	% % 		&\leq \scalebox{0.8}{\tikzfig{laxnaturality/copier/step5}} \tag{\ref{ax:copiernat}} \\
	% % 		&\leq \scalebox{0.8}{\tikzfig{laxnaturality/copier/step6}} \tag{\ref{ax:copieradj1}} \\
	% % 		&= \scalebox{0.8}{\tikzfig{laxnaturality/copier/step7}} \tag{\ref{ax:diagnat}} \\
	% % 		&\leq \copier{P} ; (\trace_{S} \t' \per \trace_{S} \t') \tag{\Cref{prop:trace-per}} \\
	% % 		&= \copier{P} ; (\t \per \t)
	% % 	\end{align*}
	% % \end{minipage}
	% % \; \vline \;
	% % \begin{minipage}{0.44\textwidth}
	% % 	\begin{align*}
	% % 		\t ; \discharger{Q} 
	% % 		&= \trace_{S} \t' ; \discharger{Q}  \\
	% % 		&= \scalebox{0.8}{\tikzfig{laxnaturality/discard/step1}} \\
	% % 		&\leq \scalebox{0.8}{\tikzfig{laxnaturality/discard/step2}} \tag{\ref{ax:dischargeradj2}} \\
	% % 		&= \scalebox{0.8}{\tikzfig{laxnaturality/discard/step3}}  \tag{\ref{ax:trace:sliding}} \\
	% % 		&= \scalebox{0.8}{\tikzfig{laxnaturality/discard/step4}} \tag{\ref{ax:diagnat}, \ref{ax:codiagnat}} \\
	% % 		&\leq \scalebox{0.8}{\tikzfig{laxnaturality/discard/step5}} \tag{\ref{ax:dischargernat}} \\
	% % 		&\leq \scalebox{0.8}{\tikzfig{laxnaturality/discard/step6}} \tag{\ref{ax:dischargeradj1}} \\
	% % 		&= \scalebox{0.8}{\tikzfig{laxnaturality/discard/step7}} \tag{\ref{ax:diagnat}} \\
	% % 		&= \scalebox{0.8}{\tikzfig{laxnaturality/discard/step8}} \tag{\ref{ax:bi}} \\
	% % 		&= \scalebox{0.8}{\tikzfig{laxnaturality/discard/step9}} \tag{\ref{}}
	% % 	\end{align*}
	% % \end{minipage}
	% \endgroup
\end{proof}

% \begin{table}
% \tiny{
% \begin{center}
% \begin{tabular}{ccccc}
% 	\toprule
% $\CBdsem{\CBRel{R}{U}{V}}_{\interpretation} = \alpha_{\sign}(R) $&$ \CBdsem{\CBcopier{A}}_{\interpretation} = \copier{X}  $&$ \CBdsem{\CBdischarger{A}}_{\interpretation} = \discharger{X}  $&$ \CBdsem{\CBcocopier{A}}_{\interpretation} = \cocopier{X}  $&$ \CBdsem{\CBcodischarger{A}}_{\interpretation} = \codischarger{X}$\\
% %
% $\CBdsem{\id{A}}_{\interpretation}= \id{A} $&$ \CBdsem{\id{1}}_{\interpretation}= \id{1} $&$ \CBdsem{\symmt{A}{A}}_{\interpretation} = \symmt{A}{A}  $&$ \CBdsem{c_1;c_2}_{\interpretation} = \CBdsem{c_1}_{\interpretation}; \CBdsem{c_2}_{\interpretation}  $ & $ \CBdsem{c_1\per c_2}_{\interpretation} = \CBdsem{c_1}_{\interpretation} \per \CBdsem{c_2}_{\interpretation}$\\
% %
% \midrule
% $\TCBdsem{\Tcirc{c}{U}{V}}_{\interpretation}= \CBdsem{c}_{\interpretation} $&$ \TCBdsem{\Tcomonoid{U}}_{\interpretation}= \diag{W} $&$ \TCBdsem{\Tcounit{U}}_{\interpretation} = \bang{W}$ & $\TCBdsem{\Tmonoid{U}}_{\interpretation}= \codiag{W} $&$ \TCBdsem{\Tunit{U}}_{\interpretation} = \cobang{W}$ \\
% %
% $\TCBdsem{\id{U}}_{\interpretation}= \id{W} $&$ \TCBdsem{\id{\zero}}_{\interpretation} = \id{\zero}  $&$ \TCBdsem{\symmp{U}{U'}}_{\interpretation}= \symmp{W}{W'} $&$ \TCBdsem{\s;\t}_{\interpretation} = \TCBdsem{\s}_{\interpretation} ; \TCBdsem{\t}_{\interpretation} $&$ \TCBdsem{\s \piu \t}_{\interpretation} = \TCBdsem{\s}_{\interpretation} \piu \TCBdsem{\t}_{\interpretation} $ \\
% \bottomrule
% \end{tabular}
% \end{center}}
% \caption{The morphisms $\CBdsem{\cdot}_{\interpretation} \colon \CB \to \Rel$ and $\TCBdsem{\cdot}_{\interpretation} \colon \CatTapeCB \to \Rel$ extending an interpretation $\interpretation=(\alpha_{\sort}, \alpha_{\sign})$ of a monoidal signature $\sign$ in $\Rel$. We write $X,W,W'$ for $\alpha_\sort(A)$, $\alpha^\sharp_\sort(U)$ and $\alpha^\sharp_\sort(U')$ respectively, and $\cocopier{X}$, $\codischarger{X}$, $\copier{X}$, $\discharger{X}$, $\codiag{W}$ $\cobang{W}$, $\diag{W}$, $\bang{W}$ for the (co)monoids in $\Rel$ defined as in~\eqref{eq:comonoidsREL}.}
% \label{tabSemantic}
% \end{table}


Given a monoidal signature $(\sort,\sign)$, a (sesquistrict) kc rig category $\Cat{C}$ and an interpretation $\mathcal{I}=(\alpha_\sort,\alpha_\sign)$ of $\sign$ in $\Cat{C}$, 
the inductive extension of $\mathcal{I}$, hereafter referred as $\CBdsem{\cdot}_{\interpretation} \colon \KTCB \to \Cat{C}$, is defined as follows. %\marginpar{aggiustare questa tabella, farla carina se possibile}
% \ale{Con o senza $\sharp$?}
\small{
\renewcommand{\arraystretch}{1.5}
\begin{tabular}{lllll}
$\CBdsem{s}_{\interpretation} = \alpha_{\sign}(s) $&$ \CBdsem{\copier{A}}_{\interpretation} = \copier{\alpha_\sort(A)}  $&$ \CBdsem{\discharger{A}}_{\interpretation} = \discharger{\alpha_\sort(A)}  $&$ \CBdsem{\cocopier{A}}_{\interpretation} = \cocopier{\alpha_\sort(A)}  $&$ \CBdsem{\codischarger{A}}_{\interpretation} = \codischarger{\alpha_\sort(A)}$\\
$\CBdsem{\id{A}}_{\interpretation}= \id{\alpha_\sort(A)} $&$ \CBdsem{\id{1}}_{\interpretation}= \id{1} $&$ \CBdsem{\symmt{A}{B}}_{\interpretation} = \symmt{\alpha_\sort(A)}{\alpha_\sort(B)}  $&$ \CBdsem{c;d}_{\interpretation} = \CBdsem{c}_{\interpretation}; \CBdsem{d}_{\interpretation}  $ & $ \CBdsem{c\per d}_{\interpretation} = \CBdsem{c}_{\interpretation} \per \CBdsem{d}_{\interpretation}$\\
$\CBdsem{\, \tapeFunct{c} \,}_{\interpretation}= \CBdsem{c}_{\interpretation} $&$ \CBdsem{\diag{U}}_{\interpretation}= \diag{\alpha^\sharp_\sort(U)} $&$ \CBdsem{\bang{U}}_{\interpretation} = \bang{\alpha^\sharp_\sort(U)}$ & $\CBdsem{\codiag{U}}_{\interpretation}= \codiag{\alpha^\sharp_\sort(U)} $&$ \CBdsem{\cobang{U}}_{\interpretation} = \cobang{\alpha^\sharp_\sort(U)}$  \\
$\CBdsem{\id{U}}_{\interpretation}= \id{\alpha^\sharp_\sort(U)} $&$ \CBdsem{\id{\zero}}_{\interpretation} = \id{\zero}  $&$ \CBdsem{\symmp{U}{V}}_{\interpretation}= \symmp{\alpha^\sharp_\sort(U)}{\alpha^\sharp_\sort(V)} $&$ \CBdsem{\s;\t}_{\interpretation} = \CBdsem{\s}_{\interpretation} ; \CBdsem{\t}_{\interpretation} $&$ \CBdsem{\s \piu \t}_{\interpretation} = \CBdsem{\s}_{\interpretation} \piu \CBdsem{\t}_{\interpretation} $\\
\multicolumn{5}{c}{
	$\CBdsem{\trace_{U}\t}_{\interpretation} = \trace_{\alpha^\sharp_\sort(U)} \CBdsem{\t}_{\interpretation}$
}
\end{tabular}
}

It turns out that  $\CBdsem{\cdot}_{\interpretation}$ is a kc rig morphism and it is actually the unique one  respecting the interpretation $\mathcal{I}$.

\begin{theorem}\label{thm:KleeneCartesiantapesfree}
$\KTCB$ is the free sesquistrict kc rig category generated by the monoidal signature $(\sort, \sign)$.
\end{theorem}



% \subsection{Functorial Semantics}\label{ssec:funsem}
% %
% % COMMENTED BELOW
% %
% \begin{comment}
% One can immediately see that by $(r)$ and $(t)$, $\precongB$ is a preorder and that by $(;)$, $(\piu)$ and $(\per)$, $\precongB$ is closed by the rig operation. To see that its is closed by traces, it is enough to take in ($ut$-1) and ($ut$-2), $\s_2=\s_1=id$.

% By enriching $\Cat{C}$ with $\precongB$, we obtain a \emph{preorder enriched traced rig category} (namely, $\trace$, $\piu$, $\per$ and $;$ are monotone) that we denote hereafter by $\Cat{C}_{\basicR}$.
% For an arbitrary category $\Cat{C}$ enriched over a preorder $\leq$, one can define a corresponding poset enriched category $\posetification{\Cat{C}}$ by quotienting the homsets of $\Cat{C}$ by the equivalence relation $\sim$ defined as $\sim  \defeq  \leq \cap \geq$. Moreover, if $\Cat{C}$ is a preorder enriched traced rig category, then $\posetification{\Cat{C}}$ is a \emph{poset enriched traced rig category}. 


% Particularly relevant for this paper will be $\posetification{\PreCatTrTapeI{\basicR}}$. %Similarly, for a monoidal theory $(\sign, \basicR)$, one can construct preorder and poset enriched monoidal categories, hereafter denoted by $\Cat{C}_{\sign,\basicR}$ and $\posetification{\Cat{C}_{\sign,\basicR}}$, respectively.


% Formally, we call $\CatKTape$ the category of tapes generated by \eqref{}
% quotiented by the laws in Figure BLA LA INSERT LAWS AND TABLES FOR THE KLEENE LAWS.
% \end{comment}
% %
% % END OF COMMENT
% %

% The usual way of reasoning through string diagrams is based on monoidal theories, namely a signature plus a set of axioms: either equations or inequations. Similarly a \emph{kc tape theory} is a pair $(\sign, \basicR)$ where $\sign$ is a monoidal signature and $\basicR$ is a set of pairs $(\t_1, \t_2)$ of arrows in $\KTCB$ with same domain and codomain. Hereafter, we think of each pair $(\t_1, \t_2)$ as an inequation $\t_1 \leq \t_2$, but the results that we develop in this section trivially hold  also for equations: it is enough to add in $\basicR$ a pair $(\t_2, \t_1)$ for each $(\t_1, \t_2) \in \basicR$.

% Given a kc tape theory $(\sign, \basicR)$, we will write $\precongB$ for $\precongR{\basicKC \cup \basicR}$ where the latter is generated from $\basicKC \cup \basicR$ by the rules  in \eqref{eq:uniformprecong}. Since the pairs of arrows in $\basicKC$
% express the laws of kc rig categories, it is safe to always keep $\basicKC$ implicit.

% \begin{remark}
% Derivations using $\precongB$ might end up being not entirely graphical because they may rely on  the decomposition via $\per$: see, e.g., Example 5.14 in \cite{bonchi2023deconstructing}.
% The solution devised in \cite{bonchi2023deconstructing} also works for kc tapes: take the kc tape theory $(\sign, \wiskbasicR)$, where $\wiskbasicR = \{ (\t_1 \per \id{U}, \t_2 \per \id{U}) \mid (\t_1, \t_2) \in \basicR \text{ and } U\in \sort^\star \}$ and define $\WprecongBA$ as in \eqref{eq:uniformprecong} but without the rules for $\per$, i.e., with the following rules. 
% \[
%     \begin{array}{ccccc}
%         \inferrule*[right=($\wiskbasicR$)]{\t_1 \mathbin{\wiskbasicR} \t_2}{\t_1 \mathrel{\WprecongBA} \t_2}
%         &
%         \inferrule*[right=($r$)]{-}{\t \mathrel{\WprecongBA} \t}
%         &    
%         \inferrule*[right=($t$)]{\t_1 \mathrel{\WprecongBA} \t_2 \quad \t_2 \mathrel{\WprecongBA} \t_3}{\t_1 \mathrel{\WprecongBA} \t_3}
%         &
%         \inferrule*[right=($;$)]{\t_1 \mathrel{\WprecongBA} \t_2 \quad \s_1 \mathrel{\WprecongBA} \s_2}{\t_1;\s_1 \mathrel{\WprecongBA} \t_2;\s_2}
%         &
%         \inferrule*[right=($\piu$)]{\t_1 \mathrel{\WprecongBA} \t_2 \quad \s_1 \mathrel{\WprecongBA} \s_2}{\t_1\piu\s_1 \mathrel{\WprecongBA} \t_2 \piu \s_2}
%         \\[8pt]
%         \multicolumn{5}{c}{
%         \inferrule*[right=($ut$-1)]{\s_2 \mathrel{\WprecongBA} \s_1 \qquad \t_1 ; (\s_1 \piu \id{}) \mathrel{\WprecongBA} (\s_2 \piu \id{}) ; \t_2}{\trace_{S_1}\t_1 \mathrel{\WprecongBA} \trace_{S_2}\t_2}
%         \qquad
%         \inferrule*[right=($ut$-2)]{ \s_2 \mathrel{\WprecongBA} \s_1 \qquad (\s_1 \piu \id{}) ; \t_1 \mathrel{\WprecongBA} \t_2 ; (\s_2 \piu \id{})}{\trace_{S_1}\t_1 \mathrel{\WprecongBA} \trace_{S_2}\t_2}
%         }
%     \end{array}
% \]
% Then, by  the same proof of Theorem 5.15 in~\cite{bonchi2023deconstructing}, it holds that  $\t_1 \precongB \t_2$ if and only if $\t_1 \WprecongBA \t_2$.
% \end{remark}

% %Recall that $\basicKC$ contains the pairs of arrows expressing the laws of Kleene and cartesian bicategories. Hereafter we will consider $\precongR{\basicKC \cup \basicR}$ as given by the rules  in \eqref{eq:uniformprecong} but we will always keep 
% % $\basicKC$ implicit and write simply $\precongB$.
% %,  and $\sim_{\basicKC \cup \basicR} \defeq \leq_{\basicKC \cup \basicR} \cap \geq_{\basicKC \cup \basicR}$. Hereafter, we will  write $\precongB$ and $\sim_{\basicR}$ keeping $\basicKC$ implicit.


% Recall that an interpretation $\mathcal{I}=(\alpha_{\sort}, \alpha_{\sign})$ of a monoidal signature $(\sort,\sign)$ in a sesquistrict rig category  $\Cat{C}$ consists of $\alpha_{\sort}\colon \sort \to Ob(\Cat{C})$ and $\alpha_{\sign}\colon \sign \to Ar(\Cat{C})$ preserving (co)arities of symbols $s\in \sign$. Whenever $\Cat{C}$ is a kc rig category, $\mathcal{I}$ gives rises uniquely, by freeness of $\KTCB$, to the morphisms of kc rig categories $\TCBdsem{\cdot}_{\interpretation} \colon \KTCB \to \Cat{C}$. We say that an intepretation $\interpretation$ of $\sign$ is \emph{a model of the theory} $(\sign, \basicR)$ whenever $\TCBdsem{\cdot}_{\interpretation}$ preserves $\precongB$: if $\t_1 \precongB \t_2$, then $\TCBdsem{\t_1}_{\interpretation} $ is below $\TCBdsem{\t_2}_{\interpretation}$ in $\Cat{C}$.

% \begin{example}\label{ex:totalorder}
% 	Consider the signature $(\sort, \sign)$ where $\sort$ contains a single sort $A$ and $\sign = \{ R \colon A \to A \}$. Take as $\basicR$ the set consisting of the following inequalities:
% 	\mylabel{R:refl}{refl}
% 	\mylabel{R:tr}{tr}
% 	\mylabel{R:anti}{anti}
% 	\mylabel{R:lin}{lin}
% 	\[
% 		\begin{array}{c@{}c@{}c c@{}c@{}c}
% 			\tikzfig{linOrd/id} &\stackrel{(\text{refl})}{\leq}& \tikzfig{linOrd/R} & \tikzfig{linOrd/RR} &\stackrel{(\text{tr})}{\leq}& \tikzfig{linOrd/R}
% 			\\[10pt]
% 			\tikzfig{linOrd/and} &\stackrel{(\text{anti})}{\leq}& \tikzfig{linOrd/id} & \tikzfig{linOrd/top} &\stackrel{(\text{lin})}{\leq}& \tikzfig{linOrd/or}		
% 		\end{array}
% 	\]
% 	An interpretation of $(\sign, \basicR)$ in the kc rig category $\Rel$ is a set $X$, together with a relation $R \subseteq X \times X$. It is a model iff $R$ is a linear order, i.e. it is reflexive, transitive, antisymmetric and linear.
% \end{example}


% Models enjoy a beautiful characterisation provided by Proposition \ref{funct:sem} below. Let $\KTCBI$ be the category having the same objects as $\KTCB$ and arrows $\sim_{\basicR}$-equivalence classes of arrows of $\KTCB$ ordered by $\precongB$.
% Since $\KTCB$ is a kc rig category, thus so is also $\KTCBI$.

% \begin{proposition}\label{funct:sem}
% 	Let $(\sign, \basicR)$ be a kc tape theory and $\Cat{C}$ a sesquistrict kc rig category.  Models of $(\sign, \basicR)$ are in bijective correspondence with  morphisms of sesquistrict kc rig categories from $\KTCBI$ to $\Cat{C}$.
% \end{proposition} 











%%%%%%%%%%%%%%%%%
%
%
% COMMENTED BELOW
%
%%%%%%%%%%%%%%%%%%



\begin{comment}
\subsection{Commentaries by Pippo}
The first (and I guess the second) definition of $\mathrel{\precongB}$ by means of the inference rules seems to be wrong because the categories resulting from the quotient is not uniform: see the explanation at the end of the paper.

Accordingly to what developed in the main case, one should have:
\[
    \begin{array}{c@{\qquad}c@{\qquad}c}
        \inferrule*[right=($\basicR$)]{\t_1 \mathbin{\basicR} \t_2}{\t_1 \mathrel{\precongB} \t_2}
        &
        \inferrule*[right=($r$)]{-}{\t \mathrel{\precongB} \t}
        &    
        \inferrule*[right=($t$)]{\t_1 \mathrel{\precongB} \t_2 \quad \t_2 \mathrel{\precongB} \t_3}{\t_1 \mathrel{\precongB} \t_3}
        \\[8pt]
        \inferrule*[right=($;$)]{\t_1 \mathrel{\precongB} \t_2 \quad \s_1 \mathrel{\precongB} \s_2}{\t_1;\s_1 \mathrel{\precongB} \t_2;\s_2}
        &
        \inferrule*[right=($\piu$)]{\t_1 \mathrel{\precongB} \t_2 \quad \s_1 \mathrel{\precongB} \s_2}{\t_1\piu\s_1 \mathrel{\precongB} \t_2 \piu \s_2}
        &
        \inferrule*[right=($\per $)]{\t_1 \mathrel{\precongB} \t_2 \quad \s_1 \mathrel{\precongB} \s_2}{\t_1\per \s_1 \mathrel{\precongB} \t_2 \per \s_2}
        \\[8pt]
        \multicolumn{3}{c}{
        \inferrule*[right=($ut$-1)]{\s_1 \mathrel{\precongB} \s_2 \qquad \s_2 \mathrel{\precongB} \s_1 \qquad \t_1 ; (\s_1 \piu \id{}) \mathrel{\precongB} (\s_2 \piu \id{}) ; \t_2}{\trace_{S_1}\t_1 \mathrel{\precongB} \trace_{S_2}\t_2}
        \qquad
        \inferrule*[right=($ut$-2)]{\s_1 \mathrel{\precongB} \s_2 \qquad \s_2 \mathrel{\precongB} \s_1 \qquad (\s_1 \piu \id{}) ; \t_1 \mathrel{\precongB} \t_2 ; (\s_2 \piu \id{})}{\trace_{S_1}\t_1 \mathrel{\precongB} \trace_{S_2}\t_2}
        }
    \end{array}
\]
Note that $\s_1 \mathrel{\precongB} \s_2$  and $\s_2 \mathrel{\precongB} \s_1$ are nedeed to guarantee that $\s_1=\s_2$ in the quotiented category.

One can drop however the premises $\s_1 \mathrel{\precongB} \s_2$ and obtain the following more compact definition.

\[
    \begin{array}{c@{\qquad}c@{\qquad}c}
        \inferrule*[right=($\basicR$)]{\t_1 \mathbin{\basicR} \t_2}{\t_1 \mathrel{\precongB} \t_2}
        &
        \inferrule*[right=($r$)]{-}{\t \mathrel{\precongB} \t}
        &    
        \inferrule*[right=($t$)]{\t_1 \mathrel{\precongB} \t_2 \quad \t_2 \mathrel{\precongB} \t_3}{\t_1 \mathrel{\precongB} \t_3}
        \\[8pt]
        \inferrule*[right=($;$)]{\t_1 \mathrel{\precongB} \t_2 \quad \s_1 \mathrel{\precongB} \s_2}{\t_1;\s_1 \mathrel{\precongB} \t_2;\s_2}
        &
        \inferrule*[right=($\piu$)]{\t_1 \mathrel{\precongB} \t_2 \quad \s_1 \mathrel{\precongB} \s_2}{\t_1\piu\s_1 \mathrel{\precongB} \t_2 \piu \s_2}
        &
        \inferrule*[right=($\per $)]{\t_1 \mathrel{\precongB} \t_2 \quad \s_1 \mathrel{\precongB} \s_2}{\t_1\per \s_1 \mathrel{\precongB} \t_2 \per \s_2}
        \\[8pt]
        \multicolumn{3}{c}{
        \inferrule*[right=($ut$-1)]{\s_2 \mathrel{\precongB} \s_1 \qquad \t_1 ; (\s_1 \piu \id{}) \mathrel{\precongB} (\s_2 \piu \id{}) ; \t_2}{\trace_{S_1}\t_1 \mathrel{\precongB} \trace_{S_2}\t_2}
        \qquad
        \inferrule*[right=($ut$-2)]{ \s_2 \mathrel{\precongB} \s_1 \qquad (\s_1 \piu \id{}) ; \t_1 \mathrel{\precongB} \t_2 ; (\s_2 \piu \id{})}{\trace_{S_1}\t_1 \mathrel{\precongB} \trace_{S_2}\t_2}
        }
    \end{array}
\]
Observe that this novel definition gives us an equivalent rephrasing of the uniformity axiom (hereafter we always drop the rightmost and consider only the leftmost)
\[\text{ If } \exists \s_1,\s_2. \; \s_2 \mathrel{\precongB} \s_1 \text{ and } \t_1 ; (\s_1 \piu \id{}) \mathrel{\precongB} (\s_2 \piu \id{}) ; \t_2 \text{, then }\trace_{S_1}\t_1 \mathrel{\precongB} \trace_{S_2}\t_2 \]

\begin{lemma}
The following are equivalent:
\begin{enumerate}
\item  If $\exists \s_1,\s_2. \; \s_2 \mathrel{\precongB} \s_1$ and $\t_1 ; (\s_1 \piu \id{}) \mathrel{\precongB} (\s_2 \piu \id{}) ; \t_2$, then $\trace_{S_1}\t_1 \mathrel{\precongB} \trace_{S_2}\t_2$;
\item  If $\exists \s . \; \t_1 ; (\s \piu \id{}) \mathrel{\precongB} (\s \piu \id{}) ; \t_2$, then $\trace_{S_1}\t_1 \mathrel{\precongB} \trace_{S_2}\t_2$.
\end{enumerate}
\end{lemma}
\begin{proof}
As the conclusions are identical, its enough to prove the equivalence of the premises.
\begin{itemize}
\item We prove that 1 entails 2. Assume that $\exists \s_1,\s_2$ such that (a) $\s_2 \mathrel{\precongB} \s_1$ and (b) $\t_1 ; (\s_1 \piu \id{}) \mathrel{\precongB} (\s_2 \piu \id{}) ; \t_2$. Thus:
\[ \t_1 ; (\s_2 \piu \id{}) \stackrel{(a)}{\mathrel{\precongB}} \t_1 ; (\s_1 \piu \id{}) \stackrel{(b)}{\mathrel{\precongB}} (\s_2 \piu \id{}) ; \t_2\]
Observe that by replacing $\s_2$ by $\s$ in the above, one obtains exactly 2.
\item We prove that 2 entails 1. Assume that 2 holds. Then 1 holds by taking both $\s_1$ and $\s_2$ to be $\s$.
\end{itemize}
\end{proof}
\end{comment}


==> oldsections/sections/cb2.tex <==
\section{Cartesian Bicategories}\label{sc:cb:background}

In Section~\ref{sec:2monREL} we gave the definition of cartesian bicategory (Definition~\ref{def:cartesian bicategory}). In this section we recall some of its properties that will be useful later on.

\begin{proposition}\label{prop:dagger}
    Let $\Cat{C}$ be a cartesian bicategory. There is an identity on objects isomorphism $\op{(\cdot)} \colon \Cat{C} \to \opcat{\Cat{C}}$ defined for all arrows $f \colon X \to Y$ as 
    \begin{equation}\label{def:dagger}\tag{\dag}
        \op{f} \defeq \stringOp{\scriptstyle f}{X}{Y}.
    \end{equation}
    Moreover, $\op{(\cdot)}$ is an isomorphism of cartesian bicategories, i.e. the laws in Table~\ref{table:re:daggerproperties} hold.
\end{proposition}
\begin{proof}
    See Theorem 2.4 in~\cite{Carboni1987}.
\end{proof}

\begin{table}[ht!]
    \centering
    % {\tiny
    $
    \begin{array}{@{}c@{\quad}c@{\quad}c@{\quad}c@{}}
        \toprule
        \multicolumn{2}{c}{
            \text{if } f \leq g \text{ then }\op{f} \leq \op{g}
        }
        &
        \multicolumn{2}{c}{
            \op{(\op{f})}= f
        }
        \\[4pt]
    \op{(f ; g)} = \op{g} ; \op{f}
    &\;\;\op{(\id{X})}=\id{X}
    &\;\;\op{(\cocopier{X})}= \copier{X}
    &\;\;\op{(\codischarger{X})}= \discharger{X}
    \\[4pt]
    \op{(f \perG g)} = \op{f} \perG \op{g}
    &\;\;\op{(\sigma^{\odot}_{X,Y})} = \sigma^{\odot}_{Y,X}
    &\;\;\op{(\copier{X})}= \cocopier{X}
    &\;\;\op{(\discharger{X})}= \codischarger{X}
    \\[4pt]
    \bottomrule
    \end{array}
    $
    % }
    \caption{Properties of $\op{(\cdot)} \colon \Cat{C} \to \opcat{\Cat{C}}$}\label{table:re:daggerproperties}
\end{table}

\begin{remark}
    From now on, we will depict a morphism $f \colon X \to Y$ as $\stringBox{f}{X}{Y}$, and use $\stringBoxOp{f}{X}{Y}$ as syntactic sugar for $\op{f}$.
\end{remark}

% \ale{Forse questo proposizione non è importante}
% \begin{proposition}
%     Let $i \colon \Cat{C} \to \Cat{D}$ be a morphism of cartesian bicategories. Then, for all $f \colon X \to Y$, $\op{i(f)} = i(\op{f})$.
% \end{proposition}
% \begin{proof}
%     See Remark 2.9 in~\cite{Carboni1987}.
% \end{proof}


\begin{definition}
    In a cartesian bicategory $\Cat{C}$, an arrow $f \colon X \to Y$ is said to be \emph{single valued} iff satisfies~\eqref{eq:cb:sv}, \emph{total} iff satisfies~\eqref{eq:cb:tot}, \emph{injective} iff satisfies~\eqref{eq:cb:inj} and \emph{surjective} iff satisfies~\eqref{eq:cb:sur}. A \emph{map} is an arrow that is both single valued and total. Similarly, a \emph{comap} is an arrow that is both injective and surjective.
    
    \smallskip


    {
    \noindent\begin{minipage}{0.48\linewidth}
        \begin{equation}\label{eq:cb:sv}\tag{SV}
            \tikzfig{cb/sv/lhs} \leq \tikzfig{cb/sv/rhs}
        \end{equation}
    \end{minipage}
    \begin{minipage}{0.48\linewidth}
        \begin{equation}\label{eq:cb:adj:sv}
            \stringSpan{f}{Y} \leq \stringId{Y}
        \end{equation}
    \end{minipage}
    
    \noindent\begin{minipage}{0.48\linewidth}
        \begin{equation}\label{eq:cb:tot}\tag{TOT}
             \tikzfig{cb/tot/lhs} \leq \tikzfig{cb/tot/rhs}
        \end{equation}
    \end{minipage}
    \begin{minipage}{0.48\linewidth}
        \begin{equation}\label{eq:cb:adj:tot}
            \stringId{X} \leq \stringCospan{f}{X}
        \end{equation}
    \end{minipage}

    
    \noindent\begin{minipage}{0.48\linewidth}
        \begin{equation}\label{eq:cb:inj}\tag{INJ}
            \tikzfig{cb/inj/lhs} \leq \tikzfig{cb/inj/rhs}
        \end{equation}
    \end{minipage}
    \begin{minipage}{0.48\linewidth}
        \begin{equation}\label{eq:cb:adj:inj}
            \stringCospan{f}{X} \leq \stringId{X}
        \end{equation}
    \end{minipage}
    
    \noindent\begin{minipage}{0.48\linewidth}
        \begin{equation}\label{eq:cb:sur}\tag{SUR}
            \tikzfig{cb/sur/lhs} \leq \tikzfig{cb/sur/rhs}
        \end{equation}
    \end{minipage}
    \begin{minipage}{0.48\linewidth}
        \begin{equation}\label{eq:cb:adj:sur}
            \stringId{Y} \leq \stringSpan{f}{Y}
        \end{equation}
    \end{minipage}
    }
\end{definition}

\begin{lemma}\label{lemma:cb:adjoints}
    In a cartesian bicategory $\Cat{C}$, an arrow $f \colon X \to Y$ is single valued iff~\eqref{eq:cb:adj:sv}, it is total iff~\eqref{eq:cb:adj:tot}, it is injective iff~\eqref{eq:cb:adj:inj} and it is surjective iff~\eqref{eq:cb:adj:sur}. In particular, an arrow is a map iff it has a right adjoint, namely $f \dashv \op{f}$; and it is a comap iff it has a left adjoint, namely $\op{f} \dashv f$.
\end{lemma}
\begin{proof}
    See Lemma 4.4 in~\cite{Bonchi2017c}.
\end{proof}

In any cartesian bicategory, one can define a convolution monoid for all objects $X,Y$ and arrows $f,g$ as
\begin{equation}\label{eq:cb:covolution}
    f \sqcap g \defeq \stringCBConvolution{f}{g}{X}{Y} \quad \text{(i.e., $\copier{X}; f \per g ;\cocopier{Y}$)} \quad\qquad \top \defeq \stringBottom{X}{Y} \quad \text{(i.e., $\discharger{X};\codischarger{Y}$).}
\end{equation}

However, unlike the case of fb categories with idempotent convolution, cartesian bicategories are not enriched over $\CMon$. In particular, each homset carries a commutative monoid structure, i.e. the laws in~\eqref{eq:cmon laws} hold; but the laws in \eqref{eq:cmon enrichment} hold only laxly, namely 
\begin{equation}
    (f \sqcap g);h \leq (f;h \sqcap g;h)
    \qquad
    h;(f \sqcap g) \leq (h;f \sqcap h;g)
    \qquad
    f ; \top \leq \top \geq \top ; f
\end{equation}

Given that the structure defined in~\eqref{eq:cb:covolution} is an idempotent monoid, and using the third inequality above, it is easy to see that each homset of a cartesian bicategory form a meet-semilattice with top.
In particular, the following holds for every arrow $f \colon X \to Y$:
\[
    \begin{tikzpicture}[scale=1.5]
        \begin{pgfonlayer}{nodelayer}
            \node [style=none] (117) at (-1, 0) {};
            \node [style=label] (118) at (-1.5, 0) {$X$};
            \node [style=bbox, scale=0.9] (120) at (0, 0) {$f$};
            \node [style=none] (121) at (1, 0) {};
            \node [style=label] (122) at (1.5, 0) {$Y$};
        \end{pgfonlayer}
        \begin{pgfonlayer}{edgelayer}
            \draw (120) to (117.center);
            \draw (120) to (121.center);
        \end{pgfonlayer}
    \end{tikzpicture}
    =
    \begin{tikzpicture}[scale=1.5]
        \begin{pgfonlayer}{nodelayer}
            \node [style=none] (117) at (-1, 0) {};
            \node [style=label] (118) at (-1.5, 0) {$X$};
            \node [style=bbox, scale=0.9] (120) at (0, 0) {$f$};
            \node [style=none] (121) at (2, 0) {};
            \node [style=label] (122) at (2.5, 0) {$Y$};
        \end{pgfonlayer}
        \begin{pgfonlayer}{edgelayer}
            \draw (120) to (117.center);
            \draw (120) to (121.center);
        \end{pgfonlayer}
    \end{tikzpicture}        
    \leq 
    \begin{tikzpicture}[scale=1.5]
        \begin{pgfonlayer}{nodelayer}
            \node [style=none] (117) at (-1.5, 0) {};
            \node [style=label] (118) at (-2, 0) {$X$};
            \node [style=bbox, scale=0.9] (120) at (0, 0) {$f$};
            \node [style=none] (121) at (2.5, 0) {};
            \node [style=label] (122) at (3, 0) {$Y$};
            \node [style=black] (123) at (1, 0) {};
            \node [style=black] (124) at (1.75, 0) {};
        \end{pgfonlayer}
        \begin{pgfonlayer}{edgelayer}
            \draw (120) to (117.center);
            \draw (123) to (120);
            \draw (124) to (121.center);
        \end{pgfonlayer}
    \end{tikzpicture}     
    \leq
    \begin{tikzpicture}[scale=1.5]
        \begin{pgfonlayer}{nodelayer}
            \node [style=none] (117) at (-1.25, 0) {};
            \node [style=label] (118) at (-1.75, 0) {$X$};
            \node [style=none] (121) at (1, 0) {};
            \node [style=label] (122) at (1.5, 0) {$Y$};
            \node [style=black] (128) at (-0.5, 0) {};
            \node [style=black] (129) at (0.25, 0) {};
        \end{pgfonlayer}
        \begin{pgfonlayer}{edgelayer}
            \draw (129) to (121.center);
            \draw (117.center) to (128);
        \end{pgfonlayer}
    \end{tikzpicture}    
\]
and the order on the homsets coincides with the one defined by the semilattice structure.

\begin{lemma}
    In a cartesian bicategory, $f \leq g$ iff $f \sqcap g = f$ for all $f,g \colon X \to Y$.
\end{lemma}
\begin{proof}
    See Lemma 4.13 in~\cite{Bonchi2017c}.
\end{proof}

% \subsection{Coreflexives in Cartesian Bicategories}

% In this section we recall the notion of \emph{coreflexive} morphisms in cartesian bicategories, along with some of their key properties. Recall that a relation $R \subseteq X \times X$ is called reflexive whenever $\id{X} \subseteq R$. Dually, $R$ is said to be coreflexive when $R \subseteq \id{X}$. The concept of coreflexive relation is abstracted in cartesian bicategories as expected.

% \begin{definition}
%     In a cartesian bicategory, a morphism $f \colon X \to X$ is a \emph{coreflexive} if $f \leq \id{X}$.
% \end{definition}

% \begin{lemma}\label{lemma:coreflexive properties}
%     In a cartesian bicategory, the following hold for all coreflexives $f,g \colon X \to X$:
%     \begin{enumerate}
%         \item $\tikzfig{coreflexive/copyR} = \tikzfig{coreflexive/Rcopy}$,
%         % \item 
%         % $\tikzfig{coreflexive/copyR} = \tikzfig{coreflexive/Rcopy}, \quad
%         % \tikzfig{coreflexive/cocopyR} = \tikzfig{coreflexive/Rcocopy},$
%         % \item[]
%         % $\tikzfig{coreflexive/copyROp} = \tikzfig{coreflexive/ROpcopy}, \quad
%         % \tikzfig{coreflexive/cocopyROp} = \tikzfig{coreflexive/ROpcocopy}$
%         \item $f ; g = f \sqcap g$,
%         \item $f$ is transitive, i.e. $f ; f = f$,
%         \item $f$ is symmetric, i.e. $f = \op{f}$,
%         \item $f$ is single valued,
%         \item $f$ is injective.
%     \end{enumerate}
%      Moreover, the following hold in any cartesian bicategory \(\Cat{C}\):
%      \begin{enumerate}
%         \setcounter{enumi}{6}
%         \item there is an isomorphism $\mathsf{Corefl}(\Cat{C})[X, X] \cong \Cat{C}[I, X]$, where $\mathsf{Corefl}(\Cat{C})$ is the subcategory of $\Cat{C}$ whose morphisms are all and only the coreflexives,
%         % \item coreflexives $f \colon X \to X$ are in one-to-one correspondence with morphisms of type $I \to X$,
%         \item for all morphims $f \colon I \to X$ and coreflexives $g \colon X \to X$, $f ; g = f \sqcap g'$, where $g' \colon I \to X$ is the morphism corresponding to $g$ via the isomorphism above,
%         \item for all morphisms $f \colon X \to X$, if $f$ is transitive, symmetric and single valued, then $f$ is a coreflexive.
%     \end{enumerate}
% \end{lemma}
% \begin{proof}
%     \begin{enumerate}
%         \item We prove the two inclusions separately: 
%         \[ \tikzfig{coreflexive/Rcopy} \stackrel{\eqref{ax:copiernat}}{\leq} \tikzfig{coreflexive/1/step1} \stackrel{(\text{coreflexive})}{\leq} \tikzfig{coreflexive/copyR} \]
%         and
%         \[ \tikzfig{coreflexive/copyR} \stackrel{\text{\cite[Lemma 4.3]{Bonchi2017c}}}{\leq} \tikzfig{coreflexive/1/step2} \stackrel{(\text{coreflexive})}{\leq} \tikzfig{coreflexive/Rcopy}. \]
%         \item $\tikzfig{coreflexive/2/step1} \stackrel{\eqref{ax:specfrob}}{=} \tikzfig{coreflexive/2/step2} \stackrel{(1)}{=} \tikzfig{coreflexive/2/step3} \stackrel{(\sqcap-\text{comm.})}{=} \tikzfig{coreflexive/2/step4} \stackrel{(1)}{=} \tikzfig{coreflexive/2/step5}$.
%         \item $\tikzfig{coreflexive/3/step1} \stackrel{(2)}{=} \tikzfig{coreflexive/3/step2} \stackrel{(\sqcap-\text{idemp.})}{=} \tikzfig{coreflexive/3/step3}$.
%         \item $\tikzfig{coreflexive/4/step1} \stackrel{\eqref{def:dagger}}{=} \tikzfig{coreflexive/4/step2} \stackrel{(1)}{=} \tikzfig{coreflexive/4/step3} \stackrel{(1)}{=} \tikzfig{coreflexive/4/step4} \stackrel{\eqref{ax:frob}}{=} \tikzfig{coreflexive/4/step5} \stackrel{\eqref{ax:copierun}, \eqref{ax:cocopierun}}{=} \tikzfig{coreflexive/3/step3}$.
%         \item $\tikzfig{coreflexive/5/step1} \stackrel{(4)}{=} \tikzfig{coreflexive/5/step2} \!\!\stackrel{(\text{coreflexive})}{\leq}\!\! \tikzfig{coreflexive/5/step3}$. Thus $f$ is single valued by means of \Cref{lemma:cb:adjoints}.
%         \item $\tikzfig{coreflexive/6/step1} \stackrel{(4)}{=} \tikzfig{coreflexive/5/step2} \!\!\stackrel{(\text{coreflexive})}{\leq} \!\! \tikzfig{coreflexive/5/step3}$. Thus $f$ is injective by means of \Cref{lemma:cb:adjoints}.
%         \item Consider the functions $i \colon \mathsf{Corefl}(\Cat{C})[X, X] \to \Cat{C}[I, X]$ and $c \colon \Cat{C}[I, X] \to \mathsf{Corefl}(\Cat{C})[X, X]$ defined as follows: %$i \colon \mathsf{Corefl}(\Cat{C})[X,X] \to \Cat{C}[I,X]$ and $c \colon \Cat{C}[I,X] \to \mathsf{Corefl}(\Cat{C})[X,X]$ defined as follows:
%             \[ i(\tikzfig{coreflexive/7/f}) \defeq \tikzfig{coreflexive/7/Cf} \qquad\qquad c(\;\tikzfig{coreflexive/7/g}) \defeq \tikzfig{coreflexive/7/Cg}  \]
%         and observe that $c(\, \tikzfig{coreflexive/7/g} \!)$ is a coreflexive, i.e.
%         \[ c( \, \tikzfig{coreflexive/7/g} \!) = \tikzfig{coreflexive/7/Cg} \stackrel{\eqref{ax:dischargernat}}{\leq} \tikzfig{coreflexive/7/step1} \stackrel{\eqref{ax:cocopierun}}{=} \tikzfig{coreflexive/5/step3}.  \]
%         To conclude, observe that $i$ and $c$ are inverse to each other:
%         \[ i(c(\, \tikzfig{coreflexive/7/g} \!)) = i(\tikzfig{coreflexive/7/Cg}) = \tikzfig{coreflexive/7/step2} \stackrel{\eqref{ax:cocopierun}}{=} \tikzfig{coreflexive/7/g} \]
%         and
%         \[ c(i(\! \tikzfig{coreflexive/7/f} \!)) = c(\, \tikzfig{coreflexive/7/Cf} \!) = \tikzfig{coreflexive/7/step3} \stackrel{(1)}{=} \tikzfig{coreflexive/7/step4} \stackrel{\eqref{ax:cocopierun}}{=} \tikzfig{coreflexive/7/f}. \]
%         \item $\begin{tikzpicture}[scale=1.5]
%             \begin{pgfonlayer}{nodelayer}
%                 \node [style=label] (110) at (2.25, 0) {$X$};
%                 \node [style=none] (117) at (1.75, 0) {};
%                 \node [style=black] (121) at (1.25, 0) {};
%                 \node [style=none] (122) at (0.75, -0.375) {};
%                 \node [style=none] (123) at (0.75, 0.375) {};
%                 \node [style=none] (125) at (0.25, -0.375) {};
%                 \node [style=bbox, scale=0.9] (127) at (0.25, 0.375) {$f$};
%                 \node [style=bbox, scale=0.9] (128) at (0.25, -0.375) {$g'$};
%             \end{pgfonlayer}
%             \begin{pgfonlayer}{edgelayer}
%                 \draw [bend left] (123.center) to (121);
%                 \draw [bend left] (121) to (122.center);
%                 \draw (125.center) to (122.center);
%                 \draw (121) to (117.center);
%                 \draw (123.center) to (127);
%             \end{pgfonlayer}
%         \end{tikzpicture}
%         \stackrel{(7)}{=}
%         \begin{tikzpicture}[scale=1.5]
%             \begin{pgfonlayer}{nodelayer}
%                 \node [style=label] (110) at (2.25, 0) {$X$};
%                 \node [style=none] (117) at (1.75, 0) {};
%                 \node [style=black] (121) at (1.25, 0) {};
%                 \node [style=none] (122) at (0.75, -0.375) {};
%                 \node [style=none] (123) at (0.75, 0.375) {};
%                 \node [style=none] (125) at (-0.5, -0.375) {};
%                 \node [style=bbox, scale=0.9] (127) at (0.25, 0.375) {$f$};
%                 \node [style=bbox, scale=0.9] (128) at (0.25, -0.375) {$g$};
%                 \node [style=black] (129) at (-0.5, -0.375) {};
%             \end{pgfonlayer}
%             \begin{pgfonlayer}{edgelayer}
%                 \draw [bend left] (123.center) to (121);
%                 \draw [bend left] (121) to (122.center);
%                 \draw (125.center) to (122.center);
%                 \draw (121) to (117.center);
%                 \draw (123.center) to (127);
%             \end{pgfonlayer}
%         \end{tikzpicture}        
%         \stackrel{(1)}{=}
%         \begin{tikzpicture}[scale=1.5]
%             \begin{pgfonlayer}{nodelayer}
%                 \node [style=label] (110) at (3.25, 0) {$X$};
%                 \node [style=none] (117) at (2.75, 0) {};
%                 \node [style=black] (121) at (1.25, 0) {};
%                 \node [style=none] (122) at (0.75, -0.375) {};
%                 \node [style=none] (123) at (0.75, 0.375) {};
%                 \node [style=none] (125) at (-0.5, -0.375) {};
%                 \node [style=bbox, scale=0.9] (127) at (0.25, 0.375) {$f$};
%                 \node [style=bbox, scale=0.9] (128) at (2, 0) {$g$};
%                 \node [style=black] (129) at (-0.5, -0.375) {};
%             \end{pgfonlayer}
%             \begin{pgfonlayer}{edgelayer}
%                 \draw [bend left] (123.center) to (121);
%                 \draw [bend left] (121) to (122.center);
%                 \draw (125.center) to (122.center);
%                 \draw (121) to (117.center);
%                 \draw (123.center) to (127);
%             \end{pgfonlayer}
%         \end{tikzpicture}
%         \stackrel{\eqref{ax:cocopierun}}{=}
%         \begin{tikzpicture}[scale=1.5]
%             \begin{pgfonlayer}{nodelayer}
%                 \node [style=label] (120) at (1.75, 0) {$X$};
%                 \node [style=none] (122) at (-0.5, 0) {};
%                 \node [style=none] (125) at (1.25, 0) {};
%                 \node [style=bbox, scale=0.9] (139) at (-0.5, 0) {$f$};
%                 \node [style=bbox, scale=0.9] (140) at (0.5, 0) {$g$};
%             \end{pgfonlayer}
%             \begin{pgfonlayer}{edgelayer}
%                 \draw (125.center) to (122.center);
%             \end{pgfonlayer}
%         \end{tikzpicture}                
%         $. %Consider the coreflexive $c(f) \colon X \to X$ corresponding to $f$. Now observe that $c(f) ; g \stackrel{(2)}{=} c(f) \sqcap g$. \ale{DA finire per bene }
%         \item $\tikzfig{coreflexive/3/step3} \stackrel{(\text{transitive})}{=} \tikzfig{coreflexive/5/step2} \stackrel{(\text{symmetric})}{=} \tikzfig{coreflexive/5/step1} \stackrel{(\text{single valued})}{\leq} \tikzfig{coreflexive/5/step3}$.
%     \end{enumerate}
% \end{proof}

% \begin{remark}\label{rem:notation-coreflexives}
%     From now on we will use $\stringCorefl{f}{X}$ to depict coreflexive morphisms. This graphical representation is, in some sense, orientation agnostic, and it reflects the fact that coreflexives are symmetric, as stated by \Cref{lemma:coreflexive properties}.4.
% \end{remark}


==> oldsections/sections/cdfbrig.tex <==
%
%
%
% \begin{definition}\label{def:distributive_monoidal}
%    A \emph{distributive monoidal} category is an fc-rig category.
% \end{definition}



\subsection{Finite Coproduct-Copy Discard Rig categories }\label{sec:fccdrig}
In Section~\ref{sec:CD}, we have seen how copy discard categories generalise finite product categories. Here, we introduce finite coproduct-copy discard rig categories that, similarly, generalise finite coproduct-finite product rig categories in Definition~\ref{def:fcfprig}.


 \begin{definition}\label{def: distributive gs-monoidal category}
    A \emph{finite coproduct-copy discard (fc-cd) rig category} is a rig category $(\Cat{C}, \piu, \zero, \per, \uno)$ where every object $X$ is equipped with morphisms $\copier{X} \colon X \to X \per X$, $\discharger{X} \colon X \to \uno$, $\codiag{X}\colon X \piu X \to X$ and $\cobang{X} \colon \zero \to X$ such that
     \begin{center}
    (a) $(\Cat{C}, \piu, \zero, \codiag{}, \cobang{})$ is a fc category, \hspace{1cm}  (b) $(\Cat{C}, \per, \uno, \copier{}, \discharger{})$ is a cd category and
    \end{center}        
   %\begin{minipage}{0.5\textwidth}\noindent
   % \begin{itemize}
   % \item $(\Cat{C}, \piu, \zero, \codiag{}, \cobang{})$ is a fc category,
   % \end{itemize}
   % \end{minipage}
   % \begin{minipage}{0.5\textwidth}
   % \begin{itemize}
   %     \item $(\Cat{C}, \per, \uno, \copier{}, \discharger{})$ is a cd category and
   % \end{itemize}
   % \end{minipage}
     (c) monoids and comonoids interact according to the following coherence condition (see also Fig.~\ref{fig:cohfccd}). %$\copier{}$ and $\discharger{}$ satisfy the following coherence conditions. \marginpar{$\lambda$ e $\rho$ should be $-$, also the objects seems to be inverted}
\begin{equation}\label{equation: coherence1}%\label{equation: coherence2}
           \discharger{X\oplus Y}=(\discharger{X} \oplus \discharger{Y});\codiag{\uno} \; \;
 \copier{X\oplus Y}=(\Irunitp{X}\piu\Ilunitp{Y} ); ((\copier{X} \oplus \cobang{X\per Y}) \oplus( \cobang{Y \per X} \oplus \copier{Y}));(\Idl{X}{X}{Y}\oplus \Idl{Y}{X}{Y}); (\Idr{X}{Y}{X\oplus Y})
\end{equation}  
   %         \begin{equation}\label{equation: coherence2}
   %             \end{equation}
A morphism of fc-cd rig categories is a rig functor preserving monoids and comonoids. %\marginpar{Check later if the definition of morphism is really needed}
\end{definition}







\begin{figure}
\[% https://q.uiver.app/#q=WzAsNixbMCwwLCJYXFxwaXUgWSJdLFsyLDAsIihYXFxwaXUgWSkgXFxwZXJHIChYXFxwaXUgWSkiXSxbMCwxLCIoWFxccGl1IDAgKSBcXHBpdSBZIl0sWzAsMiwiKFhcXHBpdSAwICkgXFxwaXUgKDAgXFxwaXUgWSkiXSxbMiwyLCIoKFhcXHBlckcgWCkgXFxwaXUgKFhcXHBlckcgWSkpIFxccGl1ICgoWVxccGVyRyBYKSBcXHBpdSAoWSBcXHBlckcgWSkpIl0sWzIsMSwiKFggXFxwZXJHIChYXFxwaXUgWSkpXFxwaXUgKFlcXHBlckcgKFhcXHBpdSBZKSkiXSxbMCwxLCJcXGRpYWd7WFxccGl1IFl9Il0sWzAsMiwiXFxsYW1iZGEgXFxwaXUgXFxpZHtZfSIsMl0sWzIsMywiXFxpZHtYIFxccGl1IDB9IFxccGl1IFxccmhvIiwyXSxbMyw0XSxbNCw1LCIoXFxJZGx7WH17WH17WX1cXG9wbHVzIFxcSWRse1l9e1h9e1l9KSIsMl0sWzUsMSwiKFxcSWRye1h9e1l9e1hcXG9wbHVzIFl9KSIsMl1d
\begin{tikzcd}
	{X\piu Y} && {(X\piu Y) \per (X\piu Y)} \\
	 && {(X \per (X\piu Y))\piu (Y\per (X\piu Y))} \\
	{(X\piu 0 ) \piu (0 \piu Y)} && {((X\per X) \piu (X\per Y)) \piu ((Y\per X) \piu (Y \per Y))}
	\arrow["{\copier{X\piu Y}}", from=1-1, to=1-3]
	\arrow["{\Irunitp{X}\piu\Ilunitp{Y}  }"', from=1-1, to=3-1]
	%\arrow["{\id{X \piu 0} \piu }"', from=2-1, to=3-1]
	\arrow["{(\Idr{X}{Y}{X\oplus Y})}"', from=2-3, to=1-3]
	\arrow["(\copier{X} \oplus \cobang{X\per Y}) \oplus( \cobang{Y \per X} \oplus \copier{Y})"',from=3-1, to=3-3]
	\arrow["{(\Idl{X}{X}{Y}\oplus \Idl{Y}{X}{Y})}"', from=3-3, to=2-3]
\end{tikzcd}
\qquad
% https://q.uiver.app/#q=WzAsMyxbMCwwLCJYIFxccGl1IFkiXSxbMSwwLCJcXHVub0cgXFxwaXUgXFx1bm9HIl0sWzEsMSwiXFx1bm9HIl0sWzAsMiwiXFxiYW5ne1hcXHBpdSBZfSIsMl0sWzEsMl0sWzAsMSwiXFxiYW5ne1h9XFxwaXUgXFxiYW5ne1l9Il1d
\begin{tikzcd}
	{X \piu Y} & {\uno \piu \uno} \\
	& \uno
	\arrow["{\discharger{X}\piu \discharger{Y}}", from=1-1, to=1-2]
	\arrow["{\discharger{X\piu Y}}"', from=1-1, to=2-2]
	\arrow["{\codiag{\uno}}", from=1-2, to=2-2]
\end{tikzcd} \]
\caption{Diagrams for the coherence conditons in \eqref{equation: coherence1}.}\label{fig:cohfccd}%\marginpar{Si Riesce a Mettere il diagramma in basso a destra?}
\end{figure}



The coherence conditions in \eqref{equation: coherence1} will be fundamental in Section~\ref{sc:tapeTcd} for the diagrammatic language that we are going to introduce. Moreover, they guarantee several useful properties.



\begin{proposition}\label{prop:map}
    Let $\Cat{C}$ be a fc-cd rig category. Then, for all objects $X$, the followings hold:
    \begin{enumerate}
    \item $\codiag{X};\copier{X}= (\copier{X}\piu\copier{X});\codiag{X \per X}$,  $\quad \codiag{X};\discharger{X}=(\discharger{X} \piu \discharger{X});\codiag{\uno}$,
    $\quad \cobang{X};\copier{X}= ;\cobang{X \per X} \;$ and $\quad \cobang{X};\discharger{X}=\cobang{\uno}$; 
    \item Both $\codiag{X}$ and $\cobang{X}$ are functional and total, i.e., 
    \[\codiag{X};\copier{X}= \copier{X\piu X};(\codiag{X}\per \codiag{X})\text{,} \quad \codiag{X};\discharger{X}= \discharger{X\piu X}\text{,} \quad \cobang{X};\copier{X}= \copier{\zero};(\cobang{X}\per \cobang{X}) \quad \text{and} \quad \cobang{X};\discharger{X}= \discharger{\zero}\text{;} \]
    \item The category $\mathrm{Map}(\Cat{C})$ is a finite coproduct-finite product rig category.
    \end{enumerate}
  \end{proposition} 
%
%
%
Note that in the last point, $\mathrm{Map}(\Cat{C})$ is defined as for cd categories in Section~\ref{sec:fccdrig}. Again, the hard part of the proof consists in showing that the distributors are functional and total.



%\marginpar{Questo insieme a tutte le prove che usano esplicitamente la properieta' universale di coprodotto e prodotto, le metterei in appendice}
%Given $f \colon X\to Z$ and $g:Y\to Z$, we shall sometimes adopt the standard notation $[f,g]:X\piu Y\to Z$, used in finite coproducts categories,  for the composition $(f\piu g);\codiag{Z}$. And also $\linj{X}:X\to X\piu Y$ and $\rinj{Y}:Y\to X\piu Y$ for the arrows $\runitp{X};(\id{X}\piu \bang{Y})$ and $\lunitp{Y};(\bang{X}\piu \id{Y})$.


\begin{lemma}\label{lemma:distributive}
    Every fc-fp rig category is a fc-cd rig category.
\end{lemma}

In Proposition~\ref{prop: Kleisli of distributive monoidal}, we have seen that for a commutative monad $T$ over a finite coproduct rig category, its Kleisli category $\Cat{C}_T$ is again a finite coproduct rig category. By Proposition~\ref{prop: Kleisli gs e cogs},  $\Cat{C}_T$ is also a cd category. It turns out that it is a fc-cd category.

\begin{proposition}\label{prop:Kleislifccd}
        Let $(\Cat{C},\piu,\zero,\per, \uno)$ be a fc-cd rig category and $T \colon \Cat{C}\to \Cat{C}$ be a symmetric monoidal monad over $(\Cat{C},\per, \uno)$. Then the Kleisli category $\Cat{C}_T$ is fc-cd rig.
\end{proposition}


Since $\Cat{Set}$ is a finite coproduct-finite product rig category, by Lemma~\ref{lemma:distributive} and Proposition~\ref{prop:Kleislifccd}, the Kleisli category $\Cat{Set}_T$ of any symmetric monoidal monad over $(\Cat{Set}, \times, \uno)$ is a fc-cd rig category.




==> oldsections/sections/cdsigmaerig.tex <==


\subsection{$\mathbb{T}$-Copy Discard Rig Categories}

With no surprise, we can combine fc-cd categories (Definition~\ref{def: distributive gs-monoidal category}) with algebraic theories.

 \begin{definition}\label{def: T distributive gs-monoidal category}
 A $\mathbb{T}$-rig category  $i\colon \opcat{\lawveret} \to \Cat{C}$ is a \emph{$\mathbb{T}$-copy discard (shortly $\mathbb{T}$-cd) rig category} if $\Cat{C}$ is a fc-cd rig category.
 A morphism of $\mathbb{T}$-cd rig categories is a both a morphisms of $\mathbb{T}$ rig and fc-cd rig categories.
\end{definition}

Our main example of $\mathbb{T}$-copy discard rig category is provided by $i\colon \opcat{\lawveret} \to \Cat{Set}_{T_{\mathbb{T}}}$ in \eqref{eq:Lawdiag}. % is a $\mathbb{T}$-rig category.
\begin{proposition}\label{prop:kleisliTrig}
Let $\mathbb{T}$ be an algebraic theory such that $T_{\mathbb{T}}$ is a symmetric monoidal monad. Then $\Sets_{T_{\mathbb{T}}}$ is a $\mathbb{T}$-copy discard rig category.
\end{proposition}
%
Since $\subdistr$ is a symmetric monoidal monad (Example~\ref{ex:monoidal monads}) and $\mathbb{PCA}$ presents $\subdistr$, by Proposition~\ref{prop:kleisliTrig}, it holds that the Kleisli category $\Cat{Set}_{\subdistr}$ equipped with the structure in \eqref{ex:products}, \eqref{ex:comonoids} and \eqref{ex:op}, is a $\mathbb{PCA}$-cd rig category. Beyond the examples provided by the above proposition, there are many others.

\begin{example}\label{ex:CM}
%There are many other crucial examples. 
Consider for instance the algebraic theory $\mathbb{CM}$ of commutative monoids that presents the finitary multiset monad $M_f$. Any rig category where $\piu$ is a biproduct, i.e., both a product and a coproduct, is a $\mathbb{CM}$ rig category. The copy-discard structure is present not just in $\Sets_{M_f}$:  the category of vector spaces~\cite{johnson2021bimonoidal}, the one of finite dimension Hilbert spaces~\cite{Coecke2012a,harding2008orthomodularity} and the category of sets and relations~\cite{bonchi2023deconstructing,Bruni01somealgebraic} are all $\mathbb{CM}$-copy discard rig categories.  %\marginpar{Insert Citations} 
\end{example}


%\begin{itemize}
%\item For a commutative monad, Kleisli has both;
%\item tape diagrams can be trivially adjusted by adding copier and discard;
%\item Illustrate that one can define copier and discard for arbitrary polinomial by means of the coherence axioms;
%\item Using tapes, illustrate the enrichment over models of $(\Sigma,E)$;
%\item Considering predicates we have distributivity with the monoid of predicates;
%\end{itemize}


==> oldsections/sections/conclusion.tex <==


\section{Conclusions}

In this work, we have extended the notion of tape diagrams in \cite{bonchi2023deconstructing} to accommodate Kleisli categories of monoidal monads. To achieve this, we introduced fc-cd rig categories (Definition~\ref{def: distributive gs-monoidal category}), which govern the interactions between (natural) $\piu$-monoids and $\per$-comonoids. We then demonstrated that these Kleisli categories naturally form fc-cd rig categories (Proposition~\ref{prop:Kleislifccd}).
%
Furthermore, we observed that when a monoidal monad is equipped with an algebraic presentation $\mathbb{T}=(\Sigma, E)$, the operations in $\Sigma$ induce natural transformations within the Kleisli categories (Proposition~\ref{prop:kleisliTrig}). These monoids, comonoids, and natural transformations enabled us to define a 2-dimensional diagrammatic language for the morphisms of $\algt$-cd rig categories freely generated by a monoidal signature $\Gamma$ (Theorem~\ref{th:tapes-free-T-cd}). Collectively, our results ensure that whenever $\Gamma$ is interpreted within the Kleisli category of a monoidal monad, this interpretation can be uniquely extended to a rig functor from the category of diagrams $\CatTapeTCD[\Gamma][\algt]$. For example, by interpreting Boolean circuits in $\Sets_{\subdistr}$, we obtain a language that captures the expressiveness of \cite{piedeleu2025boolean} while naturally incorporating probabilistic control (Example~\ref{example: probabilistic control}).

This work opens several promising research directions. (a) Extending tape diagrams with monoidal traces for $\piu$ could enable the modeling of iteration and, potentially, the development of program logics akin to \cite{bonchi2024diagrammatic}, but tailored for effectful programs. The necessary constraints on monads could be drawn from \cite{jacobs2010coalgebraic,haghverdi2000categorical}. (b) We aim to further explore the connections with probabilistic Boolean circuits in \cite{piedeleu2025boolean}. Notably, an alternative encoding of the calculus in \cite{piedeleu2025boolean} into $\mathbb{PCA}$-tapes maps each wire to the identity tape of $\objn{2}$. We anticipate that this may clarify links to the theory of \emph{effectus} \cite{introductioneffectus}. (c) Our current approach does not accommodate the monad of convex sets of distributions, as it is not monoidal. To incorporate probability and non-determinism, we may leverage the graded monad from \cite{DBLP:journals/pacmpl/LiellCockS25} and extend tape diagrams for graded monads similarly to the string diagrams in \cite{DBLP:journals/corr/abs-2501-18404}. (d) As discussed in Section \ref{ssec:rig}, $\mathbb{T}$-rig categories are enriched over models of $\mathbb{T}$. Investigating whether our tape diagrams provide a principled approach to enriching string diagrams --such as the one proposed in \cite{villoria2024enriching}-- represents another intriguing avenue for future research.



\begin{comment}
\section{Conclusions}
%
We have generalised tape diagrams in \cite{bonchi2023deconstructing} in order to deal with Kleisli categories of monoidal monads. % presented by some algebraic theory $\mathbb{T}$. 
In order to do this, we have introduced fc-cd rig categories (Definition \ref{def: distributive gs-monoidal category}) ruling the interactions of (natural) $\piu$-monoids and $\per$-comonoids and we have shown that the aforementioned Kleisli categories are indeed fc-cd rig categories (Proposition \ref{prop:Kleislifccd}). Then we have observed that, whenever the monoidal monad comes with an algebraic presentation $\mathbb{T}=(\Sigma, E)$, the operations in $\Sigma$ give rise to natural transformations in the Kleisli categories (Proposition \ref{prop:kleisliTrig}). Monoids, comonoids and such natural transformations allowed us to define a 2-dimensional diagrammatic language for arrows of $\algt$-cd rig categories freely generated by a monoidal signature $\Gamma$ (Theorem \ref{th:tapes-free-T-cd}). All together our results guarantee that, whenever $\Gamma$ is interpreted within the Kleisli category of a monoidal monad, then the intepretation can be uniquely extended to a rig functor from the category of diagrams $\CatTapeTCD[\Gamma][\algt]$: for instance, by interpreting Boolean circuits into \(\Sets_{\subdistr}\), one obtains a language that is able to encode the one in \cite{piedeleu2025boolean} and come with a natural form of probabilistic control (Example \ref{}).

Our work paves the ways to various research directions. (a) By extending tapes with monoidal traces for $\piu$, one would be able to model iterations and, hopefully, obtain program logics in the style of \cite{}, but for programs with effects. The additional constraints to impose on monads should come from \cite{}. (b) We would like to deeply explore the connections with the boolean probabilistic circuits in \cite{piedeleu2025boolean}. Indeed, there exists another possible encoding which takes of the calculus in \cite{piedeleu2025boolean} into $\mathbb{PCA}$-tapes mapping each wire into the identity tape of $\objn{2}$. We expect that this may clarify the connections with the theory of \emph{effectus} \cite{}. (c) Our tapes cannot deal with the monad of convex sets of distributions, since this is not monoidal. In order to deal with probability and non-determinism, we may use the graded monad in \cite{DBLP:journals/pacmpl/LiellCockS25} and thus extend tape diagrams for graded monad similarly to the string diagrams in \cite{DBLP:journals/corr/abs-2501-18404}. (d) As mentioned in Section \ref{},  $\mathbb{T}$ rig categories are enriched over models of $\mathbb{T}$. Understanding whether our tapes allow for a principled solution to enrich string diagrams, such as the one in \cite{}, is another exciting research direction.
\end{comment}


==> oldsections/sections/hoare.tex <==

\begin{comment}
\section{Diagrammatic Program Logics}\label{sec:hoare}



%
%
% COMMENT
%
%
define a simply typed imperative programming language\\
there is a set of basic types \(T_{0}\)\\
and a set of type constructors \(C_{T}\) that contains \(\{\per \colon 2 \to 1, \piu \colon 2 \to 1, I \colon 0 \to 1, \zero \colon 0 \to 1\}\)\\
there is a set of typed variables \(\mathsf{Vars}\)\\
and a set of typed deterministic operations \(\mathsf{Op}\)\\

the set of expressions is defined as\\
\(\mathsf{Expr} \Coloneqq x \mid f(e_{1}, \ldots, e_{n})\)\\
\elena{I am confused by what the typing rules for expressions should be}
\begin{figure}[h!]
  \begin{equation*}
  \begin{array}{c@{\qquad}c@{\qquad}c}
    \inferrule*[right=(var)]{x \colon X}{x \colon X \vdash x \colon X} & \inferrule*[right=(op)]{\Gamma_{j} \vdash e_{j} \colon Y_{j} \quad f \colon Y_{1} \per \cdots \per Y_{n} \to Z}{\Gamma_{1}, \ldots, \Gamma_{n} \vdash f(e_{1}, \ldots, e_{n}) \colon Z} & \inferrule*[right=(weak)]{\Gamma \vdash e \colon Y}{\Gamma, z \colon Z \vdash e \colon Y} \\[12pt]
    \inferrule*[right=(exch)]{\Gamma, x \colon X, y \colon Y, \Delta \vdash e \colon Z}{\Gamma, y \colon Y, x \colon X, \Delta \vdash e \colon Z} & \inferrule*[right=(cont)]{\Gamma, x \colon X, y \colon X \vdash e \colon Z}{\Gamma, x \colon X \vdash e[y/x] \colon Z} & \gets \text{ should these be here?}
  \end{array}
  \end{equation*}
  \caption{Typing rules for expressions.\label{fig:typing-rules-expressions}}
\end{figure}


the set of predicates is defined as\\
\(\mathsf{Pred} \Coloneqq \top \mid \bot \mid e_{1} = e_{2} \mid e_{1} \neq e_{2} \mid P \lor P \mid P \land P \mid \lnot P\)\\
predicates are typed \(p \colon I \to X\) for some type \(X\)\\
add predicate symbols and rule for substitution of expression in a variable\\
add exchange\\
\begin{figure}[h!]
  \begin{equation*}
  \begin{array}{c@{\qquad}c@{\qquad}c@{\qquad}c}
    \inferrule*[right=(top)]{ }{\vdash \top \colon X} & \inferrule*[right=(eq)]{\Gamma \vdash e_{1} \colon Y \quad \Gamma \vdash e_{2} \colon Y}{\vdash (e_{1} = e_{2}) \colon \Gamma} & \inferrule*[right=(and)]{\vdash P \colon X \quad \vdash Q \colon X}{\vdash (P \land Q) \colon X} & \inferrule*[right=(not)]{\vdash P \colon X}{\vdash \lnot P \colon X}\\[12pt]
    \inferrule*[right=(bot)]{ }{\vdash \bot \colon X} & \inferrule*[right=(neq)]{\Gamma \vdash e_{1} \colon Y \quad \Gamma \vdash e_{2} \colon Y}{\vdash (e_{1} \neq e_{2}) \colon \Gamma} & \inferrule*[right=(or)]{\vdash P \colon X \quad \vdash Q \colon X}{\vdash (P \lor Q) \colon X} & \inferrule*[right=(co-weak)]{\vdash P \colon X}{\vdash P \colon X \per Y}
  \end{array}
  \end{equation*}
  \caption{Typing rules for predicates.\label{fig:typing-rules-predicates}}
\end{figure}

the set of statements is defined as\\
\(\mathsf{Prog} = \mathsf{abort} \mid \mathsf{skip} \mid \mathop{\mathsf{if}} P \mathop{\mathsf{then}} C \mathop{\mathsf{else}} D \mid \mathop{\mathsf{while}} P \mathop{\mathsf{do}} C \mid C ; D \mid x \coloneqq E\)\\
\elena{should there be weakening, exchange and contraction?}\\
add typing of composition\\
for while rule types need to have same input and output types\\
\begin{figure}[h!]
  \begin{equation*}
  \begin{array}{c}
    \inferrule*[right=(abort)]{ }{\Gamma \vdash \mathsf{abort} \colon \zero}\\[12pt]
    \inferrule*[right=(assn)]{y \colon Y, \Gamma \vdash e \colon Y}{y \colon Y, x_{1} \colon  X_{1}, \ldots, x_{n} \colon X_{n} \vdash y \coloneqq e \colon Y \per X_{1} \per \cdots \per X_{n}}\\[12pt]
    \inferrule*[right=(whisk)]{\Gamma \vdash C \colon Y_{1} \per \cdots \per Y_{n}}{\Gamma, x \colon X \vdash C \colon Y_{1} \per \cdots \per Y_{n} \per X}\\[12pt]
    \inferrule*[right=(skip)]{ }{x_{1} \colon  X_{1}, \ldots, x_{n} \colon X_{n} \vdash \mathsf{skip} \colon  X_{1} \per \cdots \per X_{n}}\\[12pt]
    \inferrule*[right=(if-else)]{\vdash P \colon X_{1} \per \cdots \per X_{m} \quad x_{1} \colon  X_{1}, \ldots, x_{m} \colon X_{m} \vdash C \colon Y_{1} \per \cdots \per Y_{n} \quad x_{1} \colon  X_{1}, \ldots, x_{m} \colon X_{m} \vdash D \colon Y_{1} \per \cdots \per Y_{n}}{x_{1} \colon  X_{1}, \ldots, x_{m} \colon X_{m} \vdash \mathop{\mathsf{if}} P \mathop{\mathsf{then}} C \mathop{\mathsf{else}} D \colon Y_{1} \per \cdots \per Y_{n}}\\[12pt]
    \inferrule*[right=(while)]{\vdash P \colon X_{1} \per \cdots \per X_{m} \quad x_{1} \colon  X_{1}, \ldots, x_{m} \colon X_{m} \vdash C \colon Y_{1} \per \cdots \per Y_{n}}{x_{1} \colon  X_{1}, \ldots, x_{m} \colon X_{m} \vdash \mathop{\mathsf{while}} P \mathop{\mathsf{do}} C \colon Y_{1} \per \cdots \per Y_{n}}
  \end{array}
  \end{equation*}
  \caption{Typing rules for predicates.\label{fig:typing-rules-predicates}}
\end{figure}
\elena{do we also want generators for the statements? Neither Barthe nor Winskel have them, but nothing really prevents us from adding them}

we define the interpretation of expressions, predicates and statements in \(\KTCB\)\\
we define the signature \(\Sigma\)\\
the set of generators for the objects is the set of basic types \(T_{0}\)\\
the set of generators for morphisms is the set of deterministic operations \(\mathsf{Op}\) together with a relation \(\neq_{X} \colon X \per X \to X\) for every basic type \(X\)\\

we interpret expressions\\
\(\interpret{x : X} \defeq \id{X}\)\\
\(\interpret{f(e_{1}, \ldots, e_{n})} \defeq (\interpret{e_{1}} \per \cdots \per \interpret{e_{n}}) \dcomp f\)\\

we interpret predicates\\
\(\interpret{\top} \defeq \codischarger{}\)\\
\(\interpret{\bot} \defeq \bang{I} \dcomp \cobang{}\)\\
\(\interpret{P \land Q} \defeq\) \includegraphics[scale=0.5]{figures/predicates-intersection.pdf} \\
\(\interpret{P \lor Q} \defeq\) \includegraphics[scale=0.5]{figures/predicates-union.pdf}\\
\(\interpret{e_{1} = e_{2}} \defeq\) \includegraphics[scale=0.5]{figures/expression-equality.pdf}\\
\(\interpret{e_{1} \neq e_{2}} \defeq\) \includegraphics[scale=0.5]{figures/expression-inequality.pdf}\\
\(\interpret{\lnot \top} \defeq \interpret{\bot}\)\\
\(\interpret{\lnot \bot} \defeq \interpret{\top}\)\\
\(\interpret{\lnot (e_{1} = e_{2})} \defeq \interpret{e_{1} \neq e_{2}}\)\\
\(\interpret{\lnot (e_{1} \neq e_{2})} \defeq \interpret{e_{1} = e_{2}}\)\\
\(\interpret{\lnot (P \land Q)} \defeq \interpret{\lnot P \lor \lnot Q}\)\\
\(\interpret{\lnot (P \lor Q)} \defeq \interpret{\lnot P \land \lnot Q}\)\\
\(\interpret{\lnot \lnot P} \defeq \interpret{P}\)\\

we interpret statements\\
\(\interpret{\mathsf{abort}_{X}} \defeq \bang{X}\)\\
\(\interpret{\mathsf{skip}_{X}} \defeq \id{X}\)\\
\(\interpret{\mathop{\mathsf{if}} P \mathop{\mathsf{then}} C \mathop{\mathsf{else}} D} \defeq \)
\includegraphics[scale=0.5]{figures/if-then-else.pdf}\\
\(\interpret{\mathop{\mathsf{while}} P \mathop{\mathsf{do}} C} \defeq\)
\includegraphics[scale=0.5]{figures/while-loop.pdf}\\
\(\interpret{C ; D} \defeq \interpret{C} \dcomp \interpret{D}\)\\
\(\interpret{x \coloneqq e} \defeq\) \includegraphics[scale=0.5]{figures/variable-assignment.pdf}\\


subject to the following equations\\
\((e_{1} = e_{2}) \lor (e_{1} \neq e_{2}) = \top\) and \((e_{1} = e_{2}) \land (e_{1} \neq e_{2}) = \bot\)\\
\includegraphics[scale=0.5]{figures/union-equality-inequality.pdf} \includegraphics[scale=0.5]{figures/intersection-equality-inequality.pdf} \\
from this we can show by induction that \(p \union \lnot p = \top\) and \(p \intersection \lnot p = \bot\)\\
\(e\) is deterministic\\
\includegraphics[scale=0.5]{figures/operations-deterministic.pdf}\\
\elena{the last three derivation rules are in Barthe but not in Winskel. I'm not sure what the last one means}
derivable Hoare triples\\
Hoare derivation rules\\
\begin{figure}[h!]
  \begin{equation*}
  \begin{array}{c@{\qquad}c@{\qquad}c}
    \inferrule*[right=($\mathsf{skip}$)]{ }{\{P\}\mathsf{skip}\{P\}} & \inferrule*[right=(sub)]{ }{\{P[E/x]\}x \coloneqq E\{P\}} & \inferrule*[right=(\(\subseteq\))]{P_1 \subseteq P_2 \quad \{P_2\}C\{Q_2\} \quad Q_2 \subseteq Q_1}{\{P_1\}C\{Q_1\}} \\[12pt]
    \inferrule*[right=(seq)]{\{P\}C\{Q\} \quad \{Q\}D\{R\}}{\{P\}CD\{R\}} & \inferrule*[right=(\(\mathsf{if-else}\))]{\{B \land P\}C\{Q\} \quad \{\lnot B \land P\}D\{Q\}}{\{P\}\mathop{\mathsf{if}} B \mathop{\mathsf{then}} C \mathop{\mathsf{else}} D\{Q\}} & \inferrule*[right=(\(\mathsf{while}\))]{\{P \land B\}C\{P\}}{\{P\}\mathop{\mathsf{while}} B \mathop{\mathsf{do}} C\{\lnot B \land P\}}\\[12pt]
    \inferrule*[right=(excl)]{\{P \land B\}C\{Q\} \quad \{P \land \lnot B\}C\{Q\}}{\{P\}C\{Q\}} & \inferrule*[right=(ind)]{x_{i} \colon X_{i} \vdash C \colon Y_{j} \quad \vdash B \colon Z_{k} \quad \{P\}C\{Q\}}{\{P \land B\}C\{Q \land B\}} & \inferrule*[right=(exist)]{\forall x \colon X \ \{P\}C\{Q\}}{\exists x \colon X \{P\}C\{Q\}}
  \end{array}
  \end{equation*}
  \caption{Hoare derivation rules\label{fig:hoare-rules}}
\end{figure}

\begin{proposition}
  If a Hoare triple \(\{P\}C\{Q\}\) is derivable with the rules in \Cref{fig:hoare-rules}, then \(\interpret{P} \dcomp \interpret{C} \leq \interpret{q}\) in \(\KTCB\).
\end{proposition}
\begin{proof}
  By induction on the deduction rules.\\
  \((\mathsf{skip})\) \(\interpret{P} \dcomp \interpret{\mathsf{skip}} = \interpret{P} \dcomp \id{} = \interpret{P}\).\\
  (SUB)\\
  \includegraphics[scale=0.5]{figures/derive-substitution.pdf}\\
  \((\subseteq)\) \(\interpret{P_{1}} \dcomp \interpret{C} \leq \interpret{P_{2}} \dcomp  \interpret{C} \leq \interpret{Q_{2}} \leq \interpret{Q_{1}}\).\\
  (SEQ) \(\interpret{P} \dcomp \interpret{CD} = \interpret{P} \dcomp \interpret{C} \dcomp \interpret{D} \leq \interpret{Q} \dcomp \interpret{D} \leq \interpret{R}\).\\
  \((\mathsf{if-else})\)\\
  \includegraphics[scale=0.5]{figures/derive-if-else.pdf}\\
  \((\mathsf{while})\)\\
  \includegraphics[scale=0.5]{figures/derive-while.pdf}\\
  (EXCL)\\
  \includegraphics[scale=0.5]{figures/derive-excl.pdf}\\
  (IND)\\
  \includegraphics[scale=0.5]{figures/derive-independent.pdf}\\
  (EXISTS)\\
  \includegraphics[scale=0.5]{figures/derive-exists.pdf}
\end{proof}

\begin{table}[h!]
  \centering
  \begin{tabular}{| c | c c |}
    \toprule
    Logic & Triple & Inequality \\
    \midrule
    Hoare & \(\{P\}C\{Q\}\) & \(p \dcomp c \leq q\)\\
    Incorrectness & \([P]C[Q]\) & \(p \dcomp c \geq q\)\\
    Sufficient incorrectness & \(\lAngle P \rAngle C \lAngle Q \rAngle\) & \(\op{p} \leq c \dcomp \op{q}\)\\
    Necessary & \((P)C(Q)\) & \(\op{p} \geq c \dcomp \op{q}\)\\
    \bottomrule
  \end{tabular}
  \caption{Correspondence between triples and inequalities.\label{tab:triples-inequalities}}
\end{table}
\end{comment}
%
%
% END OF COMMENT
%
%
%
%
%
%
%
%
%
%
%
%
%
%



% \section{PROVA BY PIPPO}


\section{Diagrammatic Hoare Logic}\label{sec:hoare}

In this section we illustrate how Kleene Cartesian tapes can provide a comfortable setting to reason about imperative programs. For the sake of generality, we avoid to fix basic types and operations and, rather, we work parametrically with respect to a triple $(\sort,\mathcal{F},\mathcal{P})$. $\sort$ is a set of sorts, ranging over $A,B,C, \dots$, representing basic types; $\mathcal{F}$ is a set of function symbols, ranging over $f,g,h,\dots$, equipped with an arity in $\sort^\star$ and a coarity in $\sort$. As usual, we write $f\colon U \to A$ to mean that $f$ has arity $U$ and coarity $A$;  $\mathcal{P}$ is a set of predicate symbols, ranging over $P,Q,R,\dots$, equipped only with an arity in $\sort^\star$. The coarity, for all predicate symbols, is fixed to be $1$.

For any predicate symbol $P$, we consider an extra symbol $\bar{P}$, with the same arity of $P$, that will represent its negation. We fix $\bar{\mathcal{P}} \defeq \{\bar{P} \mid P\in \mathcal{P}\}$.
% Moreover, for any $A\in \sort$, we consider an extra symbol $\neq_{A}$ of arity $A \times A$. Intuitively, $\neq_{A}$ is the binary predicate testing difference. We fix $\mathcal{N} \defeq \{\neq_A \mid A \in \sort\}$.
%
We consider the monoidal signature $\sign \defeq \mathcal{F} \cup \mathcal{P} \cup \bar{\mathcal{P}}$. %\cup \mathcal{N}$.
The kc tape theory $\basicR$ contains the following equations for all $f\colon U \to A$ in $\mathcal{F}$
\begin{equation}\label{eq:deterministic-total}
  \tikzfig{hoare/function/step1} = \tikzfig{hoare/function/step2} \qquad \tikzfig{hoare/function/step3} = \tikzfig{hoare/function/step4}
  % \includegraphics[scale=0.5]{figures/operations-deterministic.pdf} \quad \includegraphics[scale=0.5]{figures/operations-total.pdf}
\end{equation}
and for all $P\in \mathcal{P}$,\\
\[
  \!\!\!\!\!\!\!\!\!\tikzfig{hoare/EM/lhs} = \tikzfig{hoare/EM/rhs} \quad\qquad \tikzfig{hoare/NC/lhs} = \tikzfig{hoare/NC/rhs}
\]
% \includegraphics[scale=0.5]{figures/predicate-negation.pdf}\\
These axioms force any model of the theory to interpret symbols in $\mathcal{F}$ as functions and $\bar{P}$ as the complement of $P$.

\begin{remark}
Notice that, in some program logics, function symbols are not forced to be total in order to deal with errors and exceptions like, for instance, division by $0$. One can easily allow symbols in $\mathcal{F}$ to be partial functions by dropping the rightmost axiom in \Cref{eq:deterministic-total}, but we would loose in elegance. In particular, the equality in Lemma \ref{lemma:encodingsubst} will become an inequality and, consequently, the proof of the assignment rule will require some extra work.
\end{remark}

\subsection{Expressions}
As usual, expressions are defined by the following grammar
\[e \Coloneqq x \mid f(e_{1}, \ldots, e_{n})\]
where $f$ is a function symbol in $\mathcal{F}$ and $x$ is a variable taken from some fixed set of variables.

In order to encode expressions into diagrams, we need to make copying and discarding of variables explicit; this is usually kept implicit by traditional syntax. For this reason we define an elementary type systems with judgement of the form
\[\Gamma \vdash e \colon A \]
where $e$ is an expression, $A$ is a sort in $\sort$ and $\Gamma$ is a \emph{typing context}, namely, an ordered sequence $x_1\colon A_1, \dots x_n \colon A_n$ where, all the $x_i$ are distinct variables and $A_i \in \sort$.
The type system consists of the following two rules
\[ \inferrule*[right=(var)]{-}{\Gamma, x \colon A, \Delta \vdash x \colon A} \qquad \inferrule*[right=(op)]{\Gamma \vdash e_{i} \colon A_{i} \quad f \colon A_{1} \per \cdots \per A_{n} \to A}{\Gamma \vdash f(e_{1}, \ldots, e_{n}) \colon A}\]
where $\Gamma$ and $\Delta$ are arbitrary typing contexts.

To encode well typed expressions into diagrams, we first deal with  typing contexts. We fix $\encoding{x_1\colon A_1, \dots , x_n \colon A_n} \defeq A_1 \per \dots  \per A_n$. For any well typed expressions $\Gamma \vdash e \colon A$, $\encoding{\cdot}$ is defined by induction on the two rules above:
\[ \encoding{\Gamma, x \colon A, \Delta \vdash x \colon A} \defeq \discharger{\encoding{\Gamma}} \per \id{A} \per \discharger{\encoding{\Delta}}\qquad \encoding{\Gamma \vdash f(e_{1}, \ldots, e_{n}) \colon A} \defeq \copier{\encoding{\Gamma}}^n ; (\encoding{\Gamma \vdash e_1} \per \dots \per \encoding{\Gamma \vdash e_n} ) ; f\]
where $\copier{U}^n \colon U \to U^n$ is the diagram defined inductively as expected: $\copier{\encoding{\Gamma}}^0 \defeq \discharger{U}$ and $\copier{\encoding{\Gamma}}^{n+1} \defeq \copier{U} ; (\copier{U}^n \per \id{U})$.

Later on, the notion of \emph{substitution} will be crucial. Given two expression $t$ and $e$ and a variable $x$, the expression $e[t / x]$ is defined inductively as follows, where $y$ is a variable different from $x$.
\[x[t / x] \defeq t \qquad y[ t / x]\defeq y \qquad f(e_1, \dots, e_n)[t/x] \defeq f(e_1[t/x], \dots, e_n[t/x] )\]

A simple inductive argument confirms that substitutions types well.

\begin{lemma}
Let $\Gamma ' = \Gamma, x\colon A, \Delta$ for some typing contexts $\Gamma$ and $\Delta$. If $\Gamma' \vdash e\colon B$ and $\Gamma ' \vdash t\colon A$, then $\Gamma' \vdash e[t /x] \colon B$.
\end{lemma}
\begin{proof}
We proceed by induction on $\Gamma' \vdash e\colon B$.

If $e$ is the variable $x$, then by definition of substitution $e[t / x] = t$ and by hypothesis we know that $\Gamma ' \vdash t\colon A$. Observe that by the typing rule (VAR), $B$ is forced to be the type of $x$, i.e., $A$. Thus, $\Gamma' \vdash x[t /x] \colon B$.

If $e$ is a variable $y$ different from $x$, then by definition of substitution $e[t / x] = y$ and by hypothesis we know that $\Gamma ' \vdash y\colon B$.

If $e=f(e_1, \dots, e_n)$, then by definition of substitution $e[t / x] = f(e_1 [t/x], \dots , e_n [t/x])$; by typing rule (OP), we know that $f\colon A_1 \per \dots A_n \to B$ and $\Gamma' \vdash e_i \colon A_i$. From the latter and  induction hypothesis, $\Gamma' \vdash e_i [t/x] \colon A_i$. Again by the rule (OP), we have that $\Gamma' \vdash f(e_1 [t/x], \dots , e_n [t/x])\colon B$.
\end{proof}

The following result will be useful for the assignment rule below.

\begin{lemma}\label{lemma:encodingsubst}
Let $\Gamma ' = \Gamma, x\colon A, \Delta$ for some typing contexts $\Gamma$ and $\Delta$. If $\Gamma' \vdash e\colon B$ and $\Gamma ' \vdash t\colon A$, then
\[\encoding{ \Gamma' \vdash e[t /x] \colon B} = \tikzfig{hoare/subs/step1}\] %\includegraphics[scale=0.5]{figures/interpretation-substitution.pdf}\] % (\copier{\encoding{\Gamma}} \per \id{A} \copier{\encoding{\Delta}}) \, ; \, ( \id{\encoding{\Gamma}} \per \encoding{\Gamma ' \vdash t\colon A} \per \id{\encoding{\delta}}   ) \, ; \, \encoding {\Gamma' \vdash e\colon B}\]
\end{lemma}
\begin{proof}
The proof proceeds by induction on $\Gamma' \vdash e\colon B$.

If $e$ is the variable $x$, then by the rule (VAR) $A=B$. Moreover, by definition of $\encoding{\cdot}$, $\encoding{\Gamma, x\colon A, \Delta \vdash x \colon A} =  \discharger{\encoding{\Gamma}} \per \id{A} \per \discharger{\encoding{\Delta}}$. 
Thus
\[ \tikzfig{hoare/subs/step1} = \tikzfig{hoare/subs/step2} \stackrel{\eqref{ax:copierun}}{=} \tikzfig{hoare/subs/step3} = \encoding{\Gamma ' \vdash x [t / x]\colon A} \]
% \[ \includegraphics[scale=0.5]{figures/interpretation-substitution.pdf} = \includegraphics[scale=0.5]{figures/proof-substitution-variable-same.pdf} = \encoding{\Gamma ' \vdash x [t / x]\colon A}\]
% \[(\copier{\encoding{\Gamma}} \per \id{A} \copier{\encoding{\Delta}}) \, ; \, ( \id{\encoding{\Gamma}} \per \encoding{\Gamma ' \vdash t\colon A} \per \id{\encoding{\delta}}   ) \, ; \, \encoding {\Gamma' \vdash e\colon B} = \]
% \[(\copier{\encoding{\Gamma}} \per \id{A} \copier{\encoding{\Delta}}) \, ; \, ( \id{\encoding{\Gamma}} \per \encoding{\Gamma ' \vdash t\colon A} \per \id{\encoding{\delta}}   ) \, ; \, ( \discharger{\encoding{\Gamma}} \per \id{A} \per \discharger{\encoding{\Delta}}) = (SMC) \]
% \[(\copier{\encoding{\Gamma}} \per \id{A} \copier{\encoding{\Delta}}) \, ; \, (\discharger{\encoding{\Gamma}} \per \encoding{\Gamma ' \vdash t\colon A} \per \discharger{\encoding{\Delta}}  )  = (UNIT) \]
% \[  \encoding{\Gamma ' \vdash t\colon A} = (def sub)\]
% \[  \encoding{\Gamma ' \vdash x [t / x]\colon A}\]

If $e$ is a variable $y$, different from $x$, then by the rule (VAR), there are two possible cases: either $\Gamma = \Gamma_1, y\colon B , \Gamma_2$ for some typing contexts $\Gamma_1$ and $\Gamma_2$ or  $\Delta = \Delta_1, y\colon B , \Delta_2$.
We consider the first case, the second is symmetrical. Observe that, by definition of $\encoding{\cdot}$,

\[\encoding{\Gamma_1, y\colon B, \Gamma_2, x \colon A, \Delta \vdash y \colon B} =  \discharger{\encoding{\Gamma_1}} \per \id{B} \per  \discharger{\encoding{\Gamma_2}} \per  \discharger{A} \per  \discharger{\encoding{\Delta}} \]

Thus,
\[ \tikzfig{hoare/subs/step1} = \tikzfig{hoare/subs/step4} \stackrel{\eqref{eq:deterministic-total}}{=} \tikzfig{hoare/subs/step5} \stackrel{\eqref{ax:copierun}}{=} \tikzfig{hoare/subs/step6} = \encoding{\Gamma ' \vdash y [t / x]\colon A} \] 
% \[\includegraphics[scale=0.5]{figures/interpretation-substitution.pdf} = \includegraphics[scale=0.5]{figures/proof-substitution-variable-different.pdf} = \encoding{\Gamma ' \vdash y [t / x]\colon A}\]

% \[(\copier{\encoding{\Gamma_1, y\colon B , \Gamma_2}} \per \id{A} \copier{\encoding{\Delta}}) \, ; \, ( \id{\encoding{\Gamma_1, y\colon B , \Gamma_2}} \per \encoding{\Gamma_1, y\colon B , \Gamma_2, x\colon A, \Delta \vdash t\colon A} \per \id{\encoding{\delta}}   ) \, ; \, (\, \discharger{\encoding{\Gamma_1}} \per \id{B} \per  \discharger{\encoding{\Gamma_2}} \per  \discharger{A} \per  \discharger{\encoding{\Delta}} \, ) = SMC\]
% \[(\copier{\encoding{\Gamma_1, y\colon B , \Gamma_2}} \per \id{A} \copier{\encoding{\Delta}}) \, ; \, ( \discharger{\encoding{\Gamma_1}} \per \id{B} \per  \discharger{\encoding{\Gamma_2}} \per  ( \encoding{\Gamma_1, y\colon B , \Gamma_2, x\colon A, \Delta \vdash t\colon A} ;  \discharger{A}) \per \discharger{\encoding{\Delta}}   )  = (NAT \discharger{X})\]
% \[(\copier{\encoding{\Gamma_1, y\colon B , \Gamma_2}} \per \id{A} \copier{\encoding{\Delta}}) \, ; \, ( \discharger{\encoding{\Gamma_1}} \per \id{B} \per  \discharger{\encoding{\Gamma_2}} \per  ( \discharger{\encoding{\Gamma_1}} \per  \discharger{B} \per \discharger{\encoding{\Gamma_2}} \per \discharger{A} \per \discharger{\encoding{\Delta}}) \per \discharger{\encoding{\Delta}}   )  = SMC \]
% \[(\copier{\encoding{\Gamma_1, y\colon B , \Gamma_2}} \per \id{A} \copier{\encoding{\Delta}}) \, ; \, (( \discharger{\encoding{\Gamma_1}} \per \id{B} \per  \discharger{\encoding{\Gamma_2}})  \per  ( \discharger{\encoding{\Gamma_1}} \per  \discharger{B} \per \discharger{\encoding{\Gamma_2}})) \per \discharger{A} \per ( \discharger{\encoding{\Delta}} \per \discharger{\encoding{\Delta}}   )  = (UNIT)\]
% \[ \discharger{\encoding{\Gamma_1}} \per \id{B} \per  \discharger{\encoding{\Gamma_2}}   \per \discharger{A} \per  \discharger{\encoding{\Delta}}     = \]
% \[ \encoding{\Gamma' \vdash y\colon B}    = (DEF sub)\]
% \[ \encoding{\Gamma' \vdash y[t/x] \colon B} \]

If \(e\) is an application, $e=f(e_1, \dots , e_n)$, by definition of \(\encoding{\cdot}\) on operations, \(\encoding{\Gamma' \vdash f(e_{1}, \ldots, e_{n}) \colon A} \defeq \copier{\encoding{\Gamma'}}^n ; (\encoding{\Gamma' \vdash e_1} \per \dots \per \encoding{\Gamma' \vdash e_n} ) ; f\).
By naturality of copy, we obtain
\begin{align*}
  \tikzfig{hoare/subs/step1} &= \tikzfig{hoare/subs/step7} \stackrel{\eqref{eq:deterministic-total}}{=} \tikzfig{hoare/subs/step8} \\
  &= \encoding{\Gamma' \vdash f(e_{1} [t / x],\ldots ,e_{n} [t / x])\colon A} = \encoding{\Gamma' \vdash f(e_{1},\ldots ,e_{n}) [t / x]\colon A}
\end{align*}
% \[\includegraphics[scale=0.5]{figures/interpretation-substitution.pdf} = \includegraphics[scale=0.5]{figures/proof-substitution-operation.pdf}\]
% \[= \encoding{\Gamma' \vdash f(e_{1} [t / x],\ldots ,e_{n} [t / x])\colon A} = \encoding{\Gamma' \vdash f(e_{1},\ldots ,e_{n}) [t / x]\colon A}\]
\end{proof}

% \ale{Ricontrollare bene i tipi nel testo/diagrammi}



\subsection{Predicates}
We now turn to predicates, defined by the following grammar 
\[P \Coloneqq R(e_1, \dots, e_n) \mid \bar{R}(e_1, \dots, e_n) \mid \top \mid \bot  \mid P \lor P \mid P \land P  \] %\marginpar{Forse possiamo frgarcene di $=$ e $\neq$? sono comunque sussunti da $P(e_1, \dots, e_n)$ non mi pare che giochino un ruolo chiave}
where $R$ is a symbol in $\mathcal{P}$ and $e_i$ are expressions. Observe that negation $\lnot P$ can be easily defined as expected:
$$\begin{array}{c@{\qquad}c@{\qquad}c}
\neg R(e_1, \dots, e_n) \defeq \bar{R}(e_1, \dots, e_n) &   \neg \top \defeq \bot &  \neg(P \lor P) \defeq \neg P \land \neg Q \\
\neg \bar{R}(e_1, \dots, e_n) \defeq R(e_1, \dots, e_n) & \neg \bot \defeq \top & \neg(P \land P) \defeq \neg P \lor \neg Q
\end{array}
$$
As in the case of expressions, we consider a simple type system for predicates.
  \begin{equation*}
  \begin{array}{c@{\qquad}c@{\qquad}c@{\qquad}c}
    \inferrule*[right=(top)]{ }{\Gamma \vdash \top \colon 1} &  \inferrule*[right=(and)]{\Gamma \vdash P \colon 1 \quad \Gamma \vdash Q \colon 1}{\Gamma \vdash (P \land Q) \colon 1} & \inferrule*[right=($\bar{\textnormal{R}}$)]{\Gamma\vdash e_i\colon A_i \quad R \colon A_1 \per \dots \per A_n \to 1}{\Gamma \vdash \bar{R}(e_1, \dots e_n) \colon 1} \\[12pt]
    \inferrule*[right=(bot)]{ }{\Gamma \vdash \bot \colon 1} & \inferrule*[right=(or)]{\Gamma \vdash P \colon 1 \quad \Gamma \vdash Q \colon 1}{\Gamma \vdash (P \lor Q) \colon 1} & \inferrule*[right=(R)]{\Gamma\vdash e_i\colon A_i \quad R \colon A_1 \per \dots \per A_n \to 1}{\Gamma \vdash R(e_1, \dots e_n) \colon 1}
  \end{array}
  \end{equation*}
The encoding $\encoding{\cdot}$ maps well typed predicates $\Gamma \vdash P \colon 1$ into diagrams of type $\encoding{\Gamma} \to 1$.
$$\begin{array}{rcl}
\encoding{\Gamma \vdash R(e_1, \dots e_n)\colon 1} &\defeq& \copier{\encoding{\Gamma}}^n ; (\encoding{\Gamma \vdash e_1 \colon 1} \per \dots \per \encoding{\Gamma \vdash e_n \colon 1}) ; R \\
\encoding{\Gamma \vdash \bar{R}(e_1, \dots e_n)\colon 1} &\defeq& \copier{\encoding{\Gamma}}^n ; (\encoding{\Gamma \vdash e_1 \colon 1} \per \dots \per \encoding{\Gamma \vdash e_n \colon 1}) ; \bar{R} \\
\encoding{\Gamma \vdash \top\colon 1} &\defeq& \discharger{\encoding{\Gamma}}\\
\encoding{\Gamma \vdash \bot \colon 1} &\defeq& \bang{\encoding{\Gamma}} \dcomp \cobang{1}\\
\encoding{\Gamma \vdash P \lor  Q \colon 1} &\defeq& \diag{\encoding{\Gamma}} ; (\encoding{\Gamma \vdash P\colon 1} \piu \encoding{\Gamma \vdash P\colon 1} ) ; \codiag{1}\\ %\includegraphics[scale=0.5]{figures/predicates-union.pdf}\\
\encoding{\Gamma \vdash P \land Q \colon 1} &\defeq& \copier{\encoding{\Gamma}} ;  (\encoding{\Gamma \vdash P\colon 1} \per \encoding{\Gamma \vdash P\colon 1} )    %\includegraphics[scale=0.5]{figures/predicates-intersection.pdf} \\
\end{array}
$$
%\(\encoding{e_{1} = e_{2}} \defeq\) \includegraphics[scale=0.5]{figures/expression-equality.pdf}\\
%\(\encoding{e_{1} \neq e_{2}} \defeq\) \includegraphics[scale=0.5]{figures/expression-inequality.pdf}\\
%\(\encoding{\lnot \top} \defeq \interpret{\bot}\)\\
%\(\encoding{\lnot \bot} \defeq \interpret{\top}\)\\
%\(\encoding{\lnot (e_{1} = e_{2})} \defeq \encoding{e_{1} \neq e_{2}}\)\\
%\(\encoding{\lnot (e_{1} \neq e_{2})} \defeq \encoding{e_{1} = e_{2}}\)\\
%\(\encoding{\lnot (P \land Q)} \defeq \encoding{\lnot P \lor \lnot Q}\)\\
%\(\encoding{\lnot (P \lor Q)} \defeq \encoding{\lnot P \land \lnot Q}\)\\
%\(\encoding{\lnot R(e_{1}, \dots, e_n)} \defeq \interpret{\bar{R}(e_1, \dots , e_n)}\)\\
Similarly to the case of expressions, one defines substitution on a variable $x$ of a term $t$ in a predicate $P$ inductively:
\[ R(e_1, \dots, e_n) [t/x] \defeq R(e_1[t/x], \dots, e_n[t/x]) \qquad \bar{R}(e_1, \dots, e_n) [t/x] \defeq \bar{R}(e_1[t/x], \dots, e_n[t/x]) \]
\[ \top [t/x] \defeq \top \quad \bot [t/x] \defeq \bot \quad (P \lor Q)[t/x]\defeq P[t/x] \lor Q[t/x] \quad (P \land Q)[t/x]\defeq P[t/x] \land Q[t/x] \]
A simple inductive arguments confirm that substituion are well-typed. Moreover
\begin{lemma}\label{lemma:encodingsubstPed}
Let $\Gamma ' = \Gamma, x\colon A, \Delta$ for some typing contexts $\Gamma$ and $\Delta$. If $\Gamma' \vdash P\colon 1$ and $\Gamma ' \vdash t\colon A$, then
\[\encoding{ \Gamma' \vdash P[t /x] \colon 1} = \tikzfig{hoare/pred/step1} \]% (\copier{\encoding{\Gamma}} \per \id{A} \copier{\encoding{\Delta}}) \, ; \, ( \id{\encoding{\Gamma}} \per \encoding{\Gamma ' \vdash t\colon A} \per \id{\encoding{\delta}}   ) \, ; \, \encoding {\Gamma' \vdash P\colon 1}\]
% \[\encoding{ \Gamma' \vdash P[t /x] \colon 1} = \includegraphics[scale=0.5]{figures/interpretation-substitution-predicates.pdf}\]% (\copier{\encoding{\Gamma}} \per \id{A} \copier{\encoding{\Delta}}) \, ; \, ( \id{\encoding{\Gamma}} \per \encoding{\Gamma ' \vdash t\colon A} \per \id{\encoding{\delta}}   ) \, ; \, \encoding {\Gamma' \vdash P\colon 1}\]
\end{lemma}
\begin{proof}
  Proceed by induction on the typing rules for predicates.

  If \(P\) is \(\top\), then
  \[
    \tikzfig{hoare/pred/step1} =  \tikzfig{hoare/pred/step2} \stackrel{\eqref{eq:deterministic-total}}{=} \tikzfig{hoare/pred/step3} \stackrel{\eqref{ax:copierun}}{=} \tikzfig{hoare/pred/step4}  = \encoding{\Gamma' \vdash \top \colon 1} = \encoding{\Gamma' \vdash \top[t /x] \colon 1}.
  \]
  % \[\includegraphics[scale=0.5]{figures/interpretation-substitution-predicates.pdf} = \includegraphics[scale=0.5]{figures/proof-substitution-top.pdf} = \encoding{\Gamma' \vdash \top \colon 1} = \encoding{\Gamma' \vdash \top[t /x] \colon 1}\]

  If \(P\) is \(\bot\), then
  \[  
    \tikzfig{hoare/pred/step1} = \tikzfig{hoare/pred/step5}  \stackrel{\eqref{ax:bangnat}}{=} \tikzfig{hoare/pred/step6} = \encoding{\Gamma' \vdash \bot \colon 1} = \encoding{\Gamma' \vdash \bot[t /x] \colon 1}.
  \]
  % \[\includegraphics[scale=0.5]{figures/interpretation-substitution-predicates.pdf} = \includegraphics[scale=0.5]{figures/proof-substitution-bot.pdf} = \encoding{\Gamma' \vdash \bot \colon 1} = \encoding{\Gamma' \vdash \bot[t /x] \colon 1}\]

  If \(P\) is a predicate symbol \(R\), then
  \begin{align*}
    \tikzfig{hoare/pred/step1} &= \tikzfig{hoare/pred/step7} \stackrel{\eqref{eq:deterministic-total}}{=} \tikzfig{hoare/pred/step8} \\
    &= \encoding{\Gamma' \vdash R(e_{1} [t / x],\ldots ,e_{n} [t / x])\colon A} = \encoding{\Gamma' \vdash R(e_{1},\ldots ,e_{n}) [t / x]\colon A}.
  \end{align*}
  % \[\includegraphics[scale=0.5]{figures/interpretation-substitution-predicates.pdf} = \includegraphics[scale=0.5]{figures/proof-substitution-application.pdf}\]


  If \(P\) is a negated predicate symbol \(\bar{R}\), then
  \begin{align*}
    \tikzfig{hoare/pred/step1} &= \tikzfig{hoare/pred/step9} \stackrel{\eqref{eq:deterministic-total}}{=} \tikzfig{hoare/pred/step10} \\
    &= \encoding{\Gamma' \vdash \bar{R}(e_{1} [t / x],\ldots ,e_{n} [t / x])\colon A} = \encoding{\Gamma' \vdash \bar{R}(e_{1},\ldots ,e_{n}) [t / x]\colon A}.
  \end{align*}
  % \[\includegraphics[scale=0.5]{figures/interpretation-substitution-predicates.pdf} = \includegraphics[scale=0.5]{figures/proof-substitution-not-application.pdf}\]

  For the conjunction case, \(P = Q \land R\),%\(P' = P \land Q\),
  \begin{align*}
    \tikzfig{hoare/pred/step1} &= \tikzfig{hoare/pred/step11} \stackrel{\eqref{eq:deterministic-total}}{=} \tikzfig{hoare/pred/step12} \\
    &= \encoding{\Gamma' \vdash Q[t/x] \colon 1} \land \encoding{\Gamma' \vdash R[t/x] \colon 1} \\
    &= \encoding{\Gamma' \vdash Q[t/x] \land R[t/x] \colon 1} = \encoding{\Gamma' \vdash (Q \land R)[t/x] \colon 1}.
  \end{align*}
  % \[\includegraphics[scale=0.5]{figures/interpretation-substitution-predicates.pdf} = \includegraphics[scale=0.5]{figures/proof-substitution-and.pdf}\]
  % \[= \encoding{\Gamma' \vdash P[t/x] \colon 1} \land \encoding{\Gamma' \vdash Q[t/x] \colon 1} = \encoding{\Gamma' \vdash P[t/x] \land Q[t/x] \colon 1} = \encoding{\Gamma' \vdash (P \land Q)[t/x] \colon 1}\]

  For the disjunction case, \(P = Q \lor R\),%\(P' = P \lor Q\),
  \begin{align*}
    \tikzfig{hoare/pred/step1} &= \tikzfig{hoare/pred/step13} \stackrel{\eqref{ax:diagnat}}{=} \tikzfig{hoare/pred/step14} \\
    &= \encoding{\Gamma' \vdash Q[t/x] \colon 1} \lor \encoding{\Gamma' \vdash R[t/x] \colon 1} \\
    &= \encoding{\Gamma' \vdash Q[t/x] \lor R[t/x] \colon 1} = \encoding{\Gamma' \vdash (Q \lor R)[t/x] \colon 1}.
  \end{align*}
  % \[\includegraphics[scale=0.5]{figures/interpretation-substitution-predicates.pdf} = \includegraphics[scale=0.5]{figures/proof-substitution-or.pdf}\]
  % \[= \encoding{\Gamma' \vdash P[t/x] \colon 1} \lor \encoding{\Gamma' \vdash Q[t/x] \colon 1} = \encoding{\Gamma' \vdash P[t/x] \lor Q[t/x] \colon 1} = \encoding{\Gamma' \vdash (P \lor Q)[t/x] \colon 1}\]
\end{proof}



\subsection{Commands}
Commands are defined by the following grammar
\[ C = \mathsf{abort} \mid \mathsf{skip} \mid \mathop{\mathsf{if}} P \mathop{\mathsf{then}} C \mathop{\mathsf{else}} D \mid \mathop{\mathsf{while}} P \mathop{\mathsf{do}} C \mid C ; D \mid x \coloneqq e\]
where $P$ is a predicate and $e$ an expression. The type system is rather simple: the only non straightforward rule is the one for the assignment where one has to ensure that the type of $e$ is the same to the one of $x$.
% \elena{why do commands not have a codomain? is it because we implicitly assume that they are endomorphisms?}
\begin{equation*}
\begin{array}{c}
  \begin{array}{ccc}
    \inferrule*[right=(abort)]{ }{\Gamma \vdash \mathsf{abort} }&
\inferrule*[right=(skip)]{ }{\Gamma \vdash \mathsf{skip} }&
    \inferrule*[right=(assn)]{\Gamma = \Gamma',x \colon A,\Delta' \qquad \Gamma \vdash e \colon A}{\Gamma \vdash x \coloneqq e }
    \end{array}\\
    \begin{array}{ccc}
    \inferrule*[right=(;)]{\Gamma \vdash C   \quad \Gamma \vdash D }{\Gamma \vdash C ; D }&
    \inferrule*[right=(if)]{\Gamma \vdash P \colon 1 \quad \Gamma \vdash C   \quad \Gamma \vdash D  }{\Gamma \vdash \mathop{\mathsf{if}} P \mathop{\mathsf{then}} C \mathop{\mathsf{else}} D }&
\inferrule*[right=(while)]{\Gamma \vdash P \colon 1 \quad \Gamma \vdash C  }{ \Gamma \vdash \mathop{\mathsf{while}} P \mathop{\mathsf{do}} C }
\end{array}
\end{array}
\end{equation*}


The predicates occurring in a command will be regarded as the corresponding coreflexive: we fix
% \[c(P)\defeq \includegraphics[scale=0.5]{figures/def-coreflexive.pdf}\] %\copier{\encoding{\Gamma}} ;(\encoding{\Gamma \vdash P \colon 1} \per \id{\encoding{\Gamma}})\]
\[ c(P) \defeq \tikzfig{hoare/corefl/lhs} = \tikzfig{hoare/corefl/rhs} \]
which, according to the notation in \Cref{rem:notation-coreflexives}, will be drawn as a circle.

The encoding maps any well typed command $\Gamma \vdash C $ into a diagram of type $\encoding{\Gamma} \to \encoding{\Gamma}$.
$$\begin{array}{rcl}
\encoding{\Gamma \vdash \mathsf{abort}}  & \defeq & \bang{\encoding{\Gamma}} ; \cobang{\encoding{\Gamma}}\\
\encoding{\Gamma \vdash  \mathsf{skip} }  & \defeq & \id{\encoding{\Gamma}} \\
\encoding{\Gamma \vdash  C;D }  & \defeq & \encoding{\Gamma \vdash C} ; \encoding{\Gamma \vdash D}  \\
\encoding{\Gamma \vdash \mathop{\mathsf{if}} P \mathop{\mathsf{then}} C \mathop{\mathsf{else}} D}  & \defeq & (c(P); \encoding{\Gamma \vdash C} ) + (c(\neg P); \encoding{\Gamma \vdash D}) \\
%\includegraphics[scale=0.5]{figures/if-then-else.pdf}\\
\encoding{\Gamma \vdash\mathop{\mathsf{while}} P \mathop{\mathsf{do}} C}  & \defeq & \kstar{(c(P); \encoding{\Gamma \vdash C })} ; c(\neg P)  \\
%\includegraphics[scale=0.5]{figures/while-loop.pdf}\\
\interpret{\Gamma \vdash x \coloneqq e}  & \defeq & (\copier{\encoding{\Gamma'}} \per \id{A} \per \copier{\encoding{\Delta'}}) ; (\id{\encoding{\Gamma'}} \per \encoding{\Gamma \vdash e\colon A}  \per \id{\encoding{\Delta'}} )     %\includegraphics[scale=0.5]{figures/variable-assignment.pdf}\\
\end{array}$$
Apart from the assignment the encodings of the other commands is pretty standard, see for instance Kleene Algebra with tests \cite{kozen1997kleene}. The assignment instead crucially exploits the structure of cartesian bicategories to properly model data flow.
For convenience of the reader we draw the corresponding tape diagram below. %\marginpar{Inserire diagramma di questo}
\[ \tikzfig{hoare/assign} \]
% \[(\copier{\encoding{\Gamma'}} \per \id{A} \per \copier{\encoding{\Delta'}}) ; (\id{\encoding{\Gamma'}} \per \encoding{\Gamma \vdash e\colon A}  \per \id{\encoding{\Delta'}} ) \]




\subsection{Hoare Triples}
Hoare logic \cite{hoare1969axiomatic} is one of the most influential language to reason about imperative programs. Its rules --in the version appearing in \cite{winskel1993formal}-- are reported in Figure \ref{fig:hoare-rules}. 
% In partial correctness, a triple \(\{P\}C\{Q\}\) means that if the execution of the command $C$ starting from an arbitrary state satisfying the  precondition $P$, if it terminates leads to some state satisfying the postcondition $Q$.
In partial correctness, the triple \(\{P\}C\{Q\}\) asserts that if the command $C$ is executed from any state that satisfies the precondition $P$, and if the execution terminates, the resulting state will satisfy the postcondition $Q$.
%This can be expressed by our language of tape diagrams: one  encodes the predicates $P$ and $Q$ and takes their $\op{-}$, hereafter drawn as \marginpar{INSERT DIAGRAMS}
%\[ \op{\encoding{P}} \qquad \text{ and }\op{\encoding{Q}}\text{.}\]
The following result shows that if a triple \(\{P\}C\{Q\}\) is derivable within the Hoare logic, one can prove \(\op{\encoding{P}} \dcomp \encoding{C} \leq \op{\encoding{Q}}\) within tape diagrams.
%Since, its early years the connection of Hoare logic with the calculus of relation has been widely studied: \cite{pratt1976semantical}

\begin{figure}
  \begin{equation*}
  \begin{array}{c@{\quad}c@{\quad}c}
    \inferrule*[right=($\mathsf{skip}$)]{ }{\{P\}\mathsf{skip}\{P\}} & \inferrule*[right=(sub)]{ }{\{P[E/x]\}x \coloneqq E\{P\}} & \inferrule*[right=(\(\subseteq\))]{P_1 \subseteq P_2 \quad \{P_2\}C\{Q_2\} \quad Q_2 \subseteq Q_1}{\{P_1\}C\{Q_1\}} \\[12pt]
    \inferrule*[right=(seq)]{\{P\}C\{Q\} \quad \{Q\}D\{R\}}{\{P\}C ; D\{R\}} & \inferrule*[right=(\(\mathsf{if-else}\))]{\{P \land B\}C\{Q\} \quad \{P \land \lnot B \}D\{Q\}}{\{P\}\mathop{\mathsf{if}} B \mathop{\mathsf{then}} C \mathop{\mathsf{else}} D\{Q\}} & \inferrule*[right=(\(\mathsf{while}\))]{\{P \land B\}C\{P\}}{\{P\}\mathop{\mathsf{while}} B \mathop{\mathsf{do}} C\{P \land \lnot B\}} %\\[12pt]
  %  \inferrule*[right=(excl)]{\{P \land B\}C\{Q\} \quad \{P \land \lnot B\}C\{Q\}}{\{P\}C\{Q\}} & \inferrule*[right=(ind)]{x_{i} \colon X_{i} \vdash C \colon Y_{j} \quad \vdash B \colon Z_{k} \quad \{P\}C\{Q\}}{\{P \land B\}C\{Q \land B\}} & \inferrule*[right=(exist)]{\forall x \colon X \ \{P\}C\{Q\}}{\exists x \colon X \{P\}C\{Q\}}
  \end{array}
  \end{equation*}
  \caption{Hoare derivation rules\label{fig:hoare-rules}}
\end{figure}

\begin{proposition}\label{prop:Hoare}
  If a Hoare triple \(\{P\}C\{Q\}\) is derivable with the rules in \Cref{fig:hoare-rules}, then \(\op{\encoding{P}} \dcomp \encoding{C} \leq \op{\encoding{Q}}\) in \(\KTCB\).
\end{proposition}
\begin{proof}
  By induction on the deduction rules in \Cref{fig:hoare-rules}.\\
  
  \medskip

  \noindent\((\mathsf{skip})\). \; \(\encoding{P} \dcomp \encoding{\mathsf{skip}} \stackrel{\text{(Def. of $\encoding{\cdot}$)}}{=} \encoding{P} \dcomp \id{} = \encoding{P}\).\\

  \medskip

  \noindent(SUB). \;
  \[ \tikzfig{hoare/triples/sub/step1} \stackrel{\eqref{ax:copieradj1}}{\leq} \tikzfig{hoare/triples/sub/step3} \stackrel{\eqref{eq:cb:adj:sv}}{\leq} \tikzfig{hoare/triples/sub/step2}. \] 
  % \includegraphics[scale=0.5]{figures/derive-substitution.pdf}\\
  % \elena{diagrams should have \(\op{\encoding{P}}\) instead of \(P\)}

  \medskip

  \noindent\((\subseteq)\). \; \(\encoding{P_{1}} \dcomp \encoding{C} \stackrel{(P_1 \subseteq P_2)}{\leq} \encoding{P_{2}} \dcomp  \encoding{C} \stackrel{\text{(Ind. hyp.)}}{\leq} \encoding{Q_{2}} \stackrel{(Q_1 \subseteq Q_2)}{\leq} \encoding{P_{2}} \encoding{Q_{1}}\).\\

  \medskip

  \noindent(SEQ). \; \(\encoding{P} \dcomp \encoding{C ; D} \stackrel{\text{(Def. of $\encoding{\cdot}$)}}{=} \encoding{P} \dcomp \encoding{C} \dcomp \encoding{D} \stackrel{\text{(Ind. hyp.)}}{\leq} \encoding{Q} \dcomp \encoding{D} \stackrel{\text{(Ind. hyp.)}}{\leq} \encoding{R}\).\\

  \medskip

  \noindent\((\mathsf{if-else})\). \;\\
  \begin{align*}
    \tikzfig{hoare/triples/if/step1} \stackrel{\eqref{ax:diagnat}}{=} \tikzfig{hoare/triples/if/step2} \stackrel{\text{(Ind. hyp.)}}{\leq} \tikzfig{hoare/triples/if/step3} \stackrel{(+\text{-idemp.})}{=} \tikzfig{hoare/triples/if/step4}.
  \end{align*}

  \medskip


  % \includegraphics[scale=0.5]{figures/derive-if-else.pdf}\\
  \noindent\((\mathsf{while})\). \; First, observe that the following holds:
    \[ \tikzfig{hoare/triples/while/preunif/step1} \stackrel{\eqref{ax:codiagnat}, \eqref{ax:diagnat}}{=} \tikzfig{hoare/triples/while/preunif/step2} \stackrel{\text{(Ind. hyp.)}}{\leq} \tikzfig{hoare/triples/while/preunif/step3}. \]
    Then, by~\eqref{ax:trace:tape:AU2}, the inequality below holds and the derivation concludes the proof.
    \[ \tikzfig{hoare/triples/while/postunif/step1} \leq \tikzfig{hoare/triples/while/postunif/step2} \stackrel{\eqref{ax:trace:tape:kstar-id}}{=} \tikzfig{hoare/triples/while/postunif/step3}. \]
  % \includegraphics[scale=0.5]{figures/derive-while.pdf}\\
  % (EXCL)\\
  % \includegraphics[scale=0.5]{figures/derive-excl.pdf}\\
  % (IND)\\
  % \includegraphics[scale=0.5]{figures/derive-independent.pdf}\\
  % (EXISTS)\\
  % \includegraphics[scale=0.5]{figures/derive-exists.pdf}
\end{proof}





\subsection{Other Program Logics}
While the calculus of relations, Kleene Algebra and Kleene algebra with tests express binary relations, tape diagrams are able to express relations with arbitrary source and target. For instance a tape $\t\colon U \to 1$ represents a predicate over $U$, typically intended as the set of all memories. This ability allows tape diagrams to easily express triples occurring in different programs logics, such as incorrectness \cite{o2019incorrectness}, sufficient incorrectness \cite{DBLP:journals/corr/abs-2310-18156} and necessary \cite{DBLP:conf/vmcai/CousotCFL13} logic. The correspondence between the triples of these logics and inequalities in tapes is illustrated in \Cref{tab:triples-inequalities}.
\begin{table}[H]
  \centering
  \renewcommand{\arraystretch}{1.7}
  \begin{tabular}{ c @{\qquad} c @{\qquad} c }
    \toprule
    Logic & Triple & Inequality \\
    \midrule
    Hoare & \(\{P\}C\{Q\}\) & $\tikzfig{hoare/inclusions/hoare/lhs} \leq \tikzfig{hoare/inclusions/hoare/rhs}$\\ %\(\op{\encoding{P}} \dcomp \encoding{C} \leq \op{\encoding{Q}}\)\\
    Incorrectness & \([P]C[Q]\) & $\tikzfig{hoare/inclusions/hoare/lhs} \geq \tikzfig{hoare/inclusions/hoare/rhs}$\\ %\(\op{\encoding{P}} \dcomp \encoding{C} \geq \op{\encoding{Q}}\)\\
    Sufficient incorrectness & \(\lAngle P \rAngle C \lAngle Q \rAngle\) & $\tikzfig{hoare/inclusions/suffInc/lhs} \leq \tikzfig{hoare/inclusions/suffInc/rhs}$\\ %\(\encoding{P} \leq \encoding{C} \dcomp \encoding{Q}\)\\
    Necessary & \((P)C(Q)\) & $\tikzfig{hoare/inclusions/suffInc/lhs} \geq \tikzfig{hoare/inclusions/suffInc/rhs}$\\[4pt] %\( \encoding{P} \geq \encoding{C} \dcomp \encoding{Q}\)\\
    \bottomrule
  \end{tabular}
  \caption{Correspondence between triples and inequalities.\label{tab:triples-inequalities}}
\end{table}




==> oldsections/sections/intro.tex <==

\section{Introduction}\label{sec:intro}


Motivated by the growing interest in formal languages that are both diagrammatic and compositional, an increasing number of works~\cite{BaezErbele-CategoriesInControl,DBLP:journals/pacmpl/BonchiHPSZ19,Bonchi2015,coecke2011interacting,Fong2015,DBLP:journals/corr/abs-2009-06836,Ghica2016,DBLP:conf/lics/MuroyaCG18,Piedeleu2021,DBLP:journals/jacm/BonchiGKSZ22} leverage \emph{string diagrams}~\cite{joyal1991geometry,selinger2010survey}. These diagrams formally represent arrows in a strict symmetric monoidal category freely generated by a monoidal signature. A symbol $\gen$ in the signature is depicted as a box $\Cgen{\gen}{}{}$, and arbitrary string diagrams are constructed through horizontal ($;$) and vertical ($\per$) composition of such symbols. 

While string diagrammatic languages are typically expressive enough to represent all relevant systems, they often become cumbersome when dealing with \emph{control}. For example, representing quantum control within the ZX-calculus~\cite{Coecke2008,Coecke2017} or probabilistic control of Boolean circuits~\cite{piedeleu2025boolean} requires ingenuity. Various works~\cite{DBLP:journals/corr/abs-2103-07960,zhao2021analyzing,stollenwerk2022diagrammatic,villoria2024enriching,DBLP:conf/fossacs/BoisseauP22} adopt a hybrid approach combining diagrammatic and algebraic syntax. Others~\cite{duncan2009generalised, james2012information, staton2015algebraic} extend beyond monoidal categories to \emph{rig categories}~\cite{laplaza_coherence_1972,johnson2021bimonoidal}, roughly categories equipped with two monoidal products, $\per$ and $\piu$, where $\per$ distributes over $\piu$.

A key challenge in visualizing arrows in rig categories arises from the need to compose them not only horizontally ($;$) and vertically ($\per$) but also using the additional monoidal product $\piu$. One natural approach, implemented by \emph{sheet diagrams}~\cite{comfort2020sheet}, utilizes three dimensions. An alternative, which remains within two dimensions, is offered by \emph{tape diagrams}~\cite{bonchi2023deconstructing}.

Intuitively, tape diagrams are \emph{string diagrams of string diagrams}: the vertical composition of inner diagrams represents $\per$, whereas the vertical composition of outer diagrams represents $\piu$.
\begin{equation*}\label{eq:example intro}
    \tikzfig{zx/control} \qquad\qquad \scalebox{0.8}{\tikzfig{addition/additionDef}} \qquad {\texttt{while(x>0)\{x:=x-1; y:=y+1\}; return y}}
\end{equation*}

For instance, the leftmost tape diagram above represents a controlled unitary using ZX-circuits inside the tapes. The central tape diagram denotes the imperative program on the right. In both cases, the inner diagrams correspond to data flow, while the outer diagrams capture control flow. The leftmost diagram is interpreted within the category of complex matrices, whereas the central diagram within the category of sets and relations. In both categories, $\piu$ is a \emph{biproduct}, namely a product and a coproduct. This fact guarantees the existence of natural \emph{comonoids} and \emph{monoids} for $\piu$, which provide the crucial linguistic primitives for representing both the branching and the join of tapes:
\begin{center}
$\smash{\Tcomonoid{\!\!\!\!}}$ and $\smash{\Tmonoid{\!\!\!\!}}$
\end{center}
Unfortunately, in many contexts, such as probabilistic systems, $\piu$ cannot be assumed to be a biproduct.

\medskip

In this paper, we generalize the framework of tape diagrams from~\cite{bonchi2023deconstructing} to accommodate categories where $\piu$ is not necessarily a biproduct. Specifically, our proposed tape diagrams represent arrows of rig categories that share the structure of Kleisli categories for \emph{monoidal monads}~\cite{kock1972strong}. Like in~\cite{bonchi2023deconstructing}, we deliberately avoid \emph{monoidal traces}, which --while useful for iteration as illustrated in~\cite{bonchi2024diagrammatic} and in the central tape above-- are not essential for our development.

Our starting observation is that in Kleisli categories, when the monoidal monad is presented by an algebraic theory $\mathbb{T}=(\Sigma,E)$, each symbol $f$ of the signature $\Sigma$ induces a natural transformation $\scalebox{0.8}{\Talgop{\!\!\!\!}{f}}$ that we use in place of the missing $\smash{\Tcomonoid{\!\!\!\!}}$. Conveniently, $\smash{\Tmonoid{\!\!\!\!}}$ always exists in any Kleisli category, as $\piu$ remains a coproduct~\cite{borceux2}. Notably, when $\mathbb{T}$ corresponds to the algebraic theory of commutative monoids, our $\mathbb{T}$-tape diagrams naturally generalize those in~\cite{bonchi2023deconstructing} (see Remark~\ref{remark:Generalization}).

Another fundamental aspect of our work concerns comonoids for the product $\per$. These structures, which reside within the Kleisli category of any commutative monad~\cite{fritz_2020}, have recently gained attention due to their significance in copy-discard~\cite{cho2019disintegration} (aka gs-monoidal~\cite{GadducciCorradini-termgraph}) and Markov categories~\cite{fritz_2020}.

We analyze, in the setting of rig categories, the interaction between $\per$-comonoids and $\piu$-monoids in Kleisli categories of monoidal monads, introducing the notion of \emph{finite coproduct-copy discard rig categories} (Definition~\ref{def: distributive gs-monoidal category}). By further considering the natural transformation arising from the algebraic theory $\mathbb{T}$, we obtain  \emph{$\mathbb{T}$-copy discard rig categories} (Definition~\ref{def: T distributive gs-monoidal category}). We demonstrate that any Kleisli category arising from a monoidal monad presented by $\mathbb{T}$ inherently possesses this structure (Proposition~\ref{prop:kleisliTrig}). Furthermore, we establish that our tape diagrammatic language  provides a $\mathbb{T}$-copy discard rig category freely generated by a monoidal signature (Theorem~\ref{th:tapes-free-T-cd}). These results ensure that, whenever the monoidal signature is interpreted within such a Kleisli category, the interpretation extends uniquely to a rig functor, thus providing a compositional semantics for tapes. We conclude by illustrating how interpreting Boolean circuits within the Kleisli category of subdistributions yields a language of tapes that both encodes~\cite{piedeleu2025boolean} and easily manages probabilistic control (Example~\ref{example: probabilistic control}).

\textbf{Synopsis.} Section~\ref{sec:running} illustrates the key structures within the Kleisli category of subdistributions. Section~\ref{sec:CD} recalls the fundamental concepts of copy-discard and finite (co)product categories, alongside monoidal monads. Section~\ref{sec:rigcategories} provides an overview of rig categories, followed by our definition of finite coproduct-copy discard rig categories in Section~\ref{sec:fccdrig}. Section~\ref{sec:Trig} introduces $\mathbb{T}$-rig categories and $\mathbb{T}$-copy discard rig categories, while their corresponding tape diagrams are in Section~\ref{sec:tapediagrams}. The appendix includes coherence diagrams and proofs. We assume familiarity with monads, Kleisli categories, and monoidal categories. For a symmetric monoidal category $(\Cat{C}, \perG, \unoG)$, we denote symmetries by $\sigma^\perG_{X,Y}$ and the remaining structural isomorphisms by $\assoc{X}{Y}{Z}$, $\lunit{X}$, and $\runit{X}$. For a natural isomorphism $\phi$, its inverse is denoted by $\phi^-$. 



% \begin{itemize}
% \item String Diagrams: very popular
% \item Limited: For instance in the ZX or BLA
% \item Considering Rig categories --> One need three dimensions --> Tape Diagrams
% \item Tape Diagrams are limited to those whether category has biproducts
% \item We extend Tape diagrams
% \item Observe that whenever the symmetric monoidal monad is presented by an algebraic theory, the operator in $\Sigma$ give rise to natural transformations. The old fashioned tape diagrams are now tape diagram for the algebraic theory of commutative monoids.
% \item Monoids and Comonoids interact in the context of a Kleisli category
% \item Main results guarantee that the interpretation give rise to a rig functor
% \item We illustrate an example of such approach...
% \end{itemize}

%Computer scientists often rely on diagrammatic notations to model and design systems: data and control flow diagrams, message sequence charts, petri nets, different sorts of circuits and state machines are just a few of the many graphical languages commonly used by software engineers.  On the one hand, diagrams provide  an intuitive and human-readable specification of the relationships and the interactions occurring amongst the various components of a system. On the other hand, diagrammatic languages often lack a formal semantics or, when given, this is rarely compositional.

% AGGIUSTARE SOPRA 



%
%The following is our first example of string diagram.
%\[ \tikzfig{functoriality} \]
%Observe that the above diagram can be regarded as both $(f_1;g_1) \per (f_2;g_2)$ and $(f_1 \per f_2); (g_1 \per g_2)$. Such ambiguity is not an issue, since in any monoidal category the law $(f_1;g_1) \per (f_2;g_2) = (f_1 \per f_2); (g_1 \per g_2)$ holds for all arrows $f_1,f_2,g_1,g_2$. More generally, it turns out that the diagrammatic representation identifies exactly \emph{all and only the laws of monoidal categories}~\cite{joyal1991geometry}. This is  the key feauture of string diagrams. 
%Indeed, by virtue of this fact, one can safely exploit diagrams to make proofs, which in this way often amount to simple and suggestive manipulations of diagrams that abstract away from the laws of monoidal categories.
%
%By carefully crafting the monoidal signature, hereafter denoted by $\Gamma$, one obtains the syntaxes of several languages specifying a large variety of systems: quantum protocols~\cite{Coecke2017}, linear dynamical systems~\cite{Bonchi2015}, Petri nets~\cite{DBLP:journals/pacmpl/BonchiHPSZ19}, concurrent connectors~\cite{Bruni2006}, digital circuits~\cite{Ghica2016}, automata~\cite{Piedeleu2021}, or conjunctive queries~\cite{GCQ} used in databases. In these approaches, the semantics are often defined by monoidal functor 
%$\dsem{-}\colon \Cat{C}_\Gamma \to \Cat{D}$ from the category fo string diagram $\Cat{C}_\Gamma$ to some monoidal category $\Cat{D}$. Since $\dsem{-}$ is functorial, it preserves $;$ and $\per$ and thus the semantics is guaranteed to be compositional.

%In these cases, the authors often introduce novel kinds of diagrams  to convey the intuition to the reader, but without a soundness and completeness theorem like in the aforementioned~\cite{joyal1991geometry} for string diagrams.  
%
%several authors \cite{DBLP:journals/corr/abs-2103-07960,zhao2021analyzing,stollenwerk2022diagrammatic} need to use a mixture of diagrammatic and algebraic syntax, like for instance linear combinations of diagrams frequently used in~\cite{Coecke2017}, or  $\sqcup$-props introduced in~\cite{DBLP:conf/fossacs/BoisseauP22} as a way to enrich string diagrams with a join operation. % $\sqcup$ expressing, somehow, union of diagrams. %A similar operation seems necessary, for instance, to extend the aforementioned conjunctive queries~\cite{GCQ} to conjunctive-disjunctive queries.
%Sometimes, the structure of monoidal categories is not enough and one needs to depict arrows  of \emph{rig categories}~\cite{laplaza_coherence_1972, johnson2021bimonoidal}, roughly categories equipped with two monoidal products $\per$ and $\piu$. In these cases, the authors often introduce novel kinds of diagrams \cite{}\marginpar{Mettere quei tre citati da Sheet} to convey the intuition to the reader, but without a soundness and completeness theorem like in the aforementioned~\cite{joyal1991geometry} for string diagrams.  
%


\begin{comment}
\section{Introduction}\label{sec:intro}
Motivated by the interest in dealing with formal languages that are, at the same time, diagrammatic and compositional, a growing number of works~~\cite{BaezErbele-CategoriesInControl,DBLP:journals/pacmpl/BonchiHPSZ19,Bonchi2015,coecke2011interacting, Fong2015,DBLP:journals/corr/abs-2009-06836,Ghica2016,DBLP:conf/lics/MuroyaCG18,Piedeleu2021,DBLP:journals/jacm/BonchiGKSZ22}  exploits \emph{string diagrams}~\cite{joyal1991geometry,selinger2010survey}, formally arrows of a strict symmetric monoidal category freely generated by a monoidal signature $\sign$.  A symbol $\gen$ in the signature is represented as a box $\Cgen{\gen}{}{}$ and arbitrary string diagrams are obtained by composing horizontally ($;$) and vertically ($\per$) such symbols. In these approaches, the semantics are often defined by monoidal functor 
$\dsem{-}\colon \DiagS \to \Cat{D}$ from the category of string diagram $\DiagS$ to some monoidal category $\Cat{D}$. Since $\dsem{-}$ is functorial, it preserves $;$ and $\per$ and thus the semantics is guaranteed to be \emph{compositional}. A key problem consists in Typically, the languages come with a set of axioms, namely equalities between diagrams, that are sound with respect to the semantics interpretation. As usual, completeness is a desirable properties which is hard to achieve.

While string diagrammatic languages are usually expressive enough to denote all the systems of interest, in several occasions the diagrammatic syntax appears a bit unhandy to represent \emph{control}: for instance, representing quantum control within the  ZX-calculus~\cite{Coecke2008,Coecke2017} or probabilistic control of boolean circuits~\cite{piedeleu2025boolean} requires some ingenuity. Several works \cite{DBLP:journals/corr/abs-2103-07960,zhao2021analyzing,stollenwerk2022diagrammatic,villoria2024enriching,DBLP:conf/fossacs/BoisseauP22} make use of a mixture of diagrammatic and algebraic syntax. Other works~\cite{duncan2009generalised, james2012information, staton2015algebraic} depart from monoidal categories to \emph{rig categories}~\cite{laplaza_coherence_1972, johnson2021bimonoidal}, roughly categories equipped with two monoidal products: $\per$ and $\piu$. 

The main challenge in depicting arrows of a rig category is given by the possibility of composing them not only with $;$ (horizontally) and  $\per$ (vertically), but also with the novel monoidal product $\piu$. The natural solution, implemented by sheet diagrams~\cite{comfort2020sheet}, consists in exploiting 3 dimensions.  Another solution -- which allows to remain in 2 dimensions-- is provided by \emph{tape diagrams} \cite{bonchi2023deconstructing}.

Intuitively, tape diagrams are \emph{string diagrams of string diagrams}: the vertical composition of inner diagrams represents $\per$, while vertical composition of the outer ones represents $\piu$.
\begin{equation*}\label{eq:example intro}
    \tikzfig{zx/control} \qquad\qquad \tikzfig{addition/additionDef} \qquad {\texttt{while(x>0)\{x:=x-1; y:=y+1\}; return y}}
\end{equation*}

The tape above on the left, for example, is a representation of a controlled unitary, that makes use of the ZX-calculus inside the tapes.
The tape on the center denotes the imperative program on the right. In both tapes, the inner diagram represent data-flow, while the outer diagrams control flow.
The leftmost diagram is interpreted with the category of complexes matrices, the central diagram within the category of sets and relations.
In both categories $\piu$ is a \emph{biproduct}, i.e., a categorical product and a coproduct. This fact gives us, by means of the Fox Theorem \cite{fox1976coalgebras}, natural \emph{comonoids} and \emph{monoids} for $\piu$ that are the key linguistic primitives to represent both quantum and classical control in tapes: 
\begin{center}
$\smash{\Tcomonoid{\!\!\!\!}}$ and $\smash{\Tmonoid{\!\!\!\!}}$
\end{center}
Unfortunately, in many cases, such as probabilistic system, one cannot assume $\piu$ to be a biproduct.

\medskip

In this paper we generalise tape diagrams from \cite{bonchi2023deconstructing} to deal with categories where $\piu$ is not required a biproduct. More precisely, the tapes that we introduce are able to represent arrows of rig categories having the same structure of Kleisli categories of \emph{monoidal monads}. Like in \cite{bonchi2023deconstructing}, in order to keep our developement general, we avoid to consider \emph{monoidal traces} that are used --for instance in \cite{bonchi2024diagrammatic} and in the central tape above-- to represent iteration.

Our starting observation is that in Kleisli categories, whenever the monoidal monad is presented by an algebraic theory $\mathbb{T}=(\Sigma,E)$, each symbol $f$ in the signature $\Sigma$ gives rise to a natural transformation $\scalebox{0.8}{\Talgop{\!\!\!\!}{f}}$ that one can use in place of the missing $\smash{\Tcomonoid{\!\!\!\!}}$. Luckly enough, $\smash{\Tmonoid{\!\!\!\!}}$ exists in any Kleisli category since $\piu$ is always a coproduct \cite{}. Interestingly, when \(\mathbb{T}\) is the algebraic theory of commutative monoids, our \(\mathbb{T}\)-tape diagrams generalise those in \cite{bonchi2023deconstructing} (see Remark \ref{remark:Generalization}).

Another essential ingredient for our work is provided by comonoids for the monoidal product $\per$. These structures, which leaves inside the Kleisli category of any commutative monad \cite{}, have recently received a growing attention as they are foundamental in copy discard categories \cite{} (also known as gs-monoidal~\cite{GadducciCorradini-termgraph}) and Markov categories \cite{}. 

We study the interaction of $\per$-comonoids and $\piu$-monoids within rig categories representing Kleisli categories of monoidal monads and we name the resulting structure \emph{finite coproduct-copy diacard rig categories} (Definition \ref{def: distributive gs-monoidal category}). By further considering the natural transformation arising from the algebraic theory $\mathbb{T}$, we obtain  \emph{$\mathbb{T}$-copy diacard rig categories} (Definition \ref{}). We shows that any Kleisli category for a monoidal monad presented by $\mathbb{T}$ has indeed such structure  (Proposition \ref{prop:kleisliTrig}) and we show that our diagrammatic language of tapes provides a $\mathbb{T}$-copy discard rig categories freely generated by a monoidal signature (Theorem \ref{th:tapes-free-T-cd}).
These facts entail that, whenever the monoidal signature is interpreted within such a Kleisli category, the interpretation can be uniquely extended to a functor, providing a compositonal semantics to tapes. We conclude by illustrating how by interpreting Boolean circuits within the Kleisli category of subdistributions one obtains a language that is able, at the same time, to encode~\cite{piedeleu2025boolean} and easily manage probabilistic control (Example \ref{example: probabilistic control}).

{\bf Synopsis.} We begin in Section \ref{}, by illustrating the structure of interest within the Kleisli category of subdistributions. The key notions of copy discard and finite (co)products categories are recalled in Section \ref{}, together with the definition of monoidal monad. In Section \ref{}, we first recall rig categories and, in Section \ref{}, we introduce finite coproduct-copy discard rig categories. In Section \ref{}, after recalling algebraic theories, we illustrate $\mathbb{T}$ rig categories and $\mathbb{T}$-copy discard rig categories. The corresponding tape diagrams are given in Section \ref{} together with a final example. The appendix contains the diagrams for all the already-known coherence conditions as well as all the proofs.
%
%
We assume the reader to be familiar with monads, Kleisli categories and monoidal categories. For a symmetric monoidal category $(\Cat C, \perG, \unoG)$
we denote symmetries by $\sigma^\perG_{X,Y}\colon X\perG Y \to Y \perG X$ and the remaining natural isomorphism by $\assoc{X}{Y}{Z}\colon (X \perG Y) \perG Z \to X\perG (Y \perG Z)$, $\lunit{X}\colon \unoG \perG X \to X$ and $\runit{X} \colon X \perG \unoG \to X$. For a natural isomorphism $\phi$, we write $\phi^-$ for its inverse.

\end{comment}


==> oldsections/sections/kleene.tex <==


\section{Kleene Bicategories}\label{sec:kleene}

In this section we leave the rig structure aside and we consider a special type of categories with finite biproducts and traces that resembles more closely the monoidal category $(\Rel,\piu,\zero)$. 
In the next section, we will enrich such categories with the rig structure and study the corresponding tape diagrams.


\begin{comment}
The notion of traced monoidal category has often been studied in the special cases where the monoidal product coincides with the categorical product, coproduct or biproduct: see \cite{} for a survey. 
In \cite{cuazuanescu1994feedback}, it is shown that in a finite biproduct category $\Cat{B}$, traces are equivalent to the so-called \emph{repetition operations}, namely a family of operators \(\kstar{(\cdot)} \colon \Cat{B}(S,S) \to  \Cat{B}(S,S)\) indexed by the objects $S$ of $\Cat{B}$ satisfying certain axioms. The correspondence is illustrated by means of string diagrams in Figure \ref{fig:star-trace}. 
\begin{figure}[h!]
  \centering
  % \includegraphics{figures/star-trace.pdf}
  \[
  \begin{array}{l@{\qquad}l}
    a \colon S \to S & f \colon S \piu X \to S \piu Y \\[5pt]
    \kstar{a} \defeq \Crepetition{a}{S}{S} & \trace_S f \defeq \Ctracerep{f}{S}{X}{Y}
  \end{array}
  \]
  \caption{Repetition from trace and trace from repetition in finite biproduct categories.\label{fig:star-trace}}
\end{figure}
In \cite{cuazuanescu1994feedback}, it also been illustrated that whenever the traces is uniform the aforementioned axioms can be sensibly simplified. In this section we introduce Kleene bicategories that, in first approximation, can be thought as the poset-enriched version of the ut-fb categories in \cite{cuazuanescu1994feedback}. The name Kleene is justified by the fact that the repetition operations $\kstar{(\cdot)}$ coincides with the star of a Kleene algebras as axiomatised by Kozen in \cite{Kozen94acompleteness}.
\end{comment}


\subsection{Finite Biproduct Categories with Idempotent Convolution}\label{ssec:fbic}
In any fb category $\Cat{C}$, the \emph{convolution monoid} is defined for all objects $X,Y$ and arrows $f,g\colon X \to Y$ as %\marginpar{PLS ALESSANDRO, INSERISCI DIAGRAMMI}
\begin{equation}\label{eq:covolution}
f+g \defeq \stringConvolution{f}{g}{X}{Y} \quad \text{(i.e., $\diag{X}; f \piu g ;\codiag{Y}$)} \quad\qquad 0 \defeq \stringBottom{X}{Y} \quad \text{(i.e., $\bang{X};\cobang{Y}$).}
\end{equation}
With this definition one can readily see that $\Cat{C}$ is enriched over $\Cat{CMon}$, the category of commutative monoids, namely each homset carries a commutative monoid
\begin{equation}\label{eq:cmon laws}
(f+g)+h = f+(g+h)
\quad
f+g=g+f
\quad
f+0=f
\end{equation}
and such monoid distributes over the composition $;$
\begin{equation}\label{eq:cmon enrichment}
(f+g);h = (f;h + g;h)
\quad
h;(f+g) = (h;f + h;g+)
\quad
f;0 =0= 0;f
\end{equation}

In this section we focus on a special kind of fb category, defined as follows. 
\begin{definition}\label{def:fbidempotent}
  A poset enriched monoidal category \(\Cat{C}\) is a \emph{finite biproduct category with idempotent convolution} iff $\Cat{C}$ has finite biproducts and the monoids $(\codiag{X},\cobang{X})$ are left adjoint to the comonoids $(\diag{X},\bang{X})$, i.e.,
  \[\id{X\piu X} \leq \codiag{X} ; \diag{X} \qquad  \diag{X};\codiag{X} \leq \id{X} \qquad \id{0} \leq \cobang{X};\bang{X} \qquad \bang{X};\cobang{X} \leq \id{X}\]
 \end{definition}
The axioms of adjunction for are illustrated by means of string diagrams in \Cref{fig:adjoint-biproducts}.
  \begin{figure}[h!]
    \centering
    \mylabel{ax:comonoid:assoc}{$\diag{}$-as}
    \mylabel{ax:comonoid:unit}{$\diag{}$-un}
    \mylabel{ax:comonoid:comm}{$\diag{}$-co}
    \mylabel{ax:comonoid:nat:copy}{$\diag{}$-nat}
    \mylabel{ax:comonoid:nat:discard}{$\bang{}$-nat}
    \mylabel{ax:monoid:assoc}{$\codiag{}$-as}
    \mylabel{ax:monoid:unit}{$\codiag{}$-un}
    \mylabel{ax:monoid:comm}{$\codiag{}$-co}
    \mylabel{ax:monoid:nat:copy}{$\codiag{}$-nat}
    \mylabel{ax:monoid:nat:discard}{$\cobang{}$-nat}
    \[
    \begin{array}{c@{}c@{}c @{\qquad} c@{}c@{}c @{\qquad} c@{}c@{}c}
      \tikzfig{fbAx/comonoid/assoc/lhs} & \stackrel{\text{($\diag{}$-as)}}{=} & \tikzfig{fbAx/comonoid/assoc/rhs}
      &
      \tikzfig{fbAx/comonoid/unit/lhs} & \stackrel{\text{($\diag{}$-un)}}{=} & \tikzfig{fbAx/comonoid/unit/rhs}
      &
      \tikzfig{fbAx/comonoid/comm/lhs} & \stackrel{\text{($\diag{}$-co)}}{=} & \tikzfig{fbAx/comonoid/comm/rhs}
      \\[10pt]
      \tikzfig{fbAx/monoid/assoc/lhs} & \stackrel{\text{($\codiag{}$-as)}}{=} & \tikzfig{fbAx/monoid/assoc/rhs}
      &
      \tikzfig{fbAx/monoid/unit/lhs} & \stackrel{\text{($\codiag{}$-un)}}{=}& \tikzfig{fbAx/monoid/unit/rhs}
      &
      \tikzfig{fbAx/monoid/comm/lhs} & \stackrel{\text{($\codiag{}$-co)}}{=} & \tikzfig{fbAx/monoid/comm/rhs}
      \\[10pt]
      \multicolumn{9}{c}{
        \begin{array}{c@{}c@{}c @{\qquad} c@{}c@{}c}
          \tikzfig{fbAx/comonoid/nat/copy/lhs}  & \stackrel{\text{($\diag{}$-nat)}}{=} & \tikzfig{fbAx/comonoid/nat/copy/rhs}
          &
          \tikzfig{fbAx/comonoid/nat/discard/lhs}  & \stackrel{\text{($\bang{}$-nat)}}{=} & \tikzfig{fbAx/comonoid/nat/discard/rhs}
          \\[10pt]
          \tikzfig{fbAx/monoid/nat/copy/lhs}  & \stackrel{\text{($\codiag{}$-nat)}}{=} & \tikzfig{fbAx/monoid/nat/copy/rhs}
          &
          \tikzfig{fbAx/monoid/nat/discard/lhs}  & \stackrel{\text{($\cobang{}$-nat)}}{=} & \tikzfig{fbAx/monoid/nat/discard/rhs}
        \end{array}
      }
    \end{array}
    \]
    \caption{Axioms of fb categories in string diagrams.}
    \label{fig:ax-fb-string}
  \end{figure}
  \begin{figure}[h!]
    \centering
    \mylabel{ax:adjbiprod:1}{AA1}
    \mylabel{ax:adjbiprod:2}{AA2}
    \mylabel{ax:adjbiprod:3}{AA3}
    \mylabel{ax:adjbiprod:4}{AA4}
    % \includegraphics{figures/adjoint-biproducts.pdf}
    \[
    \begin{array}{c@{}c@{}c @{\qquad} c@{}c@{}c}
      \tikzfig{adjbiprod/AA1_lhs} & \axsubeq{\ref*{ax:adjbiprod:1}} & \tikzfig{adjbiprod/AA1_rhs} & \tikzfig{adjbiprod/AA2_lhs} & \axsubeq{\ref*{ax:adjbiprod:2}} & \tikzfig{adjbiprod/AA2_rhs} \\[15pt]
      \tikzfig{adjbiprod/AA3_lhs} & \axsubeq{\ref*{ax:adjbiprod:3}} & \tikzfig{adjbiprod/AA3_rhs} & \tikzfig{adjbiprod/AA4_lhs} & \axsubeq{\ref*{ax:adjbiprod:4}} & \tikzfig{adjbiprod/AA4_rhs}
    \end{array}
    \]
    \caption{Duality between the monoid and comonoid structures.\label{fig:adjoint-biproducts}}
  \end{figure}

As expected, the name refers to the fact that the convolution monoid in \eqref{eq:covolution} turns out to be idempotent, 
\[f+f=f\]
and thus any fb category with idempotent convolution turns out to be enriched over $\Cat{Jsl}$, the category of join semilattices. In particular, the posetal enrichement in the definition above coincides with the one induced by the semilattice structure.
\begin{lemma}\label{lemma:order-adjointness}
  In a fb category with idempotent convolution, $f \leq g$ iff $f+g=g$ for all $f,g \colon X \to Y$.
\end{lemma}
Viceversa, one can also show that in an arbitrary fb category $\Cat{C}$, if $+$ is idempotent then $\Cat{C}$ is poset enriched and the axioms in \Cref{fig:adjoint-biproducts} holds. %: see BLA BLA in Appendix \ref{app:Kleene}.
A more useful fact, it is the following normal form.

\begin{proposition}[Matrix normal form]\label{prop:matrixform}
In a fb category $\Cat{C}$, any arrow $f\colon S \piu X \to T \piu Y$ has a normal form %\marginpar{PLS ALESSANDRO, INSERISCI DIAGRAMMA}
\[f = \stringMatrix{f}{S}{T}{X}{Y} \]
where $f_{ST}\colon S \to T$,  $f_{SY}\colon S \to Y$, $f_{XT}\colon X \to T$ and  $f_{XY}\colon X \to Y$ are defined as follows.
\begin{equation}\label{eq:components}
\begin{array}{cc}
f_{ST} \defeq (\id{S} \piu \cobang{X}); f ; (\id{T} \piu \cobang{Y}) &  f_{SY} \defeq (\id{S} \piu \cobang{X}); f ; (\cobang{T} \piu \id{Y} )\\
f_{XT} \defeq (\cobang{S} \piu \id{X} ); f ; (\id{T} \piu \cobang{Y}) &  f_{XY} \defeq(\cobang{S} \piu \id{X} ); f ; (\cobang{T} \piu \id{Y} )
\end{array}
\end{equation}
Moreover, if $\Cat{C}$ has idempotent convolution, for all $f,g\colon S \piu X \to T \piu Y$, it holds that $f\leq g$ iff
\[\begin{array}{cccc}
f_{ST} \leq g_{ST}, &  f_{SY} \leq g_{SY}, &
f_{XT} \leq g_{XT} ,&  f_{XY} \leq g_{XY}.
\end{array}
\]
\end{proposition}
The reader can easily check that $(\Rel,\piu,\zero)$ (Section \ref{sec:2monREL}) is a finite biproduct category with idempotent convolution by checking that the four inequalities in Definition \ref{def:fbidempotent} hold using the definition of monoids and comonoids from \eqref{eq:comonoidsREL}. Moreover one can easily see that the four morphisms defined by \eqref{eq:components} instantiate, in the case of $(\Rel,\piu,\zero)$, to those in \eqref{eq:dec}.
% \ale{non capsico questo riferimento mancante}


\subsection{Kleene Bicategories are Typed Kleene Algebras}

We can now introduce the main structures of this section: Kleene bicategories. These are fb categories with idempotent convolution equipped with a trace that, intuitively, behaves well w.r.t. the poset enrichement.  


\begin{definition}\label{def:kleenebicategory}
    A \emph{Kleene bicategory} is a fb category with idempotent convolution that is traced monoidal such that %and satisfy the laws in Figures \ref{fig:ineq-uniformity} and \ref{fig:happy-trace}.
    \begin{enumerate}
%    \item $\Cat{B}$ is a finite biproduct category, with monoids $\codiag{X} \colon X \perG X \!\to\! X, \;\; \cobang{X} \colon \unoG \!\to\! X, \;\; \diag{X} \colon X \!\to\!  X \perG X, \;\; \bang{X} \colon X \!\to\! \unoG$;
%    \item $\Cat{B}$ is a traced monoidal category;
%    \item The monoids $(\codiag{X},\cobang{X})$ are left adjoint to the comonoids $(\diag{X},\bang{X})$: see the axioms in \Cref{fig:adjoint-biproducts};
    \item the trace satisfies the laws in Figure \ref{fig:ineq-uniformity}: for all $f\colon S\piu X \to S \piu Y$ and $g \colon T\piu X \to T \piu Y$,
    \begin{itemize}
    \item[(AU1)] if $\exists r\colon S \to T$ such that  $f ; (r \piu \id{Y}) \leq (r \piu \id{X}) ; g$, then $\trace_{S}f \leq \trace_{S}g$.
    \item[(AU2)] if $\exists r\colon T \to S$ such that  $(r \piu \id{X})  ; f \leq  g ; (r \piu \id{Y})$, then $\trace_{S}f \leq \trace_{S}g$.
    \end{itemize}
    \item the trace satisfies the axiom in Figure \ref{fig:happy-trace}: $\trace_{X}(\codiag{X};\diag{X}) \leq \id{X}$
    \end{enumerate}
A \emph{morphism of Kleene bicategories} is a poset enriched symmetric monoidal functor preserving (co)monoids and traces. Kleene bicategories and their morphisms form a category \(\KBicat\).
\end{definition}

% \marginpar{ALESSANDRO PLS: In the conclusion of both laws replace the rightmost $X$ of both $f$ and $g$ by $Y$. In the premise of the second law exchange $S$ and $T$}
  \begin{figure}[h!]
    \centering
    % \includegraphics{figures/ineq-uniformity-trace.pdf}
    \mylabel{ax:posetunif:1}{AU1}
    \mylabel{ax:posetunif:2}{AU2}
    \[
    \begin{array}{c}
      \tikzfig{posetunif/AU1_lhs} \leq \tikzfig{posetunif/AU1_rhs} \stackrel{(\ref*{ax:posetunif:1})}{\implies} \tikzfig{posetunif/AU1TR_lhs} \leq \tikzfig{posetunif/AU1TR_rhs}
      \\[20pt]
      \tikzfig{posetunif/AU2_lhs} \leq \tikzfig{posetunif/AU2_rhs} \stackrel{(\ref*{ax:posetunif:2})}{\implies} \tikzfig{posetunif/AU2TR_lhs} \leq \tikzfig{posetunif/AU2TR_rhs}
    \end{array}
    \]
    \caption{Uniformity axioms for posetal bicategories.\label{fig:ineq-uniformity}}
  \end{figure}
  \begin{figure}[h!]
    \centering
    \mylabel{ax:kb:traceid}{AT1}
    % \includegraphics{figures/happy-trace.pdf}
    \[ \tikzfig{kb/traceid_lhs} \axsubeq{\ref*{ax:kb:traceid}} \tikzfig{kb/traceid_rhs} \]
    \caption{Repeating the identity.\label{fig:happy-trace}}
  \end{figure}

The axioms in Figure \ref{fig:ineq-uniformity} can be understood as the posetal extension of the uniformity axioms defined in Section \ref{sec:traced}. Note that, by antisymmetry of $\leq$, the axioms in Figure \ref{fig:ineq-uniformity} entail those in Figure \ref{fig:uniformity}. Moreover, (see Lemma \ref{lemma:equivalentUnif} in Appendix \ref{app:Kleene}) the laws (AU1) and (AU2) can equivalently be expressed by the following one.

\begin{equation}\label{eq:equivalentuni1}\tag{AU1'}
\text{If }\exists r_1,r_2\colon S \to T\text{ such that } r_2 \leq r_1\text{ and }f ; (r_1 \piu \id{Y}) \leq (r_2 \piu \id{X}) ; g\text{, then }\trace_{S}f \leq \trace_{T}g\text{;}
\end{equation}
\begin{equation}\label{eq:equivalentuni2}\tag{AU2'}
\text{If }\exists r_1,r_2\colon T \to S\text{ such that } r_2 \leq r_1\text{ and }(r_1 \piu \id{X}) ; f   \leq   g; (r_2 \piu \id{Y})\text{, then }\trace_{S}f \leq \trace_{T}g\text{;}
\end{equation}





It is worth remarking that, while the axiom of uniformity has been widely studied (see e.g. \cite{hasegawa2003uniformity}), its posetal extension in Figure \ref{fig:ineq-uniformity} is, to the best of our knowledge, novel. Instead, the axioms in Figure \ref{fig:happy-trace} already appeared in the literature (see e.g. \cite{lmcs:10963}).













%%%%%%%%%%%%%%%%
%
% COMMENT
%
%%%%%%%%%%%%%%

\begin{comment}
\begin{definition}
  A posetal bicategory \(\Cat{B}\) has \emph{adjoint biproducts} if it has biproducts and the monoids arising from it are left adjoint to the comonoids with respect to the 2-cells (\Cref{fig:adjoint-biproducts}).
  \begin{figure}[h!]
    \centering
    \mylabel{ax:comonoid:assoc}{$\diag{}$-as}
    \mylabel{ax:comonoid:unit}{$\diag{}$-un}
    \mylabel{ax:comonoid:comm}{$\diag{}$-co}
    \mylabel{ax:comonoid:nat:copy}{$\diag{}$-nat}
    \mylabel{ax:comonoid:nat:discard}{$\bang{}$-nat}
    \mylabel{ax:monoid:assoc}{$\codiag{}$-as}
    \mylabel{ax:monoid:unit}{$\codiag{}$-un}
    \mylabel{ax:monoid:comm}{$\codiag{}$-co}
    \mylabel{ax:monoid:nat:copy}{$\codiag{}$-nat}
    \mylabel{ax:monoid:nat:discard}{$\cobang{}$-nat}
    \[
    \begin{array}{c@{}c@{}c @{\qquad} c@{}c@{}c @{\qquad} c@{}c@{}c}
      \tikzfig{fbAx/comonoid/assoc/lhs} & \stackrel{\text{($\diag{}$-as)}}{=} & \tikzfig{fbAx/comonoid/assoc/rhs}
      &
      \tikzfig{fbAx/comonoid/unit/lhs} & \stackrel{\text{($\diag{}$-un)}}{=} & \tikzfig{fbAx/comonoid/unit/rhs}
      &
      \tikzfig{fbAx/comonoid/comm/lhs} & \stackrel{\text{($\diag{}$-co)}}{=} & \tikzfig{fbAx/comonoid/comm/rhs}
      \\[10pt]
      \tikzfig{fbAx/monoid/assoc/lhs} & \stackrel{\text{($\codiag{}$-as)}}{=} & \tikzfig{fbAx/monoid/assoc/rhs}
      &
      \tikzfig{fbAx/monoid/unit/lhs} & \stackrel{\text{($\codiag{}$-un)}}{=}& \tikzfig{fbAx/monoid/unit/rhs}
      &
      \tikzfig{fbAx/monoid/comm/lhs} & \stackrel{\text{($\codiag{}$-co)}}{=} & \tikzfig{fbAx/monoid/comm/rhs}
      \\[10pt]
      \multicolumn{9}{c}{
        \begin{array}{c@{}c@{}c @{\qquad} c@{}c@{}c}
          \tikzfig{fbAx/comonoid/nat/copy/lhs}  & \stackrel{\text{($\diag{}$-nat)}}{=} & \tikzfig{fbAx/comonoid/nat/copy/rhs}
          &
          \tikzfig{fbAx/comonoid/nat/discard/lhs}  & \stackrel{\text{($\bang{}$-nat)}}{=} & \tikzfig{fbAx/comonoid/nat/discard/rhs}
          \\[10pt]
          \tikzfig{fbAx/monoid/nat/copy/lhs}  & \stackrel{\text{($\codiag{}$-nat)}}{=} & \tikzfig{fbAx/monoid/nat/copy/rhs}
          &
          \tikzfig{fbAx/monoid/nat/discard/lhs}  & \stackrel{\text{($\cobang{}$-nat)}}{=} & \tikzfig{fbAx/monoid/nat/discard/rhs}
        \end{array}
      }
    \end{array}
    \]
    \caption{Axioms of fb categories in string diagrams.}
    \label{fig:ax-fb-string}
  \end{figure}
  \begin{figure}[h!]
    \centering
    \mylabel{ax:adjbiprod:1}{AA1}
    \mylabel{ax:adjbiprod:2}{AA2}
    \mylabel{ax:adjbiprod:3}{AA3}
    \mylabel{ax:adjbiprod:4}{AA4}
    % \includegraphics{figures/adjoint-biproducts.pdf}
    \[
    \begin{array}{c@{}c@{}c @{\qquad} c@{}c@{}c}
      \tikzfig{adjbiprod/AA1_lhs} & \axsubeq{\ref*{ax:adjbiprod:1}} & \tikzfig{adjbiprod/AA1_rhs} & \tikzfig{adjbiprod/AA2_lhs} & \axsubeq{\ref*{ax:adjbiprod:2}} & \tikzfig{adjbiprod/AA2_rhs} \\[15pt]
      \tikzfig{adjbiprod/AA3_lhs} & \axsubeq{\ref*{ax:adjbiprod:3}} & \tikzfig{adjbiprod/AA3_rhs} & \tikzfig{adjbiprod/AA4_lhs} & \axsubeq{\ref*{ax:adjbiprod:4}} & \tikzfig{adjbiprod/AA4_rhs}
    \end{array}
    \]
    \caption{Duality between the monoid and comonoid structures.\label{fig:adjoint-biproducts}}
  \end{figure}
\end{definition}

\begin{definition}\label{def:uniformity-ineq}
  A posetal monoidal bicategory \(\Cat{B}\) is \emph{uniformly traced} if it is uniformly traced as monoidal category and uniformity extends to the two-cells (\Cref{fig:ineq-uniformity}):
  if \(f \dcomp (r \perG \id{}) \leq (r \perG \id{}) \dcomp g\), then \(\trace_{S} f \leq \trace_{T} g\) and, if \(f \dcomp (r \perG \id{}) \geq (r \perG \id{}) \dcomp g\), then \(\trace_{S} f \geq \trace_{T} g\).
\end{definition}
\begin{remark}
  uniformity with \(=\) follows from uniformity with \(\leq\) (if we assume antisymmetry, which we should)\\
  so we do not need to require uniformity with \(=\) in \Cref{def:uniformity-ineq}
\end{remark}

\begin{definition}
  A \emph{Kleene bicategory} is a posetal bicartesian monoidal bicategory with dual biproducts and uniform trace such that \(\trace_{X}(\codiag{X} \dcomp \diag{X}) \leq \id{X}\) (\Cref{fig:happy-trace}).
  \begin{figure}[h!]
    \centering
    \mylabel{ax:kb:traceid}{AT1}
    % \includegraphics{figures/happy-trace.pdf}
    \[ \tikzfig{kb/traceid_lhs} \axsubeq{\ref*{ax:kb:traceid}} \tikzfig{kb/traceid_rhs} \]
    \caption{Repeating the identity.\label{fig:happy-trace}}
  \end{figure}
\end{definition}

\begin{definition}
  A \emph{Kleene functor} \(\fun{F} \colon \Cat{B} \to \Cat{C}\) between two Kleene bicategories \(\Cat{B}\) and \(\Cat{C}\) is a bifunctor between the underlying bicategories that preserves biproducts and trace.
\end{definition}

\begin{proposition}
  Kleene bicategories and Kleene functors form a category \(\KBicat\).
\end{proposition}




\end{comment}

%%%%%%%%%%%%%%%%
%
% END OF COMMENT
%
%%%%%%%%%%%%%%

% \marginpar{PLS ALESSANDRO, nel diag di sin cambia $a$ con $f$ e in quello di destra $f$ con $a$. Inoltre nel diagramma di sinistra $S$ dovrebbe essere $X$}
\begin{figure}[h!]
  \centering
  % \includegraphics{figures/star-trace.pdf}
  \[
  \begin{array}{l@{\qquad}l}
    f \colon X \to X & a \colon S \piu X \to S \piu Y \\[5pt]
    \kstar{f} \defeq \Crepetition{f}{X}{X} & \trace_S a \defeq \Ctracerep{a\vphantom{\kstar{a}_{SS}}}{S}{X}{Y}
  \end{array}
  \]
  \caption{Repetition from trace and trace from repetition in finite biproduct categories.\label{fig:star-trace}}\end{figure}


Like in any finite biproduct category with trace (see e.g. \cite{cuazuanescu1994feedback}), in a Kleene bicategory one can define for each endomorphism $f\colon X \to X$, a morphism $\kstar{f}\colon X \to X$ as in Figure \ref{fig:star-trace}.
The distinguishing property of Kleene bicategories is that $\kstar{(\cdot)}$ satisfies the laws of Kleene star as axiomatised by Kozen in \cite{Kozen94acompleteness}.

\begin{definition}
A \emph{Kleene star operator} on a category $\Cat{C}$ enriched over join-semi lattices consists of a family of operations \(\kstar{(\cdot)} \colon \Cat{C}(X,X) \to  \Cat{C}(X,X)\)  such that for all $f\colon X\to X$, $r\colon X \to Y$ and $l\colon Y \to X$:\begin{equation}\label{eq:Kllenelaw}
    \begin{array}{c@{\qquad}c}
      \id{X} + f \dcomp \kstar{f} \leq \kstar{f} & f \dcomp r \leq r \implies  \kstar{f} \dcomp r \leq r  \\
      \id{X} + \kstar{f} \dcomp f \leq \kstar{f} & l \dcomp f  \leq l \implies   l \dcomp \kstar{f} \leq l
    \end{array}
\end{equation}
A \emph{typed Kleene algebra} is a category enriched over join-semi lattices that has a Kleene star operator. A \emph{morphism of typed Kleene algebras} is a functor preserving both the structures of join semilattice and Kleene star.
Typed Kleene algebras and their morphism form a category referred as $\TKAlg$.
%satisfying \eqref{eq:Kllenelaw}.
% Kleene star operator on a category \(\Cat{B}\) enriched over commutative idempotent monoids: \(\kstar{(\cdot)} \colon \Cat{B}(X,X) \to  \Cat{B}(X,X)\) satisfying
\end{definition}
\begin{remark}
The notion of typed Kleene algebra has been introduced by Kozen in \cite{kozen98typedkleene} in order to deal with Kleene algebras \cite{Kozen94acompleteness} with multiple sorts. In other words, a Kleene algebra is a typed Kleene algebra with a single object.
\end{remark}

On the one hand, the laws of Kleene bicategories are sufficient for defining a Kleene star operation. On the other, any Kleene star operation gives rise to a trace as in the right of Figure \ref{fig:star-trace} satisfying the laws of Kleene bicategories.

\begin{proposition}\label{prop:trace-star}
  Let $\Cat{C}$ be a fb category with idempotent convolution. $\Cat{C}$ is a Kleene bicategory iff $\Cat{C}$ has a Kleene-star operator.
\end{proposition}
Since Kleene bicategories are enriched over join semilattices, from the above result we have that

\begin{corollary}\label{cor:kleeneareka}
  All Kleene bicategories are typed Kleene algebras.
\end{corollary}
%\begin{proof}
%  Every Kleene bicategory is enriched over commutative monoids by \Cref{lemma:convolution-monoid}.
%  The Kleene star is defined using the trace (\Cref{prop:trace-star}).
%\end{proof}
The opposite does not hold: not all typed Kleene algebras are monoidal categories. Nevertheless, from an arbitrary Kleene algebra, one can canonically build a Kleene bicategory by means of the matrix construction, illustrated in the next section.







%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% COMMENT
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
\begin{itemize}
\item definition of typed kleene algebra
\item correspondence between traces and star, together with all the axioms and bla bla
\item Illustration of the forgetful functor; quickly say that it has a left adjoint that is given by the usual matrix costruction.
\end{itemize}

a repetition operator (axioms in Selinger's survey) corresponds to a uniform trace, if we have biproducts\\
a Kleene star operator (axioms in~\cite{Kozen94acompleteness,kozen98typedkleene}) corresponds to a uniform trace together with the axiom in \Cref{fig:happy-trace}, if we have biproducts\\

\begin{definition}
  A repetition operator on a category $\Cat{B}$ enriched over commutative idempotent monoids consists of a family of operations \(\kstar{(\cdot)} \colon \Cat{B}(X,X) \to  \Cat{B}(X,X)\) satisfying
  % repetition operator on a category \(\Cat{B}\) enriched over commutative idempotent monoids: \(\kstar{(\cdot)} \colon \Cat{B}(X,X) \to  \Cat{B}(X,X)\) satisfying
  \[
    \begin{array}{c@{\qquad}c}
      1 + f \dcomp \kstar{f} \leq \kstar{f}  & f \dcomp r \leq r \dcomp g \implies  \kstar{f} \dcomp r \leq r \dcomp \kstar{g}\\
      1 + \kstar{f} \dcomp f \leq \kstar{f} & f \dcomp r \geq r \dcomp g \implies  \kstar{f} \dcomp r \geq r \dcomp \kstar{g}
    \end{array}
  \]
\end{definition}

\begin{definition}
  A Kleene star operator on a category $\Cat{B}$ enriched over commutative idempotent monoids consists of a family of operations \(\kstar{(\cdot)} \colon \Cat{B}(X,X) \to  \Cat{B}(X,X)\) satisfying
  % Kleene star operator on a category \(\Cat{B}\) enriched over commutative idempotent monoids: \(\kstar{(\cdot)} \colon \Cat{B}(X,X) \to  \Cat{B}(X,X)\) satisfying
  \[
    \begin{array}{c@{\qquad}c}
      1 + f \dcomp \kstar{f} \leq \kstar{f} & f \dcomp r \leq r \implies  \kstar{f} \dcomp r \leq r  \\
      1 + \kstar{f} \dcomp f \leq \kstar{f} & f \dcomp r \geq r \implies  \kstar{f} \dcomp r \geq r
    \end{array}
  \]
\end{definition}

rephrase the definition by Kozen\\
Kozen has some work on Kleene algebras and Hoare logic~\cite{kozen00hoarekleene,kozen02hoarekleene}



we may define a repetition operator from a trace and vice versa (\Cref{fig:star-trace})



\begin{proposition} % this is not really needed so far
  In a Kleene bicategory, \(\kstar{f}\) is the least fixpoint of \(\phi_{f}\) as defined in \Cref{prop:star-fixpoint}.
\end{proposition}
\begin{proof}
  By \Cref{prop:star-fixpoint}, we already know that \(\kstar{f}\) is a fixpoint of \(\phi_{f}\).
  Suppose that \(r \colon S \to S\) is another fixpoint of \(\phi_{f}\), i.e.~that \(\phi_{f}(r) \leq r\).
  By definition of \(\phi_{f}\), \(\id{S} + f \dcomp r \leq r\).
  Then, by adjointness and \Cref{cor:bounds-star}, \(f \dcomp r \leq \id{} + f \dcomp r \leq r\).
  By strong uniformity, we obtain \(\kstar{f} \dcomp r \leq r\).
  By \Cref{cor:bounds-star}, \(\id{} \leq \id{} + f \dcomp r \leq r\).
  Then, \(\kstar{f} = \kstar{f} \dcomp \id{} \leq \kstar{f} \dcomp r \leq r\).
\end{proof}


equivalence of trace and star is a known result\\
uniformity with \(=\) is also known~\cite{someone}
\end{comment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% END OF COMMENT
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\subsection{The Matrix Construction}\label{ssec:matrix}
Thanks to Corollary \ref{cor:kleeneareka}, one can easily construct a forgetful functor $U\colon \KBicat \to \TKAlg$: any Kleene bicategory is a typed Kleene algebra and any morphism of Kleene bicategories is a morphism of typed Kleene algebras. To see the latter, observe that preserving $\kstar{(\cdot)}$, as defined in \Cref{fig:star-trace}, and the join-semi lattice, as in \eqref{eq:covolution}, is enough to preserve traces, monoidal product and (co)monoids.

We now illustrate that $U\colon \KBicat \to \TKAlg$ has a left adjoint provided by the \emph{matrix construction}, also known as \emph{biproduct completion} \cite{coecke2017two,mac2013categories}. In \cite[Exercises VIII.2.5-6]{mac2013categories}, it is shown that there exists an adjunction in between $\CMonCat$, the category of $\Cat{CMon}$-enriched categories, and $\FBC$, the category of fb categories.
\begin{equation}\label{eq:matrixadj}
\begin{tikzcd}
        \CMonCat
        \arrow[r, "\MatFun"{name=F}, bend left] &
        \FBC
        \arrow[l, "\fun{U}"{name=U}, bend left]
        \arrow[phantom, from=F, to=U, "\vdash" rotate=90]
    \end{tikzcd}
\end{equation}
The functor $U$ is the obvious forgetful functor: as recalled in Section \ref{ssec:fbic}, every fb category is  $\Cat{CMon}$-enriched. 
Given a $\CMon$-enriched category $\Cat S$, one can form the biproduct completion of $\Cat S$, denoted as $\Mat{\Cat S}$. Its objects are formal sums of objects of $\Cat S$, while a morphism $M \colon \Piu[k=1][n]{A_k} \to \Piu[k=1][m]{B_k}$ is a $m \times n$ matrix where $M_{ji} \in \Cat S[A_i,B_j]$. Composition is given by matrix multiplication, with the addition being the plus operation on the homsets (provided by the enrichment) and multiplication being composition. The identity morphism of $\Piu[k=1][n]{A_k}$ is given by the $n \times n$ matrix $(\delta_{ji})$, where $\delta_{ji} = \id{A_j}$ if $i=j$, while if $i \neq j$, then $\delta_{ji}$ is the zero morphism of $\Cat S[A_i,A_j]$.




\begin{proposition}\label{prop:matrices-kleene-bicategory}
Let  \(\Cat{K}\) be a typed Kleene algebra. Then  \(\Mat{\Cat{K}}\) is a Kleene bicategory.
\end{proposition}


More generally, one can show that  the functor \(\MatFun \colon \CMonCat \to \fbCat\) restricts to typed Kleene algebras and Kleene bicategories
and that this gives rise to the left adjoint to $U\colon \KBicat \to \TKAlg$.

\begin{corollary}\label{cor:adjKleene}
The adjunction in \eqref{eq:matrixadj} restricts to 
\[
\begin{tikzcd}
        \TKAlg
        \arrow[r, "\MatFun"{name=F}, bend left] &
        \;\; \KBicat \;\;
        \arrow[l, "\fun{U}"{name=U}, bend left]
        \arrow[phantom, from=F, to=U, "\vdash" rotate=90]
    \end{tikzcd}
\]
\end{corollary}
% \marginpar{SE ABBIAMO TEMPO E VOGLIA INSEIRE UNA PROVA A MODO}


% \subsection{Free Kleene bicategories}

% can we reuse the results in \Cref{sec:UTConstruction,sec:UTConstruction-products} to construct the free Kleene bicategory?


==> oldsections/sections/leading.tex <==
\section{Leading Example: The Calculus of Relations}\label{sec:leading}

==> oldsections/sections/monoidal.tex <==
\section{Monoidal Categories and String Diagrams}\label{sec:monoidal}
In this Appendix we recall the key aspects of the correspondence between monoidal categories and string diagrams \cite{joyal1991geometry,selinger2010survey}. Our starting point is regarding string diagrams as terms of a typed language. Given a set $\sort$ of basic \emph{sorts}, hereafter denoted by $A,B\dots$, types are elements of $\sort^\star$, i.e.\ words over $\sort$. Terms are defined by the following context free grammar
\begin{equation}\label{eq:syntaxsymmetricstrict}
\begin{array}{rcl}
f & ::=& \; \id{A} \; \mid \; \id{I} \; \mid \; \gen \; \mid \; \sigma_{A,B}^{\perG} \; \mid \;   f ; f   \; \mid \;  f \perG f \\
\end{array}
\end{equation}  
where $s$ belongs to a fixed set $\sign$ of \emph{generators} and $I$ is the empty word. Each $s\in \sign$ comes with two types: arity $\ar(s)$ and coarity $\coar(s)$. The tuple $(\sort, \sign, \ar, \coar)$, $\sign$ for short, forms a \emph{monoidal signature}. Amongst the terms generated by  \eqref{eq:syntaxsymmetricstrict}, we consider only those that can be typed according to the inference rules in Table~\ref{fig:freestricmmoncatax}. String diagrams are such terms modulo the axioms in Table~\ref{fig:freestricmmoncatax} where,  for any $X,Y\in \sort^\star$,  $\id{X}$ and $\sigma_{X,Y}^{\perG}$ can be easily built using $\id I$, $\id{A}$, $\sigma_{A,B}^{\perG}$, $\perG$ and $;$ (see e.g.~\cite{ZanasiThesis}).
\begin{table}[h]
    \centering
    \scalebox{0.8}{
    \begin{tabular}{c c}
        % Left column
        \begin{tabular}{c}
            \toprule
            Objects ($A\in \sort$) \\
            \midrule
            $X \; ::=\; \; A \; \mid \; \unoG \; \mid \;  X \perG X \vphantom{\sigma_{A,B}^{\perG}}$ \\
            \midrule
            \makecell{
                \\[-2pt] $(X\perG Y)\perG Z=X \perG (Y \perG Z)$ \\ 
                $X \perG \unoG = X $ \\ 
                $\unoG \perG X = X$ \\[2pt]
            } \\[13pt]
            \bottomrule
        \end{tabular}
        &
        % Right column
        \begin{tabular}{cc}
            \toprule
            \multicolumn{2}{c}{Arrows ($A\in \sort$, $s\in \sign$)} \\
            \midrule
            \multicolumn{2}{c}{$f \; ::=\; \; \id{A} \; \mid \; \id{\unoG} \; \mid \; \gen  \; \mid \;   f ; f   \; \mid \;  f \perG f \; \mid \; \sigma_{A,B}^{\perG}$} \\
            \midrule
            $(f;g);h=f;(g;h)$ & $id_X;f=f=f;id_Y$\\
            \multicolumn{2}{c}{$(f_1\perG f_2) ; (g_1 \perG g_2) = (f_1;g_1) \perG (f_2;g_2)$} \\
            $id_{\unoG}\perG f = f = f \perG id_{\unoG}$ & $(f \perG g)\, \perG h = f \perG \,(g \perG h)$ \\
            $\sigma_{A, B}^{\perG}; \sigma_{B, A}^{\perG}= id_{A \perG B}$ & $(\gen \perG id_Z) ; \sigma_{Y, Z}^{\perG} = \sigma_{X,Z}^{\perG} ; (id_Z \perG \gen)$ \\
            \bottomrule
        \end{tabular}
    \end{tabular}
    } % End of scalebox

    \vspace{2em} % Adjust spacing between tables

    \scalebox{0.75}{
    \begin{tabular}{c}
        \toprule
        Typing rules \\
        \midrule
        $
        {id_A \colon A \!\to\! A} \qquad  {id_\unoG \colon \unoG \!\to\! \unoG} \qquad {\sigma_{A, B}^{\perG} \colon A \perG B \!\to\! B \perG A} \qquad 
            \inferrule{\gen \colon \ar(s) \!\to\! \coar(s) \in \sign}{\gen \colon \ar(s) \!\to\! \coar(s)} \qquad
            \inferrule{f \colon X_1 \!\to\! Y_1 \and g \colon X_2 \!\to\! Y_2}{f \perG g \colon X_1 \perG X_2 \!\to\! Y_1 \perG Y_2}  \qquad
            \inferrule{f \colon X \!\to\! Y \and g \colon Y \!\to\! Z}{f ; g \colon X \!\to\! Z}
        $\\    
        \bottomrule  
    \end{tabular}
    } % End of scalebox

    \caption{Axioms for $\CatString$}
    \label{fig:freestricmmoncatax}
\end{table}



String diagrams enjoy an elegant graphical representation: a generator $\gen$ in $\sign$ with arity $X$ and coarity $Y$ is depicted as  a \emph{box} having \emph{labelled wires} on the left and on the right representing, respectively, the words $X$ and $Y$. For instance $\gen \colon AB \to C$ in $\sign$ is depicted as the leftmost diagram below. Moreover, $\id{A}$ is displayed as one wire,  $id_{\unoG} $ as the empty diagram and $\sigma_{A,B}^{\perG}$ as a crossing:
\begin{center}
    $\tikzfig{generator} \qquad \qquad \tikzfig{id} \qquad  \qquad     \tikzfig{empty} \qquad  \qquad   \tikzfig{symm}$
\end{center}
Finally, composition $f;g$ is represented by connecting the right wires 
of $f$ with the left wires of $g$ when their labels match, 
while the monoidal product $f \perG g$ is depicted by stacking the corresponding 
diagrams on top of each other: 
\begin{center}
    $\tikzfig{seq_comp} \qquad \qquad \qquad  \tikzfig{par_comp}$
\end{center}
The first three rows of axioms for arrows in Table~\ref{fig:freestricmmoncatax}
are implicit in the 
graphical representation while the axioms in the last row  are displayed as 
\begin{center}
    $\tikzfig{stringdiag_ax1_left} = \tikzfig{stringdiag_ax1_right} \quad\qquad \tikzfig{stringdiag_ax2_left} = \tikzfig{stringdiag_ax2_right}$
\end{center}


Hereafter, we call  $\CatString$ the category having as objects words in $\sort^\star$ and as arrows string diagrams. Theorem 2.3 in~\cite{joyal1991geometry} states that  $\Cat{C}_\sign$ is a \emph{symmetric strict monoidal category freely generated} by $\sign$.
\begin{definition} A \emph{symmetric monoidal category}  consists 
of a category $\Cat{C}$, a functor $\perG \colon \Cat{C} \times \Cat{C} \to \Cat{C}$,
an object $\unoG$  and natural isomorphisms \[ \alpha_{X, Y, Z} \colon (X \perG Y) \perG Z \to X \perG (Y \perG Z) \qquad \lambda_X \colon \unoG \perG X \to X \qquad \rho_X \colon X \perG \unoG \to X \qquad \sigma_{X, Y}^{\perG} \colon X \perG Y \to Y \perG X \]
satisfying some coherence axioms (in Figures~\ref{fig:moncatax} and~\ref{fig:symmmoncatax}).
A monoidal category is said to be \emph{strict} when $\alpha$, $\lambda$ and $\rho$ are all identity natural isomorphisms. A \emph{strict symmetric monoidal functor} is a functor $F \colon \Cat{C} \to \Cat{D}$  preserving $\perG$, $\unoG$ and $\sigma^{\perG}$. We write $\SMC$ for the category of ssm categories and functors. 

\end{definition}
\begin{remark}\label{rmk:symstrict}
In \emph{strict}  symmetric monoidal (ssm) categories  the symmetry $\sigma$ is not forced to be the identity, since this would raise some problems: for instance, $(f_1;g_1) \perG (f_2;g_2) = (f_1;g_2) \perG (f_2;g_1)$ for all $f_1,f_2\colon A \to B$ and $g_1,g_2\colon B \to C$. %As we will see in  Section~\ref{sec:rigcategories}, 
This fact will make the issue of strictness for rig categories rather subtle.
\end{remark}


To illustrate in which sense $\Cat{C}_\sign$ is freely generated, it is convenient to introduce \emph{interpretations} in a fashion similar to~\cite{selinger2010survey}: an interpretation $\interpretation$ of $\sign$ into an ssm category $\Cat{D}$ consists of two functions $\alpha_{\sort} \colon \sort \to Ob(\Cat{D})$ and $\alpha_{\sign}\colon \sign \to Ar(\Cat{D})$ such that, for all $s\in \sign$, $\alpha_{\sign}(s)$ is an arrow having as domain $\alpha_{\sort}^\sharp(\ar(s))$ and codomain $\alpha_{\sort}^\sharp(\coar(s))$, for $\alpha_{\sort}^\sharp\colon \sort^\star \to Ob(\Cat{D})$ the inductive extension of  $\alpha_{\sort}$.  $\CatString$ is freely generated by $\sign$ in the sense that, for all symmetric strict monoidal categories $\Cat{D}$ and  all interpretations $\interpretation$ of $\sign$ in $\Cat{D}$, there exists a unique ssm-functor $\dsem{-}_{\interpretation}\colon \Cat{C}_\sign \to \Cat{D}$ extending $\interpretation$ (i.e. $\dsem{s}_\interpretation=\alpha_{\sign}(s)$ for all $s\in \sign$).

One can easily extend the notion of interpretation of $\sign$ into a symmetric monoidal category $\Cat D$ that is not necessarily strict. In this case we set $\alpha^\sharp_\sort \colon \sort^\star \to Ob(\Cat D)$ to be the \emph{right bracketing} of the inductive extension of $\alpha_\sort$. For instance, $\alpha^\sharp_\sort(ABC) = \alpha_\sort(A) \perG (\alpha_\sort(B) \perG \alpha_\sort(C))$.

%%%%%%CIPRIANO: TAGLIATO QUI





%
%
%
%
%
%
\subsection{Finite Product and Finite Coproduct Categories}\label{ssec:fbcat}
%
%An important feature of (symmetric) monoidal categories is the fact the existence of certain (co)limits, usually defined by means of universal properties, can be characterised through some algebraic structures in a monoidal category. 
%A result by Fox \cite{}, will play an important role for the development of our work: categor


Within a symmetric monoidal category it is possible to define certain algebraic structures that can characterise $\perG$ as certain (co)limits: Fox's theorem \cite{fox1976coalgebras} states that if every object of a symmetric monoidal category is equipped with a natural and commutative comonoid structure, then $\perG$ is the categorical product $\times$.
%\begin{definition}
%Let $\Cat{C}$ be a symmetric monoidal category. A \emph{commutative monoid} in $\Cat{C}$ consists of an object $X$ and arrows $\cobang{X} \colon \unoG \to X$ and $\codiag{X}\colon X \perG X \to X$ making the diagrams in Figure~\ref{fig:monoidax} commute. 
%A \emph{cocommutative comonoid} in $\Cat{C}$ is a commutative monoid in $\Cat{C}^{op}$, namely, it is an object $X$ with arrows $\bang{X} \colon X \to \unoG$ and $\diag{X}\colon X \to X \perG X$ making the diagrams in Figure~\ref{fig:comonoidax} commute.
%\end{definition}
%Hereafter we will often avoid to specify (co)commutative and just write (co)monoids.






%\begin{figure}[t]
 %   \begin{equation}\tag{Mon1}
  %      \input{tikz-cd/monoid_assoc.tikz}
   % \end{equation}
    %\begin{minipage}[t]{0.50\textwidth}
     %   \begin{equation}\tag{Mon2}
      %      \input{tikz-cd/monoid_unit.tikz}
       % \end{equation}
%    \end{minipage}
 %   \hfill
  %  \begin{minipage}[t]{0.46\textwidth}
   %     \begin{equation}\tag{Mon3}
    %        \input{tikz-cd/monoid_comm.tikz}
%     %   \end{equation}
 %   \end{minipage}
  %  \caption{Commutative monoid axioms}
   % \label{fig:monoidax}
%\end{figure}

%
%\begin{figure}[t]
 %   \begin{equation}
  %      \input{tikz-cd/comonoid_assoc.tikz}\tag{Com1}
  %  \end{equation}
   % \begin{minipage}[t]{0.50\textwidth}
    %    \begin{equation}\tag{Com2}
     %       \input{tikz-cd/comonoid_unit.tikz}
      %  \end{equation}
   % \end{minipage}
    %\hfill
    %\begin{minipage}[t]{0.46\textwidth}
     %   \begin{equation}\tag{Com3}
      %      \input{tikz-cd/comonoid_comm.tikz}
      %  \end{equation}
   %% \end{minipage}
    %\caption{Cocommutative comonoid axioms}
   % \label{fig:comonoidax}
%\end{figure}



%\begin{definition}
%Let $(\Cat C, \perG, \unoG)$ be a symmetric monoidal category. $\Cat C$ is called:
%\noindent \begin{enumerate}
%\item a \emph{finite product} (fp, for short) \emph{category} %is a symmetric monoidal category where
%if every object has a comonoid structure $(\diag X, \bang X)$ satisfying the coherence axioms in Figure~\ref{fig:fpcoherence} (p.~\pageref{fig:fpcoherence}) and making $\diag{}$ and $\bang{}$ natural transformations.
%\item a \emph{finite coproduct} (fc) \emph{category} %is a symmetric monoidal category where 
%if every object has a monoid structure $(\codiag X, \cobang X)$ satisfying the coherence axioms in Figure~\ref{fig:fccoherence} (p.~\pageref{fig:fccoherence}) and making $\codiag{}$ and $\cobang{}$ natural transformations.
%\item a \emph{finite biproduct} (fb) \emph{category} %is a symmetric monoidal category where 
%if every object has both natural (in the sense above)  monoid and comonoid structures satisfying the coherence axioms in Figures~\ref{fig:fpcoherence} and~\ref{fig:fccoherence}.
%\end{enumerate}
%\end{definition}

\begin{remark}\label{rem:productcomonoids}
	\begin{enumerate}[leftmargin=*]
\item For any two objects $X_1$, $X_2$ of a  fp-category $\Cat C$ (see Definition~\ref{def:fp}), $X_1 \per X_2$ is the categorical product $X_1 \times X_2$: the projections $\pi_1\colon X_1 \per X_2 \to X_1$ and $\pi_2\colon X_1 \ X_2 \to X_2$ are  
\[\begin{tikzcd}[column sep=3em]
X_1 \per X_2 \ar[r,"\id{X_1} \per \, \discharger{X_2}"] &  X_1 \per \unoG \ar[r,"\runit{X_1}"]  & X_1
	\end{tikzcd}
\quad \text{and} \quad
\begin{tikzcd}[column sep=3em]
X_1 \per X_2 \ar[r," \discharger{X_1} \per \id{X_2} "] &  \unoG \per X_2 \ar[r,"\lunit{X_2}"]  & X_2.
	\end{tikzcd}	
\]
The unit $\unoG$ is the terminal object and $\discharger{X}$ the unique morphism of type $X \to \unoG$. 
For $f_1\colon Y\to X_1$, $f_2 \colon Y \to X_2$, their pairing $\pairing{f_1,f_2}\colon Y \to X_1 \per X_2$ is given by %\[\diag{Y}; (f_1 \perG f_2)\]
\[\begin{tikzcd}
Y  \ar[r,"\copier{Y}"] & Y \per Y \ar[r,"f_1 \per f_2"] &  X_1 \per X_2.
	\end{tikzcd}\]
	
\item In a fc category, $X_1 \piu X_2$ is instead a categorical coproduct, with injections $\iota_i \colon X_i \to X_1 \piu X_2$ and copairing $\copairing{f_1,f_2} \colon X_1 \piu X_2 \to Y$, for $f_1 \colon X_1 \to Y$ and $f_2 \colon X_2 \to Y$, in the dual way. Also dually $\unoG$ is the initial object 0 and $\cobang X$ the unique morphism of type $0 \to X$.
\end{enumerate}
\end{remark}




Like for (symmetric) monoidal categories, we are interested in freely generated fp (fc) categories. We will illustrate first the case for fc categories.

%To freely generate a fb category from a signature $\sign$ one has to take the usual symmetric monoidal structure, add $\bang{X}$, $\diag{X}$, $\cobang{X}$, $\codiag{X}$ for all $X \in\sort^\star$ and impose the axioms expressing naturality (ninth row in Table~\ref{fig:freerigcat}, p.~\pageref{fig:freerigcat}), those for (comonoids) in Figures~\ref{fig:monoidax},~\ref{fig:comonoidax} and those for coherence in Figures~\ref{fig:fpcoherence},~\ref{fig:fccoherence} (pp.~\pageref{fig:fpcoherence}-\pageref{fig:fccoherence}).

\begin{comment}
\begin{definition}\label{def:freesymmonoidalcat}
Given a monoidal signature $\sign$, we denote by $\Cat{fbC}_\sign$ the free fb category generated by $\sign$:
objects are terms in $\terms{\sign}(\sort)$; arrows are inductively generated by the rules in Tables~\ref{fig:freemmoncat},~\ref{fig:freesymmmoncat},~\ref{fig:freefbcat}  modulo the axioms in the same tables and the axioms in Figures~\ref{fig:moncatax},~\ref{fig:symmmoncatax},~\ref{fig:monoidax},~\ref{fig:comonoidax},~\ref{fig:fpcoherence},~\ref{fig:fccoherence}.
\end{definition}





\begin{table}
\begin{center}
\begin{tabular}{|c|}
\hline
Rules \\
\hline
$\inferrule{X \in \terms{\sigMon}(\sort)}{\bang{X} \colon X \to \unoG} \qquad
\inferrule{X \in \terms{\sigMon}(\sort)}{\diag{X} \colon X \to X \perG X} \qquad 
\inferrule{X \in \terms{\sigMon}(\sort)}{\cobang{X} \colon \unoG \to X} \qquad
\inferrule{X \in \terms{\sigMon}(\sort)}{\codiag{X} \colon X \perG X \to X} $ \\
\hline
\hline
Axioms \\
\hline
$f; \bang{Y}=\bang{X} \qquad f; \diag{Y}=\diag{X}; (f \perG f) \qquad \cobang{X};f =\cobang{Y} \qquad \codiag{X};f =(f\perG f); \codiag{Y}$ \\
\hline
\end{tabular}
\end{center}
\caption{Additional rules and axioms for freely generating a finite biproduct category.}\label{fig:freefbcat}
\end{table}
\end{comment}

Like for symmetries, it is enough to add as generators  $\cobang{A}$, $\codiag{A}$ for all $A \in \sort$ and define $\cobang{X}$, $\codiag{X}$ for all $X \in \sort^*$ inductively as follows:
%\begin{equation}\label{eq:diagind}\begin{array}{rcl|rcl}
%\bang{\unoG} &\defeq& \id{\unoG} & \diag{\unoG} &\defeq& \id{\unoG}  \\
%\bang{A \perG W} &\defeq& \bang{A} \perG \bang{W} & \diag{A \perG W}&\defeq& (\diag{A}\perG \diag{W}) ; (\id{A} \perG \sigma_{A,W} \perG \id{W})\\
%\end{array}\end{equation}

\begin{equation}\label{eq:codiagind}\begin{array}{rcl|rcl}
\cobang{\unoG} &\defeq& \id{\unoG} & \codiag{\unoG} &\defeq& \id{\unoG} \\
\cobang{A \perG W} &\defeq& \cobang{A} \perG \cobang{W} & \codiag{A \perG W}&\defeq& (\id{A} \perG \sigma_{A,W} \perG \id{W}) ; (\codiag{A}\perG \codiag{W})\\
\end{array}
\end{equation}
With these definitions the coherence axioms in Figures~\ref{fig:fccoherence} are automatically satisfied. In the strict setting also the monoid and comonoid axioms get simplified, as illustrated in the second row of Table~\ref{fig:freestrictfbcat}. Like for symmetries, to obtain naturality of  $\cobang{X}$, $\codiag{X}$ for arbitrary arrows, it is enough to impose naturality just with respect to the generators in $\Sigma$. %However, one has to take care also of naturality of  $\bang{A}$, $\diag{A}$ with respect to $\cobang{A}$, $\codiag{A}$: these are exactly the so called \emph{bialgebra axioms} in the third row  of Table~\ref{fig:freestrictfbcat}.

\begin{table}
\begin{center}
\begin{tabular}{c}
$\copier{ A}; (\id{ A}\perG \copier{ A}) = \copier{ A};(\copier{ A}\perG \id{ A}) \qquad \copier{ A} ; (\discharger{ A}\perG \id{ A}) = \id{ A} \qquad \copier{ A};\sigma_{ A, A}=\copier{ A}$ \\
$(\id{ A}\perG \codiag{ A}) ; \codiag{ A} = (\codiag{ A}\perG \id{ A}) ; \codiag{ A} \qquad (\cobang{ A}\perG \id{ A}) ; \codiag{ A}  = \id{ A} \qquad \sigma_{ A, A};\codiag{ A}=\codiag{ A}$ \\

%$\codiag{ A};\diag{ A} = \diag{ A\perG  A} ; (\codiag{ A} \perG \codiag{ A}) \qquad \cobang{ A}; \bang{ A}= \id{\unoG} \qquad \cobang{ A}; \diag{ A}= \cobang{ A\perG  A} \qquad \diag{ A}; \bang{ A}= \bang{ A\perG  A}$\\

$\gen; \discharger{Y}=\discharger{X} \qquad \gen; \copier{Y}=\copier{X}; (\gen \perG \gen)  $\\
$\cobang{X};\gen =\cobang{Y}\qquad
\codiag{X};\gen =(\gen \perG \gen); \codiag{Y}$ \\
\end{tabular}
\end{center}
\caption{Additional axioms for freely generated strict fp and fc categories.}\label{fig:freestrictfbcat}
\end{table}

\begin{comment}
\begin{table}
\begin{center}
\begin{tabular}{|c|}
\hline
Rules \\
\hline
$\inferrule{A \in \sort}{\bang{A} \colon A \to \unoG} \qquad
\inferrule{A \in \sort}{\diag{A} \colon A \to A \perG A} \qquad 
\inferrule{A \in \sort}{\cobang{A} \colon \unoG \to A} \qquad
\inferrule{A \in \sort}{\codiag{A} \colon A \perG A \to A} $ \\
\hline
\hline
Axioms \\
\hline
$\diag{A}; (\id{A}\perG \diag{A}) = \diag{A};(\diag{A}\perG \id{A}) \qquad \diag{A} ; (\bang{A}\perG \id{A}) = \id{A} \qquad \diag{A};\sigma_{A,A}=\diag{A}$ \\
$(\id{A}\perG \codiag{A}) ; \codiag{A} = (\codiag{A}\perG \id{A}) ; \codiag{A} \qquad (\cobang{A}\perG \id{A}) ; \codiag{A}  = \id{A} \qquad \sigma_{A,A};\codiag{A}=\codiag{A}$ \\

$\codiag{A};\diag{A} = \diag{A\perG A} ; (\codiag{A} \perG \codiag{A}) \qquad \cobang{A}; \bang{A}= \id{\unoG} \qquad \cobang{A}; \diag{A}= \cobang{A\perG A} \qquad \diag{A}; \bang{A}= \bang{A\perG A}$\\

$f; \bang{Y}=\bang{X} \qquad f; \diag{Y}=\diag{X}; (f \perG f) \qquad \cobang{X};f =\cobang{Y} \qquad \codiag{X};f =(f\perG f); \codiag{Y}$ \\
\hline
\end{tabular}
\end{center}
\caption{Additional rules and axioms for freely generating a strict fb category.}\label{fig:freestrictfbcat}
\end{table}

\begin{definition}\label{def:freesymmonoidalcat}
   Given a monoidal signature $\sign$, we denoted by $\Cat{sfbC}_\sign$ the free strict fb category generated by $\sign$:
   objects are elements of $\sort^\star$; arrows are inductively generated by the rules in Tables~\ref{fig:freestricmmoncatax},~\ref{fig:freestrictsymmmoncat} and~\ref{fig:freestrictfbcat} modulo the axioms in the same tables.
   \end{definition}
\end{comment}




%\begin{definition}\label{def:freesymmonoidalcat}
In a nutshell, the free strict fc category generated by $\sign$ is defined as follows. Objects are elements of $\sort^\star$; 
   arrows are the $\sign$-terms inductively generated as 
   \begin{equation}
\begin{array}{rcl}
f & ::=& \; \id{A} \; \mid \; \id{I} \; \mid \; \gen  \; \mid \;   f ; f   \; \mid \;  f \perG f \; \mid \; \sigma_{A,B}^{\perG} \; \mid \; \cobang{A}\; \mid \; \codiag{A}\\
%&& \alpha^{\perG}_{X,Y,Z} \; \mid \; \lambda^{\perG}_X  \; \mid \; \rho^{\perG}_{X} \; \mid \; \alpha^{-\perG}_{X,Y,Z} \; \mid \; \lambda^{-\perG}_X  \; \mid \; \rho^{-\perG}_{X}  \\
%&& \assoct{X}{Y}{Z} \; \mid \; \lunitt{X} \; \mid \; \runitt{X} \; \mid \; \Iassoct{X}{Y}{Z} \; \mid \; \Ilunitt{X} \; \mid \; \Irunitt{X}  \\
%& &   \dl{X}{Y}{Z} \; \mid \; \dr{X}{Y}{Z}  \; \mid \annl X \; \mid \annr X \; \mid \;   \Idl{X}{Y}{Z} \; \mid \; \Idr{X}{Y}{Z}  \; \mid \Iannl X \; \mid \Iannr X \\
\end{array}
\end{equation}  
modulo the axioms in   Tables~\ref{fig:freestricmmoncatax} and those in the second and fourth rows of Figure~\ref{fig:freestrictfbcat}. 

The free strict fp category generated by $\Sigma$ is obtained similarly, considering adding as generators $\copier{A}$ and $\discharger{A}$ for all $A\in \sort$ and defining $\copier{X}$, $\discharger{X}$ for all $X \in \sort^*$ inductively as follows:
\begin{equation}\label{eq:diagind}\begin{array}{rcl|rcl}
\discharger{\unoG} &\defeq& \id{\unoG} & \copier{\unoG} &\defeq& \id{\unoG}  \\
\discharger{A \perG W} &\defeq& \discharger{A} \perG \discharger{W} & \copier{A \perG W}&\defeq& (\copier{A}\perG \copier{W}) ; (\id{A} \perG \sigma_{A,W} \perG \id{W})\\
\end{array}\end{equation}
modulo the axioms in   Tables~\ref{fig:freestricmmoncatax} and those in the first and third rows of Figure~\ref{fig:freestrictfbcat}. 

Also the arrows of free strict fc (fp) categories enjoy an elegant graphical representation in terms of string diagrams.  However we are not going to illustrate it now since this would be redundant with tape diagrams.

\begin{comment}

$\bang{A}$, $\diag{A}$, $\cobang{A}$, $\codiag{A}$ are depicted as

\[ \counit A \quad \comonoid A \quad \unit A \quad \monoid A \quad \]

The axioms of Table~\ref{fig:freestrictfbcat} are graphically rendered as in Figure~\ref{fig:comonoidaxD},~\ref{fig:bialgaxD},~\ref{fig:nataxD}.

\newpage

\begin{figure}[h]
    \[ \tikzfig{comonoid_assoc_left} = \tikzfig{comonoid_assoc_right} \;\;\hfill
    \tikzfig{comonoid_unit_left} = \wire A \;\;\hfill 
    \tikzfig{comonoid_comm_left} = \comonoid A \]
    \[ \tikzfig{monoid_assoc_left} = \tikzfig{monoid_assoc_right} \;\;\hfill
    \tikzfig{monoid_unit_left} = \wire A \;\;\hfill 
    \tikzfig{monoid_comm_left} = \monoid A \]
    \caption{(Co)monoid axioms} %    \label{fig:comonoidaxD}
%\end{figure}
%
%\begin{figure}[ht]
    \begin{align*}
        \tikzfig{bialgax1_left} =& \tikzfig{bialgax1_right} \qquad \tikzfig{bialgax4_left} = \tikzfig{empty} \\
        \tikzfig{bialgax2_left} =& \tikzfig{bialgax2_right} \qquad\qquad\; \tikzfig{bialgax3_left} = \tikzfig{bialgax3_right}
    \end{align*}
    \caption{Bialgebra axioms}
%    \label{fig:bialgaxD}
%\end{figure}
%
%\begin{figure}[ht]
    \[\tikzfig{monoidnat_left} = \tikzfig{monoidnat_right} \quad \tikzfig{unitnat_left} = \unit X\]
    \[\tikzfig{comonoidnat_left} = \tikzfig{comonoidnat_right} \quad \tikzfig{counitnat_left} = \counit X\]
    \caption{(Co)monoid homomorphism axioms}
    \label{fig:nataxD}
\end{figure}
\end{comment}

% \newpage
%%%%%%%%%%%%%%%%%%%%%%%%%%%%CIPRIANO TABELLA Axioms for freely generated monoidal/symmetric monoidal/fb/rig categories OSCURATA


%\begin{table}[h]
%\begin{center}
%\begin{tabular}{cl}
%$(f;g);h=f;(g;h) \qquad id_X;f=f=f;id_Y$& (cat)\\

%$id_{X\perG Y}= id_{X} \perG id_{Y} \qquad (f_1\perG f_2) ; (g_1 \perG g_2) = (f_1;g_1) \perG (f_2;g_2) $ & (fun)\\

%$(id_{\unoG}\perG f) ; \lambda_Y^{\perG} = \lambda_X^{\perG} ; f \qquad (f \perG id_{\unoG}) ; \rho_Y^{\perG} = \rho_X^{\perG} ; f $ & (nat)\\
%$(\,(f \perG g)\, \perG h) ; \alpha_{X_2,Y_2,Z_2}^{\perG} = \alpha_{X_1,Y_1,Z_1}^{\perG} ; (f \perG \,(g \perG h)\, ) $ & (nat)\\

%$\lambda_X^{\perG} ; \lambda^{-\perG}_X = id_{\unoG \perG X } \qquad \lambda^{-\perG}_{X};\lambda_X^{\perG} = id_X \qquad 
%\rho_X^{\perG} ; \rho^{-\perG}_X = id_{X  \perG \unoG  } \qquad \rho^{-\perG}_{X};\rho_X^{\perG} = id_X $& (inv)\\
%$\alpha_{X,Y,Z}^{\perG} ; \alpha_{X,Y,Z}^{-\perG} = id_{ (X \perG Y) \perG Z} \qquad \alpha_{X,Y,Z}^{-\perG} ; \alpha_{X,Y,Z}^{\perG}=id_{X \perG (Y \perG Z)} $ & (inv)\\
%\\
%$(f \perG id_Z) ; \sigma_{Y, Z} = \sigma_{X,Y} ; (id_Z \perG f)$& (nat)\\ 
%$\sigma_{X, Y}; \sigma_{Y, X}= id_{X \perG Y}$ & (inv)\\
%\\
%$f; \bang{Y}=\bang{X} \qquad f; \diag{Y}=\diag{X}; (f \perG f) \qquad \cobang{X};f =\cobang{Y} \qquad \codiag{X};f =(f\perG f); \codiag{Y}$ & (nat)\\
%\\
 %   $(f \per (g \piu h)) ; \dl{X_2}{Y_2}{Z_2} = \dl{X_1}{Y_1}{Z_1} ; ((f \per g) \piu (f \per h)) $& (nat)\\
%    $((f \piu g) \per h) ; \dr{X_2}{Y_2}{Z_2} = \dr{X_1}{Y_1}{Z_1} ; ((f \per h) \piu (g \per h)) $ & (nat) \\
%    $(f \per id_\zero) ; \annl Y = \annl X ; id_\zero \qquad (id_\zero \per f) ; \annr Y = \annr X ; id_\zero$ & (nat) \\
%    $\dl{X}{Y}{Z} ; \Idl{X}{Y}{Z} = id_{X \per (Y \piu Z)} \qquad \Idl{X}{Y}{Z} ; \dl{X}{Y}{Z} = id_{(X \per Y) \piu (X \per Z)}$ & (inv) \\
%    $\dr{X}{Y}{Z} ; \Idr{X}{Y}{Z} = id_{(X \piu Y) \per Z} \qquad \Idl{X}{Y}{Z} ; \dl{X}{Y}{Z} = id_{(X \per Z) \piu (Y \per Z)}$ & (inv) \\
%    $\annl X ; \Iannl X = id_{\zero \per X } \qquad \Iannl X;\annl X = id_\zero \qquad 
%    \annr X ; \Iannr X = id_{X  \per \zero  } \qquad \Iannr X;\annr X = id_\zero $ & (inv)\\
%    \end{tabular}
 %   \end{center}
 %    \caption{Axioms for freely generated monoidal/symmetric monoidal/fb/rig categories. Here $f \colon X \to Y$. }
  %      \label{fig:freerigcat}
%\end{table}







==> oldsections/sections/peano.tex <==

\section{The Kleene-Cartesian Tape Theory of Peano}\label{sec:peano}
In Section \ref{ssec:funsem}, we introduced kc tape theories and in Example \ref{ex:totalorder} we illustrated the theory of linear orders.
In this section we illustrate a further example of theory that fully exploits the expressive power of Kleene-Cartesian rig categories: Peano's axiomatisation of natural numbers. This  theory is not expressible in first order logic \cite{harsanyi1983mathematics}
but it can be succinctly expressed by a kc tape theory.

As expected we begin by fixing  the  signature:
\[\sort\defeq \{A\} \qquad \text{and} \qquad \sign \defeq \{ \; \tikzfig{peano/zero}, \tikzfig{peano/succ}  \}\text{.} \]
An interpretation of $\sign$ in $\Rel$ consists of 
\begin{center}
\begin{tabular}{rl}
a set $X$ &(i.e., $\alpha_\sort(A)$), \\
a relation $0 \subseteq 1 \times X$ & (i.e., $\alpha_\sign( \, \tikzfig{peano/zero} )$) and \\
a relation $s\subseteq  X \times X$ & (i.e., $\alpha_\sign(  \tikzfig{peano/succ} )$)\text{.}
\end{tabular}
\end{center}

The set of axioms $\mathbb{P}$ contains those illustrated in Figure \ref{fig:tape-theory-natural-numbers}.
The axioms at the top force the copairing of $0$ and $s$, that is $[0,s]  \defeq (0 \piu s) ; \codiag{A}$ to be an isomorphism of type $1+X \to X$.
The axiom on the left states that $\op{[0,s]}; [0,s] = \id{A}$; the one on the right that $[0,s];\op{[0,s]}= \id{A \piu A}$.
The axiom at the bottom of Figure \ref{fig:tape-theory-natural-numbers} is the induction axiom. Intuitively, it states that every element of $X$ should be contained in $0;s^* \colon 1\to X$.
Thus, overall an interpretation in $\Rel$ is a model of the theory $(\sign, \mathbb{P})$ iff $X$ is isomorphic to $X+1$ and equal to $0;s^*$.

An example of a model is obviously given by the set of natural numbers $\N$, equipped with the element zero $0\colon 1 \to \N$ and the successor function $s\colon \N \to \N$. 
We will see soon that  this is the unique --up-to isomorphism-- model of $(\sign, \mathbb{P})$.


\begin{figure}[H]
    \mylabel{ax:peanoT:zero:sv}{$0$-sv}
    \mylabel{ax:peanoT:zero:tot}{$0$-tot}
    \mylabel{ax:peanoT:succ:sv}{$s$-sv}
    \mylabel{ax:peanoT:succ:tot}{$s$-tot}
    \mylabel{ax:peanoT:ind}{ind}
    \mylabel{ax:peanoT:iso:1}{iso-1}
    \mylabel{ax:peanoT:iso:2}{iso-2}
    \[
        \begin{array}{c@{\qquad}c}
                \tikzfig{peano/ax1/iso1/lhs} \stackrel{\eqref{ax:peanoT:iso:1}}{=} \tikzfig{peano/ax1/iso1/rhs}
                &
                \tikzfig{peano/ax1/iso2/lhs} \stackrel{\eqref{ax:peanoT:iso:2}}{=} \tikzfig{peano/ax1/iso2/rhs}
                \\[20pt]
                \hline
                \multicolumn{2}{c}{
                    \begin{array}{c}
                        \\
                        \tikzfig{peano/ax1/ind/lhs} \stackrel{\eqref{ax:peanoT:ind}}{=} \tikzfig{peano/ax1/ind/rhs}
                    \end{array}
                }
        \end{array}
    \]
    \caption{Tape theory of the natural numbers.}
    \label{fig:tape-theory-natural-numbers}
\end{figure}
% \begin{figure}[ht!]
%     \mylabel{ax:peanoT:zero:sv}{$0$-sv}
%     \mylabel{ax:peanoT:zero:tot}{$0$-tot}
%     \mylabel{ax:peanoT:succ:sv}{$s$-sv}
%     \mylabel{ax:peanoT:succ:tot}{$s$-tot}
%     \mylabel{ax:peanoT:ind}{ind}
%     \mylabel{ax:peanoT:iso:1}{iso-1}
%     \mylabel{ax:peanoT:iso:2}{iso-2}
%     \[
%         \begin{array}{c|c}
%             \begin{array}{cc}
%                 \begin{array}[c]{c@{}c@{}c}
%                     \tikzfig{peano/ax1/zeroSV/lhs} &\stackrel{\eqref{ax:peanoT:zero:sv}}{\leq}& \tikzfig{peano/ax1/zeroSV/rhs} 
%                     \\[15pt]
%                     \tikzfig{peano/ax1/zeroTOT/lhs} &\stackrel{\eqref{ax:peanoT:zero:tot}}{\leq}& \tikzfig{peano/ax1/zeroTOT/rhs}
%                 \end{array}
%                 &
%                 \begin{array}[c]{c@{}c@{}c}
%                     \tikzfig{peano/ax1/succSV/lhs} &\stackrel{\eqref{ax:peanoT:succ:sv}}{\leq}& \tikzfig{peano/ax1/succSV/rhs} 
%                     \\[15pt]
%                     \tikzfig{peano/ax1/succTOT/lhs} &\stackrel{\eqref{ax:peanoT:succ:tot}}{\leq}& \tikzfig{peano/ax1/succTOT/rhs}
%                 \end{array}        
%             \end{array}
%             &
%             \begin{array}[c]{c@{}c@{}c}
%                 \tikzfig{peano/ax1/iso1/lhs} &\stackrel{\eqref{ax:peanoT:iso:1}}{=}& \tikzfig{peano/ax1/iso1/rhs}
%                 \\[20pt]
%                 \tikzfig{peano/ax1/iso2/lhs} &\stackrel{\eqref{ax:peanoT:iso:2}}{=}& \tikzfig{peano/ax1/iso2/rhs}
%             \end{array}
%             \\[40pt]
%             \hline
%             \multicolumn{2}{c}{
%                 \begin{array}{c}
%                     \\
%                     \tikzfig{peano/ax1/ind/lhs} \stackrel{\eqref{ax:peanoT:ind}}{=} \tikzfig{peano/ax1/ind/rhs}
%                 \end{array}
%             }
%         \end{array}
%     \]
%     \caption{Tape theory of the natural numbers.}
%     \label{fig:tape-theory-natural-numbers}
% \end{figure}





First we show that $(\sign, \mathbb{P})$ is equivalent to Peano's axiomatisation of natural numbers. Possibly, the most interesting axiom is the principle of induction that, as illustrated below, follows easily from uniformity and \eqref{ax:peanoT:ind}.

\begin{theorem}[Principle of Induction]\label{thm:induction}
    For all morphisms $P \colon \uno \to A$ in $\KTCBP$,
    \[ 
        \text{if } \quad
        \tikzfig{peano/ax2/ind/base/lhs} \leq \;\tikzfig{peano/ax2/ind/base/rhs} 
        \quad \text{ and } \quad 
        \tikzfig{peano/ax2/ind/hp/lhs} \leq \;\tikzfig{peano/ax2/ind/hp/rhs},
        \quad \text{ then } \quad
        \tikzfig{peano/ax2/ind/concl/lhs} = \tikzfig{peano/ax2/ind/concl/rhs} 
    \]
\end{theorem}
\begin{proof} %\marginpar{Aggiustare qua}
    Observe that the following holds:
    \[
        \tikzfig{peano/induction/step1} \stackrel{\text{(Hypothesis)}}{\leq} \; \tikzfig{peano/induction/step2} \stackrel{\eqref{ax:diagnat}, \eqref{ax:codiagnat}}{=} \; \tikzfig{peano/induction/step3}.
    \]
    Thus, by~\eqref{ax:trace:tape:AU2} the inclusion below holds and the derivation concludes the proof.
    \[
        \tikzfig{peano/ax1/ind/rhs} \stackrel{\eqref{ax:peanoT:ind}}{=} \tikzfig{peano/induction/step4} \leq \tikzfig{peano/induction/step5} \stackrel{\eqref{ax:trace:tape:kstar-id}}{=} \tikzfig{peano/ax2/ind/base/rhs}.
    \]
\end{proof}

The common form of Peano's axioms state that $0$ is a natural number, $s$ is an injective function and that $0$ is not the successor of any natural number. These are illustrated by means of tape diagrams in Figure \ref{fig:peano-theory-natural-numbers}, where we use the characterisation of total, single valued and injective relations provided by \Cref{lemma:cb:adjoints} in Section \ref{sc:cb:background}. Observe that the axiom \eqref{ax:peano:bottom} states that $\{x\in X \mid (x,0)\in s \} \subseteq \emptyset$.
At the bottom of Figure \ref{fig:peano-theory-natural-numbers}, there is the induction principle as expressed by Peano. Note that, since \eqref{ax:peano:ind} is an implication this is not a kc tape theory. Nevertheless, one can see that this set of laws is equivalent to $\mathbb{P}$.



\begin{figure}[H]
    \mylabel{ax:peano:zero:sv}{$0$-sv}
    \mylabel{ax:peano:zero:tot}{$0$-tot}
    \mylabel{ax:peano:succ:sv}{$s$-sv}
    \mylabel{ax:peano:succ:tot}{$s$-tot}
    \mylabel{ax:peano:succ:inj}{$s$-inj}
    \mylabel{ax:peano:bottom}{$\bot$}
    \mylabel{ax:peano:ind}{ind-princ}
    \[
        \begin{array}{cc}
            \begin{array}{cc}
                \begin{array}[c]{c@{}c@{}c}
                    \tikzfig{peano/ax1/zeroSV/lhs} &\stackrel{\eqref{ax:peano:zero:sv}}{\leq}& \tikzfig{peano/ax1/zeroSV/rhs} 
                    \\[15pt]
                    \tikzfig{peano/ax1/zeroTOT/lhs} &\stackrel{\eqref{ax:peano:zero:tot}}{\leq}& \tikzfig{peano/ax1/zeroTOT/rhs}  
                \end{array}
                &
                \begin{array}[c]{c@{}c@{}c}
                    \tikzfig{peano/ax1/succSV/lhs} &\stackrel{\eqref{ax:peano:succ:sv}}{\leq}& \tikzfig{peano/ax1/succSV/rhs} 
                    \\[15pt]
                    \tikzfig{peano/ax1/succTOT/lhs} &\stackrel{\eqref{ax:peano:succ:tot}}{\leq}& \tikzfig{peano/ax1/succTOT/rhs}
                \end{array}        
            \end{array}
            &
            \begin{array}[c]{c@{}c@{}c}
                \tikzfig{peano/ax2/succINJ/lhs} &\stackrel{\eqref{ax:peano:succ:inj}}{\leq}& \tikzfig{peano/ax2/succINJ/rhs}
                \\[15pt]
                \tikzfig{peano/ax2/bottom/lhs} &\stackrel{\eqref{ax:peano:bottom}}{\leq}& \tikzfig{peano/ax2/bottom/rhs}
            \end{array}
            \\[30pt]
            \hline
            \multicolumn{2}{c}{
                \begin{array}{c}
                    \\
                    \tikzfig{peano/ax2/ind/base/lhs} \leq \tikzfig{peano/ax2/ind/base/rhs}, \;\; \tikzfig{peano/ax2/ind/hp/lhs} \leq \tikzfig{peano/ax2/ind/hp/rhs} 
                    \stackrel{\eqref{ax:peano:ind}}{\implies }
                    \tikzfig{peano/ax2/ind/concl/lhs} = \tikzfig{peano/ax2/ind/concl/rhs}
                \end{array}
            }
        \end{array}
    \]
    \caption{Peano's theory of the natural numbers.}
    \label{fig:peano-theory-natural-numbers}
\end{figure}


% \ale{mettere le label precise degli assiomi che si usano}
\begin{lemma}\label{lemma:Peano}
    The laws in Figures~\ref{fig:tape-theory-natural-numbers} and \ref{fig:peano-theory-natural-numbers} are equivalent. 
    % In particular, the following equivalences hold:
    % \begin{enumerate}
    %     \item $\eqref{ax:peanoT:iso:1} \iff \eqref{ax:peano:succ:sv}, \eqref{ax:peano:zero:sv}$
    %     \item $\eqref{ax:peanoT:iso:2} \iff \eqref{ax:peano:succ:tot}, \eqref{ax:peano:zero:tot}, \eqref{ax:peano:succ:inj}, \eqref{ax:peano:bottom}$
    %     \item $\eqref{ax:peanoT:ind} \iff \eqref{ax:peano:ind}$
    % \end{enumerate}
\end{lemma}
\begin{proof}
    First, we prove that the axioms in Figure~\ref{fig:tape-theory-natural-numbers} entail those in Figure~\ref{fig:peano-theory-natural-numbers}.
    \begin{itemize}
        \item \eqref{ax:peano:succ:sv},\eqref{ax:peano:zero:sv} follow from \eqref{ax:peanoT:iso:1}, i.e.
        \[
            \tikzfig{peano/ax1/succSV/lhs} \stackrel{\eqref{ax:diagun}, \eqref{ax:codiagun}}{=} \tikzfig{peano/equivalence/sv/succ/step1} \leq \tikzfig{peano/ax1/iso1/lhs} \stackrel{\eqref{ax:peanoT:iso:1}}{=} \tikzfig{peano/ax1/iso1/rhs}
        \]
        and
        \[
            \tikzfig{peano/ax1/zeroSV/lhs} \stackrel{\eqref{ax:diagun}, \eqref{ax:codiagun}}{=} \tikzfig{peano/equivalence/sv/zero/step1} \leq \tikzfig{peano/ax1/iso1/lhs} \stackrel{\eqref{ax:peanoT:iso:1}}{=} \tikzfig{peano/ax1/iso1/rhs}.
        \]
        % \[
        % \tikzfig{peano/ax1/iso1/lhs} = \tikzfig{peano/ax1/iso1/rhs} \stackrel{\text{Lemma~\ref{lemma:order-adjointness}}}{\implies} \left\{ \begin{array}[c]{c@{\;}c@{\;}c}
        %     \tikzfig{peano/ax1/succSV/lhs} &\leq& \tikzfig{peano/ax1/succSV/rhs} \\[7pt]
        %     \tikzfig{peano/ax1/zeroSV/lhs} &\leq& \tikzfig{peano/ax1/zeroSV/rhs}
        % \end{array} \right.
        % \]
        \item \eqref{ax:peano:succ:tot}, \eqref{ax:peano:succ:inj}, \eqref{ax:peano:zero:tot}, \eqref{ax:peano:bottom} follow from the matrix normal form of~\eqref{ax:peanoT:iso:2} and Proposition~\ref{prop:matrixform}, i.e.
        \begin{equation}\label{eq:peano:iso2-equivalence}
            \tikzfig{peano/ax1/iso2/lhs} = \tikzfig{peano/ax1/iso2/rhs} \stackrel{\text{(Proposition~\ref{prop:matrixform})}}{\iff} \left\{ \begin{array}[c]{c@{\;}c@{\;}c}
                \tikzfig{peano/ax2/succINJ/lhs} &=& \tikzfig{peano/ax2/succINJ/rhs} \\[7pt]
                \tikzfig{peano/ax2/bottom/lhs} \;\; &=& \tikzfig{peano/ax2/bottom/rhs} \\[7pt]
                \;\tikzfig{peano/ax2/bottomOp/lhs} &=& \;\;\tikzfig{peano/ax2/bottomOp/rhs} \\[7pt]
                \tikzfig{peano/ax1/zeroTOT/rhs} &=& \tikzfig{peano/ax1/zeroTOT/lhs}
            \end{array} \right.  
        \end{equation}
        Observe that the last equality on the right imposes injectivity of $0$ as well, however this is always the case for morphisms $1 \to A$ that are total.
        \item \eqref{ax:peano:ind} holds by Theorem~\ref{thm:induction}.
    \end{itemize}
    Similarly, we prove that the axioms in Figure~\ref{fig:peano-theory-natural-numbers} entail those in Figure~\ref{fig:tape-theory-natural-numbers}. It is convenient to prove them in the following order.
    \begin{itemize}
        \item For \eqref{ax:peanoT:ind}, let $P \colon 1 \to A$ be the following morphism
        \[\tikzfig{peano/ax2/ind/base/rhs} \defeq  \tikzfig{peano/ax1/ind/lhs}\]
        and observe that the first condition of~\eqref{ax:peano:ind} holds:
        \[
            \tikzfig{peano/ax1/ind/lhs} \stackrel{\eqref{ax:relBangCobang}}{\geq} \tikzfig{peano/equivalence/ind/step1} \stackrel{\eqref{ax:trace:tape:sliding}}{=} \tikzfig{peano/equivalence/ind/step2} \stackrel{\eqref{ax:cobangnat}, \eqref{ax:codiagun}, \eqref{ax:diagun}}{=} \tikzfig{peano/ax2/ind/base/lhs}.
        \]
        For the second condition observe that $P$ is defined as $0 ; \kstar{s}$, and recall that $\kstar{s} ; s \leq \kstar s$ by \Cref{cor:bounds-star}. Thus $P ; s = 0 ; \kstar{s} ; s \leq 0 ; \kstar{s} = P$. We conclude using~\eqref{ax:peano:ind}.
        \item For \eqref{ax:peanoT:iso:1} we prove the two inclusions separately, starting with the one below.
        \[
            \tikzfig{peano/ax1/iso1/lhs} \stackrel{\eqref{ax:peano:succ:sv}, \eqref{ax:peano:zero:sv}}{\leq} \tikzfig{peano/equivalence/iso1/sub/step1} \stackrel{\eqref{ax:relDiagCodiag}}{\leq} \tikzfig{peano/ax1/iso1/rhs} 
        \]
        For the other inclusion, observe that by~\Cref{lemma:cb:adjoints}
        \[ 
            \tikzfig{peano/ax1/iso1/rhs} \leq \tikzfig{peano/ax1/iso1/lhs}  \iff  \tikzfig{peano/equivalence/iso1/surjective/lhs} \leq \tikzfig{peano/equivalence/iso1/surjective/rhs}.
        \]
        Thus, we prove the following:
        \begin{align*}
            \tikzfig{peano/equivalence/iso1/surjective/rhs} &\stackrel{\eqref{ax:peanoT:ind}}{=} \tikzfig{peano/equivalence/iso1/sup/step1} \stackrel{\eqref{ax:diagnat}}{=} \tikzfig{peano/equivalence/iso1/sup/step2} \\
                                                            &\leftstackrel{\text{(Proposition~\ref{prop:star-fixpoint})}}{=} \tikzfig{peano/ax1/ind/lhs} \stackrel{\eqref{ax:peanoT:ind}}{=} \tikzfig{peano/equivalence/iso1/surjective/lhs}
        \end{align*}
        \item \eqref{ax:peanoT:iso:2} follow from \eqref{ax:peano:succ:tot}, \eqref{ax:peano:succ:inj}, \eqref{ax:peano:zero:tot}, \eqref{ax:peano:bottom} as shown in \eqref{eq:peano:iso2-equivalence}.
    \end{itemize}
    % For the $\impliedby$ part, we prove the two inclusions separately:
    % \[
    %     \tikzfig{peano/ax1/iso1/lhs} \stackrel{\eqref{ax:peano:succ:sv}, \eqref{ax:peano:zero:sv}}{\leq} \tikzfig{peano/equivalence/iso1/sub/step1}  = \tikzfig{peano/ax1/iso1/rhs} 
    % \]
    % \ale{Questa è sbagliata.}
    % \[
    %     \tikzfig{peano/ax1/iso1/rhs} \leq  \tikzfig{peano/ax1/zeroSV/lhs} = \tikzfig{peano/equivalence/iso1/sup/step1} = \tikzfig{peano/equivalence/iso1/sup/step2} \leq  \tikzfig{peano/ax1/iso1/lhs}
    % \]
    
    % \[
    %     \tikzfig{peano/ax1/iso2/lhs} = \tikzfig{peano/ax1/iso2/rhs} \iff \left\{ \begin{array}[c]{c@{\;}c@{\;}c c c}
    %         \tikzfig{peano/ax2/succINJ/lhs} &=& \tikzfig{peano/ax2/succINJ/rhs} & \iff & \eqref{ax:peano:succ:tot}, \eqref{ax:peano:succ:inj} \\[7pt]
    %         \tikzfig{peano/ax2/bottom/lhs} \;\; &=& \tikzfig{peano/ax2/bottom/rhs} & \iff & \eqref{ax:peano:bottom} \\[7pt]
    %         \;\tikzfig{peano/ax2/bottomOp/lhs} &=& \;\;\tikzfig{peano/ax2/bottomOp/rhs} & \iff & \eqref{ax:peano:bottom} \\[7pt]
    %         \tikzfig{peano/ax1/zeroTOT/rhs} &=& \tikzfig{peano/ax1/zeroTOT/lhs} & \iff & \eqref{ax:peano:zero:tot}
    %     \end{array} \right.
    % \]
    % Observe that the last equality on the right imposes injectivity of $0$ as well, however this is always the case for morphisms $1 \to A$ that are total.

    % \bigskip

    % \textsc{Proof of 3.} The $\implies$ part holds by Theorem~\ref{thm:induction}. For the $\impliedby$ part, 
\end{proof}

In \cite{dedekind1888nature}, Dedekind showed that any two models of Peano's axioms are isomorphic, and thus any model of $(\sign, \mathbb{P})$ is isomorphic to the one on natural numbers.



\subsection{First Steps in Arithmetic}
To give to the reader a taste of how one can program with tapes, we now illustrate how to start to encode arithmetic within  $(\sign, \mathbb{P})$.
The tape for addition is illustrated below.
\begin{equation}\label{eq:add}
    \tikzfig{addition/addCirc} \defeq \tikzfig{addition/additionDef}
\end{equation}
As it will be clearer later, this tape can be thought as a simple imperative program:
\begin{center}
\texttt{add(x,y) = while (x>0) \{ x:=x-1; y:=y+1 \}; return y}
\end{center}
The variable \texttt{x} corresponds to the top wire in \eqref{eq:add}, while \texttt{y} to the bottom one. At any iteration, the program checks whether 
 \texttt{x} is $0$, in which case it returns \texttt{x}, or the successor of some number, in which case \texttt{x} takes such number, while \texttt{y} takes its own successor.

One can easily prove that $\tikzfig{addition/addCirc}$ satisfies the usual inductive definition of addition in Peano's arithmetics.
\begin{lemma}
    The following hold in $\KTCBP$:
    \begin{enumerate}
        \item $\tikzfig{addition/addZero} = \tikzfig{addition/addZeroRhs} \qquad \textnormal{(\texttt{ add(0,y) = y })}$ 
        \item $\tikzfig{addition/addSuccLhs} = \tikzfig{addition/addSuccRhs} \qquad \textnormal{(\texttt{ add(succ(x),y) = succ(add(x,y)) })}$
    \end{enumerate}
\end{lemma}
\begin{proof}
    First, recall that by Proposition~\ref{prop:star-fixpoint},
    \begin{equation}\label{eq:add-fixpoint}
        \tikzfig{addition/additionDef} = \tikzfig{addition/addStar}. 
    \end{equation}
    Then, observe that for $1.$ the following holds:
    % \textsc{Proof of 1.}  The following holds:
    \begin{align*}
        \tikzfig{addition/addZero} &\leftstackrel{\eqref{eq:add-fixpoint}}{=} \tikzfig{addition/partialEval/zero/step1} \stackrel{\eqref{ax:diagnat}, \eqref{ax:codiagnat}}{=} \tikzfig{addition/partialEval/zero/step2} \\
                                   &\leftstackrel{\eqref{ax:peano:bottom}}{=} \tikzfig{addition/partialEval/zero/step3} \stackrel{\eqref{ax:cobangnat}}{=} \tikzfig{addition/partialEval/zero/step4} \stackrel{\eqref{ax:diagun}, \eqref{ax:codiagun}}{=} \tikzfig{addition/partialEval/zero/step5} \\
                                   &\leftstackrel{\eqref{ax:peano:zero:tot}}{=} \tikzfig{addition/partialEval/zero/step6}. \\
    \end{align*}
    And for $2.$ the following holds:
    \begingroup
    \allowdisplaybreaks
    \begin{align*}
        \tikzfig{addition/addSuccLhs} &\leftstackrel{\eqref{eq:add-fixpoint}}{=} \tikzfig{addition/partialEval/succ/step1} \stackrel{\eqref{ax:diagnat}, \eqref{ax:codiagnat}}{=} \tikzfig{addition/partialEval/succ/step2} \\
                                      &\leftstackrel{\eqref{ax:peano:succ:inj}, \eqref{ax:peano:succ:tot}}{=} \tikzfig{addition/partialEval/succ/step3} \stackrel{\eqref{ax:peano:bottom}}{=} \tikzfig{addition/partialEval/succ/step4} \\
                                      &\leftstackrel{\eqref{ax:diagun}, \eqref{ax:codiagun}}{=} \tikzfig{addition/partialEval/succ/step5} \stackrel{\eqref{ax:trace:tape:sliding}}{=} \tikzfig{addition/partialEval/succ/step6}  \stackrel{\eqref{ax:codiagnat}, \eqref{ax:diagnat}}{=} \tikzfig{addition/partialEval/succ/step7} \\
                                      &\leftstackrel{\eqref{eq:add-fixpoint}}{=} \tikzfig{addition/addSuccRhs}.
    \end{align*}
    \endgroup
\end{proof}

While, it is straightforward that $\tikzfig{addition/addCirc}$ terminates with all possible inputs, it is interesting to see how this can be proved within the kc tape theory $\mathbb{P}$.


\begin{lemma}
    The function $\tikzfig{addition/addCirc}$ is total, i.e. the following equality holds:
    \[ \tikzfig{addition/terminates/lhs} = \tikzfig{addition/terminates/rhs} \]
\end{lemma}
\begin{proof}
    First observe that the following holds:
    % \begin{equation}\label{eq:top-add}
    %     \tikzfig{addition/terminates/rhs}  \leq \tikzfig{addition/terminates/derivation/unif_lhs}
    % \end{equation}
    \begin{align*}
        \tikzfig{addition/terminates/derivation/step1} &\leftstackrel{\eqref{ax:dischargeradj2}}{\leq} \tikzfig{addition/terminates/derivation/step2} \stackrel{\eqref{ax:codiagnat}, \eqref{ax:diagnat}}{=} \tikzfig{addition/terminates/derivation/step3} \stackrel{\eqref{ax:dischargeradj1}}{\leq} \tikzfig{addition/terminates/derivation/step4} \\
                                                       &\leftstackrel{\eqref{ax:peano:succ:sv}, \eqref{ax:peano:succ:tot}}{=} \tikzfig{addition/terminates/derivation/step5}.
    \end{align*}
    Then, by~\eqref{ax:trace:tape:AU1}, the inequality below holds and the derivation concludes the proof.
    \[
        \tikzfig{addition/terminates/rhs}  \stackrel{\eqref{ax:peanoT:ind}}{=} \tikzfig{addition/terminates/derivation/unif_lhs} \leq \tikzfig{addition/terminates/derivation/unif_rhs}
    \]
\end{proof}


==> oldsections/sections/poset.tex <==


\section{Kleene Tapes}\label{sec:kleene-tapes}
In this section, we combine the structure of Kleene bicategories from Section \ref{sec:kleene} with the one of rig categories from Section \ref{sec:rigcategories}.
We illustrate the corresponding tape diagrams, named Kleene tapes, and the corresponding notion of theories. We begin by introducing the structures of interest.

\begin{definition}\label{def:kcrig}
A poset enriched rig category $\Cat{C}$ is said to be a \emph{Kleene rig category}  if
$(\Cat{C}, \piu, \zero)$ is a Kleene bicategory. A \emph{morphism of Kleene rig categories} is a poset enriched rig functor that is also a Kleene morphism.
\end{definition}

In any Kleene rig category $\per$ distributes over the convolution monoid, or more precisely the join-semi lattice, in \eqref{eq:covolution}.

\begin{lemma}\label{lemma:ditributivityper}
For all $f_1,f_2\colon X \to Y$ and $g\colon S \to T$  in a Kleene rig category, it holds that
\[(f_1+f_2)\per g =(f_1\per g +f_2\per g) \qquad g \per (f_1+f_2) = (f_1\per g + f_2 \per g) \qquad 0 \per g = 0 = g \per 0\text{.}\] 
\end{lemma}
%



The following two results illustrate the interaction of the product $\per$  with the Kleene star and  trace.

\begin{proposition}\label{prop:star-per}
	For all $a \colon X \to X$ and $b \colon Y \to Y$ in a Kleene rig category, it holds that \[\kstar{(a \per b)} \leq \kstar{a} \per \kstar{b}\text{.}\]
	% Let $\Cat{C}$ be a Kleene rig category. The following hold for all $a \colon X \to X$ and $b \colon Y \to Y$ in $\Cat{C}$
	% \[ \kstar{(a \per b)} \leq \kstar{a} \per \kstar{b} \] 
\end{proposition}
\begin{proof}
	First observe that the following inequality holds:
	\begin{align*}
		(a \per b) ; (\kstar{a} \per \kstar{b})
		&= (a ; \kstar{a}) \per (b ; \kstar{b}) \tag{\Cref{fig:freestricmmoncatax}} \\ 
		&\leq (\kstar{a} \per \kstar{b}) \tag{\ref{eq:Kllenelaw}} \\
	\end{align*}

	Thus, by~\eqref{eq:Kllenelaw}, it follows that
	
	\begin{equation}\label{eq:A}
		\kstar{(a \per b)} ; (\kstar{a} \per \kstar{b}) \leq \kstar{a} \per \kstar{b}.
	\end{equation}

	To conclude, observe that the following holds:
	\begin{align*}
		\kstar{(a \per b)} 
		&= \kstar{(a \per b)} ; \id{X \per Y} \tag{\Cref{fig:freestricmmoncatax}} \\ 
		&= \kstar{(a \per b)} ; (\id{X} \per \id{Y}) \tag{\Cref{fig:freestricmmoncatax}} \\ 
		&\leq \kstar{(a \per b)} ; (\kstar{a} \per \kstar{b}) \tag{\ref{eq:Kllenelaw}} \\
		&\leq \kstar{a} \per \kstar{b} \tag{\ref{eq:A}}
	\end{align*}
	
\end{proof}

\begin{proposition}\label{prop:trace-per}
	For all $f \colon S \piu X \to S \piu Y$ and $f' \colon S' \piu X' \to S' \piu Y'$ in a Kleene rig category, it holds that 
	\[ 
		\trace_{S \per S'} \begin{psmallmatrix}
			f_{SS} \per f'_{S' S'} & f_{SY} \per f'_{S'Y'} \\
			f_{XS} \per f'_{X' S'} & f_{XY} \per f'_{X'Y'}
		\end{psmallmatrix}
		\; \leq \;
		\trace_{S} f \; \per \; \trace_{S'} f'
	 \]
	 where $\begin{psmallmatrix} f_{SS} & f_{SY} \\ f_{XS} & f_{XY} \end{psmallmatrix}$ and $\begin{psmallmatrix} f'_{S'S'} & f'_{S'Y'} \\ f'_{X'S'} & f'_{X'Y'} \end{psmallmatrix}$ are, respectively, the matrix normal forms of $f$ and $f'$.
\end{proposition}
\begin{proof}
	\begin{align*}
		\trace_{S} f \; \per \; \trace_{S'} f'
		&= (f_{XS} ; \kstar{f_{SS}} ; f_{SY} + f_{XY}) \per (f'_{X'S'} ; \kstar{(f'_{S'S'})} ; f'_{S'Y'} + f'_{X'Y'}) \tag{\Cref{fig:star-trace}} \\
		&= \begin{array}[t]{cl}
			\multicolumn{2}{c}{ ((f_{XS} ; \kstar{f_{SS}} ; f_{SY}) \per (f'_{X'S'} ; \kstar{(f'_{S'S'})} ; f'_{S'Y'})) } \\ 
			+ & ((f_{XS} ; \kstar{f_{SS}} ; f_{SY} + f_{XY}) \per f'_{X'Y'}) \\
			+ & (f_{XY} \per (f'_{X'S'} ; \kstar{(f'_{S'S'})} ; f'_{S'Y'})) \\
			+ & (f_{XY} \per f'_{X'Y'})
		\end{array} \tag{Lemma \ref{lemma:ditributivityper}}  \\
		&\geq { ((f_{XS} ; \kstar{f_{SS}} ; f_{SY}) \per (f'_{X'S'} ; \kstar{(f'_{S'S'})} ; f'_{S'Y'})) \; + \; (f_{XY} \per f'_{X'Y'}) }  \tag{\Cref{lemma:order-adjointness}} \\
		&= (f_{XS} \per f'_{X'S'}) ; (\kstar{f_{SS}} \per \kstar{(f'_{S'S'})}) ; (f_{SY} \per f'_{X'Y'}) + (f_{XY} \per f'_{X'Y'}) \tag{\Cref{fig:freestricmmoncatax}} \\
		&\geq (f_{XS} \per f'_{X'S'}) ; \kstar{(f_{SS} \per f'_{S'S'})} ; (f_{SY} \per f'_{X'Y'}) + (f_{XY} \per f'_{X'Y'}) \tag{\Cref{prop:star-per}} \\
		&= \trace_{S \per S'} \begin{psmallmatrix}
			f_{SS} \per f'_{S' S'} & f_{SY} \per f'_{S'Y'} \\
			f_{XS} \per f'_{X' S'} & f_{XY} \per f'_{X'Y'}
		\end{psmallmatrix} \tag{\Cref{fig:star-trace}}
	\end{align*}
\end{proof}






\subsection{From Traced Tapes to Kleene Tapes}

\begin{figure}
    \begin{subfigure}{0.6\linewidth}
        \mylabel{ax:relCobangBang}{$\cobang{}\bang{}$}
        \mylabel{ax:relBangCobang}{$\bang{}\cobang{}$}
        \mylabel{ax:relCodiagDiag}{$\codiag{}\diag{}$}
        \mylabel{ax:relDiagCodiag}{$\diag{}\codiag{}$}
        \scalebox{0.9}{
            \begin{tabular}{c@{}c@{}c @{\;} c@{}c@{}c}
                \tikzfig{empty} & $\axsubeq{\cobang{}\bang{}}$ & \tikzfig{tapes/whiskered_ax/bialg2_left} & \Tcounit{U}\Tunit{U} & $\axsubeq{\bang{}\cobang{}}$ & \Twire{U} \\[2ex]
                $\begin{aligned}\begin{gathered}\Twire{U} \\ \Twire{U} \end{gathered}\end{aligned}$ & $\axsubeq{\codiag{}\diag{}}$ & \tikzfig{tapes/whiskered_ax/bialg1_left} & \TRelCodiagDiag{U} & $\axsubeq{\diag{}\codiag{}}$ & \Twire{U}
            \end{tabular}
        }
        \caption{Axioms for  $\cobang{}  \dashv \bang{}$ and $\codiag{} \dashv \diag{}$.}
        \label{fig:rel axioms}
    \end{subfigure}
    \begin{subfigure}{0.38\linewidth}
        \mylabel{ax:trace:tape:kstar-id}{AT1}
        \[
            \scalebox{0.9}{\tikzfig{traceTapeAx/rep/lhs}} \stackrel{\text{(AT1)}}{=} \scalebox{0.9}{\tikzfig{traceTapeAx/rep/rhs}}
        \]
        \caption{Repeating the identity.}
        \label{fig:id* tape axiom}
    \end{subfigure}
    \\[15pt]
    \begin{subfigure}{\linewidth}
        \mylabel{ax:trace:tape:AU1}{AU1}
        \mylabel{ax:trace:tape:AU2}{AU2}
        \[ \tikzfig{traceTapeAx/posetUnif/1/lhs} \leq \tikzfig{traceTapeAx/posetUnif/1/rhs} \stackrel{(\text{AU1})}{\implies} \tikzfig{traceTapeAx/posetUnif/1/TR_lhs} \leq \tikzfig{traceTapeAx/posetUnif/1/TR_rhs} \]
        \[ \tikzfig{traceTapeAx/posetUnif/2/lhs} \leq \tikzfig{traceTapeAx/posetUnif/2/rhs} \stackrel{(\text{AU2})}{\implies} \tikzfig{traceTapeAx/posetUnif/2/TR_lhs} \leq \tikzfig{traceTapeAx/posetUnif/2/TR_rhs} \]
        \caption{Posetal uniformity axioms in tape diagrams.}
        \label{fif:poset unif tape axioms}
    \end{subfigure}
    \caption{Additional axioms for Kleene Tape Diagrams}\label{fig:add}
\end{figure}

We now introduce \emph{Kleene tapes}, in a nutshell tape diagrams for Kleene rig categories.

Kleene tapes are constructed as traced tape diagrams quotiented by the additional axioms of Kleene bicategories illustrated in the form of tapes in Figure \ref{fig:add}. Since these axioms include the posetal uniformity laws ((AU1) and (AU2) in Definition \ref{def:kleenebicategory}) that are not equational, such quotient needs to be performed with some care.

Let $\basicR$ be a a set of pairs $(\t_1, \t_2)$ of arrows of $\CatTrTape$ with the same domain and codomain. We define $\precongB$ to be the set generated by the following inference system (where $\t \precongB \s$ is a shorthand for $(\t,\s)\in \precongB$).
\begin{equation}\label{eq:uniformprecong}
        \!\!\begin{array}{@{\qquad}c@{\qquad\qquad}c@{\qquad}c@{\qquad}}
            \inferrule*[right=($\basicR$)]{\t_1 \mathbin{\basicR} \t_2}{\t_1 \mathrel{\precongB} \t_2}
            &
            \inferrule*[right=($r$)]{-}{\t \mathrel{\precongB} \t}
            &    
            \inferrule*[right=($t$)]{\t_1 \mathrel{\precongB} \t_2 \quad \t_2 \mathrel{\precongB} \t_3}{\t_1 \mathrel{\precongB} \t_3}
            \\[8pt]
            \inferrule*[right=($;$)]{\t_1 \mathrel{\precongB} \t_2 \quad \s_1 \mathrel{\precongB} \s_2}{\t_1;\s_1 \mathrel{\precongB} \t_2;\s_2}
            &
            \inferrule*[right=($\piu$)]{\t_1 \mathrel{\precongB} \t_2 \quad \s_1 \mathrel{\precongB} \s_2}{\t_1\piu\s_1 \mathrel{\precongB} \t_2 \piu \s_2}
            &
            \inferrule*[right=($\per $)]{\t_1 \mathrel{\precongB} \t_2 \quad \s_1 \mathrel{\precongB} \s_2}{\t_1\per \s_1 \mathrel{\precongB} \t_2 \per \s_2}
            \\[8pt]
            \multicolumn{3}{c}{
            \inferrule*[right=($ut$-1)]{\s_2 \mathrel{\precongB} \s_1 \qquad \t_1 ; (\s_1 \piu \id{}) \mathrel{\precongB} (\s_2 \piu \id{}) ; \t_2}{\trace_{S_1}\t_1 \mathrel{\precongB} \trace_{S_2}\t_2}
            \quad\;\;
            \inferrule*[right=($ut$-2)]{ \s_2 \mathrel{\precongB} \s_1 \qquad (\s_1 \piu \id{}) ; \t_1 \mathrel{\precongB} \t_2 ; (\s_2 \piu \id{})}{\trace_{S_1}\t_1 \mathrel{\precongB} \trace_{S_2}\t_2}
            }
        \end{array}
\end{equation}


We then take $\basicK$ to be the set of pairs of tapes containing those in Figure \ref{fig:rel axioms} and in Figure \ref{fig:id* tape axiom}. More explicitly,

\begin{align*}
 \basicK\defeq & \{(\id{P\piu P}  \, , \, \codiag{P};\diag{P} \mid P \in Ob(\CatTrTape) \} \cup \{( \diag{P}; \codiag{P} \,,\, \id{P} ) \mid P \in Ob(\CatTrTape)\} \cup \\
 & \{(\id{\zero}  \, , \, \cobang{P};\bang{P} \mid P \in Ob(\CatTrTape) \} \cup \{( \bang{P}; \cobang{P} \,,\, \id{P} ) \mid P \in Ob(\CatTrTape)\} \cup \\
 & \{(\trace_{P}(\codiag{P};\diag{P}) \,,\, \id{P})\mid P \in Ob(\CatTrTape)\}\text{.}
\end{align*}
We fix $\sim_\basicK \defeq \leq_{\basicK} \cap \leq_{\basicK}$.

With these definitions we can construct $\CatKTape$, the Kleene rig category of Kleene tapes. Objects are the same of $\CatTrTape$. Arrows are $\sim_\basicK$-equivalence classes of arrows of $\CatTrTape$. Every homset $\CatKTape[P,Q]$ is ordered by $\precongK$. One can easily check that the construction of $\CatKTape$ is well defined and that it gives rise to a sesquistrict Kleene rig category (see Proposition \ref{prop:tapeisKleenerig}). More importantly, $\CatKTape$ is the freely generated one.


\begin{theorem}\label{thm:Kleenetapesfree}
$\CatKTape$ is the free sesquistrict Kleene rig category generated by the monoidal signature $(\sort, \sign)$.
\end{theorem}




% \subsection{Traced Tape Theories}

% The usual way of reasoning through string diagrams is based on monoidal theories, namely a signature plus a set of axioms: either equations or inequations. Similarly a \emph{traced tape theory} is a pair $(\sign, \basicR)$ where $\sign$ is a monoidal signature (or by Theorem~\ref{thm:equivalentsignature} even a rig signature) and $\basicR$ is a set of pairs $( \st{\t_1}{S_1}, \st{\t_2}{S_2} )$ of arrows in $\UTr(\CatTape)$ with same domain and codomain. Hereafter, we think of each pair $( \st{\t_1}{S_1}, \st{\t_2}{S_2} )$ as an inequation $\st{\t_1}{S_1} \leq \st{\t_2}{S_2}$, but the results that we develop in this section trivially hold  also for equations: it is enough to add in $\basicR$ a pair $(\st{\t_2}{S_2}, \st{t_1}{S_1})$ for each $(\st{t_1}{S_1}, \st{t_2}{S_2}) \in \basicR$.

% In the following, we write $\st{\t_1}{S_1} \mathbin{\basicR} \st{\t_2}{S_2}$ for $( \st{\t_1}{S_1}, \st{\t_2}{S_2})\in \basicR$ and $\precongB$ for the smallest precongruence (w.r.t. $\piu$, $\per$ and $;$) generated by $\basicR$, i.e.\ the relation inductively generated as 
% \ale{La regola (tr) serve davvero o si deriva dall free trace construction?}
% \[
%     \begin{array}{c@{\qquad}c}
%         \inferrule*[right=($\basicR$)]{\st{\t_1}{S_1} \mathbin{\basicR} \st{\t_2}{S_2}}{\st{\t_1}{S_1} \mathrel{\precongB} \st{\t_2}{S_2}}
%         &
%         \inferrule*[right=($r$)]{-}{\st{\t}{S} \mathrel{\precongB} \st{\t}{S}}
%         \\[8pt]
%         \multicolumn{2}{c}{
%             \inferrule*[right=($tr$)]{\st{\t_1}{S_1} \mathrel{\precongB} \st{\t_2}{S_2} \quad \st{\t_1}{S_1}, \st{\t_2}{S_2} \colon S \piu P \to S \piu Q}{\st{\t_1}{S_1 \piu S} \mathrel{\precongB} \st{\t_2}{S_2 \piu S}}
%         }
%         \\[8pt]
%         \inferrule*[right=($t$)]{\st{\t_1}{S_1} \mathrel{\precongB} \st{\t_2}{S_2} \quad \st{\t_2}{S_2} \mathrel{\precongB} \st{\t_3}{S_3}}{\st{\t_1}{S_1} \mathrel{\precongB} \st{\t_3}{S_3}} 
%         &
%         \inferrule*[right=($;$)]{\st{\t_1}{S_1} \mathrel{\precongB} \st{\t_2}{S_2} \quad \st{\t_1'}{S_1'} \mathrel{\precongB} \st{\t_2'}{S_2'}}{\st{\t_1}{S_1};\st{\t_1'}{S_1'} \mathrel{\precongB} \st{\t_2}{S_2};\st{\t_2'}{S_2'}}
%         \\[8pt]
%         \inferrule*[right=($\piu$)]{\st{\t_1}{S_1} \mathrel{\precongB} \st{\t_2}{S_2} \quad \st{\t_1'}{S_1'} \mathrel{\precongB} \st{\t_2'}{S_2'}}{\st{\t_1}{S_1}\piu\st{\t_1'}{S_1'} \mathrel{\precongB} \st{\t_2}{S_2} \piu \st{\t_2'}{S_2'}} 
%         &
%         \inferrule*[right=($\per $)]{\st{\t_1}{S_1} \mathrel{\precongB} \st{\t_2}{S_2} \quad \st{\t_1'}{S_1'} \mathrel{\precongB} \st{\t_2'}{S_2'}}{\st{\t_1}{S_1}\per \st{\t_1'}{S_1'} \mathrel{\precongB} \st{\t_2}{S_2} \per \st{\t_2'}{S_2'}}
%     \end{array}
% \]

% By enriching $\UTr(\CatTape)$ with $\precongB$, we obtain a \emph{preorder enriched rig category} (namely, $\piu$, $\per$ and $;$ are monotone) that we denote hereafter by $\UTr(\PreCatTapeI{\basicR})$.
% For an arbitrary category $\Cat{C}$ enriched over a preorder $\leq$, one can define a corresponding poset enriched category $\posetification{\Cat{C}}$ by quotienting the homsets of $\Cat{C}$ by the equivalence relation $\sim$ defined as $\sim  \defeq  \leq \cap \geq$. Moreover, if $\Cat{C}$ is a preorder enriched rig category, then $\posetification{\Cat{C}}$ is a \emph{poset enriched rig category}. Particularly relevant for this paper will be $\posetification{\UTr(\PreCatTapeI{\basicR})}$. %Similarly, for a monoidal theory $(\sign, \basicR)$, one can construct preorder and poset enriched monoidal categories, hereafter denoted by $\Cat{C}_{\sign,\basicR}$ and $\posetification{\Cat{C}_{\sign,\basicR}}$, respectively.

% \begin{example}
%     QUA UN BEL ESEMPIO DI TRACED TAPE THEORY
% \end{example}

% Observe that the proof above is not entirely graphical because of the decomposition via $\per$. This inconvenience can be avoided by taking 




==> oldsections/sections/rig.tex <==


\section{Rig Categories}\label{sec:rigcategories}

%Rig categories~\cite{laplaza_coherence_1972}, also known as \emph{bimonoidal categories}, involve two (symmetric) monoidal structures where one distributes over the other. An extensive treatment was recently given in~\cite{johnson2021bimonoidal}, from which we borrow most of the notation in this paper.

We have seen that $\Cat{Set}_{\subdistr}$ carries two monoidal categories $(\Cat{Set}_{\subdistr},\per,\uno)$ and $(\Cat{Set}_{\subdistr},\piu, \zero)$. The appropriate categorical setting to study their interactions is provided by rig categories~\cite{laplaza_coherence_1972}. %, also known as \emph{bimonoidal categories}. 
An extensive treatment was recently given in~\cite{johnson2021bimonoidal}, from which we borrow most of the notation in this paper.


\begin{definition}\label{def:rig}
    A \emph{rig category} is a category $\Cat{C}$ with 
    two symmetric monoidal structures $(\Cat{C}, \per, \uno)$ and 
    $(\Cat{C}, \piu, \zero)$ and natural isomorphisms 
    \[ \dl{X}{Y}{Z} \colon X \per (Y \piu Z) \to (X \per Y) \piu (X \per Z) \qquad  \annl{X} \colon \zero \per X \to \zero \]
    \[ \dr{X}{Y}{Z} \colon (X \piu Y) \per Z \to (X \per Z) \piu (Y \per Z) \qquad \annr{X} \colon X \per \zero \to \zero \]
satisfying the coherence axioms in Figure~\ref{fig:rigax}.  A rig functor is a functor that is strong symmetric monoidal for both $(\Cat{C}, \per, \uno, \symmt)$ and $(\Cat{C}, \piu, \zero, \symmp)$ and that preserves the four above natural isomorphisms.
%  A rig category is said to be \emph{right} (respectively \emph{left}) \emph{strict} when both its monoidal structures are 
%    strict and $\lambda^\bullet, \rho^\bullet$ and $\delta^r$ (respectively $\delta^l$) are all identity 
%    natural isomorphisms. A \emph{right strict rig functor} is a strict symmetric monoidal functor for both $\per$ and $\piu$ preserving $\delta^l$. We write $\RIG$ for the category of right strict rig categories and functors.\marginpar{be carefull about strictness here}
\end{definition}

%On many occasions, one is interested in rig categories where $\piu$ has some additional structure like, for instance, in the Kleisli category of a commutative monad where $\piu$ is a coproduct. % For instance, distributive monoidal categories are rig categories where $\piu$ is a coproduct. In \cite{bonchi2023deconstructing}, the focus is on rig categories where $\piu$  is a biproduct, like the category of sets and relations $\Rel$ (see Section \ref{sec:2monREL}).

%In this work, we focus on \emph{distributive monoidal categories}, namely those rig categories where $\piu$ is a coproduct. We choose a different name for uniformity with the  structures in Sec. \ref{sec:fccdrig} and \ref{sec:Trig}.

In this work, we focus on those rig categories where $\piu$ is a coproduct. %We choose a different name for uniformity with the  structures in Sec. \ref{sec:fccdrig} and \ref{sec:Trig}.

\begin{definition}\label{def:fcrig}
A \emph{finite coproduct (fc) rig category} is a rig category $(\Cat{C}, \piu, \zero, \per, \uno)$  such that $(\Cat{C}, \piu, \zero)$ is a finite coproducts category. A \emph{morphism of fc rig categories} is both a rig functor and a morphism of fc categories. %We write $\FCRIG$ for the category of fc rig categories and their morphisms.
\end{definition}
By definition, in a finite coproduct rig category, every object $X$ has a natural monoid $\codiag{X}\colon X \piu X \to X $ and $\cobang{X}\colon \zero \to X$. The following result from \cite{bonchi2023deconstructing} illustrates the interactions of $\codiag{}$ and $\cobang{}$ with $\per$.
 \begin{lemma}\label{prop:fcrig}
	In any finite coproduct rig category the following equalities hold. 
	%\[
%	\begin{tikzcd}[column sep=4em]
%		X \per (Y \piu Y) \ar[dr,"\id X \per \codiag Y"] \\
%		(X \per Y) \piu (X \per Y) \ar[u,"{\Idl X Y Y}"] \ar[r,"\codiag{X \per Y}"] \ar[d,"{\Idr X Y Y}"'] & X \per Y \\
%		(X \piu X) \per Y \ar[ur,"\codiag X \per \id Y"']
%	\end{tikzcd}
%	\qquad
%	\begin{tikzcd}
%		X \per \zero \ar[dr,"\id X \per \cobang Y"] \\
%		\zero \ar[u,"\Iannr X"] \ar[r,"\cobang{X \per Y}"] \ar[d,"\Iannl Y"'] & X \per Y \\
%		\zero \per Y \ar[ur,"\cobang X \per \id Y"']
%	\end{tikzcd}
%	\]
\[
	\codiag{X\per Y}=\Idr{X}{Y}{Y};(\codiag{X}\per \id{Y})	=\Idl{X}{Y}{Y};(\id{X}\per \codiag{Y})\qquad \qquad
	\cobang{X\per Y}=\Iannl{Y};(\cobang{X}\per\id{Y})=\Iannr{X};(\id{X}\per\cobang{Y})
	\]
\end{lemma}


We expect the following result to be known but we cannot find a reference for it. 
\begin{proposition}\label{prop: Kleisli of distributive monoidal}
Let $(\Cat{C},\piu,\zero,\per, \uno)$ be a finite coproduct rig category and $T \colon \Cat{C}\to \Cat{C}$ be a symmetric monoidal monad over $(\Cat{C},\per, \uno)$. Then the Kleisli category $\Cat{C}_T$ is a finite coproduct rig category. 
\end{proposition}
The fact that $\Cat{C}_T$ has coproducts easily follows by standard arguments. The hard part of the proof, in Appendix~\ref{app:section:rigcategories}, consists in proving naturality of the distributors $\delta^l$ and $\delta^r$.
%
%
%In Sections \ref{sec:fccdrig} and \ref{sec:Trig}, we will consider some additional structures on fc rig categories.  For later use, we fix the following definition.
%
Before combining fc rig categories with cd categories in Section~\ref{sec:fccdrig}, it is convenient to fix the following definition.
%
%
%In the next sections, we will enrich fc rig categories with some additional structures. For the time being, it is useful to record the following definition.
\begin{definition}\label{def:fcfprig}
A \emph{finite coproduct-finite product (fc-fp) rig category} is a rig category $(\Cat{C}, \piu, \zero, \per, \uno)$  such that $(\Cat{C}, \piu, \zero)$ is a finite coproduct category and $(\Cat{C}, \per, \uno)$ is a finite product category. %A \emph{morphism of fc-fp categories} is a rig functor that is also a morphism of both finite product and finite coproduct categories. \marginpar{If not needed comment the definition of morphism}%We write $\FCRIG$ for the category of fb rig categories and their morphisms.
\end{definition}
%\begin{definition}
%A \emph{distributive category} is a rig category $(\Cat{C}, \piu, \zero, \per, \uno)$  such that $(\Cat{C}, \piu, \zero)$ is a finite coproduct category. %A \emph{morphism of distributive category categories} is a rig functor that and a morphisms of fb categories. We write $\FCRIG$ for the category of fb rig categories and their morphisms.
%\end{definition}
\begin{remark}\label{remark: distributive arrows in distriutive categories}
Note that, by definition, any fc-fp rig category has both finite coproducts (given by $\piu$) and products ($\per$). The reader may wonder whether any category with finite products and finite coprodutcs is also a fc-fp rig category. This is not the case, since the canonical morphism $(X\times Y)+ (X\times Z) \to X\times (Y + Z)$ induced by the universal properties of (co)products is not necessarily an iso. Categories with this property are known as \emph{distributive categories} \cite{carboni1993introduction}: note that the only difference with the structures in Definition~\ref{def:fcfprig} consists in the fact that in fc-fp rig categories the distributors $\delta^l$ and $\delta^r$ are not forced to be the canonical ones.  
However, as shown in \cite{lacknoncanonical}, the assumption of  natural isomorphisms $\delta^l$ and $\delta^r$ implies that the canonical morphisms are isos. Hence, every fc-fp rig category is also distributive. A similar mismatch arises amongst fc rig categories and \emph{monoidal distributive categories} \cite{annalabella}.
\end{remark}












==> oldsections/sections/sigmaerig.tex <==

\section{Combining Rig Categories with Algebraic Theories}\label{sec:Trig}
%
%
% COMMENTATO
%
%
\begin{comment}
\marginpar{The following two proposition might be moved}
\begin{definition}
 A \emph{cartesian signature} consists of a pair $(\Sigma, \operatorname{ar})$, where $\Sigma$ is a set of symbols and $\operatorname{ar}: \Sigma \to \mathbb{N}$ is a function that assigns to each symbol $f \in \Sigma$ a natural number $\operatorname{ar}(f)$, called its arity.

A \emph{$\Sigma$-term} is an expression formed using symbols from $\Sigma$ and a set of variables $V$, according to the context-free grammar:
\[
t ::= x \mid f^0 \mid f^n(t, \dots, t)
\]
where $x \in V$, and $f^0, f^n \in \Sigma$ satisfy $\operatorname{ar}(f^0) = 0$ and $\operatorname{ar}(f^n) = n$.

An \emph{algebraic theory} is defined as a pair $\mathbb{T} = (\Sigma, E)$, where $\Sigma$ is a cartesian signature and $E$ is a collection of equations between $\Sigma$-terms, represented as pairs $(t_1, t_2)$.
\end{definition}

\begin{definition}
Consider an algebraic theory $\mathbb{T} = (\Sigma, E)$. 
The associated Lawvere theory, denoted as $\lawveret$, is a category where objects correspond 
to natural numbers, and a morphism $n \to m$ is given by a tuple $\langle t_1, \dots, t_m \rangle$ 
of $\Sigma$-terms, modulo the equivalence relation induced by $E$. Each term $t_i$ depends only 
on the variables $x_1, \dots, x_n$. 

The composition of morphisms is defined via substitution:
\[
\big( \langle t_1, \dots, t_m \rangle : n \to m \big) \, ; \, 
\big( \langle s_1, \dots, s_o \rangle : m \to o \big) 
= \big\langle u_1, \dots, u_o \big\rangle : n \to o
\]
where each $u_i$ is obtained by substituting occurrences of $x_i$ in $s_i$ with $t_i$, formally:
\[
u_i = s_i[t_i/x_i \mid 1 \leq i \leq m].
\]
Furthermore, the categorical product $\times$ in $\lawveret$ is determined by 
addition on natural numbers.
\end{definition}
\end{comment}
%
%
%
%
%
%
%
%
%
%INIZIA QUA
%

In the previous section, we have illustrated how monoids for $\piu$ and comonoids for $\per$ interact within the Kleisli category of a symmetric monoidal monads. In Section \ref{sec:running}, we have seen that in $\Sets_{\subdistr}$, there are two more interesting arrows $\Br{+_p}_X$ and $\Br{\star}_X$ which arise from an algebraic theory presenting the monad $\subdistr$. In this section we focus on such arrows arising from algebraic theories.




\subsection{Preliminaries on Algebraic Theories}
%\elena{cite~\cite{staton2014freyd} for the correspondence between distributive Freyd categories and Lawvere theories for the doctrine of finite products}
A \emph{cartesian signature} is a couple $(\Sigma, \ar)$ where $\Sigma$ is a set of symbols and $\ar \colon \Sigma \to \mathbb{N}$ the arity function. %, shortly a single sorted monoidal signature where all symbols have coarity $1$. 
An \emph{algebraic theory} is a pair $\mathbb{T} = (\Sigma, E)$, where $\Sigma$ is a cartesian signature and $E$ is a set of equations between $\Sigma$-terms, represented as pairs $(t_1, t_2)$. Hereafter we write $T_{\mathbb{T}}$ for the \emph{term monad} on $\Sets$, i.e., the monad assigning to each set $X$ the set of all $E$-equivalence classes of $\Sigma$-terms with variables in $X$, and  $\lawveret$ for the \emph{Lawvere theory} associated to $\mathbb{T}$, i.e., the strict finite product category freely generated by $(\Sigma, E)$. In this category, objects are natural numbers, and a morphism $n \to m$ is a tuple $\langle t_1, \dots, t_m \rangle$ 
of $\Sigma$-terms --modulo the equivalence relation induced by $E$-- where each term $t_i$ has variables in  $x_1, \dots, x_n$. The categorical product in $\lawveret$ is determined by addition on natural numbers. %We write $\Cat{Mod}(\mathbb{T})$ for the category of \emph{models} of $\mathbb{T}$: this can be regarded either as the category of  Eilbenberg-Moore algebras for $T_{\mathbb{T}}$ or as the category of finite product morphisms from $\lawveret$ to $\Sets$.

Particularly relevant for our exposition is $\aleph_0$, the strict finite coproduct category freely generated by a single object. In $\aleph_0$, objects are finite ordinals --we write $n$ for the ordinal $\{0,\dots , n-1\}$--  and arrows are functions. By freeness, there exists an identity on object functor $d\colon \aleph_0 \to \opcat{\lawveret}$ for any algebraic theory $\mathbb{T}$. 
Moreover, there is a morphism of finite coproduct categories $c\colon \aleph_0 \to \Sets_{T_{\mathbb{T}}}$ that is obtained by  composing the embedding $\aleph_0 \to \Sets$ with the canonical left adjoint $\Sets \to \Sets_{T_{\mathbb{T}}}$. We write $ \Sets_{T_{\mathbb{T}}}^{\aleph_0}$ for the the full subcategory of $\Sets_{T_{\mathbb{T}}}$ having as object only finite ordinals. It is crucial for our development the well known fact \cite{hylandpoweruniversalalgebra} that $\Sets_{T_{\mathbb{T}}}^{\aleph_0}$ and $\opcat{\lawveret}$ are isomorphic as finite coproduct categories. We call $i\colon \opcat{\lawveret} \to  \Sets_{T_{\mathbb{T}}}$ the morphism obtained by postcomposing the isomorphism $\opcat{\lawveret} \to \Sets_{T_{\mathbb{T}}}^{\aleph_0}$ with the embedding $\Sets_{T_{\mathbb{T}}}^{\aleph_0}\to \Sets_{T_{\mathbb{T}}}$. In summary, we are interested in the morphisms of finite coproduct categories illustrated below.
%\[\begin{tikzcd}[column sep=4em]
%		\lawveret \ar[r,"\cong"] & \Sets_{T_{\mathbb{T}}}^{\aleph_0}  \ar[r,""]  &  \Sets_{T_{\mathbb{T}}}\\
%		 & \aleph_0 \ar[ur,"c"] \ar[u] \ar[ul,"d"]
%\end{tikzcd}\]
%
\begin{equation}\label{eq:Lawdiag}
\begin{tikzcd}[column sep=2em]
		\opcat{\lawveret} \ar[rr,"i"] &  &  \Sets_{T_{\mathbb{T}}}\\
		 & \aleph_0 \ar[ur,"c"']  \ar[ul,"d"]
\end{tikzcd}
\end{equation}
\begin{example}\label{ex:algebraic-theory-convex}
Consider $\mathbb{PCA}$, the algebraic theory of \emph{pointed convex algebras}: the signature $\Sigma$ consists of a binary operation $+_p$ for all $p\in(0,1)$ and a constant $\star$; the set of equations $E$ contains
\[(x_1+_q x_2)+_p x_3 =  x_1 +_{pq} (x_2+_{\frac{p(1-q)}{1-pq}} x_3) \qquad x_1+_px_2=x_2+_{1-p}x_1 \qquad  x_1+_p x_1 = x_1\]
It is well known, see e.g., \cite{swirszcz1974monadic,semadeni1973monads,jacobs2010convexity,doberkat2006eilenberg}, that the above theory provides a presentation for the monad $\subdistr$, in the sense that $T_\mathbb{PCA}$ and $\subdistr$ are isomorphic as monad. We will take the freedom to tacitly identify their Kleisli categories. 
Consider the morphism $x_1 +_p x_2 \colon 2 \to 1$ and $\star \colon 0 \to 1$ in $\Cat{L}_{\mathbb{PCA}}$. These are mapped, by $i$ into the function $i(+_p) \colon \{0\} \to \subdistr (\{0,1\})$ mapping the only element $0$ into the distribution where $0$ has probability $p$ and $1$ has probability $1-p$ and into $i(\star)\colon \{0\} \to \subdistr(\{\})$ mapping $0$ into the null subdistribution. %To conclude observe that $\Sets_{T_{\mathbb{PCA}}}^{\aleph_0}$ can be thought as the category having natural numbers as objects and sub-stochatic matrices as arrows.
\end{example}


%
%
%
%
%
%
%
%
%
%
%
%
%

\subsection{$\mathbb{T}$-rig categories}\label{ssec:rig}
We can now combine algebraic theories with finite coproduct rig categories (Definition~\ref{def:fcrig}). 

We start by observing that in a rig category, for any natural number $n$, there exists an object $\objn{n}\defeq \PiuL[i=1][n]{\uno}$, where $n$-ary sums are defined as in Table~\ref{tab:equationsonobject}.(b). Then, we show that, like for Kleisli categories,  for any  fc rig category $\Cat{C}$, there exists a canonical morphism of fc categories $c\colon \aleph_0 \to \Cat{C}$.
\begin{lemma}\label{lemma:aleph}
Let $\Cat{C}$ be a finite coproduct rig category. Then there exists a canonical morphism of finite coproduct categories $c\colon \aleph_0 \to \Cat{C}$ mapping each object $n$ of $\aleph_0$  into $\objn{n}$.
\end{lemma}

This lemma justifies the following definition.

\begin{definition}\label{def:Trig cat}
Let $\mathbb{T}$ be an algebraic theory. A \emph{$\mathbb{T}$-rig category} is a finite coproduct rig category $\Cat{C}$ together with a morphism of fc categories $i\colon \opcat{\lawveret} \to \Cat{C}$ making the following diagram commute. A morphism of $\mathbb{T}$-rig categories from $i \colon \opcat{\lawveret} \to \Cat{C}$ to $j \colon \opcat{\lawveret} \to \Cat{D}$ is a morphism of fc rig categories $f\colon \Cat{C} \to \Cat{D}$ such that $ i;f = j$. We will write simply $\Cat{C}$ whenever $i\colon \opcat{\lawveret} \to \Cat{C}$ is clear from the context.
%We write $\sigmaeRIG$ for the category of $\mathbb{T}$-rig categories and their morphisms.
\[\begin{tikzcd}[column sep=2em]
		\opcat{\lawveret} \ar[rr,"i"] &  &  \Cat{C}\\
		 & \aleph_0 \ar[ur,"c"']  \ar[ul,"d"]
\end{tikzcd}\]
\end{definition}
%
%
%
Note that commutativity of the above diagrams entails that for all $t\colon n \to 1$ in $\lawveret$, $i(t)$ is an arrow of type $1 \to \objn{n}$ in $\Cat{C}$. This gives rise to a natural transformation:
for all objects $X$,
\begin{equation}\label{eq:natf}
\Br{t}_X \defeq 
\begin{tikzcd}
	X & {1\per X} & { (\PiuL[i=1][n]{1})\per  X} & {\PiuL[i=1][n]{ X}}
    \arrow["{\Ilunitt{X}}", from=1-1, to=1-2]
	\arrow["{ i(t)\per \id{X}}", from=1-2, to=1-3]
	\arrow["{\delta^r_{n,X}}", from=1-3, to=1-4]
\end{tikzcd}
\end{equation}
where ${\delta^r_{n,X}}$ is the arrow inductively defined as $  \delta^r_{0,X}\defeq \annl{X}$ and ${\delta^r_{1,X}}\defeq \lunitt{X}$ and $\delta^r_{n+1,X} \defeq \dr{1}{\objn{n}}{X};(\lunitt{X}\piu \delta^r_{n,X})$.
In Appendix~\ref{app:Trig categories}, we show that $t$ is indeed natural (Lemma~\ref{lemma: f_X naturale}) and that it allows to monoidally enrich $\Cat{C}$ over the category of models of $\mathbb{T}$, a.k.a. Eilenberg-Moore algebras (Proposition \ref{prop:enrichement}). Moreover, $\Br{t}_X$ will play a crucial role in the tape diagrams in Section~\ref{sec:tapediagrams}.





%Table \ref{tab:equationsonobject}.(b) gives an inductive definition for $n$-ary sums: we will sometimes write $n$ for the object $\PiuL[i=1][n]{\uno}$ and  $\delta^r_{n,X}\colon (\PiuL[i=1][n]{1})\otimes X \to \PiuL[i=1][n]{X}$ for the arrow inductively defined as
%\begin{equation}
%\begin{array}{ccc}
%  \delta^r_{0,X}\defeq \annl{X} \;&\; \text{ and } \;&\; \delta^r_{n+1,X} \defeq \dr{1}{n}{X};(\lunitt{X}\piu \delta^r_{n,X}) \text{.}
%      \end{array}
%\end{equation}
%Simple inductive arguments confirm that both  $\delta^r_{n,X}$ and $\codiag{X}^n$ are natural in $X$. 

% shows that 
    





% \subsection{Tape diagrams for $(\Sigma,E)$-rig categories}\label{sc:tape}




% THE FOLLOWING SHOULD BE ALL ADJUSTED DIRECTLY TO $(\Sigma,E)$-rig categories

% THE ORIGINAL THEORY WITH ALL THE AXIOMS CAN BE IN THE APPENDIX

% ONE SHOULD ONLY ILLUSTRATE THE CHANGES TO THE ORIGINAL THEORY




% \begin{table}[t]
% {
% \begin{center}
% \begin{tabular}{cccc}
%     \toprule
%     \multicolumn{2}{c}{$\diag{ A}; (\id{ A}\perG \diag{ A}) = \diag{ A};(\diag{ A}\perG \id{ A})$} & $\diag{ A} ; (\bang{ A}\perG \id{ A}) = \id{ A} $ & $ \diag{ A};\sigma_{ A, A}=\diag{ A}$ \\
%     \multicolumn{2}{c}{$(\id{ A}\perG \codiag{ A}) ; \codiag{ A} = (\codiag{ A}\perG \id{ A}) ; \codiag{ A}$} & $(\cobang{ A}\perG \id{ A}) ; \codiag{ A}  = \id{ A} $ & $ \sigma_{ A, A};\codiag{ A}=\codiag{ A}$ \\
%     $\codiag{ A};\diag{ A} = \diag{ A\perG  A} ; (\codiag{ A} \perG \codiag{ A}) $ & $ \cobang{ A}; \bang{ A}= \id{\unoG} $ & $ \cobang{ A}; \diag{ A}= \cobang{ A\perG  A} $ & $ \diag{ A}; \bang{ A}= \bang{ A\perG  A}$\\
%     $\tapeFunct{c}; \bang{B}=\bang{A} $ & $ \tapeFunct{c}; \diag{B}=\diag{A}; (\tapeFunct{c} \perG \tapeFunct{c}) $ & $ \cobang{A};\tapeFunct{c} =\cobang{B} $ & $ \codiag{A};\tapeFunct{c} =(\tapeFunct{c} \perG \tapeFunct{c}); \codiag{B}$ \\
%     \multicolumn{2}{c}{$\tape{\id{A}} = \id{A}$} & \multicolumn{2}{c}{$\tape{c ; d} = \tape{c} ; \tape{d}$} \\
%     \bottomrule
%     \end{tabular}
% \end{center}
% }
% \caption{Additional axioms for $F_2(\Cat{C})$. Above, $c\colon A \to B$ is an arbitrary arrow of $\Cat{C}$}\label{fig:freestrictfbcat}
% \end{table}


% We have seen in Section~\ref{sec:monoidal} that string diagrams provide a convenient graphical language for strict monoidal categories.
% In this section, we recall tape diagrams, a sound and complete graphical formalism for sesquistrict rig categories introduced in~\cite{bonchi2023deconstructing}.


% The construction of tape diagrams goes through the adjunction in~\eqref{eq:adjunction}, where $\CAT$ is the category  of categories and functors, $\SMC$ is the category 
%  of ssm categories and functors, and $\FBC$ is the category of strict finite biproduct categories and their morphisms. 
% \begin{equation}\label{eq:adjunction} \begin{tikzcd}
% 		\SMC \ar[r,"U_1"] & \CAT \ar[r,bend left,"F_2"] \ar[r,draw=none,"\bot"description] & \FBC \ar[l,bend left,"U_2"]
% \end{tikzcd}
% \end{equation}
% The functors $U_1$ and $U_2$ are the obvious forgetful functors. The functor $F_2$ is the left adjoint to $U_2$, and can be described as follows.

% \begin{definition}\label{def:strict fb freely generated by C}
% Let $\Cat{C}$ be a category. The  strict fb category freely generated by $\Cat{C}$, hereafter denoted by $F_2(\Cat{C})$, has as objects words of objects of $\Cat{C}$. Arrows are terms inductively generated by the following grammar, where $A,B$ and $c$ range over arbitrary objects and arrows of $\Cat{C}$,\begin{equation}
%     \begin{array}{rcl}
%         f & ::=& \; \id{A} \; \mid \; \id{I} \; \mid \; \tapeFunct{c} \; \mid \; \sigma_{A,B}^{\perG} \; \mid \;   f ; f   \; \mid \;  f \perG f  \; \mid \; \bang{A} \; \mid \; \diag{A} \;  \mid \; \cobang{A}\; \mid \; \codiag{A}\\
%         \end{array}
% \end{equation}  
% modulo the axioms in  Tables~\ref{fig:freestricmmoncatax} and~\ref{fig:freestrictfbcat}. Notice in particular the last two from Table~\ref{fig:freestrictfbcat}:
% \begin{equation}\label{ax:tape}\tag{Tape}
% \tape{\id{A}} = \id{A} \qquad \tape{c;d}= \tape{c} ; \tape{d}
% \end{equation}
% \end{definition}
% The assignment $\Cat{C} \mapsto F_2({\Cat{C}})$ easily extends to functors $H\colon \Cat{C} \to \Cat{D}$.
% The unit of the adjunction $\eta \colon Id_{\CAT} \Rightarrow F_2U_2$ is defined for each category $\Cat{C}$ as the functor ${\tapeFunct{\cdot} \; \colon \Cat{C} \to U_2F_2(\Cat{C})}$ which is the identity on objects and maps every arrow $c$ in $\Cat{C}$ into the arrow $\tapeFunct{c}$ of $U_2F_2(\Cat{C})$. Observe that $\tapeFunct{\cdot}$ is indeed a functor, namely an arrow in $\CAT$, thanks to the axioms \eqref{ax:tape}. We will refer hereafter to this functor as the \emph{taping functor}.


% % \begin{lemma}\label{lemma:F2 left adjoint to U2}
% % $F_2 \colon \CAT \to \FBC$ is left adjoint to $U_2 \colon \FBC \to \CAT$.
% % \end{lemma}

% \medskip

% % \ale{POSSIAMO EVITARE LA SESQUISTRICTNESS(?)}

% The sesquistrict fb rig category freely generated by a monoidal signature $\sign$ is $F_2U_1(\CatString)$, hereafter referred to as $\CatTape$, and it is presented as follows.
% % This is somehow the fb rig category analogue to Theorem 2.3 in \cite{joyal1991geometry} mentioned in Section~\ref{sec:monoidal}. Let us see why.

% Recall that the set of objects of 
% $\CatString$ is $\sort^\star$, i.e.\ words of sorts in $\sort$. The set of objects of $\CatTape$ is thus $(\sort^\star)^\star$, namely words of words of sorts in $\sort$. For arrows, consider the following two-layer grammar where $s \in \sign$, $A,B \in \sort$ and $U,V \in \sort^\star$.
% \begin{equation}\label{tapesGrammar}
%     \begin{tabular}{rc ccccccccccccccccccccc}\setlength{\tabcolsep}{0.0pt}
%         $c$  & ::= & $\id{A}$ & $\!\!\! \mid \!\!\!$ & $ \id{\uno} $ & $\!\!\! \mid \!\!\!$ & $ \gen $ & $\!\!\! \mid \!\!\!$ & $ \sigma_{A,B} $ & $\!\!\! \mid \!\!\!$ & $   c ; c   $ & $\!\!\! \mid \!\!\!$ & $  c \per c$ & \multicolumn{8}{c}{\;} \\
%         $\t$ & ::= & $\id{U}$ & $\!\!\! \mid \!\!\!$ & $ \id{\zero} $ & $\!\!\! \mid \!\!\!$ & $ \tapeFunct{c} $ & $\!\!\! \mid \!\!\!$ & $ \sigma_{U,V}^{\piu} $ & $\!\!\! \mid \!\!\!$ & $   \t ; \t   $ & $\!\!\! \mid \!\!\!$ & $  \t \piu \t  $ & $\!\!\! \mid \!\!\!$  & $\cobang{U}$ & $\!\!\! \mid \!\!\!$ & $\codiag{U}$ & $\!\!\! \mid \!\!\!$ & $f_U$
%     \end{tabular}
% \end{equation}  
% The terms of the first row, denoted by $c$, are called \emph{circuits}. Modulo the axioms in Table~\ref{fig:freestricmmoncatax} (after replacing $\perG$ with $\per$), these are exactly the arrows of $\CatString$.
% The terms of the second row, denoted by $\t$, are called \emph{tapes}. Modulo the axioms in Tables \ref{fig:freestricmmoncatax} and \ref{fig:freestrictfbcat} (after replacing $\perG$ with $\piu$ and $A,B$ with $U,V$), these are exactly the arrows of $F_2U_1(\CatString)$, i.e.\  $\CatTape$. 

% Since circuits are arrows of $\CatString$, these can be graphically represented as string diagrams. Also tapes can be represented as string diagrams, since they satisfy all of the axioms of ssmc. Note however that \emph{inside} tapes, there are string diagrams: this justifies the motto \emph{tape diagrams are string diagrams of string diagrams}.
% Two layers grammars can be rendered graphically and formally~\cite{braithwaite2023collages}.
% The grammar in~\eqref{tapesGrammar} becomes:
% % \begin{equation*}\label{tapesDiagGrammar}
% %     \setlength{\tabcolsep}{2pt}
% %     \begin{tabular}{rc c@{$\,\mid\,$}c@{$\,\mid\,$}c@{$\,\mid\,$}c@{$\,\mid\,$}c@{$\,\mid\,$}c@{$\,\mid\,$}c@{$\,\mid\,$}c@{$\,\mid\,$}c}
% %         $c$  & $\Coloneqq$ &  $\wire{A}$ & $ \tikzfig{empty} $ & $ \Cgen{\gen}{A}{B}  $ & $ \Csymm{A}{B} $ & $ \tikzfig{seq_compC}   $ & $  \tikzfig{par_compC}$ \\
% %         $\t$ & $\Coloneqq$ & $\Twire{U}$ & $ \tikzfig{empty} $ & $ \Tcirc{c}{U}{V}  $ & $ \Tsymmp{U}{V} $ & $ \tikzfig{tapes/seq_comp}  $ & $  \tikzfig{tapes/par_comp}$  & $\Tunit{U}$  & $\Tmonoid{U}$ & $\Talgop{U}{f}$
% %     \end{tabular}
% % \end{equation*}  
% \begin{equation*}\label{tapesDiagGrammar}
%     \setlength{\tabcolsep}{2pt}
%     \begin{tabular}{rc c@{$\,\mid\,$}c@{$\,\mid\,$}c@{$\,\mid\,$}c@{$\,\mid\,$}c@{$\,\mid\,$}c@{$\,\mid\,$}c@{$\,\mid\,$}c@{$\,\mid\,$}c}
%         $c$  & $\Coloneqq$ &  $\wire{A}$ & $ \tikzfig{empty} $ & $ \Cgen{\gen}{A}{B}  $& $ \Csymm{A}{B} $ & $ \tikzfig{seq_compC}   $ & $  \tikzfig{par_compC}$ \\
%         $\t$ & $\Coloneqq$ & $\Twire{U}$ & $ \tikzfig{empty} $ & $ \Tcirc{c}{U}{V}  $ & $ \Tsymmp{U}{V} $ & $ \tikzfig{tapes/seq_comp}  $ & $  \tikzfig{tapes/par_comp}$ & $\Tunit{U}$  & $\Tmonoid{U}$ & $\Talgop{U}{f_U}$
%     \end{tabular}
% \end{equation*}  
% The identity $\id\zero$ is rendered as the empty tape $\tikzfig{empty}$, while $\id\uno$ is $\tikzfig{tapes/empty}$: a tape filled with the empty circuit. 
% For a monomial $U \!=\! A_1\dots A_n$, $\id U$ is depicted as a tape containing  $n$ wires labelled by $A_i$. For instance, $\id{AB}$ is rendered as $\TRwire{A}{B}$. When clear from the context, we will simply represent it as a single wire  $\Twire{U}$ with the appropriate label.
% Similarly, for a polynomial $P = \Piu[i=1][n]{U_i}$, $\id{P}$ is obtained as a vertical composition of tapes, as illustrated below on the left. \[ \id{AB \piu \uno \piu C} = \begin{aligned}\begin{gathered} \TRwire{A}{B} \\[-1.5mm] \Twire{\uno} \\[-2mm] \Twire{C} \end{gathered}\end{aligned} \qquad \qquad \tapesymm{AB}{C} = \tikzfig{tapes/examples/tapesymmABxC} \qquad\qquad \symmp{AB \piu \uno}{C} = \tikzfig{tapes/examples/symmpABp1pC} \]
% We can render graphically the symmetries $\tapesymm{U}{V} \colon UV \!\to\! VU$ and $\symmp{P}{Q} \colon P \piu Q \!\to\! Q \piu P$ as crossings of wires and crossings of tapes,  see the two rightmost diagrams above.
% The diagonal $\diag{U} \colon U \!\to\! U \piu U$ is represented as a splitting of tapes, while the bang $\bang{U} \colon U \!\to\! \zero$ is a tape closed on its right boundary. 
% Codiagonals and cobangs are represented in the same way but mirrored along the y-axis. Exploiting the coherence axioms in Figure~\ref{fig:fbcoherence}, we can construct (co)diagonals and (co)bangs for arbitrary polynomials $P$.
% For example, $\diag{AB}$, $\bang{CD}$, $\codiag{A\piu B \piu C}$ and $\cobang{AB \piu B \piu C}$ are depicted as:
% \[ 
%     \diag{AB} = \TLcomonoid{B}{A} \qquad \bang{CD} = \TLcounit{D}{C} \qquad  \codiag{A\piu B \piu C} = \tikzfig{tapes/examples/codiagApBpC} \qquad   \cobang{AB \piu B \piu C} = \tikzfig{tapes/examples/cobangABpBpC} 
% \]

% When the structure inside a tape is not relevant the graphical language can be ``compressed'' in order to simplify the diagrammatic reasoning. For example, for arbitrary polynomials $P, Q$ we represent $\id{P}, \symmp{P}{Q}, \diag{P}, \bang{P}, \codiag{P}, \cobang{P}$ as follows:
% \[ \TPolyWire{P} \qquad \TPolySymmp{P}{Q} \qquad \TPolyDiag{P} \qquad \TPolyCounit{P} \qquad \TPolyCodiag{P} \qquad \TPolyUnit{P} \]
% Moreover, for an arbitrary tape diagram $\t \colon P \to Q$ we write $\Tbox{\t}{P}{Q}$.



% It is important to observe that the graphical representation takes care of the two axioms in \eqref{ax:tape}: both sides of the leftmost axiom are depicted as $\Twire{A}$ while both sides of the rightmost axiom as
% $\tikzfig{tapes/ax/c_poi_d}$. The axioms of monoidal categories are also implicit in the graphical representation, while those for symmetries and the fb-structure (in Table~\ref{fig:freestrictfbcat}) have to be depicted explicitly as in Figure~\ref{fig:tapesax}. In particular, the diagrams in the first row express the inverse law and naturality of $\symmp$. In the second group there are the (co)monoid axioms and in the third group the bialgebra ones. Finally, the last group depicts naturality of the (co)diagonals and (co)bangs. 

% % \ale{POTREMMO ACCORPARE GLI ASSIOMI E LA GRAMMATICA GRAFICA}

% \begin{figure}[ht!]
%     \mylabel{ax:symmpinv}{$\symmp$-inv}
%     \mylabel{ax:symmpnat}{$\symmp$-nat}
%     \mylabel{ax:diagas}{$\diag{}$-as}
%     \mylabel{ax:diagun}{$\diag{}$-un}
%     \mylabel{ax:diagco}{$\diag{}$-co}
%     \mylabel{ax:codiagas}{$\codiag{}$-as}
%     \mylabel{ax:codiagun}{$\codiag{}$-un}
%     \mylabel{ax:codiagco}{$\codiag{}$-co}
%     \mylabel{ax:bi}{bi}
%     \mylabel{ax:bo}{bo}
%     \mylabel{ax:diagbi}{$\diag{}$-bi}
%     \mylabel{ax:codiagbi}{$\codiag{}$-bi}
%     \mylabel{ax:diagnat}{$\diag{}$-nat}
%     \mylabel{ax:bangnat}{$\bang{}$-nat}
%     \mylabel{ax:codiagnat}{$\codiag{}$-nat}
%     \mylabel{ax:cobangnat}{$\cobang{}$-nat}
%     \begin{center}
%         \scalebox{0.9}{
%     \begin{tabular}{C{1px} C{2.3cm} c C{2.5cm} C{5px} C{2.5cm} c C{2.3cm} C{1px}}
%         &\tikzfig{tapes/ax/symminv_left} &$\stackrel{(\symmp\text{-inv})}{=}$& \tikzfig{tapes/ax/symminv_right}  && \tikzfig{tapes/ax/symmnat_left}  &$\stackrel{(\symmp\text{-nat})}{=}$&  \tikzfig{tapes/ax/symmnat_right} & \\
% \hline
% &\tikzfig{tapes/whiskered_ax/comonoid_assoc_left}  &$\stackrel{(\diag{}\text{-as})}{=}$&  \tikzfig{tapes/whiskered_ax/comonoid_assoc_right} && \tikzfig{tapes/whiskered_ax/monoid_assoc_left} &$\stackrel{(\codiag{}\text{-as})}{=}$& \tikzfig{tapes/whiskered_ax/monoid_assoc_right} & \\
%         &\tikzfig{tapes/whiskered_ax/comonoid_unit_left} &$\stackrel{(\diag{}\text{-un})}{=}$& \Twire{U} && \tikzfig{tapes/whiskered_ax/monoid_unit_left} &$\stackrel{(\codiag{}\text{-un})}{=}$& \Twire{U} & \\
%         &\tikzfig{tapes/whiskered_ax/comonoid_comm_left} &$\stackrel{(\diag{}\text{-co})}{=}$& \Tcomonoid{U} && \tikzfig{tapes/whiskered_ax/monoid_comm_left} &$\stackrel{(\codiag{}\text{-co})}{=}$& \Tmonoid{U} &\\[-0.5ex]
% \hline
%         \\[-2.2ex]
%         &\tikzfig{tapes/whiskered_ax/bialg1_left} &$\stackrel{(\text{bi})}{=}$& \tikzfig{tapes/whiskered_ax/bialg1_right} && \tikzfig{tapes/whiskered_ax/bialg2_left}  &$\stackrel{(\text{bo})}{=}$&  \tikzfig{empty} & \\[-1ex]
%         &\tikzfig{tapes/whiskered_ax/bialg3_left}  &$\stackrel{(\diag{}\text{-bi})}{=}$&  \tikzfig{tapes/whiskered_ax/bialg3_right} && \tikzfig{tapes/whiskered_ax/bialg4_left}  &$\stackrel{(\codiag{}\text{-bi})}{=}$&  \tikzfig{tapes/whiskered_ax/bialg4_right} & \\
% \hline
%         \\
%         &\tikzfig{tapes/ax/comonoidnat_left} &$\stackrel{(\diag{}\text{-nat})}{=}$& \tikzfig{tapes/ax/comonoidnat_right} && \tikzfig{tapes/ax/monoidnat_left} &$\stackrel{(\codiag{}\text{-nat})}{=}$& \tikzfig{tapes/ax/monoidnat_right} & \\[-1ex]
%         &\tikzfig{tapes/ax/counitnat_left}  &$\stackrel{(\bang{}\text{-nat})}{=}$& \tikzfig{tapes/ax/counitnat_right} && \tikzfig{tapes/ax/unitnat_left}  &$\stackrel{(\cobang{}\text{-nat})}{=}$& \tikzfig{tapes/ax/unitnat_right} &
%     \end{tabular}}
%     \end{center}
%     \caption{Axioms for tape diagrams}
%     \label{fig:tapesax}
% \end{figure}


% \begin{theorem}\label{thm:Tapes is free sesquistrict generated by sigma}
% 	$\CatTape$ is the free sesquistrict fb rig category generated by the monoidal signature $(\sort, \sign)$.
% \end{theorem}
% The proof~\cite{bonchi2023deconstructing} of the above theorem mostly consists in illustrating that $\CatTape$ carries the structure of a rig category: $\per$ is defined on objects as in \eqref{def:productPolynomials}; the definition of symmetries for $\per$ and left distributors is given inductively in Table \ref{table:def dl symmt}; the definition of  $\per$ on tapes relies on the definition of \emph{left and right whiskerings}: see Table \ref{tab:producttape}. We will come back to whiskerings in Section \ref{ssec:tracerig}. For the time being, the reader can have a concrete grasp by means of the following example borrowed from \cite{bonchi2023deconstructing}.

% \begin{example}\label{ex:diagPer}
%     %The graphical representation of $\per$ follows from its definition. Indeed, it is enough to render the diagrams for the two polynomial whiskerings and compose them together in sequence. For example, 
%     Consider $\t\colon U\piu V \to W\piu Z$ and $\s\colon U'\piu V' \to W'\piu Z'$ illustrated below on the left. Then $\t \per \s$ is simply the sequential composition of $\LW{U\piu V}{\s}$ and $\RW{W' \piu Z'}{\t}$:
%     \[  \tikzfig{tapes/examples/t1} \per \tikzfig{tapes/examples/t2} = \tikzfig{tapes/examples/t1xt2_line} \]
%     The dashed line highlights the boundary between left and right polynomial whiskerings: $\LW{U \piu V}{\s}$, on the left, is simply the vertical composition of the monomial whiskerings $\LW{U}{\s}$ and $\LW{V}{\s}$ while, on the right, $\RW{W' \piu Z'}{\t}$ is rendered as the vertical composition of $\RW{W'}{\t}$ and $\RW{Z'}{\t}$, precomposed and postcomposed with left distributors.
% \end{example}

% \begin{table}[ht!]
%     \begin{center}
%     % \tiny{
%         % \hfill
%         \begin{subtable}{0.60\textwidth}
%             \begin{tabular}{l}
%                 \toprule
%                 $\dl{P}{Q}{R} \colon P \per (Q\piu R)  \to (P \per Q) \piu (P\per R) \vphantom{\symmt{P}{Q}}$ \\
%                 \midrule
%                 $\dl{\zero}{Q}{R} \defeq \id{\zero} \vphantom{\symmt{P}{\zero} \defeq \id{\zero}}$ \\
%                 $\dl{U \piu P'}{Q}{R} \defeq (\id{U\per (Q \piu R)} \piu \dl{P'}{Q}{R});(\id{U\per Q} \piu \symmp{U\per R}{P'\per Q} \piu \id{P'\per R}) \vphantom{\symmt{P}{V \piu Q'} \defeq \dl{P}{V}{Q'} ; (\Piu[i]{\tapesymm{U_i}{V}} \piu \symmt{P}{Q'})}$ \\
%                 \bottomrule
%             \end{tabular}
%             \caption{}
%             \label{table:def dl}
%         \end{subtable}
%         \;
%         \begin{subtable}{0.35\textwidth}
%             \begin{tabular}{l}
%                 \toprule
%                 $\symmt{P}{Q} \colon P\per Q \to Q \per P$, with $P = \Piu[i]{U_i}$ \\
%                 \midrule
%                 $\symmt{P}{\zero} \defeq \id{\zero}$ \\
%                 $\symmt{P}{V \piu Q'} \defeq \dl{P}{V}{Q'} ; (\Piu[i]{\tapesymm{U_i}{V}} \piu \symmt{P}{Q'})$ \\
%                 \bottomrule
%             \end{tabular}
%             \caption{}
%             \label{table:def symmt}
%         \end{subtable}
%         % \hfill
%         \caption{Inductive definition of $\delta^l$ and $\symmt$}
%         \label{table:def dl symmt}
%     % }
%     \end{center}
% \end{table}

% \begin{table}[ht!]
%     \begin{center}
%     {
%         \hfill
%   \[\begin{array}{c}
%         \def\arraystretch{1.5}
%         \begin{array}{rcl|rcl}
%             \toprule
%             \LW U {\id\zero} &\defeq& \id\zero& \RW U {\id\zero} &\defeq& \id\zero \\
%             % \LW U {\id\uno} &\defeq& \id U& \RW U {\id\uno} &\defeq& \id U \\
%             % \LW U {\id V} &\defeq& \id {UV}& \RW U {\id V} &\defeq& \id {VU} \\
%             % \LW U {\tape{\gen}} &\defeq& \tape{\id U \per \gen}& \RW U {\tape{\gen}} &\defeq& \tape{\gen \per \id U} \\
%             \LW U {\tape{c}} &\defeq& \tape{\id U \per c}& \RW U {\tape{c}} &\defeq& \tape{c \per \id U} \\
%             % &\LW U {\symmt{V}{W}} &\defeq& \symmp{UV}{UW}& \RW U {\symmt{V}{W}} &\defeq& \symmp{VU}{WU} \\
%             % \LW U {\tapesymm{V}{W}} &\defeq& \tapesymm{UV}{UW}& \RW U {\tapesymm{V}{W}} &\defeq& \tapesymm{VU}{WU} \\
%             \LW U {\symmp{V}{W}} &\defeq& \symmp{UV}{UW}& \RW U {\symmp{V}{W}} &\defeq& \symmp{VU}{WU} \\
%             \LW U {\diag V} &\defeq& \diag{UV}& \RW U {\diag V} &\defeq& \diag{VU} \\
%             \LW U {\bang V} &\defeq& \bang{UV}& \RW U {\bang V} &\defeq& \bang{VU} \\
%             \LW U {\codiag V} &\defeq& \codiag{UV}& \RW U {\codiag V} &\defeq& \codiag{VU} \\
%             \LW U {\cobang V} &\defeq& \cobang{UV}& \RW U {\cobang V} &\defeq& \cobang{VU} \\
%             \LW U {\t_1 ; \t_2} &\defeq& \LW U {\t_1} ; \LW U {\t_2}& \RW U {\t_1 ; \t_2} &\defeq& \RW U {\t_1} ; \RW U {\t_2} \\
%             \LW U {\t_1 \piu \t_2} &\defeq& \LW U {\t_1} \piu \LW U {\t_2}& \RW U {\t_1 \piu \t_2} &\defeq& \RW U {\t_1} \piu \RW U {\t_2} \\
%             \hline \hline
%             \LW{\zero}{\t} &\defeq& \id{\zero} & \RW{\zero}{\t} &\defeq& \id{\zero} \\
%             \LW{W\piu S'}{\t} &\defeq& \LW{W}{\t} \piu \LW{S'}{\t} & \RW{W \piu S'}{\t} &\defeq& \dl{P}{W}{S'} ; (\RW{W}{\t} \piu \RW{S'}{\t}) ; \Idl{Q}{W}{S'} \\
%             \hline \hline
%             \multicolumn{6}{c}{
%                 \t_1 \per \t_2 \defeq \LW{P}{\t_2} ; \RW{S}{\t_1}   \quad \text{ ( for }\t_1 \colon P \to Q, \t_2 \colon R \to S   \text{ )}
%             }
%             \\
%             \bottomrule
%         \end{array}
%     \end{array}        
%       \]
%       \hfill
%       \caption{Inductive definition of left and right monomial whiskerings (top); inductive definition of polynomial whiskerings (center); definition of $\per$ (bottom).}\label{tab:producttape}
%        }
%     \end{center}
% \end{table}


% CONTINUE LIKE THIS



% \begin{theorem}
%  BLA BLA is the sesqui-strict freely generated $(\Sigma,E)$-rig category
% \end{theorem}

% This result generalizes the one in \cite{} when taking $(\Sigma,E)$ to be the theory of commutative monoids.




==> oldsections/sections/sigmaetapes.tex <==

\section{Tape Diagrams}\label{sec:tapediagrams}
%
In this section we introduce diagrammatic languages for $\mathbb{T}$-rig categories (Section~\ref{sc:tape}) and $\mathbb{T}$-cd rig categories (Section~\ref{sc:tapeTcd}). Our main results are  analogous to Theorem 2.3 in~\cite{joyal1991geometry} showing that string diagrams are arrows of a strict symmetric monoidal category freely generated by a monoidal signature. To begin, we need to recall what strict and freely generated means in the context of rig categories.



\subsection{Freely Generated Sesquistrict Rig Categories} 

In Section \ref{sec:CD}, we mentioned that the strictification theorem for monoidal categories allows us to safely forgets about the structural isomorphisms  $\assoc{X}{Y}{Z}$, $\lunit{X}$ and $\runit{X}$ and, thus, drastically simplify definitions and proofs. A strictification result also holds for rig categories (Theorem 5.4.6 in~\cite{johnson2021bimonoidal}): it states that every rig category is equivalent to a \emph{right} strict rig category, defined as follows.

\begin{definition}
A rig category is said to be \emph{right} (respectively \emph{left}) \emph{strict} when both its monoidal structures are 
strict and $\lambda^\bullet, \rho^\bullet$ and $\delta^r$ (respectively $\delta^l$) are all identity 
natural isomorphisms. A \emph{right strict rig functor} is a strict symmetric monoidal functor for both $\per$ and $\piu$ preserving $\delta^l$. %We write $\RIG$ for the category of right strict rig categories and functors.\marginpar{be carefull about strictness here}
\end{definition}
Note that only one of the two distributors is forced to be the identity within a strict rig category. The curious reader is referred to \cite[Section 4]{bonchi2023deconstructing} for a brief explanation of this asymmetry. In loc. cit., it is also explained that the above notion of strictness is somewhat inconvenient when studying  freely generated categories: consider a right strict rig category freely generated by a signature $\Gamma$ with sorts $\sort$. The objects of this category are terms generated by the grammar in Table~\ref{table:eq objects fsr} modulo the equations in the first three rows of the same table. These equivalence classes of terms do not come with a very handy form, unlike, for instance, the objects of a strict monoidal category, which are words. %For this reason several authors, like~\cite{comfort2020sheet,johnson2021bimonoidal}, prefer to take as objects polynomials in $\sort$ at the price of working with a category that is not freely generated but only equivalent to a freely generated one. This fact forces one to consider functors that are not necessarily strict,  thus most of the constructions need to properly deal with the tedious natural isomorphisms.

\begin{table}
	\begin{center}
		\begin{subtable}{0.52\textwidth}
            \scalebox{0.8}{
            \begin{tabular}{c}
				\toprule
				$X \; ::=\; \; A \; \mid \; \uno \; \mid \; \zero \; \mid \;  X \per X \; \mid \;  X \piu X$\\
				\midrule
				\begin{tabular}{ccc}
					$ (X \per Y) \per Z = X \per (Y \per Z)$ & $\uno \per X = X$ &  $X \per \uno = X $\\
					$(X \piu Y) \piu Z = X \piu (Y \piu Z)$ & $\zero \piu X = X$  & $X \piu \zero =X  $\\
					$(X \piu Y) \per Z = (X \per Z) \piu (Y \per Z)$ &  $\!\zero \per X = \zero$ & $X \per \zero=X $\\
				\end{tabular}\\
				$A \per (Y \piu Z) = (A \per Y) \piu (A \per Z)$\\
				\bottomrule
			\end{tabular}
            }
            \caption{}
            \label{table:eq objects fsr}
        \end{subtable}
		\begin{subtable}{0.45\textwidth}
            \scalebox{0.8}{
            \begin{tabular}{c}
				\toprule
				$n$-ary sums and products $\vphantom{\mid}$\\
				\midrule
				\makecell{
					\\[-1pt]
					$\Piu[i=1][0]{X_i} = \zero \; \Piu[i=1][1]{X_i}= X_1 \; \Piu[i=1][n+1]{X_i} = X_1 \piu (\Piu[i=1][n]{X_{i+1}} )$ \\[1em]
					$\Per[i=1][0]{X_i} = \uno \; \Per[i=1][1]{X_i}= X_1 \; \Per[i=1][n+1]{X_i} = X_1 \per (\Per[i=1][n]{X_{i+1}} )$ \\[3pt]
				} \\
				\bottomrule
			\end{tabular}
            }
            \caption{}
            \label{table:n-ary sums and prod}
        \end{subtable}
	\end{center}
	\caption{Equations for the objects of a free sesquistrict rig category}\label{tab:equationsonobject}
\end{table}

An alternative solution is proposed in \cite{bonchi2023deconstructing}: the focus is  on  freely generated rig categories that are \emph{sesquistrict}, i.e.\ right strict but only partially left strict: namely the left distributor  $\dl{X}{Y}{Z} \colon X \per (Y \piu Z) \to (X \per Y) \piu (X \per Z)$ is the identity only when $X$ is a basic sort $A\in \sort$. In terms of the equations to impose on objects, this amounts to the one in the fourth row in Table~\ref{table:eq objects fsr} for each $A\in \sort$.  By orienting from left to right \emph{all} the equations in Table~\ref{table:eq objects fsr}, one obtains a rewriting system that is confluent and terminating and, most importantly, the unique normal forms are exactly polynomials: a term $X$  is in \emph{polynomial} form if there exist $n$, $m_i$ and $A_{i,j}\in \sort$ for $i=1 \dots n$ and $j=1 \dots m_i$ such that $X=\Piu[i=1][n]{\Per[j=1][m_i]{A_{i,j}}}$ (for $n$-ary sums and products as in Table~\ref{table:n-ary sums and prod}).
We will always refer to terms in polynomial form as \emph{polynomials} and, for a polynomial like the aforementioned  $X$, we will call \emph{monomials} of $X$ the $n$ terms $\Per[j=1][m_i]{A_{i,j}}$. For instance the monomials of $(A \per B) \piu \uno$ are $A \per B$ and $1$. Note that, differently from the polynomials we are used to dealing with, here neither $\piu$ nor $\per$ is commutative so, for instance, $(A \per B) \piu \uno$ is different from both $\uno \piu (A \per B)$ and $(B \per A) \piu \uno$. Note that non-commutative polynomials are in one to one correspondence with \emph{words of words} over $\sort$, while monomials are words over $\sort$. 
\begin{notation}
Hereafter, we will denote by $A,B,C\dots$ the sorts in $\sort$, by $U,V,W \dots$ the words in $\sort^\star$ and by $P,Q,R,S \dots$ the words of words in $(\sort^\star)^\star$. Given two words $U,V\in \sort^\star$, we will write $UV$ for their concatenation and $1$ for the empty word. Given two words of words $P,Q\in (\sort^\star)^\star$, we will write $P\piu Q$ for their concatenation and $\zero$ for the empty word of words. Given a word of words $P$, we will write $\pi P$ for the corresponding term in polynomial form, for instance $\pi(A \piu BCD\piu 1 )$ is the term $A \piu ((B \per (C \per D)) \piu \uno)$. Throughout this paper  we  often omit $\pi$, thus we implicitly identify words of words with polynomials.
\end{notation}


Beyond concatenation ($\piu$), one can define a product operation $\per$ on $(\sort^\star)^\star$ by taking the unique normal form of $\pi(P) \per \pi(Q)$ for any $P,Q\in (\sort^\star)^\star$. More explicitly for
$P = \Piu[i]{U_i}$ and $Q = \Piu[j]{V_j}$, 
\begin{equation}\label{def:productPolynomials} P \per Q \defeq \Piu[i]{\Piu[j]{U_iV_j}}.
\end{equation}
Observe that, if both $P$ and $Q$ are monomials, namely, $P=U$ and $Q=V$ for some $U,V\in \sort^\star$, then $P\per Q = UV$. We can thus safely write $PQ$ in place of $P\per Q$ without the risk of any confusion.








%It is useful to observe that the addition of these equations avoids the problem of using left and right strictness at the same time. Indeed $(A\piu B) \per (C \piu D)$ turns out to be equal to $(A \per C) \piu (A \per D) \piu (B \per C) \piu (B \per D)$ but not to $(A \per C) \piu (B \per C) \piu (A \per D)  \piu (B \per D)$. 











%Words of words are also exploited in the traditional \emph{strictification} theorem for rig categories (see e.g.\ Theorem 5.4.6 in~\cite{johnson2021bimonoidal}):
%given a rig category $\Cat C$, one can build a right strict rig category $\sCatT C$ that is equivalent to it. The objects of the strictification $\sCatT C$ are words of words of objects of $\Cat C$, while $\sCatT C[P,Q] = \Cat C[\pi P, \pi Q]$. It is easy to see that $\Cat C$ embeds into $\sCatT C$: a morphism $f \!\colon\! X \!\to\! Y$ in $\Cat C$ can be seen as a morphism in $\sCatT C[X,Y]$, where $X$ and $Y$ are considered as unary words made of a single unary word. This embedding forms an equivalence of rig categories $\Cat C \simeq \sCatT C$. See~\cite{johnson2021bimonoidal} for further details.
%
%
%
%It turns out that $\sCatT C$ does actually satisfy a partial left distribution, with $Ob(\Cat C)$ playing the role of $\sort$, as it were. To make this statement precise, we introduce the following notion.






\begin{definition}\label{def:sesquistrict rig category}
	A \emph{sesquistrict rig category} is a functor $H \colon \Cat S \to \Cat C$, where $\Cat S$ is a discrete category and $\Cat C$ is a right strict rig category, such that for all $A \in \Cat S$
	\[
	\dl{H(A)}{X}{Y} \colon H(A) \per (X \piu Y) \to (H(A) \per X) \piu (H(A) \per Y)
	\]
	is an identity morphism. We will also say, in this case, that $\Cat C$ is a $\Cat S$-sesquistrict rig category.
	
	Given $H \!\colon\! \Cat S \!\to\! \Cat C$ and $H' \!\colon\! \Cat S' \!\to\! \Cat C'$ two sesquistrict rig categories, a \emph{sesquistrict rig functor} from $H$ to $H'$ is a pair $(\alpha \!\colon\! \Cat S \!\to\! \Cat S', \beta \!\colon\! \Cat C \!\to\! \Cat C')$, with $\alpha$ a functor and $\beta$ a strict rig functor, such that $\alpha; H' = H; \beta$.
\end{definition}
\begin{remark}
In \cite{bonchi2023deconstructing}, it was shown that for any rig category $\Cat{C}$, one can construct its strictification $\overline{\Cat{C}}$ as in \cite{johnson2021bimonoidal} and then consider the obvious embedding from  $ob(\Cat{C})$, the discrete category of the objects of $\Cat{C}$, into $\overline{\Cat{C}}$. The embedding $ob(\Cat{C}) \to \overline{\Cat{C}}$ forms a sesquistrict category and it is equivalent (as a rig category) to the original $\Cat{C}$ \cite[Corollary 4.5]{bonchi2023deconstructing}. Hereafter, when dealing with a rig category $\Cat{C}$, we will often implicitly refer to the equivalent sesquistrict $ob(\Cat{C}) \to \overline{\Cat{C}}$.
\end{remark}



% \begin{theorem}\label{thm:strict(C) is sesquistrict}
% Let $\Cat C$ be a rig category. Then its strictification $\sCatT C$ is a $Ob(\Cat C)$-sesquistrict rig category.\end{theorem}
% \begin{proof}
% 	We recall from~\cite{johnson2021bimonoidal} some facts regarding the strictification $\sCatT C$ of $\Cat C$.
	
% 	Let $P$ and $Q$ be objects of $\sCatT C$. Then $P \per Q$ is given as in~\eqref{def:productPolynomials} and it is immediate to see that $A \per (P \piu Q) = (A \per P) \piu (A \per Q)$ when $A \in Ob(\Cat C)$. In order to prove that $\id{A \per (P \piu Q)} = \dl{A}{P}{Q}$ in $\sCatT C$, one needs to expand the definition of the left distributor $\delta^l$ and the symmetries $\sigma^\otimes$ in $\sCatT C$, which involve structural isomorphisms of $\Cat C$, and use the coherence theorem for rig categories, as stated in Theorem~3.9.1 of~\cite{johnson2021bimonoidal}. For this it is enough to observe that $\pi(A \per (P \piu Q))$ is \emph{regular} in the sense of~\cite[Definition 3.1.25]{johnson2021bimonoidal}. 
% \end{proof}

%
%
%
%\ale{Dire questo corollario a parole}
%\begin{corollary}[Sesquistrictification]
%Any rig category is rig equivalent to a sesquistrict rig category.
%\end{corollary}

% In light of the corollary above, from now on we will only consider strictified rig categories. Moreover, in the rest of the article, whenever we will be considering strict symmetric monoidal functors $F \colon \Cat C \to \Cat D$ where $\Cat D$ is a rig category, we will actually mean that $F \colon \Cat C \to \sCatT D$ and we will assume that $F$ sends objects of $\Cat C$ to objects of $\Cat D$ (embedded in $\sCatT D$). This assumption is not restrictive, as witnessed by the following lemma.

Given a set of sorts $\sort$, a \emph{rig signature} is a tuple $(\sort,\Gamma,\ar,\coar)$ where $\ar$ and $\coar$ assign to each $\gen \in \Gamma$ an arity and a coarity respectively, which are polynomials. A \emph{monoidal signature} is a rig signature where arity and coarity of any $s\in \Gamma$ are monomials. An \emph{interpretation} of a rig signature $(\sort,\Gamma,\ar,\coar)$ in a sesquistrict  rig category $H \colon \Cat M \to \Cat D$ is a pair of functions $(\alpha_{\sort} \colon \sort \to Ob(\Cat M), \alpha_\Gamma \colon \Gamma \to Ar(\Cat D))$ such that, for all $\gen \in \Gamma$, $\alpha_{\Gamma}(s)$ is an arrow having as domain and codomain $(\alpha_{\sort};H)^\sharp(\ar(s))$ and  $(\alpha_{\sort};H)^\sharp(\coar(s))$, where $-^\sharp$ stands for the expected inductive extension.

\begin{definition}\label{def:freesesqui}
Let $(\sort,\Gamma,\ar,\coar)$ (simply $\Gamma$ for short) be a rig signature. A sesquistrict  rig category $H \colon \Cat M \to \Cat D$ is said to be \emph{freely generated} by $\Gamma$ if there is an interpretation $(\alpha_S,\alpha_\Gamma)$ of $\Gamma$ in $H$ such that for every sesquistrict rig category $H' \colon \Cat M' \to \Cat D'$ and every interpretation $(\alpha_\sort' \colon \sort \to Ob(\Cat M'), \alpha_\Gamma' \colon \Gamma \to Ar(\Cat D'))$ there exists a unique sesquistrict rig functor $(\alpha \colon \Cat M \to \Cat M', \beta \colon \Cat D \to \Cat D')$ such that $\alpha_\sort ; \alpha = \alpha_\sort'$ and $\alpha_\Gamma ; \beta = \alpha_{\Gamma}'$. 
\end{definition}
%This is the definition of free object on a generating one instantiated in the category of sesquistrict rig categories and the category of rig signatures.
%Thus, sesquistrict rig categories generated by a given signature are isomorphic to each other and we may refer to ``the'' free sesquistrict rig category generated by a signature.
%
\begin{remark}
Theorem 4.9 in \cite{bonchi2023deconstructing} guarantees that, whenever $\piu$ is forced to be a biproduct, every rig signature can be reduced to a monoidal one. 
When $\piu$ is not necessarily a biproduct, as it is the case of $\mathbb{T}$-rig categories, monoidal signatures are less expressive than rig ones. 

The diagrammatic language introduced in the next section is limited to monoidal signatures: on the one hand, this restriction is what  allows having intuitive 2 dimensional diagrams; on the other, the use of the natural transformations in \eqref{eq:natf} makes the language expressive enough to generalise  \cite{bonchi2023deconstructing}.
\end{remark}













% THE FOLLOWING SHOULD BE ALL ADJUSTED DIRECTLY TO $(\Sigma,E)$-rig categories

% THE ORIGINAL THEORY WITH ALL THE AXIOMS CAN BE IN THE APPENDIX

% ONE SHOULD ONLY ILLUSTRATE THE CHANGES TO THE ORIGINAL THEORY

% \bigskip
% \bigskip

\begin{table}[t]
    % \centering
    \scalebox{0.7}{
        \[
        \begin{array}{@{}c@{}}
        \toprule
        \begin{array}{c@{\qquad}c}
            \begin{array}{c@{\qquad}c@{\qquad}c@{\qquad}c@{\qquad}c}
                \id{\uno} \colon \uno \to \uno 
                &
                \id{A} \colon A \to A  
                &
                {id_\zero \colon \zero \to \zero} 
                & 
                {id_U \colon U \to U} 
                & 
                s \colon \ar(s) \to \coar(s)
                \\
                \symmt{A}{B} \colon A \per B \to B \per A
                &
                {\sigma_{U, V}^{\piu} \colon U \piu V \to V \piu U} 
                &
                {\codiag{U}\colon U \piu U \to U}
                &
                { \cobang{U} \colon \zero \to U}   
                &
                \inferrule{c \colon U \to V}{\tapeFunct{c}\colon U \to V} 
            \end{array}    
            &
            \inferrule{\ar{(f)}=n }{\textstyle{\Br{f}_U \colon U \to \bigoplus^n U}}
        \end{array}
        \\
        \begin{array}{c@{\qquad}c@{\qquad}c@{\qquad}c}
            \inferrule{c \colon U \to V \and d \colon V \to W}{c ; d \colon U \to W}
            &
            \inferrule{c \colon U_1 \to V_1 \and d \colon U_2 \to V_2}{c \per d \colon U_1 \per  U_2 \to V_1 \per  V_2}
            &
            \inferrule{\t \colon P \to Q \and \s \colon Q \to R}{\t ; \s \colon P \to R}
            &
            \inferrule{\t \colon P_1 \to Q_1 \and \s \colon P_2 \to Q_2}{\t \piu \s \colon P_1 \piu P_2 \to Q_1 \piu Q_2}       
        \end{array}
        \\
        \midrule
        \midrule
        \begin{array}{@{}l @{\quad}|@{\quad} r}
            \begin{array}{cc}
                (f;g);h=f;(g;h) & id_X;f=f=f;id_Y
                \\
                \multicolumn{2}{c}{(f_1\perG f_2) ; (g_1 \perG g_2) = (f_1;g_1) \perG (f_2;g_2)}
                \\
                id_{\unoG}\perG f = f = f \perG id_{\unoG} & (f \perG g)\, \perG h = f \perG \,(g \perG h)
                \\
                \sigma_{A, B}^{\perG}; \sigma_{B, A}^{\perG}= id_{A \perG B} & (\gen \perG id_Z) ; \sigma_{Y, Z}^{\perG} = \sigma_{X,Z}^{\perG} ; (id_Z \perG \gen)
            \end{array}
            &
            \begin{array}{cc}
                (\id{ U}\piu \codiag{ U}) ; \codiag{ U} = (\codiag{ U}\piu \id{ U}) ; \codiag{ U} & \codiag{U};\tapeFunct{c} =(\tapeFunct{c} \piu \tapeFunct{c}); \codiag{V} \quad \cobang{U};\tapeFunct{c} =\cobang{V} \\ %\codiag{U} ; f_U = (f_U \piu f_U) ; \codiag{U \piu \ldots \piu U} \\
                \multicolumn{2}{c}{
                (\cobang{ U}\piu \id{ U}) ; \codiag{ U}  = \id{ U} 
                \quad\;\;
                \codiag{U} ; \Br{f}_U = (\Br{f}_U \piu \Br{f}_U) ; \codiag{\Piu[][n]{U}} 
                \quad\;\;
                \cobang{U};\Br{f}_U = \cobang{\Piu[][n]U}  % \cobang{U} ; f_U = \cobang{U} \piu \ldots \piu \cobang{U} \\
                } \\
                \sigma_{ U, U}^\piu;\codiag{ U}=\codiag{ U} & \t ; \Br{f}_Q = \Br{f}_P ; \Piu[][n] \t  \\ %               \tapeFunct{c} ; f_V = f_U ; (\tapeFunct{c} \piu \ldots \piu \tapeFunct{c}) \\
                \multicolumn{2}{c}{\tape{\id{U}} = \id{U} \qquad \tape{c ; d} = \tape{c} ; \tape{d} \qquad t_U = t'_U, \text{ with } (t,t') \in E}
                % \tape{\id{U}} = \id{U} & \tape{c ; d} = \tape{c} ; \tape{d}
            \end{array}
        \end{array}
        \\
        \midrule
        \midrule
        \begin{array}{@{}l | l | l}

            \begin{array}{@{}l}
                % \toprule
                \codiag{P} \colon P \per P \to P
                \\
                \midrule
                \codiag{\zero} \defeq \id{\zero} 
                \qquad\qquad
                \codiag{U \piu P'} \defeq (\id{U} \piu \symmp{U}{P'} \piu \id{P'}) ; (\codiag{U} \piu \codiag{P'})
                \phantom{\quad}
                % \\
                % \bottomrule
            \end{array}
        &
        % \multicolumn{2}{l}{
            \begin{array}{@{}l}
            % \toprule
            \smash{\cobang{P} \colon \zero \to P}
            \\
            \midrule
            \cobang{\zero} \defeq \id{\zero} 
            \qquad\qquad
            \cobang{U \piu P'} \defeq \cobang{U} \piu \cobang{P'}
            \phantom{\qquad}
            \end{array}
        % }
        &
        \begin{array}{@{}l}
            % \toprule
            \smash{\id{P} \colon P \to P}
            \\
            \midrule
            \id{\zero} \defeq \id{\zero} 
            \qquad
            \id{U \piu P'} \defeq \id{U} \piu \cobang{P'}
        \end{array}
            \\
            \midrule
            \begin{array}{@{}l@{\qquad\qquad}l}
                \multicolumn{2}{@{}l}{
                    \sigma^\piu_{P,Q} \colon P \piu Q \to Q \piu P
                }
                \\
                \midrule
                \sigma^\piu_{\zero,Q} \defeq \id{Q} 
                &
                \sigma^\piu_{U \piu P',Q} \defeq (\id{U} \piu \sigma^\piu_{P', Q}) ; (\sigma^\piu_{U,Q} \piu \id{P'})
                \\
                \sigma^\piu_{P, \zero} \defeq \id{P}
                &
                \sigma^\piu_{P, W \piu Q'} \defeq (\sigma^\piu_{P,W} \piu \id{Q'}) ; (\id{W} \piu \sigma^\piu_{P,Q'})
                \phantom{\quad}
                \end{array}
                &
            \multicolumn{2}{l}{
                    \begin{array}{@{}l@{\qquad\qquad}l}
                    \multicolumn{2}{@{}l}{
                        \sigma_{U,V} \colon U \per V \to V \per U
                    }
                        \\
                        \midrule
                        \sigma_{U, \uno} \defeq \id{U}
                        &
                        \sigma_{A \per U',W} \defeq (\id{A} \per \sigma_{U', W}) ; (\sigma_{A,W} \per \id{U'})
                        \\
                        \sigma{\uno, W} \defeq \id{W}
                        &
                        \sigma_{U, B \per W'} \defeq (\sigma_{U,B} \per \id{W'}) ; (\id{B} \per \sigma_{U,W'})
                        \phantom{\qquad\qquad\qquad}
                    \qquad
                \end{array}
            }
            \\
            \midrule
            \begin{array}{@{}l}
                % \toprule
                \dl{P}{Q}{R} \colon P \per (Q\piu R)  \to (P \per Q) \piu (P\per R) \vphantom{\symmt{P}{Q}} \\
                \midrule
                \dl{\zero}{Q}{R} \defeq \id{\zero} \vphantom{\symmt{P}{\zero} \defeq \id{\zero}} \\
                \dl{U \piu P'}{Q}{R} \defeq (\id{U\per (Q \piu R)} \piu \dl{P'}{Q}{R});(\id{U\per Q} \piu \symmp{U\per R}{P'\per Q} \piu \id{P'\per R}) \vphantom{\symmt{P}{V \piu Q'} \defeq \dl{P}{V}{Q'} ; (\Piu[i]{\tapesymm{U_i}{V}} \piu \symmt{P}{Q'})} \\
                % \bottomrule
            \end{array}
            &
            \begin{array}{@{}l}
                % \toprule
                \symmt{P}{Q} \colon P\per Q \to Q \per P, \text{ with } P = \Piu[i]{U_i} \\
                \midrule
                \symmt{P}{\zero} \defeq \id{\zero} \\
                \symmt{P}{V \piu Q'} \defeq \dl{P}{V}{Q'} ; (\Piu[i]{\tapesymm{U_i}{V}} \piu \symmt{P}{Q'})
                \phantom{\quad}
                % \bottomrule
            \end{array}
            &
            \begin{array}{@{}l}
                \Br{f}_P \colon P \to \bigoplus^n P \\
                \midrule
                \Br{f}_\zero \defeq \id{\zero} \\
                \Br{f}_{U \piu P'} \defeq (\Br{f}_U \piu \Br{f}_{P'}) ; \Idl{\piu^n \uno}{U}{P'} 
                % \phantom{\qquad}
            \end{array}
        \end{array}
        \\
        \bottomrule
        \end{array}
        \]
    }
    \caption{Typing rules (top), axioms (middle) and syntactic sugar (bottom) for $\algt$-tapes.}
    \label{tab:tape typing and axioms}%\label{tab:axiomTAPE}
    \label{table:def syn sugar}
\end{table}

% \begin{table}[ht!]
%     \begin{center}
%         \begin{tabular}{c|c}
%             \toprule
%             \begin{tabular}{l}
%                 % \toprule
%                 $\dl{P}{Q}{R} \colon P \per (Q\piu R)  \to (P \per Q) \piu (P\per R) \vphantom{\symmt{P}{Q}}$ \\
%                 \midrule
%                 $\dl{\zero}{Q}{R} \defeq \id{\zero} \vphantom{\symmt{P}{\zero} \defeq \id{\zero}}$ \\
%                 $\dl{U \piu P'}{Q}{R} \defeq (\id{U\per (Q \piu R)} \piu \dl{P'}{Q}{R});(\id{U\per Q} \piu \symmp{U\per R}{P'\per Q} \piu \id{P'\per R}) \vphantom{\symmt{P}{V \piu Q'} \defeq \dl{P}{V}{Q'} ; (\Piu[i]{\tapesymm{U_i}{V}} \piu \symmt{P}{Q'})}$ \\
%                 % \bottomrule
%             \end{tabular}
%             &
%             \begin{tabular}{l}
%                 % \toprule
%                 $\symmt{P}{Q} \colon P\per Q \to Q \per P$, with $P = \Piu[i]{U_i}$ \\
%                 \midrule
%                 $\symmt{P}{\zero} \defeq \id{\zero}$ \\
%                 $\symmt{P}{V \piu Q'} \defeq \dl{P}{V}{Q'} ; (\Piu[i]{\tapesymm{U_i}{V}} \piu \symmt{P}{Q'})$ \\
%                 % \bottomrule
%             \end{tabular}
%             \\[20pt]
%             \midrule
%             \multicolumn{2}{c}{
%                 \begin{tabular}{c|c|c}
%                     \begin{tabular}{l}
%                         % \toprule
%                         $\codiag{P} \colon P \per P \to P$
%                         \\
%                         \midrule
%                         $\codiag{\zero} \defeq \id{\zero} $
%                         \\
%                         $\codiag{U \piu P'} \defeq (\id{U} \piu \symmp{U}{P'} \piu \id{P'}) ; (\codiag{U} \piu \codiag{P'})$
%                         % \\
%                         % \bottomrule
%                     \end{tabular}
%                     &
%                     \begin{tabular}{l}
%                         % \toprule
%                         $\cobang{P} \colon \zero \to P
%                         \vphantom{\copier{U} \colon U \to U \per U}$
%                         \\
%                         \midrule
%                         $\cobang{\zero} \defeq \id{\zero} $
%                         \\
%                         $\cobang{U \piu P'} \defeq \cobang{U} \piu \cobang{P'}
%                         \vphantom{\cocopier{U \piu P'} \defeq \Tcocopier{U} \piu \bang{UP'} \piu (\dl{P'}{U}{P'} ; (\bang{P'U} \piu \cocopier{P'}))}$
%                         % \\
%                         % \bottomrule
%                     \end{tabular}
%                     &
%                     \begin{tabular}{l}
%                         % \toprule
%                         $f_P \colon P \to \piu^n P$ \\
%                         \midrule
%                         $f_\zero \defeq \id{\zero}$ \\
%                         $f_{U \piu P'} \defeq (f_U \piu f_{P'}) ; \Idl{\piu^n \uno}{U}{P'}$ 
%                         % \bottomrule
%                     \end{tabular}
%                 \end{tabular}
%             }
%             \\
%             \bottomrule
%         \end{tabular}
%         \caption{Syntactic sugar for $\algt$-tapes.}
%         \label{table:def syn sugar}
%     % }
%     \end{center}
% \end{table}


% \begin{equation}\label{eq:adjunction} \begin{tikzcd}
%     \SMC \ar[r,"U_1"] & \CAT \ar[r,bend left,"F_2"] \ar[r,draw=none,"\bot"description] & \Cat{FCC} \ar[l,bend left,"U_2"]
% \end{tikzcd}
% \end{equation}
% The functors $U_1$ and $U_2$ are the obvious forgetful functors. The functor $F_2$ is the left adjoint to $U_2$, and can be described as follows.

% \begin{definition}\label{def:strict fb freely generated by C}
% Let $\Cat{C}$ be a category. The  strict fc category freely generated by $\Cat{C}$, hereafter denoted by $F_2(\Cat{C})$, has as objects words of objects of $\Cat{C}$. Arrows are terms inductively generated by the following grammar, where $A,B$ and $c$ range over arbitrary objects and arrows of $\Cat{C}$,\begin{equation} 
%     \begin{array}{rcl}
%         f & ::=& \; \id{A} \; \mid \; \id{I} \; \mid \; \tapeFunct{c} \; \mid \; \sigma_{A,B}^{\perG} \; \mid \;   f ; f   \; \mid \;  f \perG f  \;  \mid \; \cobang{A}\; \mid \; \codiag{A} \\ 
%         \end{array}
% \end{equation}  
% modulo the axioms in  Table~\label{tab:tape typing and axioms}. Notice in particular the last two from the bottom right of Table\label{tab:tape typing and axioms}:
% \begin{equation}\label{ax:tape}\tag{Tape}
% \tape{\id{A}} = \id{A} \qquad \tape{c;d}= \tape{c} ; \tape{d}
% \end{equation}
% \end{definition}
% The assignment $\Cat{C} \mapsto F_2({\Cat{C}})$ easily extends to functors $H\colon \Cat{C} \to \Cat{D}$.
% The unit of the adjunction $\eta \colon Id_{\CAT} \Rightarrow F_2U_2$ is defined for each category $\Cat{C}$ as the functor ${\tapeFunct{\cdot} \; \colon \Cat{C} \to U_2F_2(\Cat{C})}$ which is the identity on objects and maps every arrow $c$ in $\Cat{C}$ into the arrow $\tapeFunct{c}$ of $U_2F_2(\Cat{C})$. Observe that $\tapeFunct{\cdot}$ is indeed a functor, namely an arrow in $\CAT$, thanks to the axioms \eqref{ax:tape}. We will refer hereafter to this functor as the \emph{taping functor}.


% \begin{lemma}\label{lemma:F2 left adjoint to U2}
% $F_2 \colon \CAT \to \FBC$ is left adjoint to $U_2 \colon \FBC \to \CAT$.
% \end{lemma}

% \smallskip

% AGGIUSTARE DA QUA IN POI

% \smallskip

\subsection{Tape Diagrams for $\algt$-Rig Categories}\label{sc:tape}
%
For an algebraic theory $\algt = (\Sigma, E)$, we want to identify a $\algt$-rig category freely generated from a monoidal signature $(\sort, \Gamma)$. Our work is an adaptation of the tape diagrams in~\cite{bonchi2023deconstructing}.
%We consider the sesquistrict rig category that has objects in $(\sort^\star)^\star$ and as arrows the terms generated by the following :

Consider terms generated by the following two-layer grammar
\begin{equation}\label{tapesGrammar}
    \begin{tabular}{rc ccccccccccccccccccccc}\setlength{\tabcolsep}{0.0pt}
        $c$  & ::= & $\id{A}$ & $\!\!\! \mid \!\!\!$ & $ \id{\uno} $ & $\!\!\! \mid \!\!\!$ & $ \gen $ & $\!\!\! \mid \!\!\!$ & $ \sigma_{A,B} $ & $\!\!\! \mid \!\!\!$ & $   c ; c   $ & $\!\!\! \mid \!\!\!$ & $  c \per c$ & \multicolumn{8}{c}{\;} \\
        $\t$ & ::= & $\id{U}$ & $\!\!\! \mid \!\!\!$ & $ \id{\zero} $ & $\!\!\! \mid \!\!\!$ & $ \tapeFunct{c} $ & $\!\!\! \mid \!\!\!$ & $ \sigma_{U,V}^{\piu} $ & $\!\!\! \mid \!\!\!$ & $   \t ; \t   $ & $\!\!\! \mid \!\!\!$ & $  \t \piu \t  $ & $\!\!\! \mid \!\!\!$  & $\cobang{U}$ & $\!\!\! \mid \!\!\!$ & $\codiag{U}$ & $\!\!\! \mid \!\!\!$ & $\Br{f}_U$
    \end{tabular}
\end{equation}  
where $A,B \in \sort$, $U,V \in \sort^\star$, $s \in \Gamma$ and $f \in \Sigma$. Terms are typed according to the rules at the top of Table~\ref{tab:tape typing and axioms}: each type is an arrow $P \to Q$ where $P,Q\in (\sort^\star)^\star$. As expected, we consider only those terms that are typeable. Constants in~\eqref{tapesGrammar} can be extended to arbitrary $P \in (\sort^\star)^\star$, according to the inductive definitions at the bottom of Table~\ref{table:def syn sugar}. %\marginpar{manca la simmetria del piu e l'identita'} %For instance, $\codiag{P}$ is inductively defined as $\codiag{\zero} = \id{\zero}$ and $\codiag{U \piu Q} = (\id{U} \piu \sigma_{Q,U}^\piu \piu \id{Q}) ; (\codiag{U} \piu \codiag{Q})$.

Terms in the first layer of the grammar are called \emph{circuits}; those in the second layer are \emph{tapes}. 
Note that (a) circuits can occur inside tapes, (b) circuits have type $U\to V$, for $U,V\in \sort^\star$ and can be composed via $\per$, (c) tapes have type $P\to Q$ for $P,Q\in (\sort^\star)^\star$ and can be composed via $\piu$. 

The key insights of \cite{bonchi2023deconstructing} is that one can define $\per$ also on tapes: for $\t_1 \colon P \to Q$, $\t_2 \colon R \to S$,  $\t_1 \per \t_2 \defeq \LW{P}{\t_2} ; \RW{S}{\t_1} $ where $\LW{P}{\cdot}$, $\RW{S}{\cdot}$ are the left and right whiskerings, defined as in Table~\ref{tab:producttape}. This stratification is what allows to draw terms in \eqref{tapesGrammar} in just two dimensions, while more direct representation of rig categories require three dimensions (see e.g. \cite{comfort2020sheet}).%\marginpar{Insert reference to sheets diagrams} 

% \marginpar{Aggiustare un po' il discorso qua}
The main novelty of tapes for \(\mathbb{T}\) lies in the \( \Br{f}_U \)'s, which allow us to represent the operations of the algebraic theory \(\algt\). By combining the \( \Br{f}_U \)'s with the monoid structure \((\codiag{U}, \cobang{U})\), we can represent every term of the theory. Specifically, for each $\sign$-term $t \colon n \to 1$ and object $U \in \sort^\star$ there is an associated term $\Br{t}_U \colon U \to \Piu[][n]{U}$ constructed inductively on the $\sign$-terms as follows:%as in \eqref{eq: definizione f(t_1,...,t_n)}, using the $f_U$'s, $\id{U}$, $\sigma_{U,U}^\piu$, $\cobang{U}$ and $\codiag{U}$.
\begin{center} %\marginpar{Definito Male: $f$ potrebbe avere un'arieta' diversa da $n$}
$
\Br{x_i}_U \defeq \cobang{\Piu[][i-1]{U}} \piu \id{U} \piu \cobang{\Piu[][n-i]{U}}
\qquad\quad
\Br{f(t_1, \ldots, t_m)}_U \defeq \Br{f}_U ; (\Br{t_1}_U \piu \ldots \piu \Br{t_m}_U) ; \codiagg{\Piu[][n]{U}}{m}
$,
\end{center}
where $f\in \sign$ has arity $m$ and $\codiagg{P}{m} \colon \Piu[][m] P \to P$ is defined inductively as 
$\codiagg{P}{0} \defeq \cobang{P}$ and $\codiagg{P}{m+1} \defeq (\id{P} \piu \codiagg{P}{m}) ; \codiag{P}$.


Next, we impose the laws of $\algt$-rig categories on tapes: the axioms of symmetric monoidal categories for both layers; the axioms in $E$ of $\mathbb{T}$, the axioms of fc categories and those stating naturality of the $\Br{f}_U$'s for the second layer.
%
Formally, for each axiom $l=r$ in the middle left of Table~\ref{tab:tape typing and axioms}, we build a set $\basicR$ containing the pairs $(l,r)$  where  $\perG$ and $\unoG$ are replaced by $\piu$ and $\zero$ and the pairs $(\tape{l},\tape{r})$ where $\perG$ and $\unoG$ are replaced by $\per$ and $\uno$. Moreover, we add a pair $(l,r)$ for each axiom $l = r$ in the middle right of Table~\ref{tab:tape typing and axioms}.
%
Now we define $\congI$, the smallest congruence relation (w.r.t. $;$, $\piu$ and $\per$) containing $\basicR$, according to the following inductive rules. % \marginpar{Non usare $s$: si usa per i generatori} \marginpar{Secondo me quelle per la naturalita' cosi' non bastano}
\begin{equation}\label{eq:congr}
        \scalebox{0.85}{$
        \centering
        \begin{array}{c}
        \begin{array}{c@{\qquad\qquad}c@{\qquad\qquad}c@{\qquad\qquad}c}
            \inferrule*[right=($\basicR$)]{\t_1 \mathbin{\basicR} \t_2}{\t_1 \mathrel{\congI} \t_2}
            &
            \inferrule*[right=($\textsc{R}$)]{-}{\t \mathrel{\congI} \t}
            &
            \inferrule*[right=($\textsc{S}$)]{\t_1 \mathrel{\congI} \t_2}{\t_2 \mathrel{\congI} \t_1}
            &    
            \inferrule*[right=($\textsc{T}$)]{\t_1 \mathrel{\congI} \t_2 \quad \t_2 \mathrel{\congI} \t_3}{\t_1 \mathrel{\congI} \t_3}
            % &
            % \inferrule*[right=($E$)]{ (t,t') \in E \and U \in \sort^\star}{ t_U \mathrel{\congI} t'_U}
        \end{array}
        \\[10pt]
        \begin{array}{c@{\qquad}c@{\qquad}c}
            \inferrule*[right=($;$)]{\t_1 \mathrel{\congI} \t_2 \quad \s_1 \mathrel{\congI} \s_2}{\t_1;\s_1 \mathrel{\congI} \t_2;\s_2}
            &
            \inferrule*[right=($\piu$)]{\t_1 \mathrel{\congI} \t_2 \quad \s_1 \mathrel{\congI} \s_2}{\t_1\piu\s_1 \mathrel{\congI} \t_2 \piu \s_2}
            &
            \inferrule*[right=($\per $)]{\t_1 \mathrel{\congI} \t_2 \quad \s_1 \mathrel{\congI} \s_2}{\t_1\per \s_1 \mathrel{\congI} \t_2 \per \s_2}       
        \end{array}
        \end{array}
        $}
\end{equation}
% Observe that the rule $(E)$ allows to incorporate the equations in $\algt$ as equations between tapes.
Finally, we construct the category $\CatTapeT[\Gamma][\algt]$ whose objects are polynomials in $(\sort^\star)^\star$ and arrows are $\congI\text{-equivalence}$ classes of typed terms generated from~\eqref{tapesGrammar}. This construction gives rise to a $\algt$-rig category $\Br{\cdot}_1\colon \opcat{\lawveret} \to \CatTapeT[\Gamma][\algt]$. Most importantly, it is the freely generated one.

\begin{theorem}\label{thm:free signametape}
    $\CatTapeT[\Gamma][\algt]$ is the free sesquistrict $\algt$-rig generated by the monoidal signature $(\sort,\Gamma)$. %and an algebraic theory $\algt$.
\end{theorem}


\begin{table}[t]
    \begin{center}
    {
        \hfill {\tiny
  \[\begin{array}{c}
        \def\arraystretch{1.2}
        \begin{array}{rclrcl|rclrcl}
            \toprule
            \LW U {\id\zero} &\defeq& \id\zero& \LW U {\t_1 \piu \t_2} &\defeq& \LW U {\t_1} \piu \LW U {\t_2} &  \RW U {\id\zero} &\defeq& \id\zero & \RW U {\t_1 \piu \t_2} &\defeq& \RW U {\t_1} \piu \RW U {\t_2} \\
            \LW U {\tape{c}} &\defeq& \tape{\id U \per c} &    \LW U {\t_1 ; \t_2} &\defeq& \LW U {\t_1} ; \LW U {\t_2}&  \RW U {\tape{c}} &\defeq& \tape{c \per \id U} & \RW U {\t_1 ; \t_2} &\defeq& \RW U {\t_1} ; \RW U {\t_2} \\
            \LW U {\symmp{V}{W}} &\defeq& \symmp{UV}{UW}       &       \LW U {\Br{f}_V} &\defeq& \Br{f}_{UV} & \RW U {\symmp{V}{W}} &\defeq& \symmp{VU}{WU}& \RW U {\Br{f}_U} &\defeq& \Br{f}_{VU} \\
            \LW U {\codiag V} &\defeq& \codiag{UV} &  \LW U {\cobang V} &\defeq& \cobang{UV}& \RW U {\codiag V} &\defeq& \codiag{VU} & \RW U {\cobang V} &\defeq& \cobang{VU} \\
            \hline \hline
            \LW{\zero}{\t} &\defeq& \id{\zero} &  \LW{W\piu S'}{\t} &\defeq& \LW{W}{\t} \piu \LW{S'}{\t} & \RW{\zero}{\t} &\defeq& \id{\zero} &
            \RW{W \piu S'}{\t} &\defeq& \dl{P}{W}{S'} ; (\RW{W}{\t} \piu \RW{S'}{\t}) ; \Idl{Q}{W}{S'} \\
            \hline \hline
            \multicolumn{12}{c}{
                \t_1 \per \t_2 \defeq \LW{P}{\t_2} ; \RW{S}{\t_1}   \quad \text{ ( for }\t_1 \colon P \to Q, \t_2 \colon R \to S   \text{ )}
            }
            \\
            \bottomrule
        \end{array}
    \end{array}        
      \]
      }
      \hfill
      \caption{Inductive definition of left and right monomial whiskerings (top); inductive definition of polynomial whiskerings (center); definition of $\per$ (bottom).}\label{tab:producttape}
       }
    \end{center}
\end{table}


\begin{remark}\label{remark:Generalization}
Theorem~\ref{thm:free signametape} generalizes Theorem 5.11 in \cite{bonchi2023deconstructing} when $\algt$ is $\mathbb{CM}$, the theory of commutative monoids (Example~\ref{ex:CM}).
\end{remark}


The arrows of $\CatTapeT[\Gamma][\algt]$ enjoy an intuitive 2 dimesional representation in terms of \emph{tape diagrams}. The grammar in~\eqref{tapesGrammar} becomes:
\begin{equation*}\label{tapesDiagGrammar}
    \setlength{\tabcolsep}{2pt}
    \begin{tabular}{rc c@{$\,\mid\,$}c@{$\,\mid\,$}c@{$\,\mid\,$}c@{$\,\mid\,$}c@{$\,\mid\,$}c@{$\,\mid\,$}c@{$\,\mid\,$}c@{$\,\mid\,$}c}
        $c$  & $\Coloneqq$ &  $\wire{A}$ & $ \tikzfig{empty} $ & $ \Cgen{\gen}{A}{B}  $& $ \Csymm{A}{B} $ & $ \tikzfig{seq_compC}   $ & $  \tikzfig{par_compC}$ \\
        $\t$ & $\Coloneqq$ & $\Twire{U}$ & $ \tikzfig{empty} $ & $ \Tcirc{c}{U}{V}  $ & $ \Tsymmp{U}{V} $ & $ \tikzfig{tapes/seq_comp}  $ & $  \tikzfig{tapes/par_comp}$ & $\Tunit{U}$  & $\Tmonoid{U}$ & $\Talgop{U}{f}$
    \end{tabular}
\end{equation*}  
The identity $\id\zero$ is rendered as the empty tape $\tikzfig{empty}$, while $\id\uno$ is $\tikzfig{tapes/empty}$: a tape filled with the empty circuit. %\marginpar{Aggiustare quanto segue a seconda dello spazio e di quello che il lettore deve capire per andare il resto}
For a monomial $U \!=\! A_1\dots A_n$, $\id U$ is depicted as a tape containing  $n$ wires labelled by $A_i$. For instance, $\id{AB}$ is rendered as $\TRwire{A}{B}$. When clear from the context, we will simply represent it as a single wire  $\Twire{U}$ with the appropriate label.
Similarly, for a polynomial $P = \Piu[i=1][n]{U_i}$, $\id{P}$ is obtained as a vertical composition of tapes, as illustrated below on the left. 


\scalebox{0.82}{$ 
    \id{AB \piu \uno \piu C} = \!\!\!\begin{aligned}\begin{gathered} \TRwire{A}{B} \\[-1.8mm] \Twire{\uno} \\[-1.8mm] \Twire{C} \end{gathered}\end{aligned}
    \qquad\;\;
    \codiag{A\piu B \piu C} = \!\!\tikzfig{tapes/examples/codiagApBpC}
    \qquad\;\;
    \cobang{AB \piu B \piu C} = \!\tikzfig{tapes/examples/cobangABpBpC}
    \qquad\;\;
    \tikzfig{tapes/examples/algt}
$}


The codiagonal $\codiag{U} \colon  U \piu U \!\to\! U$ is represented as a merging of tapes, while the cobang $\cobang{U} \colon \zero \!\to\! U$ is a tape closed on its left boundary. 
Exploiting the definitions in Table~\ref{table:def syn sugar}, we can construct codiagonals and cobangs for arbitrary polynomials.
For example, $\codiag{A\piu B \piu C}$ and $\cobang{AB \piu B \piu C}$ are depicted as the second and third diagrams above. The last diagram is the tape for 
$\Br{(\star +_p x_1)+_q x_1}_A$ when the algebraic theory is fixed to be $\mathbb{PCA}$ (Example~\ref{ex:algebraic-theory-convex}).

%associated to the $\sign$-term $f(f(g, x),x)$, where $\sign = \{f \colon 2 \to 1, g \colon 0 \to 1\}$.
For an arbitrary $\t \colon P \to Q$ we write $\Tbox{\t}{P}{Q}$. For a $\sign$-term $t \colon n \to 1$ we write \scalebox{0.8}{$\TSterm{U}{t_U}$}.%For a $\sign$-term $t \colon n \to 1$ we write its associated tape diagram $t_U \colon U \to \Piu[][n]{U}$ as \scalebox{0.8}{$\TSterm{U}{t}$}.

The graphical representation embodies several axioms such as those of symmetric monoidal categories. Those axioms that are not implicit in the graphical representation are shown in Figure~\ref{fig:tapesax}. %\marginpar{Mancano gli assiomi dei tape e delle simmetrie del per dentro i tape... No?} 





%
%
%
%
%
%
%

\begin{figure}[t]
    \mylabel{ax:symmpinv}{$\symmp$-inv}
    \mylabel{ax:symmpnat}{$\symmp$-nat}
    
    \mylabel{ax:codiagas}{$\codiag{}$-as}
    \mylabel{ax:codiagun}{$\codiag{}$-un}
    \mylabel{ax:codiagco}{$\codiag{}$-co}
    
    \mylabel{ax:codiagnat}{$\codiag{}$-nat}
    \mylabel{ax:cobangnat}{$\cobang{}$-nat}

    % \mylabel{ax:codiagf}{$\codiag{}$-$f$}
    % \mylabel{ax:cobangf}{$\cobang{}$-$f$}
    \mylabel{ax:fnat}{$f$-nat}

    \begin{center}
        \scalebox{0.9}{
            \begin{tabular}{r@{}c@{}l @{} r@{}c@{}l @{} r@{}c@{}l}
                % \multicolumn{9}{c}{
                    % \begin{tabular}{r@{}c@{}l @{\qquad\qquad} r@{}c@{}l}
                        \tikzfig{tapes/ax/symminv_left} &$\stackrel{(\symmp\text{-inv})}{=}$& \tikzfig{tapes/ax/symminv_right}  
                    & 
                    \tikzfig{tapes/ax/symmnat_left}  &$\stackrel{(\symmp\text{-nat})}{=}$&  \tikzfig{tapes/ax/symmnat_right}
                        % \end{tabular}
                % }
                &
                \multicolumn{3}{c}{
                    \begin{tabular}{r@{}c@{}l}
                        \tikzfig{cb/symm_inv_left} & $\axeq{\sigma\text{-inv}}$ & \tikzfig{cb/symm_inv_right} 
                        \\
                        \tikzfig{cb/symm_nat_left} & $\axeq{\sigma\text{-nat}}$ & \tikzfig{cb/symm_nat_right}
                    \end{tabular}
                }
                \\
                % \multicolumn{9}{c}{
                %     \begin{tabular}{c@{}c@{}c c@{}c@{}c c@{}c@{}c}
                        \tikzfig{tapes/whiskered_ax/monoid_assoc_left} &$\stackrel{(\codiag{}\text{-as})}{=}$& \tikzfig{tapes/whiskered_ax/monoid_assoc_right}  
                        &
                        \tikzfig{tapes/whiskered_ax/monoid_unit_left} &$\stackrel{(\codiag{}\text{-un})}{=}$& \Twire{U}
                        &
                        \tikzfig{tapes/whiskered_ax/monoid_comm_left} &$\stackrel{(\codiag{}\text{-co})}{=}$& \Tmonoid{U}
                    % \end{tabular}
                % }
                \\
                \multicolumn{9}{c}{
                    \begin{tabular}{r@{}c@{}l @{\qquad} r@{}c@{}l @{\qquad} r@{}c@{}l}
                        \tikzfig{tapes/ax/monoidnat_left} &$\stackrel{(\codiag{}\text{-nat})}{=}$& \tikzfig{tapes/ax/monoidnat_right}
                        &
                        \tikzfig{tapes/ax/unitnat_left}  &$\stackrel{(\cobang{}\text{-nat})}{=}$& \tikzfig{tapes/ax/unitnat_right}
                        &
                        \scalebox{0.8}{\tikzfig{tapes/ax/newax/nat/left}} & $\stackrel{(f\text{-nat})}{=} \; \; $ & \scalebox{0.8}{\tikzfig{tapes/ax/newax/nat/right}}
                        \\
                        \tikzfig{tapes/ax/newax/copyf_left} &$\stackrel{(\codiag{}\text{-nat})}{=}$& \scalebox{0.7}{\tikzfig{tapes/ax/newax/copyf_right}}
                        &
                        \tikzfig{tapes/ax/newax/discf_left} &$\stackrel{(\cobang{}\text{-nat})}{=}$& \tikzfig{tapes/ax/newax/discf_right}       
                        &
                        $\TSterm{U}{t}$ & $=$ & $\TSterm{U}{t'}$
                    \end{tabular}
                }
                % \multicolumn{3}{c}{
                %     \!\!\!\!\begin{tabular}{r@{}c@{}c}
                %         \tikzfig{tapes/ax/monoidnat_left} &$\stackrel{(\codiag{}\text{-nat})}{=}$& \tikzfig{tapes/ax/monoidnat_right}
                %         \\       
                %         \tikzfig{tapes/ax/unitnat_left}  &$\stackrel{(\cobang{}\text{-nat})}{=}$& \tikzfig{tapes/ax/unitnat_right}
                %     \end{tabular}
                % }
                % &
                % \tikzfig{tapes/ax/newax/nat/left} & $\stackrel{(f\text{-nat})}{=} \; \; $ & \tikzfig{tapes/ax/newax/nat/right}
                % \\
                % \tikzfig{tapes/ax/newax/copyf_left} &$\stackrel{(\codiag{}\text{-}f)}{=}$& \scalebox{0.8}{\tikzfig{tapes/ax/newax/copyf_right}}
                % &
                % $\TSterm{U}{t}$ & $=$ & $\TSterm{U}{t'}$
                % \multicolumn{3}{c}{
                %     \!\!\!\!\!\begin{tabular}{r@{}c@{}c}
                %         \tikzfig{tapes/ax/newax/discf_left} &$\stackrel{(\cobang{}\text{-}f)}{=}$& \tikzfig{tapes/ax/newax/discf_right}       
                %         \\
                %         \tikzfig{tapes/ax/newax/fcopies_left} &$\stackrel{(f\text{-nat})}{=}$& \tikzfig{tapes/ax/newax/fcopies_right}
                %     \end{tabular}
                % }
            \end{tabular}
        }
    \end{center}
    \caption{Axioms for $\algt$-tape diagrams. Here $(t,t') \in E$.}
    \label{fig:tapesax}
\end{figure}




\subsection{Tape Diagrams for $\algt$-cd Rig Categories}\label{sc:tapeTcd}

% INSERT HERE THE ADDITIONAL SYNTAX
% THE FACT THAT ONE DEFINE THE COPIER AND DISCHARGER ON ARBITRARY POLYNOMIALS WITH THE COHERENCE AXIOMS
% INSERT THE MAIN EXAMPLE
% \bigskip

In this section, we extend $\algt$-tape diagrams to deal with $\algt$-cd rig categories. Obviously, this requires augmenting the grammar in~\eqref{tapesGrammar} with the copy $\copier{A}$ and discard $\discharger{A}$ operations, for every $A \in \sort$.
\begin{equation}%\label{CDtapesGrammar}
    \begin{tabular}{rc ccccccccccccccccccccc}\setlength{\tabcolsep}{0.0pt}
        $c$  & ::= & $\id{A}$ & $\!\!\! \mid \!\!\!$ & $ \id{\uno} $ & $\!\!\! \mid \!\!\!$ & $ \gen $ & $\!\!\! \mid \!\!\!$ & $ \sigma_{A,B} $ & $\!\!\! \mid \!\!\!$ & $   c ; c   $ & $\!\!\! \mid \!\!\!$ & $  c \per c$ & $\!\!\! \mid \!\!\!$  & $\discharger{A}$ & $\!\!\! \mid \!\!\!$ & $\copier{A}$ & \\
        $\t$ & ::= & $\id{U}$ & $\!\!\! \mid \!\!\!$ & $ \id{\zero} $ & $\!\!\! \mid \!\!\!$ & $ \tapeFunct{c} $ & $\!\!\! \mid \!\!\!$ & $ \sigma_{U,V}^{\piu} $ & $\!\!\! \mid \!\!\!$ & $   \t ; \t   $ & $\!\!\! \mid \!\!\!$ & $  \t \piu \t  $ & $\!\!\! \mid \!\!\!$  & $\cobang{U}$ & $\!\!\! \mid \!\!\!$ & $\codiag{U}$ & $\!\!\! \mid \!\!\!$ & $\Br{f}_U$
    \end{tabular}
\end{equation}  
Next, we construct the category $\CatTapeTCD[\Gamma][\algt]$ as in Section~\ref{sc:tape}, but extending $\basicR$ to include the axioms of cocommutative comonoids for $(\copier{A}, \discharger{A})$. Graphically, we require the following equations.
\begin{center}
    $\tikzfig{cb/monoid_assoc_right} = \tikzfig{cb/monoid_assoc_left} 
    \qquad
    \tikzfig{cb/monoid_unit_left}  = \tikzfig{cb/monoid_unit_right} 
    \qquad
    \tikzfig{cb/monoid_comm_left}  = \tikzfig{cb/monoid_comm_right}$.
\end{center}
%
%
%The coherence conditions in~\eqref{eq:comonoidcoherence} ensure that the copy-discard structure can be defined for every monomial $U \in \sort^\star$. In particular, we have that:
Copier and discard can be defined  for every  $U \in \sort^\star$ via the coherence conditions in~\eqref{eq:comonoidcoherence}:
\[
    \begin{array}{rcl C{0.65cm} rcl}
        \copier{\uno} &\defeq& \id{\uno} && \discharger{\uno} &\defeq& \id{\uno}  \\
        \copier{A \per U'} &\defeq& (\copier{A} \per \copier{U'}) ; (\id{A} \per \sigma^\per_{A, U'} \per \id{U'}) && \discharger{A \piu U'} &\defeq& (\discharger{A} \per \discharger{U'})
    \end{array}
\]
%
% \marginpar{Can you please insert the definition of copier and discard for monomials?} 
However, to conclude that $\CatTapeTCD[\Gamma][\algt]$ is a $\algt$-cd rig category, we need to show that the copy-discard structure exists for every polynomial $P \in (\sort^\star)^\star$.
%
The conditions in~\eqref{equation: coherence1} provide an inductive definition:
\begin{equation}\label{eq:copierind}
    \begin{array}{rcl C{0.5cm} rcl}
        \copier{\zero} &\defeq& \id{\zero} && \discharger{\zero} &\defeq& \cobang{\uno}  \\
        \copier{U \piu P'} &\defeq& \Tcopier{U} \piu \cobang{UP'} \piu ((\cobang{P'U} \piu \copier{P'}) ; \Idl{P'}{U}{P'}) && \discharger{U \piu P'} &\defeq& (\Tdischarger{U} \piu \discharger{P'}) ; \codiag{\uno}
    \end{array}
\end{equation}
%
For instance, $\copier{A \piu B} \colon A \piu B \to (A \piu B) \per (A \piu B) = AA \piu AB \piu BA \piu BB$ and $\discharger{A \piu B} \colon A \piu B \to \uno$ are:
%
\begin{center}
    $\copier{A \piu B} = \!\!\!\tikzfig{cb/examples/copierApB} 
    \qquad\qquad
    \discharger{A \piu B} = \!\!\tikzfig{cb/examples/dischargerApB}$
\end{center}


% The fact that $(\copier{P} \colon P \to P \per P, \discharger{P} \colon P \to \uno)$, as defined in~\eqref{eq:copierind}, satisfy the axioms of cocommutative comonoids is proved in~\cite[Theorem 7.3]{bonchi2023deconstructing}. Thus, the following result holds. \marginpar{Questo si puo' nascondere nella dimostrazione del teorema?}
%With these definitions, one can easily prove our main result.
\begin{theorem}\label{th:tapes-free-T-cd}
    $\CatTapeTCD[\Gamma][\algt]$ is the free sesquistrict $\algt$-cd rig generated by the monoidal signature $(\sort,\Gamma)$.
\end{theorem}
By virtue of the above theorem, any intepretation $\interpretation$ of the monoidal signature $(\sort,\Gamma)$ into a $\algt$-cd rig category $\Cat{C}$, gives rise uniquely 
to a morphism $\CBdsem{-}_\interpretation \colon \CatTapeTCD[\Gamma][\algt] \to \Cat{C}$ which represents the \emph{compositional} semantics of tapes. Its inductive definition is reported in Figure \ref{eq:SEMANTICA}.



\begin{figure}[t]
    \renewcommand{\arraystretch}{1.5}
\!\!\!\begin{tabular}{l@{\;\;\;\;}l@{\;\;\;\;}l@{\;\;\;\;}l@{\;\;\;\;}l}
$\CBdsem{s}_{\interpretation} \defeq \alpha_{\Gamma}(s) $& $\CBdsem{\, \tapeFunct{c} \,}_{\interpretation}\defeq \CBdsem{c}_{\interpretation} $ & $\CBdsem{\codiag{U}}_{\interpretation}\defeq \codiag{\alpha^\sharp_\sort(U)} $&$ \CBdsem{\cobang{U}}_{\interpretation} \defeq \cobang{\alpha^\sharp_\sort(U)}$   &  $\CBdsem{\Br{f}_{U}}_{\interpretation} \defeq j(f) \per \id{\alpha^\sharp_\sort(U)}$\\
$\CBdsem{\id{A}}_{\interpretation}\defeq \id{\alpha_\sort(A)} $&$ \CBdsem{\id{1}}_{\interpretation}\defeq \id{1} $&$ \CBdsem{\symmt{A}{B}}_{\interpretation} \defeq \symmt{\alpha_\sort(A)}{\alpha_\sort(B)}  $&$ \CBdsem{c;d}_{\interpretation} \defeq \CBdsem{c}_{\interpretation}; \CBdsem{d}_{\interpretation}  $ & $ \CBdsem{c\per d}_{\interpretation} \defeq \CBdsem{c}_{\interpretation} \per \CBdsem{d}_{\interpretation}$\\
$\CBdsem{\id{U}}_{\interpretation}\defeq \id{\alpha^\sharp_\sort(U)} $&$ \CBdsem{\id{\zero}}_{\interpretation} \defeq \id{\zero}  $&$ \CBdsem{\symmp{U}{V}}_{\interpretation}\defeq \symmp{\alpha^\sharp_\sort(U)}{\alpha^\sharp_\sort(V)} $&$ \CBdsem{\s;\t}_{\interpretation} \defeq \CBdsem{\s}_{\interpretation} ; \CBdsem{\t}_{\interpretation} $&$ \CBdsem{\s \piu \t}_{\interpretation} \defeq \CBdsem{\s}_{\interpretation} \piu \CBdsem{\t}_{\interpretation} $ \\
 & & $\CBdsem{\copier{A}} \defeq \copier{\alpha_\sort(A)}$ & $\CBdsem{\discharger{A}} \defeq \discharger{\alpha_\sort(A)}$ & 
% \multicolumn{5}{c}{
%     \begin{tabular}{c@{\qquad\qquad}c}
%         $\CBdsem{\copier{A}} = \copier{\alpha_\sort(A)}$ & $\CBdsem{\discharger{A}} = \discharger{\alpha_\sort(A)}$
%     \end{tabular}
% }
\end{tabular}
\caption{The  morphism of $\algt$-cd rig categories $\CBdsem{-}_\interpretation \colon \CatTapeTCD[\Gamma][\algt] \to \Cat{C}$ induced by  an interpretation $\interpretation = (\alpha_\sort, \alpha_\Gamma)$ of the monoidal signature $(\sort,\Gamma)$ in $\Cat{C}$. This is the compositional semantics of tapes.}
\label{eq:SEMANTICA}
\end{figure}

% \begin{equation}\label{eq:SEMANTICA}
%     \renewcommand{\arraystretch}{1.5}
% \!\!\!\begin{tabular}{l@{\;\;\;\;}l@{\;\;\;\;}l@{\;\;\;\;}l@{\;\;\;\;}l}
% $\CBdsem{s}_{\interpretation} \defeq \alpha_{\Gamma}(s) $& $\CBdsem{\, \tapeFunct{c} \,}_{\interpretation}\defeq \CBdsem{c}_{\interpretation} $ & $\CBdsem{\codiag{U}}_{\interpretation}\defeq \codiag{\alpha^\sharp_\sort(U)} $&$ \CBdsem{\cobang{U}}_{\interpretation} \defeq \cobang{\alpha^\sharp_\sort(U)}$   &  $\CBdsem{\Br{f}_{U}}_{\interpretation} \defeq j(f) \per \id{\alpha^\sharp_\sort(U)}$\\
% $\CBdsem{\id{A}}_{\interpretation}\defeq \id{\alpha_\sort(A)} $&$ \CBdsem{\id{1}}_{\interpretation}\defeq \id{1} $&$ \CBdsem{\symmt{A}{B}}_{\interpretation} \defeq \symmt{\alpha_\sort(A)}{\alpha_\sort(B)}  $&$ \CBdsem{c;d}_{\interpretation} \defeq \CBdsem{c}_{\interpretation}; \CBdsem{d}_{\interpretation}  $ & $ \CBdsem{c\per d}_{\interpretation} \defeq \CBdsem{c}_{\interpretation} \per \CBdsem{d}_{\interpretation}$\\
% $\CBdsem{\id{U}}_{\interpretation}\defeq \id{\alpha^\sharp_\sort(U)} $&$ \CBdsem{\id{\zero}}_{\interpretation} \defeq \id{\zero}  $&$ \CBdsem{\symmp{U}{V}}_{\interpretation}\defeq \symmp{\alpha^\sharp_\sort(U)}{\alpha^\sharp_\sort(V)} $&$ \CBdsem{\s;\t}_{\interpretation} \defeq \CBdsem{\s}_{\interpretation} ; \CBdsem{\t}_{\interpretation} $&$ \CBdsem{\s \piu \t}_{\interpretation} \defeq \CBdsem{\s}_{\interpretation} \piu \CBdsem{\t}_{\interpretation} $ \\
%  & & $\CBdsem{\copier{A}} \defeq \copier{\alpha_\sort(A)}$ & $\CBdsem{\discharger{A}} \defeq \discharger{\alpha_\sort(A)}$ & 
% % \multicolumn{5}{c}{
% %     \begin{tabular}{c@{\qquad\qquad}c}
% %         $\CBdsem{\copier{A}} = \copier{\alpha_\sort(A)}$ & $\CBdsem{\discharger{A}} = \discharger{\alpha_\sort(A)}$
% %     \end{tabular}
% % }
% \end{tabular}
% \end{equation}
% In particular, note that the definition of $\CBdsem{-}_\interpretation$ in the proof of Theorem~\ref{thm:free signametape} can be extended so that $\CBdsem{\copier{A}} = \copier{\alpha_\sort(A)}$. Moreover, any other morphism of $\algt$-cd rig categories $\beta \colon \CatTapeTCD[\Gamma][\algt] \to \Cat{C}$ must preserve the copy-discard structure, ensuring the uniqueness of $\CBdsem{-}_\interpretation$.  

\begin{comment}
\bigskip

MACRO CIRCUITI

\[ \CBcopier \mid \CBdischarger \mid \Andgate \mid \Orgate \mid \Notgate \mid \Flip{0} \mid \Flip{1} \mid \CBcocopier \]

\[ \CBcopier[t] \mid \CBdischarger[t] \mid \Andgate[t] \mid \Orgate[t] \mid \Notgate[t] \mid \Flip{0}[t] \mid \Flip{1}[t] \mid \CBcocopier[t] \]


The signature $\sort = \{ A\}$, $\Gamma = \{ \Andgate , \Orgate , \Notgate , \Flip{0} , \Flip{1} , \CBcocopier \}$

\[
\begin{array}{rclrclrcl}
\alpha_{\Gamma}(\Andgate)\colon 2 \times 2& \to & 2 & \alpha_{\Gamma}(\Orgate)\colon 2 \times 2& \to & 2 & \alpha_{\Gamma}(\Notgate)\colon  2& \to & 2 \\
(x,y)&\mapsto&\delta_{x\wedge y} & (x,y)&\mapsto&\delta_{x\vee y} & x & \mapsto & \delta_{\neg x}
\end{array}
\]
\end{comment}
%
%
%
%
%
%
\begin{example}[Probabilistic Boolean circuits]\label{example: probabilistic control}
%  Probabilistic boolean circuits are boolean circuits interpreted in the Kleisli category of the finitary subdistribution monad, \(\Sets_{\subdistr}\).
 Consider a monoidal signature with a single sort, $\sort = \{ A\}$, and  generators $\Gamma = \{ \Andgate , \Orgate , \Notgate , \Flip{0} , \Flip{1}, \CBcocopier \}$. All generators have coarity $A$, while their arities are determined by the the number of ports on the left: for instance $\Andgate$ has arity $AA$, while $\Flip{0}$ has arity $1$. Intuitively, the first five generators represent operations and constants of boolean algebras ($\wedge$, $\vee$, $\neg$, $0$ and $1$); the last generator takes in input two signals on the left and, if they are equal, it outputs the same signal on the right. 
 
To make this formal we define an interpretation $\interpretation$ of $(\sort, \Gamma)$ into \(\Sets_{\subdistr}\).
The sort \(A\) is interpreted as the set of booleans, \(\alpha_{\sort}(A) = 2\), and the generators as the following arrows of $\Sets_{\subdistr}$.
  \[
    \begin{array}{rclrclrcl}
      \alpha_{\Gamma}(\Andgate)\colon 2 \times 2& \to & 2 & \alpha_{\Gamma}(\Orgate)\colon 2 \times 2& \to & 2 & \alpha_{\Gamma}(\Notgate)\colon  2& \to & 2 \\
      (x,y)&\mapsto&\delta_{x\wedge y} & (x,y)&\mapsto&\delta_{x\vee y} & x & \mapsto & \delta_{\neg x}\\[4pt]
      \alpha_{\Gamma}(\Flip{0}) \colon 1 & \to & 2 & \alpha_{\Gamma}(\Flip{1}) \colon 1 & \to & 2 & \alpha_{\Gamma}(\CBcocopier) \colon 2 \times 2 & \to & 2 \\
      \bullet &\mapsto&\delta_{0} & \bullet &\mapsto&\delta_{1} & (x,x) &\mapsto&\delta_{x}
    \end{array}
  \]
Observe that $\CBcocopier$ denotes an arrow in  \(\Sets_{\subdistr}\) that is not total, while all the remaining generators are total. Moreover, \emph{all} generators denote \emph{deterministic} arrows  in \(\Sets_{\subdistr}\). 

To add probabilistic behaviours, one can consider tape diagrams for $\mathbb{PCA}$-cd categories, where $\mathbb{PCA}$ is the algebraic theory in \Cref{ex:algebraic-theory-convex}. Indeed since  \(\Sets_{\subdistr}\) is a $\mathbb{PCA}$-cd category (Proposition~\ref{prop:kleisliTrig}), then by Theorem~\ref{th:tapes-free-T-cd}, the interpretation $\interpretation$ induces a morphism $\CBdsem{-}_\interpretation \colon \CatTapeTCD[\Gamma][\mathbb{PCA}] \to \Sets_{\subdistr}$ defined as in Figure~\ref{eq:SEMANTICA}. % \marginpar{INSERT REFERENCE}
For example, $\CBdsem{-}_\interpretation$ assigns to  the following tape on the left
\begin{equation}\label{eq:exprobabilistictapes}
        \tikzfig{tapes/examples/ANDpOR} \qquad \qquad \tikzfig{tapes/examples/1p0}
% \text{INSERT TAPE }1+_p 0\text{ ---- INSERT TAPE }AND +_p OR 
\end{equation}
the arrow $2 \times 2 \to 2$ of \(\Sets_{\subdistr}\) which maps any pair of booleans $(x,y)$ into $x\wedge y$ with probability $p$ and $x \vee y$ with probability $(1-p)$.
The tape on the right is mapped by $\CBdsem{-}_\interpretation$ into the arrow $1 \to 2$ assigning to $\bullet$ the distribution $1 \mapsto p$, $0 \mapsto (1-p)$. By denoting this tape with $ \Flip{p}[t]$, one can easily see that there is a straightforward encoding of the diagrammatic calculus in \cite{piedeleu2025boolean} into $\CatTapeTCD[\Gamma][\mathbb{PCA}]$. %preserving the semantics. \marginpar{Maybe we can say a few more things in the Appendix?}

While a more detailed comparison with \cite{piedeleu2025boolean} is left for future work, we conclude by highlighting that the use of tapes enables a natural implementation of probabilistic control, as illustrated in the leftmost diagram of \eqref{eq:exprobabilistictapes}. In \cite{piedeleu2025boolean}, control is achieved through the probabilistic multiplexer, which is represented by the tape $\Ifgate[t][A] \defeq \tikzfig{tapes/examples/multiplex}$.


Intuitively, when $ \Flip{p}[t]$, $\Tcirc{c}{\!\!\!\!}{\!\!\!\!}$ and $\Tcirc{d}{\!\!\!\!}{\!\!\!\!}$ are plugged, respectively, into the first, second and third wire of the multiplexer, the output will match that of $c$ with probability \( p \) and the one of $d$ with probability \( 1 - p \).
% Intuitively, when $ \Flip{p}[t]$ is plugged into the first wire of the multiplexer, the output will match the second wire with probability \( p \) and the third wire with probability \( 1 - p \).
%
The full picture is given by the term $(\;\Flip{p}[t] \;\per \Tcirc{c}{\!\!\!\!}{\!\!\!\!} \per \Tcirc{d}{\!\!\!\!}{\!\!\!\!}) ; \scalebox{0.7}{\Ifgate[t]}$ which, by definition of $\Flip{p}[t]$ in~\eqref{eq:exprobabilistictapes} and $\per$ in~Table~\ref{tab:producttape}, is the tape on the left below. %\marginpar{Cambiare il disegno di destra come si e detto}
\begin{equation*}%\label{eq:multi vs pchoice}
    \tikzfig{tapes/examples/multiplexT} \qquad \qquad \tikzfig{tapes/examples/pchoice}
\end{equation*}
The two diagrams above exhibit similar behavior. However, there is an important difference when  \( d \) (or similarly \( c \)) is \tikzfig{tapes/examples/failure}\!\!\!  denoting the null subdistribution, intuitively representing failure. The circuit on the left always fails (Lemma 4.4 in \cite{piedeleu2025boolean}); instead, the output of the circuit on the right 
matches the output of $c$ (or $d$) with probability $p$ (or $1-p$). 

Since multiplying ($\per$) by a null behaviour always results in a null behaviour, we believe that issues similar to the one of the multiplexer are unavoidable when having only the monoidal product $\per$. The additional use of $\piu$ provides, in our opinion, a valuable representation of control.



%The two diagrams above exhibit similar behavior. However, there is an important difference when either \( c \) or \( d \) is the circuit that always fails, i.e., \tikzfig{tapes/examples/failure}\!\!\!. If a branch of the multiplexer (above, left) always fails, then the entire circuit fails as well (Lemma 4.4 in \cite{piedeleu2025boolean}), even if that branch is never evaluated.  
%
%In contrast, if a branch of the probabilistic choice (above, right) always fails, it does not necessarily cause the entire circuit to fail.
%
%The presence of two monoidal structures, as well as the possibility to represent operations of an algebraic theory in tape diagrams, crucially, allow us to capture both behvariours. \marginpar{concludere meglio qua.}

% The two diagrams above exhibit similar behavior. However, there is a subtle difference when either \( c \) or \( d \) is the circuit that always fails, i.e., \tikzfig{tapes/examples/failure}\!\!\!. In particular, if a branch of the multiplexer always fails, then the whole circuit always fails (Lemma 4.4 in \cite{piedeleu2025boolean}), even when this branch is never evaluated.
%   On the other hand, a branch of the probabilistic choice that always fails does not make the whole circuit fail.
\end{example}


\begin{comment}

OLD STUFF

We have seen in Section~\ref{sec:monoidal} that string diagrams provide a convenient graphical language for strict monoidal categories.
In this section, we recall tape diagrams, a sound and complete graphical formalism for sesquistrict rig categories introduced in~\cite{bonchi2023deconstructing}.


The construction of tape diagrams goes through the adjunction in~\eqref{eq:adjunction}, where $\CAT$ is the category  of categories and functors, $\SMC$ is the category 
 of ssm categories and functors, and $\FBC$ is the category of strict finite biproduct categories and their morphisms. 
\begin{equation}\label{eq:adjunction} \begin{tikzcd}
		\SMC \ar[r,"U_1"] & \CAT \ar[r,bend left,"F_2"] \ar[r,draw=none,"\bot"description] & \FBC \ar[l,bend left,"U_2"]
\end{tikzcd}
\end{equation}
The functors $U_1$ and $U_2$ are the obvious forgetful functors. The functor $F_2$ is the left adjoint to $U_2$, and can be described as follows.

\begin{definition}\label{def:strict fb freely generated by C}
Let $\Cat{C}$ be a category. The  strict fb category freely generated by $\Cat{C}$, hereafter denoted by $F_2(\Cat{C})$, has as objects words of objects of $\Cat{C}$. Arrows are terms inductively generated by the following grammar, where $A,B$ and $c$ range over arbitrary objects and arrows of $\Cat{C}$,\begin{equation}
    \begin{array}{rcl}
        f & ::=& \; \id{A} \; \mid \; \id{I} \; \mid \; \tapeFunct{c} \; \mid \; \sigma_{A,B}^{\perG} \; \mid \;   f ; f   \; \mid \;  f \perG f  \; \mid \; \bang{A} \; \mid \; \diag{A} \;  \mid \; \cobang{A}\; \mid \; \codiag{A}\\
        \end{array}
\end{equation}  
modulo the axioms in  Tables~\ref{fig:freestricmmoncatax} and~\ref{fig:freestrictfbcat}. Notice in particular the last two from Table~\ref{fig:freestrictfbcat}:
\begin{equation}\label{ax:tape}\tag{Tape}
\tape{\id{A}} = \id{A} \qquad \tape{c;d}= \tape{c} ; \tape{d}
\end{equation}
\end{definition}
The assignment $\Cat{C} \mapsto F_2({\Cat{C}})$ easily extends to functors $H\colon \Cat{C} \to \Cat{D}$.
The unit of the adjunction $\eta \colon Id_{\CAT} \Rightarrow F_2U_2$ is defined for each category $\Cat{C}$ as the functor ${\tapeFunct{\cdot} \; \colon \Cat{C} \to U_2F_2(\Cat{C})}$ which is the identity on objects and maps every arrow $c$ in $\Cat{C}$ into the arrow $\tapeFunct{c}$ of $U_2F_2(\Cat{C})$. Observe that $\tapeFunct{\cdot}$ is indeed a functor, namely an arrow in $\CAT$, thanks to the axioms \eqref{ax:tape}. We will refer hereafter to this functor as the \emph{taping functor}.


% \begin{lemma}\label{lemma:F2 left adjoint to U2}
% $F_2 \colon \CAT \to \FBC$ is left adjoint to $U_2 \colon \FBC \to \CAT$.
% \end{lemma}

\medskip

% \ale{POSSIAMO EVITARE LA SESQUISTRICTNESS(?)}

The sesquistrict fb rig category freely generated by a monoidal signature $\sign$ is $F_2U_1(\CatString)$, hereafter referred to as $\CatTape$, and it is presented as follows.
% This is somehow the fb rig category analogue to Theorem 2.3 in \cite{joyal1991geometry} mentioned in Section~\ref{sec:monoidal}. Let us see why.

Recall that the set of objects of 
$\CatString$ is $\sort^\star$, i.e.\ words of sorts in $\sort$. The set of objects of $\CatTape$ is thus $(\sort^\star)^\star$, namely words of words of sorts in $\sort$. For arrows, consider the following two-layer grammar where $s \in \sign$, $A,B \in \sort$ and $U,V \in \sort^\star$.
\begin{equation}\label{tapesGrammar}
    \begin{tabular}{rc ccccccccccccccccccccc}\setlength{\tabcolsep}{0.0pt}
        $c$  & ::= & $\id{A}$ & $\!\!\! \mid \!\!\!$ & $ \id{\uno} $ & $\!\!\! \mid \!\!\!$ & $ \gen $ & $\!\!\! \mid \!\!\!$ & $ \sigma_{A,B} $ & $\!\!\! \mid \!\!\!$ & $   c ; c   $ & $\!\!\! \mid \!\!\!$ & $  c \per c$ & \multicolumn{8}{c}{\;} \\
        $\t$ & ::= & $\id{U}$ & $\!\!\! \mid \!\!\!$ & $ \id{\zero} $ & $\!\!\! \mid \!\!\!$ & $ \tapeFunct{c} $ & $\!\!\! \mid \!\!\!$ & $ \sigma_{U,V}^{\piu} $ & $\!\!\! \mid \!\!\!$ & $   \t ; \t   $ & $\!\!\! \mid \!\!\!$ & $  \t \piu \t  $ & $\!\!\! \mid \!\!\!$  & $\cobang{U}$ & $\!\!\! \mid \!\!\!$ & $\codiag{U}$ & $\!\!\! \mid \!\!\!$ & $f_U$
    \end{tabular}
\end{equation}  
The terms of the first row, denoted by $c$, are called \emph{circuits}. Modulo the axioms in Table~\ref{fig:freestricmmoncatax} (after replacing $\perG$ with $\per$), these are exactly the arrows of $\CatString$.
The terms of the second row, denoted by $\t$, are called \emph{tapes}. Modulo the axioms in Tables \ref{fig:freestricmmoncatax} and \ref{fig:freestrictfbcat} (after replacing $\perG$ with $\piu$ and $A,B$ with $U,V$), these are exactly the arrows of $F_2U_1(\CatString)$, i.e.\  $\CatTape$. 

Since circuits are arrows of $\CatString$, these can be graphically represented as string diagrams. Also tapes can be represented as string diagrams, since they satisfy all of the axioms of ssmc. Note however that \emph{inside} tapes, there are string diagrams: this justifies the motto \emph{tape diagrams are string diagrams of string diagrams}.
Two layers grammars can be rendered graphically and formally~\cite{braithwaite2023collages}.
The grammar in~\eqref{tapesGrammar} becomes:
% \begin{equation*}\label{tapesDiagGrammar}
%     \setlength{\tabcolsep}{2pt}
%     \begin{tabular}{rc c@{$\,\mid\,$}c@{$\,\mid\,$}c@{$\,\mid\,$}c@{$\,\mid\,$}c@{$\,\mid\,$}c@{$\,\mid\,$}c@{$\,\mid\,$}c@{$\,\mid\,$}c}
%         $c$  & $\Coloneqq$ &  $\wire{A}$ & $ \tikzfig{empty} $ & $ \Cgen{\gen}{A}{B}  $ & $ \Csymm{A}{B} $ & $ \tikzfig{seq_compC}   $ & $  \tikzfig{par_compC}$ \\
%         $\t$ & $\Coloneqq$ & $\Twire{U}$ & $ \tikzfig{empty} $ & $ \Tcirc{c}{U}{V}  $ & $ \Tsymmp{U}{V} $ & $ \tikzfig{tapes/seq_comp}  $ & $  \tikzfig{tapes/par_comp}$  & $\Tunit{U}$  & $\Tmonoid{U}$ & $\Talgop{U}{f}$
%     \end{tabular}
% \end{equation*}  
\begin{equation*}\label{tapesDiagGrammar}
    \setlength{\tabcolsep}{2pt}
    \begin{tabular}{rc c@{$\,\mid\,$}c@{$\,\mid\,$}c@{$\,\mid\,$}c@{$\,\mid\,$}c@{$\,\mid\,$}c@{$\,\mid\,$}c@{$\,\mid\,$}c@{$\,\mid\,$}c}
        $c$  & $\Coloneqq$ &  $\wire{A}$ & $ \tikzfig{empty} $ & $ \Cgen{\gen}{A}{B}  $& $ \Csymm{A}{B} $ & $ \tikzfig{seq_compC}   $ & $  \tikzfig{par_compC}$ \\
        $\t$ & $\Coloneqq$ & $\Twire{U}$ & $ \tikzfig{empty} $ & $ \Tcirc{c}{U}{V}  $ & $ \Tsymmp{U}{V} $ & $ \tikzfig{tapes/seq_comp}  $ & $  \tikzfig{tapes/par_comp}$ & $\Tunit{U}$  & $\Tmonoid{U}$ & $\Talgop{U}{f_U}$
    \end{tabular}
\end{equation*}  
The identity $\id\zero$ is rendered as the empty tape $\tikzfig{empty}$, while $\id\uno$ is $\tikzfig{tapes/empty}$: a tape filled with the empty circuit. 
For a monomial $U \!=\! A_1\dots A_n$, $\id U$ is depicted as a tape containing  $n$ wires labelled by $A_i$. For instance, $\id{AB}$ is rendered as $\TRwire{A}{B}$. When clear from the context, we will simply represent it as a single wire  $\Twire{U}$ with the appropriate label.
Similarly, for a polynomial $P = \Piu[i=1][n]{U_i}$, $\id{P}$ is obtained as a vertical composition of tapes, as illustrated below on the left. \[ \id{AB \piu \uno \piu C} = \begin{aligned}\begin{gathered} \TRwire{A}{B} \\[-1.5mm] \Twire{\uno} \\[-2mm] \Twire{C} \end{gathered}\end{aligned} \qquad \qquad \tapesymm{AB}{C} = \tikzfig{tapes/examples/tapesymmABxC} \qquad\qquad \symmp{AB \piu \uno}{C} = \tikzfig{tapes/examples/symmpABp1pC} \]
We can render graphically the symmetries $\tapesymm{U}{V} \colon UV \!\to\! VU$ and $\symmp{P}{Q} \colon P \piu Q \!\to\! Q \piu P$ as crossings of wires and crossings of tapes,  see the two rightmost diagrams above.
The diagonal $\diag{U} \colon U \!\to\! U \piu U$ is represented as a splitting of tapes, while the bang $\bang{U} \colon U \!\to\! \zero$ is a tape closed on its right boundary. 
Codiagonals and cobangs are represented in the same way but mirrored along the y-axis. Exploiting the coherence axioms in Figure~\ref{fig:fbcoherence}, we can construct (co)diagonals and (co)bangs for arbitrary polynomials $P$.
For example, $\diag{AB}$, $\bang{CD}$, $\codiag{A\piu B \piu C}$ and $\cobang{AB \piu B \piu C}$ are depicted as:
\[ 
    \diag{AB} = \TLcomonoid{B}{A} \qquad \bang{CD} = \TLcounit{D}{C} \qquad  \codiag{A\piu B \piu C} = \tikzfig{tapes/examples/codiagApBpC} \qquad   \cobang{AB \piu B \piu C} = \tikzfig{tapes/examples/cobangABpBpC} 
\]

When the structure inside a tape is not relevant the graphical language can be ``compressed'' in order to simplify the diagrammatic reasoning. For example, for arbitrary polynomials $P, Q$ we represent $\id{P}, \symmp{P}{Q}, \diag{P}, \bang{P}, \codiag{P}, \cobang{P}$ as follows:
\[ \TPolyWire{P} \qquad \TPolySymmp{P}{Q} \qquad \TPolyDiag{P} \qquad \TPolyCounit{P} \qquad \TPolyCodiag{P} \qquad \TPolyUnit{P} \]
Moreover, for an arbitrary tape diagram $\t \colon P \to Q$ we write $\Tbox{\t}{P}{Q}$.



It is important to observe that the graphical representation takes care of the two axioms in \eqref{ax:tape}: both sides of the leftmost axiom are depicted as $\Twire{A}$ while both sides of the rightmost axiom as
$\tikzfig{tapes/ax/c_poi_d}$. The axioms of monoidal categories are also implicit in the graphical representation, while those for symmetries and the fb-structure (in Table~\ref{fig:freestrictfbcat}) have to be depicted explicitly as in Figure~\ref{fig:tapesax}. In particular, the diagrams in the first row express the inverse law and naturality of $\symmp$. In the second group there are the (co)monoid axioms and in the third group the bialgebra ones. Finally, the last group depicts naturality of the (co)diagonals and (co)bangs. 

\begin{figure}[ht!]
    \mylabel{ax:symmpinv}{$\symmp$-inv}
    \mylabel{ax:symmpnat}{$\symmp$-nat}
    
    \mylabel{ax:codiagas}{$\codiag{}$-as}
    \mylabel{ax:codiagun}{$\codiag{}$-un}
    \mylabel{ax:codiagco}{$\codiag{}$-co}
    
    \mylabel{ax:codiagnat}{$\codiag{}$-nat}
    \mylabel{ax:cobangnat}{$\cobang{}$-nat}

    \mylabel{ax:codiagf}{$\codiag{}$-$f$}
    \mylabel{ax:cobangf}{$\cobang{}$-$f$}
    \mylabel{ax:fnat}{$f$-nat}

    \begin{center}
        \scalebox{0.9}{
            \begin{tabular}{r@{}c@{}l @{\quad} r@{}c@{}l @{\quad} r@{}c@{}l}
                \multicolumn{9}{c}{
                    \begin{tabular}{r@{}c@{}l @{\qquad\qquad} r@{}c@{}l}
                        \tikzfig{tapes/ax/symminv_left} &$\stackrel{(\symmp\text{-inv})}{=}$& \tikzfig{tapes/ax/symminv_right}  
                & 
                \tikzfig{tapes/ax/symmnat_left}  &$\stackrel{(\symmp\text{-nat})}{=}$&  \tikzfig{tapes/ax/symmnat_right}
                    \end{tabular}
                }
                \\
                % \multicolumn{9}{c}{
                %     \begin{tabular}{c@{}c@{}c c@{}c@{}c c@{}c@{}c}
                        \tikzfig{tapes/whiskered_ax/monoid_assoc_left} &$\stackrel{(\codiag{}\text{-as})}{=}$& \tikzfig{tapes/whiskered_ax/monoid_assoc_right}  
                        &
                        \tikzfig{tapes/whiskered_ax/monoid_unit_left} &$\stackrel{(\codiag{}\text{-un})}{=}$& \Twire{U}
                        &
                        \tikzfig{tapes/whiskered_ax/monoid_comm_left} &$\stackrel{(\codiag{}\text{-co})}{=}$& \Tmonoid{U}
                    % \end{tabular}
                % }
                \\
                \multicolumn{3}{c}{
                    \begin{tabular}{r@{}c@{}c}
                        \tikzfig{tapes/ax/monoidnat_left} &$\stackrel{(\codiag{}\text{-nat})}{=}$& \tikzfig{tapes/ax/monoidnat_right}
                        \\       
                        \tikzfig{tapes/ax/unitnat_left}  &$\stackrel{(\cobang{}\text{-nat})}{=}$& \tikzfig{tapes/ax/unitnat_right}
                    \end{tabular}
                }
                &
                \tikzfig{tapes/ax/newax/copyf_left} &$\stackrel{(\codiag{}\text{-}f)}{=}$& \tikzfig{tapes/ax/newax/copyf_right}
                &
                \multicolumn{3}{c}{
                    \begin{tabular}{r@{}c@{}c}
                        \tikzfig{tapes/ax/newax/discf_left} &$\stackrel{(\cobang{}\text{-}f)}{=}$& \tikzfig{tapes/ax/newax/discf_right}       
                        \\
                        \tikzfig{tapes/ax/newax/fcopies_left} &$\stackrel{(f\text{-nat})}{=}$& \tikzfig{tapes/ax/newax/fcopies_right}
                    \end{tabular}
                }
            \end{tabular}
        }
    \end{center}
    \caption{Axioms for tape diagrams}
    \label{fig:tapesax}
\end{figure}

% \begin{figure}[ht!]
%     \mylabel{ax:symmpinv}{$\symmp$-inv}
%     \mylabel{ax:symmpnat}{$\symmp$-nat}
%     \mylabel{ax:diagas}{$\diag{}$-as}
%     \mylabel{ax:diagun}{$\diag{}$-un}
%     \mylabel{ax:diagco}{$\diag{}$-co}
%     \mylabel{ax:codiagas}{$\codiag{}$-as}
%     \mylabel{ax:codiagun}{$\codiag{}$-un}
%     \mylabel{ax:codiagco}{$\codiag{}$-co}
%     \mylabel{ax:bi}{bi}
%     \mylabel{ax:bo}{bo}
%     \mylabel{ax:diagbi}{$\diag{}$-bi}
%     \mylabel{ax:codiagbi}{$\codiag{}$-bi}
%     \mylabel{ax:diagnat}{$\diag{}$-nat}
%     \mylabel{ax:bangnat}{$\bang{}$-nat}
%     \mylabel{ax:codiagnat}{$\codiag{}$-nat}
%     \mylabel{ax:cobangnat}{$\cobang{}$-nat}
%     \begin{center}
%         \scalebox{0.9}{
%     \begin{tabular}{C{1px} C{2.3cm} c C{2.5cm} C{5px} C{2.5cm} c C{2.3cm} C{1px}}
%         &\tikzfig{tapes/ax/symminv_left} &$\stackrel{(\symmp\text{-inv})}{=}$& \tikzfig{tapes/ax/symminv_right}  && \tikzfig{tapes/ax/symmnat_left}  &$\stackrel{(\symmp\text{-nat})}{=}$&  \tikzfig{tapes/ax/symmnat_right} & \\
% \hline
% &\tikzfig{tapes/whiskered_ax/comonoid_assoc_left}  &$\stackrel{(\diag{}\text{-as})}{=}$&  \tikzfig{tapes/whiskered_ax/comonoid_assoc_right} && \tikzfig{tapes/whiskered_ax/monoid_assoc_left} &$\stackrel{(\codiag{}\text{-as})}{=}$& \tikzfig{tapes/whiskered_ax/monoid_assoc_right} & \\
%         &\tikzfig{tapes/whiskered_ax/comonoid_unit_left} &$\stackrel{(\diag{}\text{-un})}{=}$& \Twire{U} && \tikzfig{tapes/whiskered_ax/monoid_unit_left} &$\stackrel{(\codiag{}\text{-un})}{=}$& \Twire{U} & \\
%         &\tikzfig{tapes/whiskered_ax/comonoid_comm_left} &$\stackrel{(\diag{}\text{-co})}{=}$& \Tcomonoid{U} && \tikzfig{tapes/whiskered_ax/monoid_comm_left} &$\stackrel{(\codiag{}\text{-co})}{=}$& \Tmonoid{U} &\\[-0.5ex]
% \hline
%         \\[-2.2ex]
%         &\tikzfig{tapes/whiskered_ax/bialg1_left} &$\stackrel{(\text{bi})}{=}$& \tikzfig{tapes/whiskered_ax/bialg1_right} && \tikzfig{tapes/whiskered_ax/bialg2_left}  &$\stackrel{(\text{bo})}{=}$&  \tikzfig{empty} & \\[-1ex]
%         &\tikzfig{tapes/whiskered_ax/bialg3_left}  &$\stackrel{(\diag{}\text{-bi})}{=}$&  \tikzfig{tapes/whiskered_ax/bialg3_right} && \tikzfig{tapes/whiskered_ax/bialg4_left}  &$\stackrel{(\codiag{}\text{-bi})}{=}$&  \tikzfig{tapes/whiskered_ax/bialg4_right} & \\
% \hline
%         \\
%         &\tikzfig{tapes/ax/comonoidnat_left} &$\stackrel{(\diag{}\text{-nat})}{=}$& \tikzfig{tapes/ax/comonoidnat_right} && \tikzfig{tapes/ax/monoidnat_left} &$\stackrel{(\codiag{}\text{-nat})}{=}$& \tikzfig{tapes/ax/monoidnat_right} & \\[-1ex]
%         &\tikzfig{tapes/ax/counitnat_left}  &$\stackrel{(\bang{}\text{-nat})}{=}$& \tikzfig{tapes/ax/counitnat_right} && \tikzfig{tapes/ax/unitnat_left}  &$\stackrel{(\cobang{}\text{-nat})}{=}$& \tikzfig{tapes/ax/unitnat_right} &
%     \end{tabular}}
%     \end{center}
%     \caption{Axioms for tape diagrams}
%     \label{fig:tapesax}
% \end{figure}


\begin{theorem}\label{thm:Tapes is free sesquistrict generated by sigma}
	$\CatTape$ is the free sesquistrict fb rig category generated by the monoidal signature $(\sort, \sign)$.
\end{theorem}
The proof~\cite{bonchi2023deconstructing} of the above theorem mostly consists in illustrating that $\CatTape$ carries the structure of a rig category: $\per$ is defined on objects as in \eqref{def:productPolynomials}; the definition of symmetries for $\per$ and left distributors is given inductively in Table \ref{table:def dl symmt}; the definition of  $\per$ on tapes relies on the definition of \emph{left and right whiskerings}: see Table \ref{tab:producttape}. We will come back to whiskerings in Section \ref{ssec:tracerig}. For the time being, the reader can have a concrete grasp by means of the following example borrowed from \cite{bonchi2023deconstructing}.

\begin{example}\label{ex:diagPer}
    %The graphical representation of $\per$ follows from its definition. Indeed, it is enough to render the diagrams for the two polynomial whiskerings and compose them together in sequence. For example, 
    Consider $\t\colon U\piu V \to W\piu Z$ and $\s\colon U'\piu V' \to W'\piu Z'$ illustrated below on the left. Then $\t \per \s$ is simply the sequential composition of $\LW{U\piu V}{\s}$ and $\RW{W' \piu Z'}{\t}$:
    \[  \tikzfig{tapes/examples/t1} \per \tikzfig{tapes/examples/t2} = \tikzfig{tapes/examples/t1xt2_line} \]
    The dashed line highlights the boundary between left and right polynomial whiskerings: $\LW{U \piu V}{\s}$, on the left, is simply the vertical composition of the monomial whiskerings $\LW{U}{\s}$ and $\LW{V}{\s}$ while, on the right, $\RW{W' \piu Z'}{\t}$ is rendered as the vertical composition of $\RW{W'}{\t}$ and $\RW{Z'}{\t}$, precomposed and postcomposed with left distributors.
\end{example}

\begin{table}[ht!]
    \begin{center}
    % \tiny{
        % \hfill
        \begin{subtable}{0.60\textwidth}
            \begin{tabular}{l}
                \toprule
                $\dl{P}{Q}{R} \colon P \per (Q\piu R)  \to (P \per Q) \piu (P\per R) \vphantom{\symmt{P}{Q}}$ \\
                \midrule
                $\dl{\zero}{Q}{R} \defeq \id{\zero} \vphantom{\symmt{P}{\zero} \defeq \id{\zero}}$ \\
                $\dl{U \piu P'}{Q}{R} \defeq (\id{U\per (Q \piu R)} \piu \dl{P'}{Q}{R});(\id{U\per Q} \piu \symmp{U\per R}{P'\per Q} \piu \id{P'\per R}) \vphantom{\symmt{P}{V \piu Q'} \defeq \dl{P}{V}{Q'} ; (\Piu[i]{\tapesymm{U_i}{V}} \piu \symmt{P}{Q'})}$ \\
                \bottomrule
            \end{tabular}
            \caption{}
            \label{table:def dl}
        \end{subtable}
        \;
        \begin{subtable}{0.35\textwidth}
            \begin{tabular}{l}
                \toprule
                $\symmt{P}{Q} \colon P\per Q \to Q \per P$, with $P = \Piu[i]{U_i}$ \\
                \midrule
                $\symmt{P}{\zero} \defeq \id{\zero}$ \\
                $\symmt{P}{V \piu Q'} \defeq \dl{P}{V}{Q'} ; (\Piu[i]{\tapesymm{U_i}{V}} \piu \symmt{P}{Q'})$ \\
                \bottomrule
            \end{tabular}
            \caption{}
            \label{table:def symmt}
        \end{subtable}
        % \hfill
        \caption{Inductive definition of $\delta^l$ and $\symmt$}
        \label{table:def dl symmt}
    % }
    \end{center}
\end{table}

\begin{table}[ht!]
    \begin{center}
    {
        \hfill
  \[\begin{array}{c}
        \def\arraystretch{1.2}
        \begin{array}{rcl|rcl}
            \toprule
            \LW U {\id\zero} &\defeq& \id\zero& \RW U {\id\zero} &\defeq& \id\zero \\
            % \LW U {\id\uno} &\defeq& \id U& \RW U {\id\uno} &\defeq& \id U \\
            % \LW U {\id V} &\defeq& \id {UV}& \RW U {\id V} &\defeq& \id {VU} \\
            % \LW U {\tape{\gen}} &\defeq& \tape{\id U \per \gen}& \RW U {\tape{\gen}} &\defeq& \tape{\gen \per \id U} \\
            \LW U {\tape{c}} &\defeq& \tape{\id U \per c}& \RW U {\tape{c}} &\defeq& \tape{c \per \id U} \\
            % &\LW U {\symmt{V}{W}} &\defeq& \symmp{UV}{UW}& \RW U {\symmt{V}{W}} &\defeq& \symmp{VU}{WU} \\
            % \LW U {\tapesymm{V}{W}} &\defeq& \tapesymm{UV}{UW}& \RW U {\tapesymm{V}{W}} &\defeq& \tapesymm{VU}{WU} \\
            \LW U {\symmp{V}{W}} &\defeq& \symmp{UV}{UW}& \RW U {\symmp{V}{W}} &\defeq& \symmp{VU}{WU} \\
            % \LW U {\diag V} &\defeq& \diag{UV}& \RW U {\diag V} &\defeq& \diag{VU} \\
            % \LW U {\bang V} &\defeq& \bang{UV}& \RW U {\bang V} &\defeq& \bang{VU} \\
            \LW U {\codiag V} &\defeq& \codiag{UV}& \RW U {\codiag V} &\defeq& \codiag{VU} \\
            \LW U {\cobang V} &\defeq& \cobang{UV}& \RW U {\cobang V} &\defeq& \cobang{VU} \\
            \LW U {f_V} &\defeq& f_{UV} & \RW U {f_V} &\defeq& f_{VU} \\
            \LW U {\t_1 ; \t_2} &\defeq& \LW U {\t_1} ; \LW U {\t_2}& \RW U {\t_1 ; \t_2} &\defeq& \RW U {\t_1} ; \RW U {\t_2} \\
            \LW U {\t_1 \piu \t_2} &\defeq& \LW U {\t_1} \piu \LW U {\t_2}& \RW U {\t_1 \piu \t_2} &\defeq& \RW U {\t_1} \piu \RW U {\t_2} \\
            \hline \hline
            \LW{\zero}{\t} &\defeq& \id{\zero} & \RW{\zero}{\t} &\defeq& \id{\zero} \\
            \LW{W\piu S'}{\t} &\defeq& \LW{W}{\t} \piu \LW{S'}{\t} & \RW{W \piu S'}{\t} &\defeq& \dl{P}{W}{S'} ; (\RW{W}{\t} \piu \RW{S'}{\t}) ; \Idl{Q}{W}{S'} \\
            \hline \hline
            \multicolumn{6}{c}{
                \t_1 \per \t_2 \defeq \LW{P}{\t_2} ; \RW{S}{\t_1}   \quad \text{ ( for }\t_1 \colon P \to Q, \t_2 \colon R \to S   \text{ )}
            }
            \\
            \bottomrule
        \end{array}
    \end{array}        
      \]
      \hfill
      \caption{Inductive definition of left and right monomial whiskerings (top); inductive definition of polynomial whiskerings (center); definition of $\per$ (bottom).}\label{tab:producttape}
       }
    \end{center}
\end{table}


CONTINUE LIKE THIS



\begin{theorem}
 BLA BLA is the sesqui-strict freely generated $(\Sigma,E)$-rig category
\end{theorem}

This result generalizes the one in \cite{bonchi2023deconstructing} when taking $(\Sigma,E)$ to be the theory of commutative monoids.

\end{comment}


==> oldsections/sections/tapes.tex <==

\section{Tape Diagrams with Uniform Traces}\label{sec:tapes}
In this section we introduce tape diagrams for rig categories with finite biproducts and uniform traces. 
The approach is similar to the one in Section~\ref{sc:tape} and it goes through the following adjunction.

% \begin{proposition}
%     $\CatTrTape$ is a $\sort$-sesquistrict ut-fb rig category.
% \end{proposition}
% \begin{proof}
%     The proof of the analogous result for plain, non-traced, tape diagrams, i.e. Theorem 5.10 in~\cite{bonchi2023deconstructing}, relies on several inductive proofs that must be extended to include the additional inductive case $\trace_{S}\t$ in~\eqref{tracedTapesGrammar}.
% \end{proof}

% \begin{theorem}
%     There is an isomorphism of $\sort$-sesquistrict ut-fb rig categories $\UTr(\CatTape) \cong \CatTrTape$.
% \end{theorem}

\begin{equation}\label{eq:adjunction-utfb}
    \begin{tikzcd}
        \SMC \ar[r,"U_1"] &
        \CAT
        \arrow[r, "F_3"{name=F}, bend left] &
        \FBUTr
        \arrow[l, "U_3"{name=U}, bend left]
        \arrow[phantom, from=F, to=U, "\vdash" rotate=90]
    \end{tikzcd}
\end{equation}

The functors $U_1$ and $U_3$ are the obvious forgetful functors. The functor $F_3$ is the left adjoint to $U_3$ and can be described as follows.


\begin{definition}\label{def:strict ut-fb freely generated by C}
Let $\Cat{C}$ be a category. The  strict ut-fb category freely generated by $\Cat{C}$, hereafter denoted by $F_3(\Cat{C})$, has as objects words of objects of $\Cat{C}$. Arrows are terms inductively generated by the following grammar, where $A,B$ and $c$ range over arbitrary objects and arrows of $\Cat{C}$,
    \begin{equation}
        \begin{array}{rcl}
            f & ::=& \; \id{A} \; \mid \; \id{I} \; \mid \; \tapeFunct{c} \; \mid \; \sigma_{A,B}^{\perG} \; \mid \;   f ; f   \; \mid \;  f \perG f  \; \mid \; \bang{A} \; \mid \; \diag{A} \;  \mid \; \cobang{A}\; \mid \; \codiag{A} \; \mid \; \trace_{A} f\\
            \end{array}
    \end{equation}  
    modulo the axioms in  Tables~\ref{fig:freestricmmoncatax},~\ref{fig:freestrictfbcat},~\ref{tab:trace-axioms} and~\ref{tab:uniformity}. %\marginpar{Modulo the axioms, for uniformity we should be clearer, maybe before}
\end{definition}

Similarly to~\eqref{eq:adjunction}, the unit of the adjunction $\eta \colon Id_{\CAT} \Rightarrow F_3U_3$ is defined for each category $\Cat{C}$ as the identity-on-objects functor $G \colon \Cat{C} \to U_3F_3(\Cat{C})$ that maps each arrow $c$ in $\Cat{C}$ into the arrow $\tapeFunct{c}$ of $U_3 F_3(\Cat{C})$.

\begin{lemma}\label{lemma:tr-adj}
    $F_3 \colon \CAT \to \FBUTr$ is left adjoint to $U_3 \colon \FBUTr \to \CAT$.
\end{lemma}

Recall from Section \ref{sec:monoidal} the category of string diagrams $\CatString$ generated by a monoidal signature $\sign$. Hereafter, we focus on  $F_3U_1(\CatString)$, referred to as $\CatTrTape$.
The set of objects of $\CatTrTape$ is the same of $\CatTape$, i.e., words of words of sorts in $\sort$. For arrows, we extend the two-layer grammar in~\eqref{tapesGrammar} with one production accounting for the trace operation.
\begin{equation}\label{tracedTapesGrammar}
    \begin{tabular}{rc ccccccccccccccccccccc}\setlength{\tabcolsep}{0.0pt}
        $c$  & ::= & $\id{A}$ & $\!\!\! \mid \!\!\!$ & $ \id{\uno} $ & $\!\!\! \mid \!\!\!$ & $ \gen $ & $\!\!\! \mid \!\!\!$ & $ \sigma_{A,B} $ & $\!\!\! \mid \!\!\!$ & $   c ; c   $ & $\!\!\! \mid \!\!\!$ & $  c \per c$ & \multicolumn{8}{c}{\;} \\
        $\t$ & ::= & $\id{U}$ & $\!\!\! \mid \!\!\!$ & $ \id{\zero} $ & $\!\!\! \mid \!\!\!$ & $ \tapeFunct{c} $ & $\!\!\! \mid \!\!\!$ & $ \sigma_{U,V}^{\piu} $ & $\!\!\! \mid \!\!\!$ & $   \t ; \t   $ & $\!\!\! \mid \!\!\!$ & $  \t \piu \t  $ & $\!\!\! \mid \!\!\!$ & $ \bang{U} $ & $\!\!\! \mid \!\!\!$ & $\diag{U}$ & $\!\!\! \mid \!\!\!$ & $\cobang{U}$ & $\!\!\! \mid \!\!\!$ & $\codiag{U}$  &  $\!\!\! \mid \!\!\!$ & $\trace_{U}\t$    
    \end{tabular}
\end{equation}  

The terms of the first row are taken modulo the axioms in Table~\ref{fig:freestricmmoncatax} (after replacing $\perG$ with $\per$).
The terms of the second row are taken modulo the axioms in Tables \ref{fig:freestricmmoncatax},~\ref{fig:freestrictfbcat},~\ref{tab:trace-axioms} and~\ref{tab:uniformity} (after replacing $\perG$ with $\piu$ and $A,B$ with $U,V$).

As for $\CatTape$, the grammar in \eqref{tracedTapesGrammar} can be rendered diagrammatically as follows.
\begin{equation*}\label{tracedTapesDiagGrammar}
    \setlength{\tabcolsep}{2pt}
    \begin{tabular}{rc cccccccccccc}
        $c$  & ::= &  $\wire{A}$ & $\mid$ & $ \tikzfig{empty} $ & $\mid$ & $ \Cgen{\gen}{A}{B}  $ & $\mid$ & $ \Csymm{A}{B} $ & $\mid$ & $ \tikzfig{seq_compC}   $ & $\mid$ & $  \tikzfig{par_compC}$ & \\
        $\t$ & ::= & $\Twire{U}$ & $\mid$ & $ \tikzfig{empty} $ & $\mid$ & $ \Tcirc{c}{U}{V}  $ & $\mid$ & $ \Tsymmp{U}{V} $ & $\mid$ & $ \tikzfig{tapes/seq_comp}  $ & $\mid$ & $  \tikzfig{tapes/par_comp}$ & $\mid$ \\
             &     & \multicolumn{12}{l}{$\Tcounit{U} \; \mid \; \Tcomonoid{U} \; \mid \; \Tunit{U} \; \mid \; \Tmonoid{U} \; \mid \; \TTraceMon{\t}[U][P][Q]$}
    \end{tabular}
\end{equation*} 

%%% COMMENTED VERSION PITH GENERIC PRODUCT
\begin{comment}
\begin{table}
\[\begin{array}{ccc}
\begin{array}{rcl}
 \bang{\unoG} & \defeq & \id{\unoG}  \\ 
 \bang{A \perG P} & \defeq & \bang{A} \perG \bang{P}  \\ 
\end{array}
&
\begin{array}{rcl}
\diag{\unoG} & \defeq &  \id{\unoG}  \\ 
\diag{A \perG P} & \defeq & (\diag{A} \perG \diag{P}) ; (\id{A} \perG \symm{A}{P} \perG \id{P})\\ 
\end{array}
\\ \\
\begin{array}{rcl}
 \cobang{\unoG} & \defeq & \id{\unoG}  \\ 
 \cobang{A \perG P} & \defeq & \cobang{A} \perG \cobang{P}  \\ 
\end{array}
&
\begin{array}{rcl}
\codiag{\unoG} & \defeq &  \id{\unoG}  \\ 
\codiag{A \perG P} & \defeq & (\id{A} \perG \symm{A}{P} \perG \id{P}) ; (\codiag{A} \perG \codiag{P}) \\ 
\end{array}
&
\begin{array}{rcl}
\trace_{\unoG}(\t) & \defeq & \t \\
\trace_{A \perG P}(\t) & \defeq & \trace_{P} \trace_A (\t) 
\end{array}
\end{array}\]
\caption{Inductive definitions of $\bang{P}$, $\diag{P}$, $\cobang{P}$,  $\codiag{P}$ and  $\trace_{P}\t$ for all words $P$}
\end{table}
\end{comment}

\begin{table}
\[\begin{array}{ccc}
\begin{array}{rcl}
 \bang{\zero} & \defeq & \id{\zero}  \\ 
 \bang{U \piu P} & \defeq & \bang{U} \piu \bang{P}  \\ 
\end{array}
&
\begin{array}{rcl}
\diag{\zero} & \defeq &  \id{\zero}  \\ 
\diag{U \piu P} & \defeq & (\diag{U} \piu \diag{P}) ; (\id{U} \piu \symm{U}{P} \piu \id{P})\\ 
\end{array}
\\ \\
\begin{array}{rcl}
 \cobang{\zero} & \defeq & \id{\zero}  \\ 
 \cobang{U \piu P} & \defeq & \cobang{U} \piu \cobang{P}  \\ 
\end{array}
&
\begin{array}{rcl}
\codiag{\zero} & \defeq &  \id{\zero}  \\ 
\codiag{U \piu P} & \defeq & (\id{U} \piu \symm{U}{P} \piu \id{P}) ; (\codiag{U} \piu \codiag{P}) \\ 
\end{array}
&
\begin{array}{rcl}
\trace_{\zero}(\t) & \defeq & \t \\
\trace_{U \piu P}(\t) & \defeq & \trace_{P} \trace_U (\t) 
\end{array}
\end{array}\]
\caption{Inductive definitions of $\bang{P}$, $\diag{P}$, $\cobang{P}$,  $\codiag{P}$ and  $\trace_{P}\t$ for all polynomial $P$}\label{tab:inddefutfb}
\end{table}


\begin{figure}[h!]
    \mylabel{ax:trace:tape:sliding}{sliding}
    \centering
    \[
        \begin{array}{c@{}c@{}c @{\quad} c@{}c@{}c}
            \tikzfig{traceTapeAx/tight/lhs} &\stackrel{\text{(tightening)}}{=}& \tikzfig{traceTapeAx/tight/rhs}
            &
            \tikzfig{traceTapeAx/strength/lhs} &\stackrel{\text{(strength)}}{=}& \tikzfig{traceTapeAx/strength/rhs}
            \\[20pt]
            \tikzfig{traceTapeAx/join/lhs} &\stackrel{\text{(joining)}}{=}& \tikzfig{traceTapeAx/join/rhs}
            &
            \tikzfig{traceTapeAx/vanish/lhs} &\stackrel{\text{(vanishing)}}{=}& \tikzfig{traceTapeAx/vanish/rhs}
            \\[40pt]
            \tikzfig{traceTapeAx/slide/lhs} &\stackrel{\text{(sliding)}}{=}& \tikzfig{traceTapeAx/slide/rhs}
            &
            \tikzfig{traceTapeAx/yank/lhs} &\stackrel{\text{(yanking)}}{=}& \tikzfig{traceTapeAx/yank/rhs}
            \\[20pt]
            \multicolumn{6}{c}{
                \tikzfig{traceTapeAx/uniformity/lhs} = \tikzfig{traceTapeAx/uniformity/rhs} \stackrel{(\text{uniformity})}{\implies} \tikzfig{traceTapeAx/uniformity/TR_lhs} = \tikzfig{traceTapeAx/uniformity/TR_rhs}
            }
          \end{array}
    \]
    \caption{Uniform trace axioms in tape diagrams.}
    \label{fig:trace-axiom-tapes}
\end{figure}

%\marginpar{Alessandro puoi fare una versione grafica tape degli assiomi delle tracce?}

%\ale{DIRE COME SI FA $\trace_{S} \t$ ?}

Observe that (co)monoids and traces are defined for arbitrary monomials $U$, but not for all polynomials $P$. They can easily be defined inductively by means of the coherence axioms for (co)monoids and joining and vanishing for traces: see  
Table \ref{tab:inddefutfb}.


%\ale{AGGIUSTARE E FINIRE QUESTI DUE}
%\begin{lemma}\label{lemma:ut-fb-iso}
%    $\CatTrTape$ and $\UTr(\CatTape)$ are isomorphic as ut-fb categories.
%\end{lemma}
In the same way in which $\CatTape$ is the free $\sort$-sesquistrict fb rig category, $\CatTrTape$ is the free uniformly traced one.
\begin{theorem}\label{thm:freeut-fb}
$\CatTrTape$ is the free sesquistrict ut-fb rig category generated by the monoidal signature $(\sort, \sign)$.
\end{theorem}
One can prove the above theorem by extending the inductive definitions of whiskerings for tapes in Table \ref{tab:producttape} with the cases for traces given in Table \ref{tab:wisktraces} and then extends the proof of \Cref{thm:Tapes is free sesquistrict generated by sigma} by considering this additional inductive case. Hereafter we illustrate a more modular proof that allows to reuse Theorem \ref{thm:Tapes is free sesquistrict generated by sigma} and the free uniform state construction discussed in Section \ref{sec:traced}.

\begin{table}
    \begin{center}
    % \tiny{
        \hfill
  \[ \begin{array}{rcl|rcl}
    \LW U {\trace_V \t } &\defeq& \trace_{UV}{ \LW{U}{\t}} & \RW U {\trace_V \t} &\defeq& \trace_{VU}{\RW{U}\t} \\
    \end{array} 
     \]
      \hfill
      \caption{Extension of the definition of left and right whiskerings in Table \ref{tab:producttape} with the case of trace}\label{tab:wisktraces}
    %    }
    \end{center}
\end{table}


\subsection{Proof of Theorem \ref{thm:freeut-fb}}


The adjunction in \eqref{eq:adjunction-utfb} can be decomposed in the following two adjunctions, where the leftmost is the one in~\eqref{eq:adjunction} and the rightmost is the one given by Corollary \ref{cor:free-uniform-trace-fb}.

\begin{equation}
    \begin{tikzcd}
        \SMC \ar[r,"U_1"] &
        \CAT
        \arrow[r, "F_2"{name=F}, bend left] &
        \FBC
        \arrow[r, "\UTr"{name=H}, bend left] 
        \arrow[l, "U_2"{name=U}, bend left]
        \arrow[phantom, from=F, to=U, "\vdash" rotate=90]&
        \FBUTr
        \arrow[l, "U"{name=G}, bend left]
        \arrow[phantom, from=H, to=G, "\vdash" rotate=90]
    \end{tikzcd}
\end{equation}

\begin{proposition}\label{prop:iso}
For all categories $\Cat{C}$, $\UTr F_2 (\Cat{C})$ and $F_3 (\Cat{C})$ are isomorphic as ut-fb-categories.
\end{proposition}
\begin{proof}
Observe that $U U_2 = U_3$. Since adjoints compose, then $\UTr F_2$ is left-adjoint to $U_3$. By uniqueness of adjoints, $\UTr F_2 (\Cat{C})$ is isomorphic to $F_3 (\Cat{C})$.
\end{proof}
\begin{corollary}
 $\CatTrTape$ and $\UTr(\CatTape)$ are isomorphic as ut-fb categories.
\end{corollary}

The above result suggests that to prove that $\CatTrTape$ is the free sesquistrict ut-fb rig category, one could rather prove that $\UTr(\CatTape)$ is the free one. This can be easily achieved by relying on Theorem \ref{thm:Tapes is free sesquistrict generated by sigma} and Proposition \ref{prop:free-uniform-trace-fb-rig}.

\begin{proposition}\label{prop:tracedtacesutfb}
$\UTr(\CatTape)$ is a $\sort$-sesquistrict ut-fb rig category.
\end{proposition}
\begin{proof}
By Proposition \ref{prop:free-uniform-trace-fb-rig}, $\UTr(\CatTape)$ is a ut-fb rig category. One only needs to show that the inclusion  functor $\sort \to \UTr(\CatTape)$ makes $\UTr(\CatTape)$ a $\sort$-sesquistrict rig category according to Definition \ref{def:sesquistrict rig category}. This means that we have to show that for all $A\in \sort$, $\dl{A}{Q}{R}=  \id{(A\per Q)\piu (A\per R)}$. The latter equivalence holds in $\CatTape$ (see e.g. the end of the proof of Theorem 5.10 in \cite{bonchi2023deconstructing}) and thus it also holds in $\UTr(\CatTape)$. %\marginpar{maybe we should have said before what is $\dl{P}{Q}{R}$ in $\UTr(-)$.}
%    It follows from sesquistrictness of $\CatTape$ and the fact that the left distributor in $\UTr(\CatTape)$ is essentially $\delta^l$ in $\CatTape$.
\end{proof}

\begin{theorem}\label{thm:uniformfree}
    $\UTr(\CatTape)$ is the free sesquistrict ut-fb rig category generated by the monoidal signature $(\sort, \sign)$.
\end{theorem}
\begin{proof}
The obvious interpretation of  $(\sign, \sort)$ into $\UTr(\CatTape)$ is $(\id{\sort}, \tape{\cdot} ; \eta)$ where $\eta$ is the unit of the adjunction provided by Proposition \ref{prop:free-uniform-trace-fb-rig} mapping any tape $\t$ in $\CatTape$ into $\St{\t}{\zero}$.

Now, suppose that $M \to D$ is a $\sort$-sesquistrict ut-fb rig category with an interpretation $(\alpha_\sort, \alpha_\sign)$. 

Since $D$ is, in particular, a fb rig category then by Theorem \ref{thm:Tapes is free sesquistrict generated by sigma}, there exists an $\sort$-sesqustrict fb rig functor $(\alpha,\beta)$ with $\alpha\colon \sort \to M$ and $\beta \colon \CatTape \to D$ such that
\begin{equation}\label{eq:one}
\id{\sort}; \alpha = \alpha_\sort \qquad \text{ and } \qquad \tape{\cdot} ; \beta = \alpha_\sign\text{.}
\end{equation}
Since $D$ is a ut-fb rig category, by the adjunction in Proposition \ref{prop:free-uniform-trace-fb-rig}, there exists a unique ut-fb rig functor $\beta^\sharp \colon \UTr(\CatTape) \to D$ such that 
\begin{equation}\label{eq:two}
\eta ; \beta^\sharp = \beta
\end{equation}
From \eqref{eq:one} and \eqref{eq:two}, it immediately follows that $\tape{\cdot}; \eta ; \beta^\sharp = \tape{\cdot}; \beta = \alpha_\sign$. In summary, we have a sesquistrict ut-fb rig functor
$(\alpha\colon \sort \to M, \beta^\sharp \colon \UTr(\CatTape) \to D)$ such that 
\begin{equation}%\label{eq:one}
\id{\sort}; \alpha = \alpha_\sort \qquad \text{ and } \qquad \tape{\cdot} ; \eta ; \beta^\sharp = \alpha_\sign\text{.}
\end{equation}
\end{proof}

%To conclude the proof of Theorem \ref{thm:freeut-fb} one has just to show that 

Thanks to the isomorphism in Proposition \ref{prop:iso}, $\CatTrTape$ inherits the rig structures from $\UTr(\CatTape)$.
Let $H \colon \UTr(\CatTape) \to \CatTrTape$ and $K \colon \CatTrTape \to \UTr(\CatTape)$  be the functors witnessing the isomorphism. Then, one can define $\per$, distributors and symmetries on $\CatTrTape$ as follows:
\begin{equation}\label{eq:rigstruct}
        \t_1 \per \t_2 \defeq H(K(\t_1) \per K(\t_2)) \qquad \dl{P}{Q}{R} \defeq H(\dl{K(P)}{K(Q)}{K(R)} \mid \zero ) \qquad \symmt{P}{Q} \defeq H(\symmt{K(P)}{K(Q)}\mid \zero )
\end{equation}
The above definitions make $\CatTrTape$ and $\UTr(\CatTape)$ isomorphic as ut-fb rig categories. By Theorem \ref{thm:uniformfree}, it follows that  $\CatTrTape$ is the free sesquistrict ut-fb rig category.

\begin{remark}
Observe that the rig structure of $\CatTrTape$ in \eqref{eq:rigstruct} is defined differently than using the whiskerings in Tables \ref{tab:producttape} and \ref{tab:wisktraces} and symmetries and distributors in Table \ref{table:def dl symmt}. 
Since the definition in \eqref{eq:rigstruct} passes through the isomorphism, it is a bit unhandy. The reader can safely use those in Tables \ref{table:def dl symmt}, \ref{tab:producttape} and \ref{tab:wisktraces}, since the two constructions coincide: see Appendix \ref{app:rigtrTape} for a detailed proof.
\end{remark}


==> oldsections/sections/traced.tex <==


\section{Uniformity in Traced Monoidal Categories}\label{sec:traced}
Tape diagrams add expressivity to languages of monoidal categories: the results in \cite{bonchi2023deconstructing} extend languages of quantum circuits \cite{coecke2011interacting} to express control gates, and provide a complete axiomatisation for the positive fragment of the calculus of relations \cite{tarski1941calculus,DBLP:conf/stacs/Pous18}.
Their expressivity, however, does not allow one to deal with the so called Kleene star, namely, the reflexive and transitive closure, that is often used to give semantics to while loops in imperative programming languages. To overcome this problem, we propose in this work to extend tape diagrams with \emph{traces} \cite{joyal1996traced}.

It turns out that the laws of traced monoidal categories are not sufficient to reuse the construction of tapes from \cite{bonchi2023deconstructing}, but one needs an additional condition on traces that is known as \emph{uniformity} \cite{cuazuanescu1994feedback}. In this section we recall uniformly traced monoidal categories and several adjunctions that will be crucial in the next section to introduce tape diagrams with traces. For the sake of brevity, hereafter all monoidal categories and functors are implicitly assumed to be symmetric and strict.




%\marginpar{Please replace everywhere \(\Cat{B}\) by $\Cat{C}$}
\begin{definition}\label{def:traced-category}
A  monoidal category $(\Cat{C}, \perG, \unoG)$  is \emph{traced} if it is endowed with an operator \(\trace_{S} \colon \Cat{C}(S \perG X, S \perG Y) \to \Cat{C}(X,Y)\), for all objects \(S\), \(X\) and \(Y\) of \(\Cat{C}\), that satisfies the axioms in \Cref{tab:trace-axioms} for all suitably typed \(f\), \(g\), \(u\) and \(v\).
 A \emph{morphism of traced  monoidal categories} is a  monoidal functor \(\fun{F} \colon \Cat{B} \to \Cat{C}\) 
  % from a \(\Cat{S}\)-uniformly traced monoidal category \(\Cat{C}\) to a \(\Cat{T}\)-uniformly traced monoidal category \(\Cat{C}\)
  %between uniformly traced monoidal categories, \(\Cat{C}\) and \(\Cat{C}\),
  %is a monoidal functor between the underlying monoidal categories 
  that preserves the trace, namely \(\fun{F}(\trace_{S}f) = \trace_{\fun{F}S}(\fun{F}f)\). We write $\TSMC$ for the category of traced monoidal categories and their morphisms.
\end{definition}

  \begin{table}[h!]
    \centering
    \mylabel{ax:trace:tightening}{tightening}
    \mylabel{ax:trace:strength}{strength}
    \mylabel{ax:trace:joining}{joining}
    \mylabel{ax:trace:vanishing}{vanishing}
    \mylabel{ax:trace:yanking}{yanking}
    \mylabel{ax:trace:sliding}{sliding}
    \begin{tabular}{l r}
      \toprule
      \(\trace_{S}((\id{} \perG u) \dcomp f \dcomp (\id{} \perG v)) = u \dcomp \trace_{S}f \dcomp v\) & (\ref*{ax:trace:tightening}) \\
      \(\trace_{S}(f \perG g) = \trace_{S}f \perG g\) & (\ref*{ax:trace:strength})\\
      \(\trace_{T} \trace_{S} f = \trace_{S \perG T} f\) & (\ref*{ax:trace:joining})\\
      \(\trace_{\unoG} f = f\) & (\ref*{ax:trace:vanishing})\\
      \(\trace_{T}(f \dcomp (u \perG \id{})) = \trace_{S}((u \perG \id{}) \dcomp f)\) & (\ref*{ax:trace:sliding})\\
      \(\trace_{S} \sigma^\perG_{S,S} = \id{S}\)& (\ref*{ax:trace:yanking})\\
      \bottomrule
    \end{tabular}
    \caption{Trace axioms.}\label{tab:trace-axioms}
  \end{table}
  
  String diagrams can be extended to deal with traces~\cite{joyal1996traced} (see e.g., \cite{selinger2010survey} for a survey). For a morphism $f\colon S \perG X \to S \perG Y$, we draw its trace as %\marginpar{Please Alessandro insert the drawing}
  \[ 
    \begin{tikzpicture}
      \begin{pgfonlayer}{nodelayer}
        \node [style=label] (105) at (-2.75, -0.625) {$X$};
        \node [style=none] (117) at (-2.25, -0.625) {};
        \node [style=none] (118) at (-1.75, 0.625) {};
        \node [style=label] (120) at (2.75, -0.625) {$Y$};
        \node [style=none] (125) at (2.25, -0.625) {};
        \node [style=none] (126) at (1.75, 0.625) {};
        \node [style=stringlongbox] (128) at (0, 0) {$f$};
        \node [style=none] (129) at (-1.75, 2.125) {};
        \node [style=none] (130) at (1.75, 2.125) {};
        \node [style=label] (131) at (-1.25, 1.125) {$S$};
        \node [style=label] (132) at (1.25, 1.125) {$S$};
      \end{pgfonlayer}
      \begin{pgfonlayer}{edgelayer}
        \draw (125.center) to (117.center);
        \draw (118.center) to (126.center);
        \draw (130.center) to (129.center);
        \draw [bend right=90, looseness=1.50] (129.center) to (118.center);
        \draw [bend left=90, looseness=1.50] (130.center) to (126.center);
      \end{pgfonlayer}
    \end{tikzpicture}.     
  \]
  Using this convention, the axioms in Table \ref{tab:trace-axioms} acquire a more intuitive flavour: see  \Cref{fig:trace-axioms}.
  
  
  
  \begin{figure}[h!]
    \centering
    % \includegraphics{figures/axioms-trace.pdf}
    \[
      \begin{array}{c@{}c@{}c @{\qquad} c@{}c@{}c}
        \tikzfig{traceAx/tight/lhs} &\stackrel{\text{(tightening)}}{=}& \tikzfig{traceAx/tight/rhs}
        &
        \tikzfig{traceAx/strength/lhs} &\stackrel{\text{(strength)}}{=}& \tikzfig{traceAx/strength/rhs}
        \\[20pt]
        \tikzfig{traceAx/join/lhs} &\stackrel{\text{(joining)}}{=}& \tikzfig{traceAx/join/rhs}
        &
        \tikzfig{traceAx/vanish/lhs} &\stackrel{\text{(vanishing)}}{=}& \tikzfig{traceAx/vanish/rhs}
        \\[20pt]
        \tikzfig{traceAx/slide/lhs} &\stackrel{\text{(sliding)}}{=}& \tikzfig{traceAx/slide/rhs}
        &
        \tikzfig{traceAx/yank/lhs} &\stackrel{\text{(yanking)}}{=}& \tikzfig{traceAx/yank/rhs}
      \end{array}
    \]
    \caption{Trace axioms in string diagrams.\label{fig:trace-axioms}}
  \end{figure}


To extend tape diagrams with traces we need to require the trace to be uniform. This constraint, that arises from technical necessity, turns out to be the key to recover the axiomatisation of Kleene algebras in Section \ref{sec:kleene}, the induction proof principle in Section \ref{sec:peano} and the proof rules for while loops in Hoare logic in Section \ref{sec:hoare}.


\begin{definition}\label{def:utr-category}
  A traced monoidal category \(\Cat{C}\)
  % with a distinguished monoidal subcategory \(\Cat{S}\) of \emph{strict} morphisms is \(\Cat{S}\)-
  is \emph{uniformly traced} if the trace operator satisfies the implication in \Cref{tab:uniformity} for all suitably typed \(f\), \(g\) and \(r\). A \emph{morphism of uniformly traced monoidal categories} is simply a morphism of traced monoidal categories. The category of uniformly traced monoidal categories and their morphisms is denoted by  \(\UTSMC\).
  \begin{table}[h!]
    \centering
    \mylabel{ax:trace:uniformity}{uniformity}
    \begin{tabular}{l r}
      \toprule
      if \(f \dcomp (r \perG \id{}) = (r \perG \id{}) \dcomp g\), then \(\trace_{S} f = \trace_{T} g\) & (\ref*{ax:trace:uniformity})\\
      \bottomrule
    \end{tabular}
    \caption{Uniformity axiom.}\label{tab:uniformity}
  \end{table}
\end{definition}

With string diagrams, the uniformity axiom is drawn as in Figure \ref{fig:uniformity}.
  \begin{figure}[h!]
    \centering
    % \includegraphics{figures/uniformity-trace.pdf}
    \[
    \begin{array}{c}
      \tikzfig{traceAx/uniformity/lhs} = \tikzfig{traceAx/uniformity/rhs} \stackrel{(\text{uniformity})}{\implies} \tikzfig{traceAx/uniformity/TR_lhs} = \tikzfig{traceAx/uniformity/TR_rhs}
    \end{array}
    \]
    \caption{Uniformity axiom in string diagrams.\label{fig:uniformity}}
  \end{figure}


\begin{remark}[Uniformity and sliding]\label{rem:uniformity-sliding}
 % % Consider an \(\Cat{S}\)-uniformly traced monoidal category \(\Cat{C}\).
 % % Suppose that all morphisms of \(\Cat{C}\) can be written as the trace of a strict morphism: for all \(u \colon S \to T\) there exist a strict \(r \colon R \perG S \to R \perG T\) such that \(u = \trace_{R} r\).
  The sliding axiom is redundant as it follows from uniformity: 
    \[ \tikzfig{ufu} = \tikzfig{ufu} \implies \tikzfig{traceAx/slide/lhs} = \tikzfig{traceAx/slide/rhs} \]
  %% We could apply uniformity to \(\id{} \perG r\) because strict morphisms are necessarily closed under monoidal products and isomorphisms, and identities in particular, are always strict~\cite{hasegawa1997models}.
 This fact will be useful for constructing the uniformly traced monoidal category freely generated by a monoidal category \(\Cat{C}\).
\end{remark}


\subsection{The Two Traced Monoidal Structures of $\Rel$}\label{sec:2trREL}
Recall from Section \ref{sec:2monREL} that the category of sets and relations $\Rel$ has two different monoidal structures:  $(\Rel, \per, \uno)$, intuitively representing data flow, and $(\Rel, \piu, \zero)$ representing control flow.
Since \cite{bainbridge1976feedback} (see also \cite{selinger1998note}), it is known that both monoidal categories are traced. For a relation $R\colon S \per X \to S \per Y$, its trace $\trace_{S}(R)$ in $(\Rel, \per, \uno)$ is defined as 
\[\trace_{S}(R) \defeq \{(x,y) \mid \exists s\in S. \; (\, (s,x) \,,\, (s,y) \, )\in R\}\subseteq X \times Y\]
To describe the trace in $(\Rel, \piu, \zero)$, we first need to observe that any relation $R\colon S \piu X \to S \piu Y$ can be decomposed as $R=R_{S,S} \cup R_{S,Y} \cup R_{X,S} \cup R_{X,Y}$ where 
\begin{equation}\label{eq:dec}
\begin{array}{rcl}
R_{S,S} &\defeq&\{(s,t)\mid (\,(s,0), (t,0) \,)\in R \} \subseteq S \times S \\ 
R_{S,Y} &\defeq&\{(s,y)\mid (\,(s,0), (y,1) \,)\in R \} \subseteq S \times Y \\ 
R_{X,S} &\defeq&\{(x,t)\mid (\,(x,1), (t,0) \,)\in R \} \subseteq X \times S \\ 
R_{X,Y} &\defeq&\{(x,y)\mid (\,(x,1), (y,1) \,)\in R \} \subseteq X \times Y 
\end{array}
\end{equation}
Then, the trace of $R\colon S \piu X \to S \piu Y$ in $(\Rel, \piu, \zero)$ is given by 
\begin{equation}%\label{eq:relTrace}
  \trace_{S}(R) \defeq ( \, R_{X,S}; (R_{S,S})^\star ; R_{S,Y} \, ) \cup R_{X,Y}
\end{equation}
where, for any relation $T\subseteq S\times S$, $T^\star$ stands for the reflexive and transitive closure of $T$ (see e.g. \cite{joyal1996traced}).
The reader will see in Section \ref{sec:kleene}, that both the decomposition in \eqref{eq:dec} and the formula for the trace  in $(\Rel, \piu, \zero)$ come from its finite biproduct structure. In the same section, it will also become clear that such trace is uniform.
Instead, the trace in $(\Rel, \per, \uno)$ is not uniform: the readers can easily convince themselves by taking $r$ in Table \ref{tab:uniformity} to be the empty relation and observe that, for all arrows $f$ and $g$, the premise of the implication always holds. To properly tackle this kind of issues, in several works (see e.g. \cite{hasegawa2003uniformity}), uniformity is required on a restricted class of morphisms $r$, named \emph{strict} but we will not make similar restrictions here.



\subsection{The Free Uniform Trace}\label{sec:UTConstruction}
We now illustrate a construction that will play a key role in the rest of the paper: from a monoidal category, we freely generate a uniformly traced one.
Our first step consists in showing that, given a traced monoidal category $\Cat{C}$, one can always transform it into a uniformly traced one, named $\Unif(\Cat{C})$.

Let $\basicR$ be a set of pairs $(f, g)$ of arrows of $\Cat{C}$ with the same domain and codomain. We define $\congB$ to be the set generated by the following inference system (where $f \congB g$ is a shorthand for $(f,g)\in \congB$).
\begin{equation}\label{eq:uniformcong}
        \!\!\begin{array}{@{\qquad}c@{\qquad\qquad}c@{\qquad}c@{\qquad}}
            
            \inferrule*[right=($r$)]{-}{f \mathrel{\congB} f}
            &    
            \inferrule*[right=($t$)]{f \mathrel{\congB} g \quad g \mathrel{\congB} h}{f \mathrel{\congB} h}
            &
            \inferrule*[right=($s$)]{f \mathrel{\congB} g}{g \mathrel{\congB} f}
            \\[8pt]
                       \inferrule*[right=($\basicR$)]{f \mathbin{\basicR} g}{f \mathrel{\congB} g}
&
            \inferrule*[right=($;$)]{f \mathrel{\congB} f' \quad g \mathrel{\congB} g'}{f;g \mathrel{\congB} f';g'}
            &
%            \inferrule*[right=($\piu$)]{f \mathrel{\congB} g \quad \s_1 \mathrel{\congB} \s_2}{f\piu\s_1 \mathrel{\congB} g \piu \s_2}
        %    &
            \inferrule*[right=($\perG$)]{f \mathrel{\congB} f' \quad g \mathrel{\congB} g'}{f\perG g \mathrel{\congB} f' \perG g'}
            \\[8pt]
            \multicolumn{3}{c}{
            \inferrule*[right=($ut$)]{u \mathrel{\congB} v \qquad f ; (u \piu \id{}) \mathrel{\congB} (v \piu \id{}) ; g}{\trace_{S}f \mathrel{\congB} \trace_{T}g}
            }
        \end{array}
\end{equation}
Observe that, for all $\basicR$, $\congB$ is an equivalence relation by (r), (t) and (s) and it is closed by composition $;$ and monoidal product $\perG$, thanks to the inference rules ($;$) and ($\perG$). By taking $u$ and $v$ in ($ut$) to be identities, $\congB$ is also closed by $\trace$: if $f\congB g$, then $\trace_{S}f \congB \trace_{S} g$.
%
When $\basicR$ is the empty set $\emptyset$, we just write $\approx$ in place of $\approx_{\emptyset}$. When we want to emphasise the underlying category $\Cat{C}$, we write $\approx_{\Cat{C}}$ in place of $\approx$.

We call $\Unif(\Cat{C})$ the quotient of $\Cat{C}$ by $\approx_{\Cat{C}}$. More explicitly, objects of $\Unif(\Cat{C})$ are the same as those of $\Cat{C}$ and arrows are $\approx_{\Cat{C}}$-equivalence classes $[f]\colon X \to Y$ of arrows $f\colon X\to Y$ in $\Cat{C}$.

\begin{proposition}\label{prop:uniformCat}
For a   traced monoidal category $\Cat{C}$, $\Unif(\Cat{C})$ is a uniformly traced monoidal category.
\end{proposition}
The assignment $\Cat{C} \mapsto \Unif(\Cat{C})$ extends to morphisms of traced monoidal categories: for $F\colon \Cat{B} \to \Cat{C}$, the functor $\Unif(F) \colon \Unif(\Cat{B}) \to \Unif(\Cat{C})$ is defined as
\[\Unif(F)(X)\defeq X \text{ for all objects }X\text{, and } \Unif(F)[f]\defeq [Ff] \text{ for all arrows }[f]\text{.}\]

\begin{lemma}\label{lemma:uniformity-quotient-functor}
  There is a functor \(\Unif \colon \TSMC \to \UTSMC\) defined as above.
\end{lemma}

Recall that $\TSMC$ and $\UTSMC$ are the categories of, respectively, traced monoidal categories and uniformly traced monoidal ones.


%\Cref{lemma:traced-monoidal-functors-preserve-equivalence} is the reason why we take just trace monoidal functors between uniformly traced monoidal categories\\

\begin{proposition}\label{prop:free-uniform}
Let $\fun{U}\colon \UTSMC \to \TSMC$ be the obvious embedding. Then $\Unif$ is left adjoint to $\fun{U}$. %In other words, the following in an adjunction.
  \[\begin{tikzcd}
        \TSMC
        \arrow[r, "\Unif"{name=F}, bend left] &
        \UTSMC
        \arrow[l, "\fun{U}"{name=U}, bend left]
        \arrow[phantom, from=F, to=U, "\vdash" rotate=90]
    \end{tikzcd}\]
\end{proposition}

The next step consists in recalling from~\cite{katis2002feedback} the construction of the free traced monoidal category \(\freeTr (\Cat{C})\) on a symmetric monoidal category \(\Cat{C}\).
 \(\freeTr (\Cat{C})\) has  the same objects as \(\Cat{C}\), and morphisms \((f \mid S) \colon X \to Y\) are pairs of an object \(S\) and a morphism \(f \colon S \perG X \to S \perG Y\) of \(\Cat{C}\).  Morphisms are quotiented by \emph{yanking} and \emph{sliding}. Compositions, monoidal products and trace in \(\freeTr (\Cat{C})\) are recalled below.
  \begin{align}
    \st{f}{S} \dcomp \st{g}{T} &\defeq \st{\CStSeq{f}{S}{X}{g}{T}{Z}}{S \perG T} \label{eq:seq in Utr} \\
    \st{f}{S} \perG \st{g}{T} &\defeq \st{\CStPar{f}{S}{X}{Y}{g}{T}{Z}{W}}{S \perG T} \label{eq:per in Utr} \\
    \trace_T\st{f}{S} &\defeq \st{f}{S \perG T} \label{eq:trace in Utr}
  \end{align}
 The assignment $\Cat{C} \mapsto \freeTr(\Cat{C})$ extends to a functor $\freeTr \colon \SMC \to \TSMC$ which is the left adjoint to the obvious forgetful
 $\fun{U}\colon \TSMC \to \SMC$.
   \begin{equation}\label{eq:nonuniform}
   \begin{tikzcd}
        \SMC
        \arrow[r, "\freeTr"{name=F}, bend left] &
        \TSMC
        \arrow[l, "\fun{U}"{name=U}, bend left]
        \arrow[phantom, from=F, to=U, "\vdash" rotate=90]
    \end{tikzcd}\end{equation}
One can compose the  adjunction above with the one of Proposition \ref{prop:free-uniform}, to obtain the following result where  $\UTr \colon \SMC \to \UTSMC$ is the composition of $\freeTr \colon \SMC \to \TSMC$ with $\Unif \colon \TSMC \to \UTSMC$.

\begin{theorem}\label{th:free-uniform-trace}
Let $\fun{U}\colon \UTSMC \to \SMC$ be the obvious forgetful. Then $\UTr$ is left adjoint to $\fun{U}$:
   \[\begin{tikzcd}
        \SMC
        \arrow[r, "\UTr"{name=F}, bend left] &
        \UTSMC
        \arrow[l, "\fun{U}"{name=U}, bend left]
        \arrow[phantom, from=F, to=U, "\vdash" rotate=90]
    \end{tikzcd}\]
%  There is an adjunction \(\UTr \colon \SMC \leftrightarrows \UTSMC \co{\colon} \fun{U}\), where \(\UTr(\Cat{C})\) gives the free \(\Cat{C}\)-uniformly traced category on a symmetric monoidal category \(\Cat{C}\).
\end{theorem}


Since, by Remark \ref{rem:uniformity-sliding}, uniformity entails sliding, one can conveniently rephrase the construction of the freely generated uniformly traced monoidal category \(\UTr (\Cat{C})\) as follows.

\begin{definition}\label{def:uniform-state-construction}
  For a symmetric monoidal category \(\Cat{C}\), define \(\UTr (\Cat{C})\) with the same objects as \(\Cat{C}\), morphisms \((f \mid S) \colon X \to Y\) are pairs of an object \(S\) and a morphism \(f \colon S \perG X \to S \perG Y\) of \(\Cat{C}\).
  The morphisms are quotiented by the \emph{yanking}  and $\approx_{\Cat{C}}$.
%  posetal two-cells given by uniformity: \((f \mid S) \leq (g \mid T)\) whenever there is \(r \colon S \to T\) in \(\Cat{C}\) such that \(f \dcomp (r \perG \id{Y}) \leq (r \perG \id{X}) \dcomp g\), or there is \(r \colon T \to S\) in \(\Cat{C}\) such that \((r \perG \id{X}) \dcomp f \leq g \dcomp (r \perG \id{Y})\).
\end{definition}






%
%
%
% COMMENTED
%
%
%
\begin{comment}


\subsection{The Free Uniform Trace}\label{sec:UTConstruction}

% we need to keep track of the strict morphisms\\
% to make the free construction work the way we want it\\
% this is the same as what is done in~\cite{effectfulstreams} but adding the yanking axiom

% uniformity does not give an equivalence relation\\
% if \(\trace_{S} f = \trace_{T} g\) by uniformity on \(u \colon S \to T\) and \(\trace_{R} h = \trace_{T} g\) by uniformity on \(v \colon R \to T\), we cannot, in general, show that \(\trace_{S} f = \trace_{R} h\) by uniformity\\
% because we cannot, in general, construct a \(w \colon S \to R\) or \(w \colon R \to S\) that satisfies the assumptions of uniformity\\
% so we need to close by transitivity\\
% and we end up with zig-zags of uniformity witnesses\\
% define n-step uniformity by induction\\

% \begin{definition}\label{def:uniformity-equivalence}
%   Let \(\Cat{C}\) be a traced monoidal category and \(\Cat{S}\) be a monoidal subcategory of \(\Cat{C}\).
%   Let \(f \colon S \perG X \to S \perG Y\) and \(g \colon T \perG X \to T \perG Y\) be two morphisms in \(\Cat{C}\).
%   Their traces are \emph{\(1\)-step uniformity equivalent}, \(\trace_{S} f \unifeq_{1} \trace_{T} g\), if there are morphisms \(h \colon R \perG X \to R \perG Y\), \(u \colon S \to R\) and \(v \colon T \to R\) such that
%   \[f \dcomp (u \perG \id{}) = (u \perG \id{}) \dcomp h \qquad\text{and}\qquad g \dcomp (v \perG \id{}) = (v \perG \id{}) \dcomp h \ .\]
%   By induction, their traces are \emph{\(n+1\)-step uniformity equivalent}, \(\trace_{S} f \unifeq_{n+1} \trace_{T} g\), if there is a morphism \(f' \colon S' \perG X \to S' \perG Y\) such that \(\trace_{S} f \unifeq_{n} \trace_{S'} f'\) and \(\trace_{S'} f' \unifeq_{1} \trace_{T} g\).

%   Uniformity equivalence is the union of all \(n\)-step uniformity equivalences: \(\trace_{S} f \unifeq \trace_{T} g\) if there is a natural number \(n\) that makes them \(n\)-step uniformity equivalent, \(\trace_{S} f \unifeq_{n} \trace_{T} g\).
% \end{definition}

define relations on a traced monoidal category as traced monoidal profunctors\\

\begin{definition}
  A \emph{relation} \(R\) on a traced monoidal category \(\Cat{B}\) is a family of relations \(R(X,Y) \subseteq \Cat{B}(X,Y) \times \Cat{B}(X,Y)\) % that assemble into a traced monoidal profunctor \(R \colon \Cat{B} \nrightarrow \Cat{B}\), i.e.\
  that are closed under compositions and monoidal products with morphisms in \(\Cat{B}\), and are closed under traces:
  \begin{itemize}
    \item if \((f,f') \in R(X,Y)\), \(g \in \Cat{B}(Y,Z)\) and \(h \in \Cat{B}(W,X)\), then \((f \dcomp g, f' \dcomp g) \in R(X,Z)\) and \((h \dcomp f, h \dcomp f') \in R(W,Y)\);
    \item if \((f,f') \in R(X,Y)\) and \(g \in \Cat{B}(W,Z)\), then \((f \perG g, f' \perG g) \in R(X \perG W, Y \perG Z)\) and \((g \perG f, g \perG f') \in R(W \perG X, Z \perG Y)\);
    \item if \((f,f') \in R(S \perG X, S \perG Y)\), then \((\trace_{S}f, \trace_{S}f') \in R(X,Y)\).
  \end{itemize}
  Such a relation is an \emph{equivalence relation} if all its components \(R(X,Y)\) are.
\end{definition}

relations on a traced monoidal category form a lattice with the pointwise inclusion order, unions and intersections\\

\begin{proposition}\label{def:operations-traced-monoidal-relations}
  Let \(R\), \(S\) and \(R_{i}\), for \(i \in J\), be relations on a traced monoidal category \(\Cat{B}\).
  The following operations are well-defined on relations on \(\Cat{B}\).
  \begin{itemize}
    \item \(\op{R}(X,Y) \defeq \op{(R(X,Y))} = \{(f,f') \mid (f',f) \in R(X,Y)\}\);
    \item \((R \cdot S)(X,Y) \defeq (R(X,Y)) \cdot (S(X,Y)) = \{(f,g) \mid \exists \ h \in \Cat{B}(X,Y) (f,h) \in R(X,Y) \land (h,g) \in S(X,Y)\}\);
    \item \((\Union_{i \in J} R_{i})(X,Y) \defeq \Union_{i \in J} R(X,Y)\);
    \item \(\oneUniform(R)(X,Y) \defeq \{(\trace_{S}f, \trace_{T}g) \mid \exists \ (r,s) \in R(S,T) \ : \ (f \dcomp (r \perG \id{Y}), (s \perG \id{X}) \dcomp g) \in R(S \perG X, T \perG Y)\}\).
  \end{itemize}
\end{proposition}
\begin{proof}
  \emph{(opposite)}
  Suppose that \((f,f') \in (\op{R})(X,Y)\), then \((f',f) \in R(X,Y)\).
  Since \(R\) is a relation on \(\Cat{B}\), for a morphism \(g \in \Cat{B}(Y,Z)\), we have that \((f' \dcomp g, f \dcomp g) \in R(X,Z)\).
  This means that \((f \dcomp g,f' \dcomp g) \in (\op{R})(X,Z)\).
  A similar reasoning shows closure under pre-compositions, monoidal products and trace.

  \emph{(relation composition)}
  Suppose that \((f,f') \in (R \cdot S)(X,Y)\), then there is a morphism \(f'' \colon X \to Y\) such that \((f,f'') \in R(X,Y)\) and \((f'',f') \in S(X,Y)\).
  Since both \(R\) and \(S\) are relations on \(\Cat{B}\), for a morphism \(g \in \Cat{B}(Y,Z)\), we have that \((f \dcomp g, f'' \dcomp g) \in R(X,Z)\) and \((f'' \dcomp g, f' \dcomp g) \in S(X,Z)\).
  This means that \((f \dcomp g,f' \dcomp g) \in (R \dcomp S)(X,Z)\).
  A similar reasoning shows closure under pre-compositions, monoidal products and trace.


  \emph{(union)}
  Suppose that \((f,f') \in (\Union_{i \in J} R_{i})(X,Y)\), then there is an index \(j \in J\) such that \((f,f') \in R_{j}(X,Y)\).
  Since all \(R_{i}\) are relations on \(\Cat{B}\), for a morphism \(g \in \Cat{B}(Y,Z)\), we have that \((f \dcomp g, f' \dcomp g) \in R_{j}(X,Z)\).
  This means that \((f \dcomp g,f' \dcomp g) \in (\Union_{i \in J} R_{i})(X,Z)\).
  A similar reasoning shows closure under pre-compositions, monoidal products and trace.

  \emph{(uniformity)}
  \elena{this part would benefit from string diagrams}
  Suppose that \((f,f') \in \oneUniform(R)(X,Y)\), then there are morphisms \(h \colon S \perG X \to S \perG Y\) and \(h' \colon T \perG X \to T \perG Y\), and \((r,s) \in R(S,T)\) such that \((h \dcomp (r \perG \id{}), (s \perG \id{}) \dcomp h') \in R(S \perG X, T \perG Y)\).
  For a morphism \(g \colon Y \to Z\), \(((h \dcomp (\id{} \perG g)) \dcomp (r \perG \id{}), (s \perG \id{}) \dcomp (h' \dcomp (\id{} \perG g))) = (h \dcomp (r \perG \id{}) \dcomp (\id{} \perG g), (s \perG \id{}) \dcomp h' \dcomp (\id{} \perG g)) \in R(S \perG X, T \perG Z)\).
  Then, \((f \dcomp g, f' \dcomp g) = (\trace_{S}h \dcomp g, \trace_{T}h' \dcomp g) = (\trace_{S}(h \dcomp (\id{} \perG g)), \trace_{T}(h' \dcomp (\id{} \perG g))) \in \oneUniform(R)(X,Z)\).
  The same reasoning shows closure under pre-compositions.

  Now, consider a morphism \(g' \colon X' \to Y'\).
  Then, \(((h \dcomp (r \perG \id{})) \perG g', ((s \perG \id{}) \dcomp h') \perG g') \in R(S \perG X \perG X', T \perG Y \perG Y')\), which implies that \((f \perG g', f' \perG g') = (\trace_{S}h \perG g', \trace_{T}h' \perG g') = (\trace_{S}(h \perG g'), \trace_{T}(h' \perG g')) \in \oneUniform(R)(X \perG X', Y \perG Y')\).

  Finally, consider \((f,f') \in \oneUniform(R)(A \perG X, A \perG Y)\).
  Then, there are morphisms \(h \colon S \perG A \perG X \to S \perG A \perG Y\) and \(h' \colon T \perG A \perG X \to T \perG A \perG Y\), and \((r,s) \in R(S,T)\) such that \((h \dcomp (r \perG \id{}), (s \perG \id{}) \dcomp h') \in R(S \perG A \perG X, T \perG A \perG Y)\).
  Since \(R\) is closed under compositions, also \(((\symm{A}{S} \perG \id{}) \dcomp h \dcomp (\symm{S}{A} \perG \id{}) \dcomp (\id{} \perG r \perG \id{}), (\id{} \perG s \perG \id{}) \dcomp (\symm{A}{T} \perG \id{}) \dcomp h' \dcomp (\symm{T}{A} \perG \id{})) = ((\symm{A}{S} \perG \id{}) \dcomp h \dcomp (r \perG \id{}) \dcomp (\symm{T}{A} \perG \id{}), (\symm{A}{S} \perG \id{}) \dcomp (s \perG \id{}) \dcomp h' \dcomp (\symm{T}{A} \perG \id{})) \in R(A \perG S \perG X, A \perG T \perG Y)\).
  The relation \(R\) is also closed under traces, then \((\trace_{A}((\symm{A}{S} \perG \id{}) \dcomp h \dcomp (\symm{S}{A} \perG \id{}) \dcomp (\id{} \perG r \perG \id{})), \trace_{A}((\id{} \perG s \perG \id{}) \dcomp (\symm{A}{T} \perG \id{}) \dcomp h' \dcomp (\symm{T}{A} \perG \id{}))) = (\trace_{A}((\symm{A}{S} \perG \id{}) \dcomp h \dcomp (\symm{S}{A} \perG \id{})) \dcomp (r \perG \id{}), (s \perG \id{}) \dcomp \trace_{A}((\symm{A}{T} \perG \id{}) \dcomp h' \dcomp (\symm{T}{A} \perG \id{}))) \in R(S \perG X, T \perG Y)\).
  By definition of \(\oneUniform\), we obtain \((\trace_{A}f, \trace_{A}f') = (\trace_{S \perG A} h, \trace_{T \perG A} h') = (\trace_{A \perG S} ((\symm{A}{S} \perG \id{}) \dcomp h \dcomp (\symm{S}{A} \perG \id{})), \trace_{A \perG T} ((\symm{A}{T} \perG \id{}) \dcomp h' \dcomp (\symm{T}{A} \perG \id{}))) \in \oneUniform(R)(X,Y)\).
\end{proof}

define a monotone function\\
take its least fixed point

\begin{proposition}
  For a (small) traced monoidal category \(\Cat{B}\), the set \(\tracedMonRel(\Cat{B})\) of relations on it forms a lattice, where the order is defined pointwise: \(R \subseteq S\) iff \(\forall X,Y \ R(X,Y) \subseteq S(X,Y)\).
  Moreover, the function \(\mathcal{H} \colon \tracedMonRel(\Cat{B}) \to \tracedMonRel(\Cat{B})\), defined in \Cref{eq:fixpoint-uniformity} is monotone.
  \begin{equation}\label{eq:fixpoint-uniformity}
    \mathcal{H}(R) \defeq \id{} \union R \union \op{R} \union (R \cdot R) \union \oneUniform(R)
  \end{equation}
\end{proposition}
\begin{proof}
  Suprema are given by unions, while infima by intersections.
  The intersection of relations on a traced monoidal category is closed under compositions, monoidal products and traces because all its components are.
  The function \(\mathcal{H}\) is monotone because unions, opposite, relation composition and \(\oneUniform\) are all monotone.
\end{proof}

\begin{definition}\label{def:uniformity-equivalence}
  For a traced monoidal category \(\Cat{B}\), the uniformity relation is the least fixed point of \(\mathcal{H}\).
\end{definition}

by Kleene fixed point theorem, this least fixed point is \((\unifeq) \defeq \Union_{n \in \N} \mathcal{H}^{n}(\emptyset)\)\\
when we need to specify the category \(\Cat{B}\) on which we construct the uniformity relation, we use subscripts \((\unifeq_{\Cat{B}})\) and \(\mathcal{H}_{\Cat{B}}\)

\begin{remark}\label{rem:increasing-uniformity-relation}
  note that, for \(m \leq n\), \(\mathcal{H}^{m}(\emptyset) \subseteq \mathcal{H}^{n}(\emptyset)\)\\
  so, if we have \(f \unifeq f'\) and \(g \unifeq g'\), there is \(n \in \N\) such that \((f,f'), (g,g') \in \mathcal{H}^{n}(\emptyset)\)\\
  because we take the max
\end{remark}

\begin{lemma}\label{lemma:uniformity-congruence}
  The uniformity relation in \Cref{def:uniformity-equivalence} is a traced monoidal congruence, i.e.\ it is an equivalence relation and it respects compositions, monoidal products and trace.
\end{lemma}
\begin{proof}
  Let \(\Cat{B}\) be a traced monoidal category.
  By \Cref{def:operations-traced-monoidal-relations}, each \(\mathcal{H}^{n}(\emptyset)\) is a relation on \(\Cat{B}\) and so is their union.
  Let \(f \unifeq f' \unifeq f'' \colon X \to Y\) be three uniformly equivalent morphisms.
  We know that \((f,f) \in \id{} = \mathcal{H}(\emptyset)\).
  Moreover, there are \(m,n \in \N\) such that \((f,f') \in \mathcal{H}^{m}(\emptyset)(X,Y)\) and \((f',f'') \in \mathcal{H}^{n}(\emptyset)(X,Y)\).
  By the definition of \(\mathcal{H}\), \((f',f) \in \mathcal{H}^{m+1}(\emptyset)(X,Y)\) and \((f,f'') \in \mathcal{H}^{\max\{m,n\}}(\emptyset)(X,Y)\).
  Then, \((\unifeq)\) is reflexive, symmetric and transitive.

  Note that, by transitivity, if \(f \unifeq f'\) and \(g \unifeq g'\), then \(f \dcomp g \unifeq f' \dcomp g \unifeq f' \dcomp g'\) and \(f \perG g \unifeq f' \perG g \unifeq f' \perG g'\).
\end{proof}

\begin{definition}\label{def:uniformity-quotient}
  For a traced monoidal category \(\Cat{B}\),
  % and a monoidal subcategory \(\Cat{S}\)
  define a category \(\Unif(\Cat{B})\) by quotienting \(\Cat{B}\) by uniformity equivalence (\Cref{def:uniformity-equivalence}).
%  We write \(\Unif(\Cat{B})\) for the particular case in which the subclass \(\Cat{S}\) is \(\Cat{B}\) itself.
\end{definition}

\begin{lemma}\label{lemma:traced-monoidal-functors-preserve-equivalence}
  Traced monoidal functors preserve uniformity equivalence.
  Explicitly, for a traced monoidal functor \(\fun{F} \colon \Cat{B} \to \Cat{C}\) and two morphisms \(f,g \colon X \to Y\) in \(\Cat{B}\), if \(f \unifeq_{\Cat{B}} g\), then \(\fun{F}(f) \unifeq_{\Cat{C}} \fun{F}(g)\).
\end{lemma}
\begin{proof}
  Let \(\Cat{B}\) and \(\Cat{C}\) be two traced monoidal categories.
  We indicate with \(\mathcal{H}_{\Cat{B}} \colon \tracedMonRel(\Cat{B}) \to \tracedMonRel(\Cat{B})\) and \(\mathcal{H}_{\Cat{C}} \colon \tracedMonRel(\Cat{C}) \to \tracedMonRel(\Cat{C})\) the function defined in \Cref{eq:fixpoint-uniformity} and instantiated in \(\Cat{B}\) and \(\Cat{C}\).
  For two morphisms \(f,g \colon X \to Y\) in \(\Cat{B}\), if \(f \unifeq_{\Cat{B}} g\), then, by definition, there is a natural number \(n \in \N\) such that \((f,g) \in \mathcal{H}_{\Cat{B}}^{n}(\emptyset)\).
  We show by induction on \(n\) that \((\fun{F}(f), \fun{F}(g)) \in \mathcal{H}_{\Cat{C}}^{n}(\emptyset)\).
  If \(n = 0\), the statement is vacuously true as \(\mathcal{H}_{\Cat{B}}^{0}(\emptyset) = \emptyset = \mathcal{H}_{\Cat{C}}^{0}(\emptyset)\).
  Suppose that \((f,g) \in \mathcal{H}_{\Cat{B}}^{n+1}(\emptyset)\).
  By definition of \(\mathcal{H}_{\Cat{B}}\), there are five possibilities: \emph{(i)} \((f,g) \in \id{}\); \emph{(ii)} \((f,g) \in \mathcal{H}_{\Cat{B}}^{n}(\emptyset)\); \emph{(iii)} \((f,g) \in \op{(\mathcal{H}_{\Cat{B}}^{n}(\emptyset))}\); \emph{(iv)} \((f,g) \in (\mathcal{H}_{\Cat{B}}^{n}(\emptyset)) \cdot (\mathcal{H}_{\Cat{B}}^{n}(\emptyset))\); \emph{(v)} \((f,g) \in \oneUniform (\mathcal{H}_{\Cat{B}}^{n}(\emptyset))\).
  We show that, in all these cases, \((\fun{F}(f), \fun{F}(g)) \in \mathcal{H}_{\Cat{C}}^{n+1}(\emptyset)\).

  \emph{(i)} If \((f,g) \in \id{}\), it means that \(f = g\).
  Then, \(\fun{F}(f) = \fun{F}(g)\) and \((\fun{F}(f), \fun{F}(g)) \in \id{} \subseteq \mathcal{H}_{\Cat{C}}^{n+1}(\emptyset)\).

  \emph{(ii)} If \((f,g) \in \mathcal{H}_{\Cat{B}}^{n}(\emptyset)\), then, by induction, \((\fun{F}(f), \fun{F}(g)) \in \mathcal{H}_{\Cat{C}}^{n}(\emptyset) \subseteq \mathcal{H}_{\Cat{C}}^{n+1}(\emptyset)\).

  \emph{(iii)} If \((f,g) \in \op{(\mathcal{H}_{\Cat{B}}^{n}(\emptyset))}\), it means that \((g,f) \in \mathcal{H}_{\Cat{B}}^{n}(\emptyset)\).
  By induction, \((\fun{F}(g),\fun{F}(f)) \in \mathcal{H}_{\Cat{C}}^{n}(\emptyset)\).
  Then, \((\fun{F}(f),\fun{F}(g)) \in \op{(\mathcal{H}_{\Cat{C}}^{n}(\emptyset))} \subseteq \mathcal{H}_{\Cat{C}}^{n+1}(\emptyset)\).

  \emph{(iv)} If \((f,g) \in (\mathcal{H}_{\Cat{B}}^{n}(\emptyset)) \cdot (\mathcal{H}_{\Cat{B}}^{n}(\emptyset))\), it means that there is \(h \colon X \to Y\) such that \((f,h) \in \mathcal{H}_{\Cat{B}}^{n}(\emptyset)\) and \((h,g) \in \mathcal{H}_{\Cat{B}}^{n}(\emptyset)\).
  By induction, \((\fun{F}(f),\fun{F}(h)) \in \mathcal{H}_{\Cat{C}}^{n}(\emptyset)\) and \((\fun{F}(h),\fun{F}(g)) \in \mathcal{H}_{\Cat{C}}^{n}(\emptyset)\).
  Then, \((\fun{F}(f),\fun{F}(g)) \in (\mathcal{H}_{\Cat{C}}^{n}(\emptyset)) \cdot (\mathcal{H}_{\Cat{C}}^{n}(\emptyset)) \subseteq \mathcal{H}_{\Cat{C}}^{n+1}(\emptyset)\).

  \emph{(v)} If \((f,g) \in \oneUniform (\mathcal{H}_{\Cat{B}}^{n}(\emptyset))\), it means that there are \(r,s \colon S \to T\) such that \((r,s) \in \mathcal{H}_{\Cat{B}}^{n}(\emptyset)\) and \((f \dcomp (r \perG \id{}), (s \perG \id{}) \dcomp g) \in \mathcal{H}_{\Cat{B}}^{n}(\emptyset)\).
  By induction, \((\fun{F}(r),\fun{F}(s)) \in \mathcal{H}_{\Cat{C}}^{n}(\emptyset)\) and \((\fun{F}(f \dcomp (r \perG \id{})), \fun{F}((s \perG \id{}) \dcomp g)) \in \mathcal{H}_{\Cat{C}}^{n}(\emptyset)\).
  Then, \((\fun{F}(f) \dcomp (\fun{F}(r) \perG \id{}), (\fun{F}(s) \perG \id{}) \dcomp \fun{F}(g)) \in \mathcal{H}_{\Cat{C}}^{n}(\emptyset)\) and \((\fun{F}(f), \fun{F}(g)) \in \oneUniform (\mathcal{H}_{\Cat{C}}^{n}(\emptyset)) \subseteq \mathcal{H}_{\Cat{C}}^{n+1}(\emptyset)\).
\end{proof}

\Cref{lemma:traced-monoidal-functors-preserve-equivalence} is the reason why we take just trace monoidal functors between uniformly traced monoidal categories\\



\begin{lemma}\label{lemma:uniformity-quotient-functor}
  The uniformity quotient extends to a functor \(\Unif \colon \TSMC \to \UTSMC\).
\end{lemma}
\begin{proof}
  By \Cref{lemma:uniformity-congruence}, the quotient respects the traced monoidal structure, thus \(\Unif(\Cat{B})\) is a traced monoidal category.
  The uniformity axiom holds by construction.
  This gives the action of \(\Unif\) on objects.

  On morphisms, \(\Unif\) assigns to a traced monoidal functor \(\fun{F} \colon \Cat{B} \to \Cat{C}\) the corresponding functor on equivalence classes:
  for \(f \in \Cat{B}(X,Y)\), \(\Unif(\fun{F})([f]) \defeq [\fun{F}(f)]\), where \([h]\) denotes the uniformity equivalence class of \(h\).
  By \Cref{lemma:traced-monoidal-functors-preserve-equivalence}, if \([f] = [g]\), then \([\fun{F}(f)] = [\fun{F}(g)]\), so \(\Unif(\fun{F})\) is well-defined on equivalence classes.
  Finally, \(\Unif(\fun{F})\) inherits the monoidal structure from \(\fun{F}\) and it preserves the trace.
  \[ \Unif(\fun{F})(\trace_{S}[f]) = \Unif(\fun{F})([\trace_{S}f]) = [\fun{F}(\trace_{S}f)] = [\trace_{\fun{F}S}(\fun{F}f)] = \trace_{\fun{F}S}[(\fun{F}f)] = \trace_{\fun{F}S}(\Unif(\fun{F})[f])\]
\end{proof}



\begin{remark}\label{rem:uniformity-quotient-idempotent}
  note that the uniformity quotient is idempotent\\
  if \(\Cat{C}\) is uniformly traced, then \(\mathcal{H}^{n}(\emptyset) = \id{}\) for all \(n > 0\)\\
  this means that uniformity equivalence is the identity relation\\
  and that the uniformity quotient does nothing
\end{remark}

%
%
%



\begin{proposition}\label{prop:free-uniform}
  For a traced monoidal category \(\Cat{B}\),
  % and a monoidal subcategory \(\Cat{S}\),
  the construction of \(\Unif(\Cat{B})\) gives the free uniformly traced monoidal category over \(\Cat{B}\).
  This means that there is an adjunction between traced monoidal categories and uniformly traced monoidal categories:
  \[\begin{tikzcd}
        \TSMC
        \arrow[r, "\Unif"{name=F}, bend left] &
        \UTSMC
        \arrow[l, "\fun{U}"{name=U}, bend left]
        \arrow[phantom, from=F, to=U, "\vdash" rotate=90]
    \end{tikzcd}.\]
\end{proposition}
\begin{proof}
  By \Cref{lemma:uniformity-quotient-functor}, \(\Unif\) is a functor.
  We show that it is a left adjoint by defining the unit of the adjunction and checking the universal property.
  The components of the unit are traced monoidal functors \(\eta_{\Cat{B}} \colon \Cat{B} \to \fun{U}(\Unif(\Cat{B}))\).
  We define them to be identity-on-objects, \(\eta_{\Cat{B}}(X) \defeq X\), and to map a morphism to its uniformity equivalence class \(\eta_{\Cat{B}}(f) \defeq [f]\).
  By \Cref{lemma:uniformity-congruence}, uniformity equivalence classes respect compositions, monoidal products and trace, which makes \(\eta_{\Cat{B}}\) a functor.
  Naturality follows from the definitions of \(\eta\) and \(\Unif\).
  \begin{align*}
    & \fun{U}(\Unif(\fun{F}))(\eta_{\Cat{B}}(X)) && \fun{U}(\Unif(\fun{F}))(\eta_{\Cat{B}}(f)) \\
    & = \fun{U}(\Unif(\fun{F}))(X) &    & = \fun{U}(\Unif(\fun{F}))([f]) \\
    & = \fun{F}(X) &    & = [\fun{F}(f)] \\
    & = \eta_{\Cat{C}}(\fun{F}(X)) &    & = \eta_{\Cat{C}}(\fun{F}(f))
  \end{align*}

  Let \(\fun{G} \colon \Cat{B} \to \fun{U}(\Cat{D})\) be a traced monoidal functor and define \(\hat{\fun{G}} \colon \Unif(\Cat{B}) \to \Cat{C}\) as \(\hat{\fun{G}}(X) \defeq \fun{G}(X)\) and \(\hat{\fun{G}}([f]) \defeq \fun{G}(f)\).
  By \Cref{lemma:traced-monoidal-functors-preserve-equivalence}, if \(f \unifeq g\), then \(\fun{G}(f) \unifeq \fun{G}(g)\).
  Since \(\Cat{C}\) is uniformly traced, by \Cref{rem:uniformity-quotient-idempotent} this shows that \(\fun{G}(f) = \fun{G}(g)\) and that \(\hat{\fun{G}}\) is well-defined.
  Since \(\fun{G}\) is a traced monoidal functor, so is \(\hat{\fun{G}}\).
  Finally, \(\hat{\fun{G}}\) is the only possible functor satisfying \(\fun{U}(\hat{\fun{G}})(\eta_{\Cat{B}}(f)) = \fun{G}(f)\).
\end{proof}

\begin{definition}\label{def:uniform-state-construction}
  For a symmetric monoidal category \(\Cat{B}\), define \(\UTr (\Cat{B})\) with the same objects as \(\Cat{B}\), morphisms \((f \mid S) \colon X \to Y\) are pairs of an object \(S\) and a morphism \(f \colon S \perG X \to S \perG Y\) of \(\Cat{B}\).
  The morphisms are quotiented by the \emph{yanking axiom}, \((\symm{S}{S} \mid S) = (\id{S} \mid \unoG)\), and the \emph{uniformity axiom}, if \((f \mid S) \unifeq (g \mid T)\), then \((f \mid S) = (g \mid T)\).
%  posetal two-cells given by uniformity: \((f \mid S) \leq (g \mid T)\) whenever there is \(r \colon S \to T\) in \(\Cat{B}\) such that \(f \dcomp (r \perG \id{Y}) \leq (r \perG \id{X}) \dcomp g\), or there is \(r \colon T \to S\) in \(\Cat{B}\) such that \((r \perG \id{X}) \dcomp f \leq g \dcomp (r \perG \id{Y})\).
\end{definition}

\begin{proposition}
  For a symmetric monoidal category \(\Cat{B}\), \(\UTr (\Cat{B})\) is a uniformly traced category.
\end{proposition}
\begin{proof}
  We rely on the construction of the free traced monoidal category \(\freeTr (\Cat{B})\) on a monoidal category \(\Cat{B}\)~\cite{katis2002feedback}.
  It has the same morphisms as \(\UTr (\Cat{B})\), they are also quotiented by yanking, but they are quotiented by sliding instead of uniformity.
  Compositions, monoidal products and trace in \(\freeTr (\Cat{B})\) are recalled below.
  \begin{align}
    \st{f}{S} \dcomp \st{g}{T} &\defeq \CStSeq{f}{S}{X}{g}{T}{Z} \label{eq:seq in Utr} \\
    \st{f}{S} \per \st{g}{T} &\defeq \CStPar{f}{S}{X}{Y}{g}{T}{Z}{W} \label{eq:per in Utr} \\
    \trace_T\st{f}{S} &\defeq \st{f}{S \perG T} \label{eq:trace in Utr}
  \end{align}
  By \Cref{prop:free-uniform}, \(\Unif(\freeTr(\Cat{B}))\) is the free uniformly traced monoidal category over \(\freeTr(\Cat{B})\) and it is obtained by quotienting \(\freeTr(\Cat{B})\) by the uniformity axiom.
  By \Cref{rem:uniformity-sliding}, \(\UTr(\Cat{B})\) also satisfies the sliding axiom.
  Thus, \(\UTr(\Cat{B})\) can be equivalently described as the quotient by uniformity of \(\freeTr(\Cat{B})\), i.e.\ \(\Unif(\freeTr(\Cat{B}))\).
\end{proof}

we need to slightly generalise the result in~\cite{katis2002feedback} to take uniformity into account\\

\begin{theorem}\label{th:free-uniform-trace}
  There is an adjunction \(\UTr \colon \SMC \leftrightarrows \UTSMC \co{\colon} \fun{U}\), where \(\UTr(\Cat{B})\) gives the free \(\Cat{B}\)-uniformly traced category on a symmetric monoidal category \(\Cat{B}\).
\end{theorem}
\begin{proof}
  The results in~\cite{katis2002feedback} construct an adjunction \(\freeTr \colon \SMC \leftrightarrows \TSMC \co{\colon} \fun{U}\) that gives the free traced monoidal category over a symmetric monoidal category.
  By \Cref{prop:free-uniform}, there is an adjunction that quotients by uniformity, \(\Unif \colon \TSMC \leftrightarrows \UTSMC \co{\colon} \fun{U}\).
  By composing these two adjunctions, we obtain the desired adjunction.

  The unit and counit of this adjunction are compositions of the units and counits of the smaller adjunctions.
  We describe them explicitly.
  The components of the unit are identity-on-objects symmetric monoidal functors \(\eta_{\Cat{B}} \colon \Cat{B} \to \fun{U}(\UTr(\Cat{B}))\).
  A morphism \(f \colon X \to Y\) in \(\Cat{B}\) is mapped to the uniformity equivalence class of \(f\) with monoidal unit state space, \(\eta_{\Cat{B}}(f) = [(f \mid I)]\).
  The components of the counit are identity-on-objects traced monoidal functors \(\epsilon_{\Cat{C}} \colon \UTr(\fun{U}(\Cat{C})) \to \Cat{C}\).
  A morphism \([(f \mid S)] \colon X \to Y\) in \(\UTr(\fun{U}(\Cat{C}))\) is mapped to the trace of \(f\) on \(S\), \(\epsilon_{\Cat{C}}([(f \mid S)]) = \trace_{S}f\).
\end{proof}
\end{comment}
%
%
%
% END OF COMMENTED
%
%
%





\subsection{The Free Uniform Trace preserves Products, Coproducts and Biproducts}\label{sec:UTConstruction-products}

A very important class of traced monoidal categories are those where the monoidal product is a product, a coproduct or a biproduct (see e.g. \cite{cstef?anescu1987flowchart,cstef?nescu1987flowchartII,esik1980identities}).
Recall that the latter have been introduced in Definition \ref{def:biproduct category}: finite products categories are defined similarly but without the monoids, finite coproducts categories without the comonoids.

\begin{proposition}\label{prop:free-uniform-trace-cartesian}
  The adjunction in \Cref{th:free-uniform-trace} restricts to finite product categories.
  In particular, if \(\Cat{C}\) is a finite product category, then so is \(\UTr(\Cat{C})\).
\end{proposition}
\begin{proof}
  Let \(f \colon X \to Y\) be a morphism in \(\UTr(\Cat{C})\).
  By the definition of \(\UTr\), there is a morphism \(g \colon S \perG X \to S \perG Y\) in \(\Cat{C}\) whose trace is \(f\), \(f = (g \mid S)\).
  By the universal property of products, \(g\) has two components: \(g = \diag{S \perG X} \dcomp (g_{1} \perG g_{2})\).
  The natural comonoid structure \((\diag{},\bang{})\) of \(\Cat{C}\) gives a comonoid structure \(((\diag{} \mid \unoG), (\bang{} \mid \unoG))\) in \(\UTr(\Cat{C})\) via the unit of the adjunction, \(\eta_{\Cat{C}}\).
  We show that this comonoid structure is natural in \(\UTr(\Cat{C})\).
  We can rewrite \(f \dcomp (\bang{Y} \mid \unoG)\) using naturality of \(\bang{Y}\) in \(\Cat{C}\).
  \[
    \tikzfig{traceProd/discard/rewrite/step1} = \tikzfig{traceProd/discard/rewrite/step2} = \tikzfig{traceProd/discard/rewrite/step3} = \tikzfig{traceProd/discard/rewrite/step4}
  \]
  By uniformity, we rewrite the trace of \(g_{1}\).
  \[
    \tikzfig{traceProd/discard/unif/lhs/step1} = \tikzfig{traceProd/discard/unif/lhs/step2} \implies \tikzfig{traceProd/discard/unif/rhs/step1} = \tikzfig{traceProd/discard/unif/rhs/step2} = \tikzfig{traceProd/discard/unif/rhs/step3}
  \]
  This shows that \(f \dcomp (\bang{Y} \mid \unoG) = (\bang{X} \mid \unoG)\), i.e.\ that the counit is natural in \(\UTr(\Cat{C})\).

  Similarly, we can rewrite \(f \dcomp (\diag{Y} \mid \unoG)\) using naturality of \(\diag{Y}\) in \(\Cat{C}\).
  \[ \tikzfig{traceProd/copy/rewrite/step1} = \tikzfig{traceProd/copy/rewrite/step2}  = \tikzfig{traceProd/copy/rewrite/step3} \]
  By uniformity, we rewrite the trace of \(g_{1}\) with the comultiplication maps.
  \[ \tikzfig{traceProd/copy/unif/lhs/step1} = \tikzfig{traceProd/copy/unif/lhs/step2} = \tikzfig{traceProd/copy/unif/lhs/step3} \implies  \tikzfig{traceProd/copy/unif/rhs/step1} = \tikzfig{traceProd/copy/unif/rhs/step2} \]
  Then, \(f \dcomp (\diag{Y} \mid \unoG) = (\diag{X} \mid \unoG) \dcomp (f \times f)\), i.e.\ the comultiplication is also natural in \(\UTr(\Cat{C})\).
  \[ \tikzfig{traceProd/copy/rewrite2/step1} = \tikzfig{traceProd/copy/rewrite/step3} = \tikzfig{traceProd/copy/rewrite2/step2} = \tikzfig{traceProd/copy/rewrite2/step3} = \tikzfig{traceProd/copy/rewrite2/step4} \]
  This shows that \(\UTr(\Cat{C})\) is a finite product category.
  Since a finite product functor is just a symmetric monoidal functor between finite product categories and a traced finite product functor is just a traced monoidal functor between traced finite product categories, the functor \(\UTr \colon \SMC \to \UTSMC\) restricts to a functor \(\UTr \colon \CMC \to \UTCMC\) from finite product categories to uniformly traced finite product categories.
  For the same reason, the unit and counit of the adjunction also restrict.
\end{proof}

\begin{remark}
Note how the above proof exploits the assumption of uniformity. In fact, it might be the case that $\Cat{C}$ has finite products but $\freeTr (\Cat{C})$ does not.
\end{remark}

\begin{definition}\label{def:utfbcategory}
A monoidal category $\Cat{C}$ is a \emph{uniformly traced finite biproduct} category (shortly ut-fb category) if it is uniformly traced and has finite biproducts.
Morphisms of ut-fb categories are monoidal functors that are both morphisms of traced monoidal categories and of finite biproduct categories.
We write $\FBUTr$  for the category of ut-fb categories and their morphisms.
\end{definition}


\begin{corollary}\label{cor:free-uniform-trace-fb}
  The adjunction in \Cref{th:free-uniform-trace} restricts to finite biproduct categories.
  \[\begin{tikzcd}
        \FBC
        \arrow[r, "\UTr"{name=F}, bend left] &
        \FBUTr
        \arrow[l, "\fun{U}"{name=U}, bend left]
        \arrow[phantom, from=F, to=U, "\vdash" rotate=90]
    \end{tikzcd}\]
\end{corollary}





%
%
%
% TRACE AND RIG
%
%
\subsection{The Free Uniform Trace preserves the Rig Structure}\label{ssec:tracerig}



So far, we have illustrated that  $\UTr(\cdot)$ (\Cref{def:uniform-state-construction})  gives the free uniformly traced category over a symmetric monoidal one (Theorem \ref{th:free-uniform-trace}) and that such construction preserves the structure of finite biproduct category (\Cref{cor:free-uniform-trace-fb}). Here, we illustrate that the same construction additionally preserves the structure of rig categories, namely that the adjunction in  Theorem \ref{th:free-uniform-trace} restricts to an adjunction between the categories $\RIG$ and $\RIGUTr$, defined as follows.

\begin{definition}
A \emph{uniformly traced (ut) rig category} is a rig category $(\Cat{C}, \piu, \zero, \per, \uno)$  such that $(\Cat{C}, \piu, \zero)$ is a uniformly traced monoidal category. A \emph{morphism of uniformly traced rig categories} is both a rig functor and a morphisms of uniformly traced categories. We write $\RIGUTr$ for the category of uniformly traced rig categories and their morphisms.
\end{definition}

Our proof exploits the notion of whiskering that, as stated by the following proposition, enjoys useful properties in any rig category.

\begin{proposition}\label{prop:whisk}
    Let $\Cat{C}$ be a rig category, $X$ an object in $\Cat{C}$ and $\fun{L}_X, \fun{R}_X \colon \Cat{C} \to \Cat{C}$ two functors defined on objects as
    $\LW{X}{Y} \defeq X \per Y$ and $\RW{X}{Y} \defeq Y \per X$,
    %$\fun{L}_X \defeq \id{X} \per -$ and $\fun{R}_X \defeq - \per \id{X}$.
    and on arrows $f \colon Y \to Z$ as 
    \[ \LW{X}{f} \defeq \id{X} \per f \qquad \text{ and } \qquad   \RW{X}{f} \defeq f \per \id{X}. \]
    $\fun{L}_X$ and $\fun{R}_X$ are called, respectively, \emph{left} and \emph{right whiskering} and they satisfy the laws in Table~\ref{table:whisk}.
\end{proposition}


\begin{table}[t]
    \centering
    {\begin{tabular}{lc lc}
        \toprule
        \multicolumn{2}{l}{$1. \ \ \LW X {\id{Y}} = \id{X \per Y}$} & $2. \ \ \RW X {\id{Y}} = \id{Y \per X}$ & (\newtag{W1}{eq:whisk:id})\\[0.3em]
        \multicolumn{2}{l}{$1. \ \ \LW{X}{f ; g} = \LW{X}{f} ; \LW{X}{g}$} & $2. \ \ \RW{X}{f ; g} = \RW{X}{f} ; \RW{X}{g}$ & (\newtag{W2}{eq:whisk:funct})\\[0.3em]
        \multicolumn{2}{l}{$1. \ \ \LW{\uno}{f} = f$} & $2. \ \ \RW{\uno}{f} = f$ & (\newtag{W3}{eq:whisk:uno}) \\[0.3em]
        \multicolumn{2}{l}{$1. \ \ \LW{\zero}{f} = \id{\zero}$} & $2. \ \ \RW{\zero}{f} = \id{\zero}$ & (\newtag{W4}{eq:whisk:zero}) \\[0.3em]
        \multicolumn{2}{l}{$1. \ \ \LW{X}{f_1 \piu f_2} = \dl{X}{X_1}{X_2} ; (\LW{X}{f_1} \piu \LW{X}{f_2}) ; \Idl{X}{Y_1}{Y_2}$}  & $2. \ \ \RW{X}{f_1 \piu f_2} = \RW{X}{f_1} \piu \RW{X}{f_2}$ & (\newtag{W5}{eq:whisk:funct piu}) \\[0.3em]
        \multicolumn{2}{l}{$1. \ \ \LW{X \piu Y}{f} = \LW{X}{f} \piu \LW{Y}{f}$}  & $2. \ \ \RW{X \piu Y}{f} = \dl{Z}{X}{Y} ; ( \RW{X}{f} \piu \RW{Y}{f} ) ; \Idl{W}{X}{Y}$ & (\newtag{W6}{eq:whisk:sum}) \\[0.3em]
        \multicolumn{3}{c}{$\LW{X_1}{f_2} ; \RW{Y_2}{f_1} = \RW{X_2}{f_1} ; \LW{Y_1}{f_2}$} & (\newtag{W7}{eq:tape:LexchangeR}) \\[0.3em]
        % $\RW S {\diag{U}} = \diag{US} \qquad \RW S {\codiag{U}} = \codiag{US}$ & (\newtag{W8}{eq:whisk:diag}) &  $\RW S {\bang{U}} = \bang{US} \qquad \RW S {\cobang{U}} = \cobang{US}$ & (\newtag{W9}{eq:whisk:bang}) \\[0.3em]
        $\RW X {\symmp{Y}{Z}} = \symmp{Y \per X}{Z \per X}$ & (\newtag{W8}{eq:whisk:symmp}) & $\symmt{X \per Y}{Z} = \LW{X}{ \symmt{Y}{Z}} ; \RW{Y}{\symmt{X}{Z}}$ & (\newtag{W9}{eq:symmper}) \\[0.3em]
        $\RW{X}{f} ; \symmt{Z}{X} = \symmt{Y}{X} ; \LW{X}{f}$ & (\newtag{W10}{eq:LRnatsym}) & $\LW{X}{\RW{Y}{f}} = \RW{Y}{\LW{X}{f}}$ & (\newtag{W11}{eq:tape:LR}) \\[0.3em]
        $\LW{X \per Y}{f} = \LW{X}{\LW{Y}{f}}$ & (\newtag{W12}{eq:tape:LL}) & $\RW{Y \per X}{f} = \RW{X}{\RW{Y}{f}}$ & (\newtag{W13}{eq:tape:RR}) \\[0.3em]
        $\RW X {\dl{Y}{Z}{W}} = \dl{Y}{Z \per X}{W \per X}$ & (\newtag{W14}{eq:whisk:dl}) & $\LW X {\dl{Y}{Z}{W}} = \dl{X \per Y}{Z}{W} ; \Idl{X}{Y \per Z}{Y \per W}$ & (\newtag{W15}{eq:whisk:Ldl}) \\
        \bottomrule
    \end{tabular}}
    \caption{The algebra of whiskerings}  
    \label{table:whisk}
\end{table}

In order to prove that $\UTr(\cdot)$ (Definition \ref{def:uniform-state-construction}) preserves the rig structure, we define below left and right whiskerings on $\UTr(\Cat{C})$ for an arbitrary rig category $\Cat{C}$.


\begin{definition}\label{def:utr-whisk}
    Let $(\Cat{C}, \piu, \zero, \per, \uno)$ be a rig category, $\UTr(\Cat{C})$ the uniformly traced category freely generated from $(\Cat{C}, \oplus, \uno)$, and $X$ an object of $\UTr(\Cat C)$. Then $\fun{L}_X, \fun{R}_X \colon \UTr(\Cat C) \to \UTr(\Cat C)$ are defined on objects as 
    $\LW{X}{Y} \defeq X \per Y$ and $\RW{X}{Y} \defeq Y \per X$,
    and on arrows $\st{f}{S} \colon Y \to Z$ as
    \[ \LW{X}{f \mid S} \defeq \st{\symmt{X}{Y}}{\zero} ; \RW{X}{f \mid S} ; \st{\symmt{Z}{X}}{\zero} \qquad \text{ and } \qquad \RW{X}{f \mid S} \defeq \st{\RW{X}{f}}{S \per X}.\] 
\end{definition}
 
 
\begin{proposition}\label{lemma:utr-whisk-algebra}
    $\fun{L}_X, \fun{R}_X \colon \UTr(\Cat{C}) \to \UTr(\Cat{C})$ satisfy the laws in Table~\ref{table:whisk}.
\end{proposition}

\begin{remark}
It is worth remarking that the proof of \eqref{eq:tape:LexchangeR} --that is equivalent to functoriality of $\per$-- crucially requires uniformity, once more.
\end{remark}

The left and right whiskerings in Definition~\ref{def:utr-whisk} allow us to define another monoidal product on $\UTr(\Cat C)$, which on objects coincides with $\per$ in $\Cat C$ and on arrows $\st{f_1}{S_1} \colon X_1 \to Y_1$, $\st{f_2}{S_2} \colon X_2 \to Y_2$ is defined as:
\begin{equation}\label{eq:utr-per}
    \st{f_1}{S_1} \per \st{f_2}{S_2} \defeq \fun{L}_{X_1}(f_2 \mid S_2) ; \fun{R}_{Y_2}(f_1 \mid S_1).
\end{equation}


% \ale{RIFRASARE MEGLIO LE PROVE DEL LEMMA~\ref{lemma:utr-per-monoidal} E TEOREMA~\ref{th:free-uniform-trace-rig}}

One can check that $\per$ makes $\UTr(\Cat C)$ a symmetric monoidal category (see Lemma \ref{lemma:utr-per-monoidal}). Moreover the following key result holds.


\begin{theorem}\label{th:free-uniform-trace-rig}
    The adjunction in \Cref{th:free-uniform-trace} restricts to $\begin{tikzcd}
        \;\; \RIG \;\;
        \arrow[r, "\UTr"{name=F}, bend left] &
        \RIGUTr
        \arrow[l, "\fun{U}_3"{name=U}, bend left]
        \arrow[phantom, from=F, to=U, "\vdash" rotate=90]
    \end{tikzcd}$. 
    \end{theorem}


%\begin{theorem}\label{th:free-uniform-trace-rig}
%    The adjunction in \Cref{th:free-uniform-trace} restricts to rig categories.
%    In other words, if \(\Cat{C}\) is a rig category, then so is \(\UTr(\Cat{C})\).
%\end{theorem}


\subsection{Rigs, Biproducts and Uniform Traces}\label{ssec:rigbiut}
In the next section we are going to extend the language of tape diagrams for rig categories that are both finite biproduct and uniformly traced. We find thus convenient to introduce the following notion.

\begin{definition}
A \emph{uniformly traced finite biproduct (ut-fb) rig category} is a rig category $(\Cat{C}, \piu, \zero, \per, \uno)$  such that $(\Cat{C}, \piu, \zero)$ is a ut-fb category (see Definition \ref{def:utfbcategory}). A \emph{morphism of ut-fb rig categories} is both a rig functor and a morphisms of ut-fb categories. We write $\FBRIGUtr$ for the category of fb rig categories and their morphisms.
\end{definition}

By combining Corollary \ref{cor:free-uniform-trace-fb} and Theorem \ref{th:free-uniform-trace-rig}, one easily obtains the following.
\begin{proposition}\label{prop:free-uniform-trace-fb-rig}
    The adjunction in \Cref{th:free-uniform-trace} restricts to  $\begin{tikzcd}
        \FBRIG
        \arrow[r, "\UTr"{name=F}, bend left] &
        \FBRIGUtr
        \arrow[l, "\fun{U}_3"{name=U}, bend left]
        \arrow[phantom, from=F, to=U, "\vdash" rotate=90]
    \end{tikzcd}$. 
\end{proposition}





% \begin{center}
% NOTES TO REMEMBER FOR THE ADJUNCTIONS PROOFS
% \end{center}

% To prove that the adjunction restricts one has to prove that

% \begin{enumerate}
% \item $\UTr$ restricts on objects
% \item $\UTr$ restricts on arrows
% \item the unit $\eta$ restricts
% \item the counit $\epsilon$ restricts
% \end{enumerate}

% We already proved 1.

% To prove 2., should be rather simple.
% Consider first the restriction to fb-categories.
% Consider a fb-functor $F \colon \Cat{C} \to \Cat{D}$. By the original adjunction  $\UTr(F) \colon \UTr(\Cat{C}) \to \UTr(\Cat{D})$ is a functor that preserves traces. We should prove that $\UTr(F)$ is a fb-functor, i.e., it preserves (co)monoids; We assume that $\UTr(F) (f\mid \zero) = (Ff \mid \zero)$ (I am not sure about this, but I guess that this is true). One also has that the comultiplications on $\UTr(C)$ and $\UTr(D)$ are $(\diag{-}\mid \zero)$ where $\diag{-}$ is the comultiplication of either $\Cat{C}$ and $\Cat{D}$. Observe that:
% \begin{align*}
% \UTr(F) (\diag{X} \mid \zero) &= (F\diag{X} \mid \zero) \tag{assumption that I guess}\\
% &= (\diag{FX} \mid \zero)  \tag{$F$ fb-functors}
% \end{align*}

% For the restriction to rig categories, we proceed similarly with the symmetries and left distributors. For the $\per$, one has to do some more steps but I guess it is anyhow simple: TO CHECK.

% To prove 3., one has to prove that whenever $\Cat{C}$ is a fb-categories than $\eta_{\Cat{C}} \colon \Cat{C} \to \UTr(\Cat{C})$ is a fb-functor, i.e., it preserves comonoids. This is obvious since the $\eta$ maps any $f$ into $(f \mid \zero)$ and in particular $\diag{X}$ into $(\diag{X} \mid \zero)$ that is exactly the comultiplication in $\UTr(\Cat{C})$.

% Then for the rig structure,  $\eta_{\Cat{C}} \colon \Cat{C} \to \UTr(\Cat{C})$ preserves the rig structure. For symmetries and distributors is as above. For the $\per$, one has to prove that $(f \mid \zero) \per (g \mid \zero) = (f\times g \mid \zero)$ that I guess is rather straightforward.








% \begin{center}
% END OF THE NOTES
% \end{center}


\begin{comment}
\begin{itemize}
\item show the pullback results: the free constructions preserves both the rig and the finite biproduct structure
\item Apply this to tape: explain tapes, their diagrammatic version and so on so forth... summarise the old result...
\item ... illustrate the meaning of the new result... with drawing traces etc etc...
\end{itemize}

The adjunction in Theorem~\ref{th:free-uniform-trace} restricts to both finite biproduct categories (Corollary~\ref{cor:free-uniform-trace-fb}) and rig categories (Theorem~\ref{th:free-uniform-trace-rig}). Pe combine these two results by taking a pullback in $\CAT$, showing that the adjunction also restricts to rig categories with finite biproducts.
\begin{equation}\label{eq:pullback-utr}
    \begin{tikzcd}%[column sep=10pt]
        \FBRIGUtr &&& \RIGUTr \\
        & \FBRIG & \RIG \\
        & \FBC & \SMC \\
        \FBUTr &&& \UTSMC
        \arrow[hook, from=1-1, to=1-4]
        \arrow[""{name=0}, start anchor=south east, end anchor=north west, bend right, shift right=4, shorten <=5pt, from=1-1, to=2-2]
        \arrow[hook, from=1-1, to=4-1]
        \arrow["\lrcorner"{anchor=center, pos=0}, draw=none, from=1-1, to=4-4]
        \arrow[""{name=1}, start anchor=south west, end anchor=north east, bend left, shift left=4, from=1-4, to=2-3]
        \arrow[hook, from=1-4, to=4-4]
        \arrow[""{name=2}, start anchor=north west, end anchor=south east, bend right, shift left=-4, shorten >=5pt, from=2-2, to=1-1]
        \arrow[hook, from=2-2, to=2-3]
        \arrow[hook, from=2-2, to=3-2]
        \arrow["\lrcorner"{anchor=center, pos=0}, draw=none, from=2-2, to=3-3]
        \arrow[""{name=3}, start anchor=north east, end anchor=south west, bend left, shift right=-4, from=2-3, to=1-4]
        \arrow[hook, from=2-3, to=3-3]
        \arrow[hook, from=3-2, to=3-3]
        \arrow[""{name=4}, start anchor=south west, end anchor=north east, bend right, shift right=4, from=3-2, to=4-1]
        \arrow[""{name=5}, start anchor=south east, end anchor=north west, bend left, shift right=-4, from=3-3, to=4-4]
        \arrow[""{name=6}, start anchor=north east, end anchor=south west,  bend right, shift left=-4, from=4-1, to=3-2]
        \arrow[hook, from=4-1, to=4-4]
        \arrow[""{name=7}, start anchor=north west, end anchor=south east, bend left, shift left=4, from=4-4, to=3-3]
        \arrow["\dashv"{anchor=center, rotate=-135}, draw=none, from=2, to=0]
        \arrow["\dashv"{anchor=center, rotate=-45}, draw=none, from=3, to=1]
        \arrow["\dashv"{anchor=center, rotate=-45}, draw=none, from=4, to=6]
        \arrow["\dashv"{anchor=center, rotate=-135}, draw=none, from=5, to=7]
    \end{tikzcd}
\end{equation}

\ale{we could put references to theorems beside the adjunction symbols}

%\begin{proposition}\label{prop:free-uniform-trace-fb-rig}
%    The adjunction in \Cref{th:free-uniform-trace} restricts to  finite biproduct rig categories.
%    In other words, if \(\Cat{C}\) is a finite biproduct rig category, then so is \(\UTr(\Cat{C})\).
%\end{proposition}
\end{comment}


==> oldsections/sections/tracedrig.tex <==




\section{Rig Categories with Uniform Trace}\label{sec:tracedrig}





% \subsection{Freely Generated Rig Categories}



==> sections/cbproductsOLD.tex <==

\section{Convex Biproduct Categories OLD}\label{sec:cbproducts}  

\begin{definition}
A \emph{convex biproduct category} is a symmetric monoidal category $(\Cat{C},\oplus, \zero)$ such that, for every object $X$, there exist arrows $\codiag{X} \colon X\oplus X \to X$, $\cobang{X}\colon 0 \to X$, $\Br{+_p}_X \colon X \to X \oplus X$ and $\Br{\star}_X \colon X \to 0$ such that
\begin{enumerate}
\item  $\codiag{X}, \cobang{X}$ form monoids that are coherent and natural (see Figure~\ref{fig:monoidax} and \ref{fig:fccoherence}).;
\item  $\Br{+_p}_X, \Br{\star}_X$ form co-PCAs that are coherent and natural (see Figure~\ref{fig:co-pca axioms} and \ref{fig:copcacoherence}).
\end{enumerate}
A morphism of convex biproduct categories is a symmetric monoidal functor preserving monoids and co-pca. We write $\Cat{CBCat}$ for the category of convex biproduct categories and their morphisms.
\end{definition}
The name convex product is due to the fact that $\oplus$ is coproduct (by point 1 and Fox theorem \cite{fox1976coalgebras}) and --at the same time-- a \emph{convex product}, a notion that we will introduce soon. 

In a convex biproduct category, every homset carries a pointed convex algebra where for all $f,g\colon X \to Y$

\begin{equation}
f +_p g \defeq \Br{+_p}_X ; (f\oplus g) ; \codiag{Y} \qquad \star_{X,Y} \defeq \Br{\star}_X ; \cobang{Y}
\end{equation}

\begin{lemma}
Any convex biproduct category is enriched over $\Cat{PCA}$. Any morphism of convex biproduct category is $\Cat{PCA}$-enriched.
\end{lemma}
\begin{proof}
For the first point see \cite{}. For the second, observe it is enough to observe  that, by definition, any morphism of convex biproduct categories has to preserve all the structure involved in the definitions of $+_p$ and $\star_{X,Y}$.
\end{proof}

For $\Cat{PCA}$-enriched categories we can define the binary convex product of two objects $X,Y$ to be an object $Z$ with two arrows $\pi_1\colon Z\to X_1$ and $\pi_2\colon Z\to X_2$ satisfying the following universal property: for any $f\colon A\to X_1$ and $g\colon A \to X_2$, and $p,q \in (0,1)$ such that $p+q\le 1$, there exists a unique arrow $h\colon A \to Z$ such that $h;\pi_1 = p\cdot f$ and $h;\pi_2 = q\cdot g$.

Similarly, we can define the $n$-ary convex product of $n$ objects $X_1,\ldots,X_n$ to be an object $Z$ with arrows $\pi_i\colon Z\to X_i$ for $i=1,\ldots,n$ such that for any $f_i\colon A\to X_i$, and $p_i \in (0,1)$ such that $\sum_{i=1}^n p_i \le 1$, there exists a unique arrow $h\colon A \to Z$ such that $h;\pi_i = p_i\cdot f_i$ for all $i=1,\ldots,n$. Observe that, by definition, the 0-ary convex product is the final object $0$ of the category.



\begin{theorem}[A Fox theorem for convex bicategory]
Let $(\Cat{C},\oplus, \zero)$ be a symmetric monoidal category. $(\Cat{C},\oplus,\zero)$ is a convex biproduct category iff $\oplus$ is both a coproduct and a binary conex product and $\zero$ is both initial and final.   
\end{theorem}
\begin{proof}
Since, $\Cat{C}$ has coproducts, by Fox theorem \cite{fox1976coalgebras}, $(\Cat{C}, \oplus, 0)$ is a symmetric monoidal category such that for all object $X$, equipped with natural transformations  $\codiag{X} \colon X\oplus X \to X$, $\cobang{X}\colon 0 \to X$ forming monoids.

The arrow $\Br{+_p}_X \colon X \to X \oplus X$ is defined as the $(p,1-p)$-product of $\id{X}$ with itself. 

PROVE ITS NATURALITY. 

PROVE THE AXIOMS OF PCA.

The arrow $\Br{\star}_X \colon X \to 0$ is defined as the unique morphism to the final object $0$

PROVE ITS NATURALITY

PLEASE CHECK THE EXTRA CONDITIONS
\end{proof}


\begin{lemma}
Let $\Cat{C}$ be a convex biproducts category. Then $\Cat{C}$ has $n$-ary convex products.
\end{lemma}
\begin{proof}

\end{proof}




\section{Convex Biproduct Categories NEW}\label{sec:cbproducts}  

So far, we have recalled that $\KlD$ is $\Cat{PCA}$-enriched. Like all Kleisli category of a monad over $\Sets$, $\KlD$ inherits coproducts from $\Sets$ \cite{}. In this section, we observe that such coproducts in $\KlD$ carries what we named \emph{convex products}.

\begin{definition}
Let $X_1$, $X_2$  be two objects of a $\Cat{PCA}$-enriched category  $\Cat{C}$. The \emph{convex product} of $X_1$ and $X_2$ is an object $Z$ with two arrows $\pi_1\colon Z\to X_1$ and $\pi_2\colon Z\to X_2$ satisfying the following property: for all $p_1,p_2 \in (0,1)$ such that $p_1+p_2\le 1$ and all arrows $f\colon A\to X_1$, $g\colon A \to X_2$, there exists a unique arrow $h\colon A \to Z$ such that $h;\pi_1 = p\cdot f$ and $h;\pi_2 = p_2 \cdot g$.
\end{definition}

Similarly, the convex product of $n$ objects $X_1,\ldots,X_n$ is an object $Z$ with arrows $\pi_i\colon Z\to X_i$ for $i=1,\ldots,n$ such that for all $p_1, \dots p_n \in (0,1)$ such that $\sum_{i=1}^n p_i \le 1$ and arrows $f_i\colon A\to X_i$, there exists a unique arrow $h\colon A \to Z$ such that $h;\pi_i = p_i\cdot f_i$ for all $i=1,\ldots,n$. Observe that, by definition, the 0-ary convex product is a final object in $\Cat{C}$. Hereafter, we will denote the unique arrow $h$ by $\langle f_1, \dots, f_n \rangle_{\vec{p}}$ where $\vec{p}$ is a compact notation for $p_1, \dots , p_n$.


%\begin{definition}\marginpar{Vedi composizione di proiezione con iniezioni}
%A \emph{convex biproduct category} is a cocartesian monoidal category $(\Cat{C}, \oplus, \zero)$ such that
%\begin{itemize}
%\item $\Cat{C}$ is $\Cat{PCA}$-enriched;
%\item the initial object $\zero$ is also a final object;
%\item the coproduct $\oplus$ is a also convex product;
%\end{itemize} 
%\end{definition}


\begin{definition}\label{def:convbicat}%\marginpar{Vedi composizione di proiezione con iniezioni}
A \emph{convex biproduct category} is a $\Cat{PCA}$-enriched $\Cat{C}$ with an object $\zero$ which is both initial and terminal such that for every pair of objects $X_1$ and $X_2$ there exists and object $X_1\oplus X_2$ and morphism $\pi_i \colon X_1\oplus X_2 \to X_i$ and $\iota_i \colon X_i \to X_1 \oplus X_2$ such that $(X_1\oplus X_2, \iota_1, \iota_2)$ is a coproduct, $(X_1\oplus X_2, \pi_1, \pi_2)$ is a convex product and
\begin{equation}\label{eq:delta}\iota_i; \pi_j = \delta_{i,j}\end{equation}
where $\delta_{i,j} \colon X_i \to X_j$ is the arrow defined as $\delta_{i,j}= \id{X_i}$ if $i=j$ and $\delta_{i,j}=\star_{X_i,X_j}$ otherwise. Moreover, the enrichment is coherent w.r.t. the (convex-co)products, namely for every pair of arrows $f,g\colon X \to Y$ and $p\in (0,1)$
\begin{equation}\label{eq: assioma aggiuntivo}
    f+_p g = \langle f,g \rangle_{(p,1-p)};\codiag{Y}\text{.}
\end{equation}

A morphism of convex biproduct categoires is a functor $F\colon \Cat{C} \to \Cat{D}$ preserving coproducts and convex products. We write $\Cat{CBCat}$ for the category of convex biproduct categories and their morphisms.
\end{definition}

\begin{remark}
    The above definition is the one of biproduct category where products are replaced by convex products. Observe that the PCA-enrichment implies that for every $X,Y\in \Cat{C}$ it holds that
    \[\star_{X,Y} = \bang{X};\cobang{Y}\]
    where $\bang{X}\colon X \to \zero$ is the unique arrow to the final object $\zero$ and $\cobang{Y}\colon \zero \to Y$ is the unique arrow from the initial object $\zero$ to $Y$.
    Moreover the above condition $\iota_i; \pi_j = \delta_{i,j}$ is equivalent to requiring that the projections $\pi_1\colon X_1\oplus X_2 \to X_1$ and $\pi_2\colon X_1\oplus X_2 \to X_2$ are equal to $(\id{X_1}\otimes \bang{X_1});\runit{X_1}$ and $(\bang{X_2}\otimes \id{X_2});\lunit{X_2}$, respectively. Indeed,  since $\iota_1;(\id{X_1}\otimes \bang{X_1});\runit{X_1} = \id{X_1}$ and $\iota_2;(\bang{X_2}\otimes \id{X_2});\lunit{X_2} = \bang{X_2};\cobang{X_2}$ the universal property of coproducts implies the equality.

\end{remark}



As expected, our main example of a convex biproduct category is $\KlD$. 

\begin{proposition}\marginpar{Aggiungi dimostrazione}
$\KlD$ is a convex biproduct category
\end{proposition}
\begin{proof} \marginpar{TO BE MOVED IN THE APPENDIX}
    Coproducts are induced by the coproducts in $\Sets$, and the empty set $\zero$ is both initial and final. Indeed, for every object $X$, the unique arrow $X\to \zero$ sends an element $x\in X$ into the null subdistribution (which is the unique element of $\Dis(\zero)$). 
    
$\KlD$ is $\Cat{PCA}$-enriched since, for every $X,Y\in \KlD$, the homset $\KlD[X,Y]$ is a pointed convex algebra with the operations defined as follows: $+_p(f,g)(y|x)\defeq p\cdot f(y|x) + (1-p)\cdot g(y|x)$ for all $f,g\colon X \to Y$ and $p\in (0,1)$, and $\star_{X,Y}(y|x) \defeq 0$ (i.e., it is the arrow which sends every $x$ into the null subdistribution over $Y$). An easy calculation shows that arrow composition is a morphism of pointed convex algebras, i.e., it preserves the operations $+_p$ and $\star_{X,Y}$. For instance $(f+_pg) ;h= (f;h +_p g;h)$ for all $f,g\colon X \to Y$ and $h\colon Y \to Z$ is obtained as follows:
\begin{align}
    ((f+_pg) ;h)(z|x) &\coloneqq \sum_{y\in Y} (f+_pg)(y|x) \cdot h(z|y) \tag*{} \\
    &= \sum_{y\in Y} (p\cdot f(y|x) + (1-p)\cdot g(y|x)) \cdot h(z|y) \tag*{}\\
    &= p\cdot \sum_{y\in Y} f(y|x) \cdot h(z|y) + (1-p)\cdot \sum_{y\in Y} g(y|x) \cdot h(z|y) \tag*{}\\
    &= p\cdot (f;h)(z|x) + (1-p)\cdot (g;h)(z|x) \tag*{}\\
    &= (f;h +_p g;h)(z|x)\text{.}\tag*{}
    \end{align}
Now observe that $X_1+ X_2$ with the projections $\pi_i\colon X_1 + X_2 \to X_i$ for $i=1,2$ given by 
\[ \pi_1(x_1|z)\defeq \begin{cases}
    \delta_{x_1} & z=\iota_1(x_1)\\
    0 & otherwise
\end{cases} \qquad \pi_2(x_2|z)\defeq \begin{cases}
     \delta_{x_2} & z=\iota_2(x_2)\\
        0 & otherwise
\end{cases}\]
 is a convex product of $X_1$ and $X_2$. Indeed, given arrows $f_1\colon A\to X_1$ and $f_2\colon A\to X_2$ and $p_1,p_2 \in (0,1)$ such that $p_1+p_2\le 1$, there exists an arrow $\langle f_1,f_2\rangle_{p_1,p_2}\colon A \to X_1\oplus X_2$ defined as follows:
\[ \langle f_1,f_2\rangle_{p_1,p_2}(z|a) \defeq \begin{cases}
    p_1\cdot f_1(x_1|a) & z=\iota_1(x_1)\\
    p_2\cdot f_2(x_2|a) & z=\iota_2(x_2) \text{.}
\end{cases}\]
Observe that, for $i\in \{1,2\}$,
\begin{align*}
\langle f_1,f_2\rangle_{p_1,p_2} ; \pi_i (x_i | a) = & \sum_{z\in X_1+X_2} \langle f_1,f_2\rangle_{p_1,p_2}(z|a) \cdot \pi_i (x_i | z) \\
= & \langle f_1,f_2\rangle_{p_1,p_2} (\iota_i(x_i)|a)\\
= & p_i\cdot f_i (x_i|a)
\end{align*}
namely, it holds that $(\langle f_1,f_2\rangle_{p_1,p_2} );\pi_i = p_i\cdot f_i$. This is the unique arrow with such property since, for any other arrow $h'\colon A \to X_1\oplus X_2$ such that $h';\pi_i = p_i\cdot f_i$ for all $i=1,2$ it follows that 
\begin{align*}
  h'(\iota_1(x_1)|a) &=    h'(\iota_1(x_1)|a) \cdot 1\\
    & =\sum_{z\in X_1\oplus X_2} h'(z|a) \cdot \pi_1(x_1|z) \tag*{}\\
   &= h' ; \pi_1(x_1|a) \\
    &= p_1\cdot f_1(\iota_1(x_1)|a) \tag*{}
\end{align*}
and similarly for $\pi_2$ one obtains that $h'(\iota_2(x_2)|a) = p_2\cdot f_2(\iota_2(x_2)|a)$, i.e., $h' = \langle f_1,f_2\rangle_{p_1,p_2}$. A trivial verification shows that the above arrows $\pi_i$ and $\iota_i$ satisfy the required properties, i.e., $\iota_i;\pi_j = \delta_{i,j}$ for all $i,j=1,2$. 

\end{proof}

By Fox theorem \cite{}, any convex biproduct category $\Cat{C}$ carries a symmetric monoidal category $(\Cat{C}, \oplus, \zero)$ where every object $X$ is equipped with a commutative monoid that is natural and coherent, i.e., morphisms $\codiag{X} \colon X\oplus X \to X$ and $\cobang{X} \colon \zero \to X$ satifying the laws in BLA BLA. 

Moreover, for every object $X$ and $p\in (0,1)$, there exists an arrow $\Br{+_p}_X \colon X \to X \oplus X$ defined as $\langle id_X, id_X \rangle_{p,1-p}$ and an arrow $\Br{\star}_X\colon X \to \zero$ defined as the unique map to the final object $\zero$. \marginpar{Dalla seconda definizione segue che $\zero$ e' finale? Se no, si deve aggiustare la definizione richiedendo di avere uno zero object}
These maps equip every obejct with a co-PCA that is natural and coherent, i.e., the axioms in BLA BLA holds.



\begin{lemma}\label{lemma:initialproperties}
In a convex biproduct category the following hold:
\begin{enumerate}
\item $\star_{X,Y} = \bang{X};\cobang{Y}$
\item  $\iota_1=\Irunit{X_1}; (\id{X_1}\oplus \bang{X_2})$ for $\iota_1\colon X_1 \to  X_1\oplus X_2 $;\label{lemma:iotai1}
\item $\iota_2 = \Ilunit{X_2} ;(\bang{X_1}\oplus \id{X_2})$  for $\iota_2\colon  X_2 \to X_1\oplus X_2 $;\label{lemma:iota2}
\item  $\pi_1=(\id{X_1}\oplus \bang{X_2});\runit{X_1}$ for $\pi_1\colon X_1\oplus X_2 \to X_1$;\label{lemma:pi1}
\item $\pi_2 =(\bang{X_1}\oplus \id{X_2});\lunit{X_2}$  for $\pi_2\colon X_1\oplus X_2 \to X_2$;\label{lemma:pi2}
\item $p \cdot f = \diagp{X}; (f \oplus \bang{X} ) ; \runit{Y} $ for all $f\colon X \to Y$;\label{lemma:pf}
\item $(1-p)\cdot  f= \diagp{X} ; ( \, (\bang{X}  \oplus f \,)  ; \lunit{y}$  for all $f\colon X \to Y$; \label{lemma:1-pf}
\item $(p\cdot f) ; g =p\cdot (f;g)$ and $f;(p\cdot g) = p\cdot ( f;g)$ ; \label{lemma:p;}
\item $p\cdot (q \cdot f) =pq \cdot f$; \label{lemma:pq}
%\item $p \cdot \diagq{X} = \langle \id{X},\id{X}\rangle_{pq, p(1-q)} $.\label{lemma:pdiag}
%\item $\diagp{X}; (\id{X} \oplus q\cdot \id{X})=\langle \id{X},\id{X}\rangle_{p,(1-p)q}$ \label{lemma:diagp}
\end{enumerate}
\end{lemma}
\begin{proof}
We prove below item by item.
\begin{enumerate}
\item Follow easily by enrichment and finality of $\zero$: 
\begin{align*}
\star_{X,Y} & = \star_{X,\zero} ; \cobang{Y} \tag{\ref{eq:enr}}\\
&= \bang{X};\cobang{Y} \tag{$\zero$ is final}
\end{align*}
\item We prove that $ \id{X_1}\oplus \bang{X_2}=\runit{X_1}; \iota_1$ by universal property of $X_1\oplus \zero$ using the injections $\iota_1^{X_1\oplus\zero} \colon X_1 \to X_1\oplus \zero$ and 
$\iota_2^{X_1\oplus\zero} \colon \zero \to X_1\oplus \zero$. First observe that, by initiality of $\zero$,
 \[\iota_2^{X_1\oplus \zero}; (\id{X_1}\oplus \bang{X_2}) = \iota_2^{X_1\oplus \zero}; \runit{X_1}; \iota_1 \text{.} \]
Moreover
\begin{align*}
\iota_1^{X_1\oplus \zero} ; (\id{X_1}\oplus \bang{X_2}) &= \iota_1^{X_1\oplus \zero} ; [\id{X_1}; \iota{1},\bang{X_2};\iota_2 ] \tag{def. of $\oplus$}\\
&=\id{X_1};\iota_1 \tag{coproduct}\\
&=\iota_1^{X_1,\zero}; \runit{X_1} ; \iota_1 \tag{def. of $\runit{}$} 
\end{align*}
Thus $ \id{X_1}\oplus \bang{X_2}=\runit{X_1}; \iota_1$.
\item Analogous to the point above.
\item Observe that, for $\iota_i\colon X_i \to X_1\oplus X_2$, 
\[\iota_1 ; (\id{X_1}\oplus \bang{X_2});\runit{X_1}=\id{X_1} \qquad \iota_2 ;  (\id{X_1}\oplus \bang{X_2});\runit{X_1} = \bang{X_2}; \cobang{X_1}= \star_{X_2,X_1}\]
namely $(\id{X_1}\oplus \bang{X_2});\runit{X_1} = [id_{X_1}, \star_{X_2,X_1}]$. Now, by \eqref{eq:delta}, one has that $[id_{X_1}, \star_{X_2,X_1}]=\pi_1$.
\item Analogous to the point above.
\item By the following derivation.
\begin{align*}
p \cdot f &= f+_p\star_{X,Y} \tag{def. of $p\cdot(-)$}\\
&= \diagp{X} ; (f \oplus \star_{X,Y}) ; \codiag{Y} \tag{\ref{eq: assioma aggiuntivo}} \\ 
&= \diagp{X} ; (f \oplus (\bang{X};\cobang{Y})) ; \codiag{Y} \tag{Lemma \ref{lemma:initialproperties}.1} \\ 
&= \diagp{X} ; (f \oplus \bang{X}) ;(\id{Y} \oplus \cobang{Y}) ; \codiag{Y} \tag{Symmetric Monoidal Category} \\ 
&= \diagp{X} ; (f \oplus \bang{X}) ;\runit{Y} \tag{\ref{ax:Mon2}} \\ 
 \end{align*}
 \item By the following derivation
\begin{align*}
(1-p) \cdot f &= f+_{1-p}\star_{X,Y} \tag{def. of $p\cdot(-)$}\\
&= \star_{X,y} +_{p} f \tag{\ref{eq:pca}}\\
&= \diagp{X} ; (\star_{X,Y} \oplus f) ; \codiag{Y} \tag{\ref{eq: assioma aggiuntivo}} \\ 
&= \diagp{X} ; ((\bang{X};\cobang{Y}) \oplus f) ; \codiag{Y} \tag{Lemma \ref{lemma:initialproperties}.1} \\ 
&= \diagp{X} ; (\bang{X} \oplus f) ;(\id{Y} \oplus \cobang{Y}) ; \codiag{Y} \tag{Symmetric Monoidal Category} \\ 
&= \diagp{X} ; ( \bang{X} \oplus f) ;\lunit{Y} \tag{\ref{ax:Mon2}} \\ 
 \end{align*} 
 \item  Follow easily by the enrichment. For instance, the first equality is proved as follows.
\begin{align*} 
(p\cdot f) ; g & = (f+_p\star_{X,Y});g \tag{def of $p\cdot(-)$} \\
&= (f;g) +_p(\star_{X,Y};g) \tag{\ref{eq:enr}}\\
&= (f;g) +_p(\star_{X,Z}) \tag{\ref{eq:enr}}\\
&= p\cdot (f ; g) \tag{def of $p\cdot(-)$} \\
\end{align*}
\item Follow easily by the laws of PCAs.
\begin{align*}
p\cdot (q \cdot f) &= (f+_q \star )+_p \star \tag{def. of $p\cdot(-)$}\\
&= f+_{pq} (\star +_{\frac{p\cdot(1-q)}{1-pq}} \star) \tag{\ref{eq:pca}} \\
&= f+_{pq} \star \tag{\ref{eq:pca}} \\
&= pq \cdot f \tag{def. of $p\cdot(-)$}
\end{align*}
\end{enumerate}
\end{proof}


\begin{lemma}\label{lemma:naturality}
In a convex bicategory, $\bang{}$ and $\diagp{}$ form natural transformations, namely 
$f;\bang{Y}=\bang{X}$  and $f;\diagp{Y} = \diagp{X};(f\oplus f)$ for all $f\colon X\to Y$.
\end{lemma}
\begin{proof}
The equation $f;\bang{Y}=\bang{X}$ for $f\colon X \to Y$ follows from the fact that $\zero$ is final. The equation
\[f;\diagp{Y} = \diagp{X};(f\oplus f)\]
follows from the universl property of convex products. Indeed, observe that
\begin{align*}
    \diagp{X};(f\oplus f);\pi_1 &= \diagp{X};(f\oplus f);(\id{Y}\piu \bang{Y});\runit{X} \tag{Lemma \ref{lemma:initialproperties}.\ref{lemma:pi1}}\\
    &= \diagp{X};(f\oplus (f;\bang{Y}));\runit{X}  \tag{Symmetric Monoidal Category}\\
    &= \diagp{X};(f\oplus \bang{X});\runit{X} \tag{Naturality of $\bang{X}$}\\
    &= p\cdot f \tag{Lemma \ref{lemma:initialproperties}.\ref{lemma:pf}}
\end{align*}
\begin{align*}
    \diagp{X};(f\oplus f);\pi_2 &= \diagp{X};(f\oplus f);(\bang{Y} \piu \id{Y} );\lunit{X} \tag{Lemma \ref{lemma:initialproperties}.\ref{lemma:pi2}}\\
    &= \diagp{X};( (f;\bang{Y})\oplus f);\lunit{X}  \tag{Symmetric Monoidal Category}\\
    &= \diagp{X};( \bang{X} \oplus f);\lunit{X} \tag{Naturality of $\bang{X}$}\\
    &= (1-p)\cdot f \tag{Lemma \ref{lemma:initialproperties}.\ref{lemma:1-pf}}
\end{align*}
and that
\begin{align*}
f;\diagp{Y};\pi_1 &= f ; \langle \id{X}, \id{X} \rangle_{p,(1-p)};\pi_1 \tag{def. of $\diagp{}$}\\
&= f; (p\cdot \id{X}) \tag{convex product} \\
&= p\cdot(f;\id{X}) \tag{Lemma \ref{lemma:initialproperties}.\ref{lemma:p;}}\\
&=p\cdot f \tag{Category}
\end{align*}
\begin{align*}
f;\diagp{Y};\pi_2 &= f ; \langle \id{X}, \id{X} \rangle_{p,(1-p)};\pi_2 \tag{def. of $\diagp{}$}\\
&= f; (\,(1-p)\cdot \id{X}\,) \tag{convex product} \\
&= (1-p)\cdot(f;\id{X}) \tag{Lemma \ref{lemma:initialproperties}.\ref{lemma:p;}}\\
&=(1-p)\cdot f \tag{Category}
\end{align*}
\end{proof}

\begin{lemma}\label{lemma:coherence}
In a convex bicategory, the coherence axioms in Figure~\ref{fig:copcacoherence} hold.
\end{lemma}
\begin{proof}
(Coh2), (Coh3) and (Coh4) follow from the fact that $\zero$ is both initial and final. (Coh1) follows from the naturality and the universal property of coproducts. 

Let $s\defeq \assoc{X}{X}{Y\piu Y}; ( {\id{X}\piu \Iassoc{X}{Y}{Y}} ); ({\id X \piu ( \symm{X}{Y}^{\piu} \piu \id Y)} ); (\id{X}\piu \assoc{Y}{X}{Y}); \Iassoc{X}{Y}{X\oplus Y}$. Let
\[\iota_1^{(X\oplus X)\oplus(Y\oplus Y)}\colon X\piu X \to (X\piu X)\piu (Y\piu Y) \text{ and }\iota_2^{(X\oplus X)\oplus(Y\oplus Y)}\colon Y\piu Y \to (X\piu X)\piu (Y\piu Y)\] be the injections. By using the definitions of the structural isomorphisms induced by the coproducts, one can easily check that
\begin{equation}\label{eq:local}
\iota_1^{(X\oplus X)\oplus(Y\oplus Y)}; s= \iota_1 \oplus \iota_1 \qquad \text{and} \qquad \iota_2^{(X\oplus X)\oplus(Y\oplus Y)}; s= \iota_2 \oplus \iota_2\text{.}
\end{equation}
Then
\begin{align*}
\iota_1; (\diagp{X}\piu \diagp{Y}) ;s &= \iota_1; [\diagp{X}; \iota_1^{(X\oplus X)\oplus(Y\oplus Y)} \, , \, \diagp{Y}; \iota_2^{(X\oplus X)\oplus(Y\oplus Y)}] ;s \tag{def. of $\oplus$}\\
& = \diagp{X};\iota_1^{(X\oplus X)\oplus(Y\oplus Y)};s  \tag{coproduct}\\
&= \diagp{X}; (\iota_1 \oplus \iota_1) \tag{\ref{eq:local}} \\
&= \iota_1;\diagp{X\piu Y} \tag{Lemma \ref{lemma:naturality}}
\end{align*}
and 
\begin{align*}
\iota_2; (\diagp{X}\piu \diagp{Y}) ;s &= \iota_2; [\diagp{X}; \iota_1^{(X\oplus X)\oplus(Y\oplus Y)} \, , \, \diagp{Y}; \iota_2^{(X\oplus X)\oplus(Y\oplus Y)}] ;s \tag{def. of $\oplus$}\\
& = \diagp{Y};\iota_2^{(X\oplus X)\oplus(Y\oplus Y)};s  \tag{coproduct}\\
&= \diagp{X}; (\iota_2 \oplus \iota_2) \tag{\ref{eq:local}} \\
&= \iota_2;\diagp{X\piu Y} \tag{Lemma \ref{lemma:naturality}}
\end{align*}
Hence, the universal property of coproducts implies that $\diagp{X\piu Y} = \diagp{X}\piu \diagp{Y};s$.
\end{proof}


\begin{lemma}\label{lemma:pdiag} \label{lemma:diagp}
In a convex biproduct category the following hold:
\begin{enumerate}
\item $p \cdot \diagq{X} = \langle \id{X},\id{X}\rangle_{pq, p(1-q)} $.%\label{lemma:pdiag}
\item $\diagp{X}; (\id{X} \oplus q\cdot \id{X})=\langle \id{X},\id{X}\rangle_{p,(1-p)q}$ %\label{lemma:diagp}
\end{enumerate}
\end{lemma}
\begin{proof}
We prove below item by item.
\begin{enumerate}
\item By the uniqueness of $\langle \id{X},\id{X}\rangle_{pq, p(1-q)}$ and the following two derivations.
\begin{align*}
(p \cdot \diagq{X})  ; \pi_1 &= p \cdot (\diagq{X};\pi_1) \tag{Lemma \ref{lemma:initialproperties}.4}\\
&=p\cdot (\langle \id{X},\id{X}\rangle_{q,1-q} ; \pi_1) \tag{def. of $\diagq{}$}\\
&= p\cdot (q \cdot \id{X}) \tag{convex product}\\
&= (p q) \cdot \id{X} \tag{\ref{lemma:pq}}
\end{align*}
\begin{align*}
(p \cdot \diagq{X})  ; \pi_2 &= p \cdot (\diagq{X};\pi_2) \tag{Lemma \ref{lemma:initialproperties}.4}\\
&=p\cdot (\langle \id{X},\id{X}\rangle_{q,1-q} ; \pi_2) \tag{def. of $\diagq{}$}\\
&= p\cdot ((1-q) \cdot \id{X}) \tag{convex product}\\
&= (p (1-q)) \cdot \id{X} \tag{\ref{lemma:pq}}
\end{align*}
\item By uniqueness of $\langle \id{X},\id{X}\rangle_{p,(1-p)q}$ and the following two derivations. \marginpar{Questa forse va messa dopo poiche si usa la naturalita}
\begin{align*}
\diagp{X}; (\id{X} \oplus q\cdot \id{X}) ; \pi_1 &= \diagp{X}; (\id{X} \oplus q\cdot \id{X}) ; (\id{X}\oplus \bang{X});\runit{X} \tag{Lemma \ref{lemma:initialproperties}.\ref{lemma:pi1}}\\
&= \diagp{X}; (\id{X} \oplus (q\cdot \id{X} ; \bang{X})); \runit{X} \tag{Symmetric Monoidal Category}\\
&= \diagp{X}; (\id{X} \oplus  \bang{X}); \runit{X} \tag{Naturality of $\bang{}$} \\
&= p\cdot \id{X} \tag{Lemma \ref{lemma:initialproperties}.\ref{lemma:pf}}
\end{align*}
\begin{align*}
\diagp{X}; (\id{X} \oplus q\cdot \id{X}) ; \pi_2 &= \diagp{X}; (\id{X} \oplus q\cdot \id{X}) ; (\bang{X}\oplus \id{X});\lunit{X} \tag{Lemma \ref{lemma:initialproperties}.\ref{lemma:pi2}}\\
&= \diagp{X}; ( \bang{X}\oplus( q\cdot \id{X}) ) ; \lunit{X} \tag{Symmetric Monoidal Category}\\
&= (1-p)\cdot (q \cdot \id{X}) \tag{Lemma \ref{lemma:initialproperties}.\ref{lemma:1-pf}}\\
&= ((1-p)q) \cdot \id{X} \tag{Lemma \ref{lemma:initialproperties}.\ref{lemma:pq}}
\end{align*}
\end{enumerate}
\end{proof}



\begin{lemma}
If $\Cat{C}$ is a convex biproduct category, then for every object $X$  the triple $(X,\diagp{X},\bangp{X})$ is a co-PCA object, i.e., the axioms in Figure~\ref{fig:co-pca axioms} and \ref{fig:copcacoherence} hold.
\end{lemma}
\begin{proof}
We proved naturality and coherence in Lemmas \ref{lemma:naturality} and \ref{lemma:coherence}. Below we prove the axioms in Figure~\ref{fig:co-pca axioms}.

    (PCA1) in Figure~\ref{fig:co-pca axioms} follows from the universal property of convex products. Indeed, observe that \marginpar{Per il primo passaggio mi sembra necessario il rmk che ho scritto dopo la def di convex biproduct category, o no?}
    \begin{align*}
        \diagp{X} ; (\diagq{X} \oplus \id{X}) ; \pi_1 &= \diagp{X} ; (\diagq{X} \oplus \id{X}) ;( \id{X \oplus X} \oplus \bang{X}) ; \runit{X\oplus X} \tag{Lemma \ref{lemma:initialproperties}.\ref{lemma:pi1}}\\
        &= \diagp{X} ; (\diagq{X} \oplus \bang{X}) ; \runit{X\oplus X} \tag{Symmetric Monoidal Category}\\
        &= p \cdot \diagq{} \tag{Lemma \ref{lemma:initialproperties}.\ref{lemma:pf}}\\
        &= \langle \id{X}, \id{X} \rangle_{pq,\,p(1-q)}\tag{Lemma \ref{lemma:pdiag}}
    \end{align*}
    
        \begin{align*}
        \diagp{X} ; (\diagq{X} \oplus \id{X}) ; \pi_2 &= \diagp{X} ; (\diagq{X} \oplus \id{X}) ;( \bang{X \oplus X} \oplus \id{X}) ; \lunit{X} \tag{Lemma \ref{lemma:initialproperties}.\ref{lemma:pi2}}\\
        & = \diagp{X} ; ( \, (\diagq{X} ; (\bang{X} \oplus \bang{X}) ) \oplus \id{X} \,)  ; \lunit{X} \tag{Symmetric Monoidal Category}\\
        &= \diagp{X} ;  (\bang{X}  \oplus \id{X} )  ; \lunit{X} \tag{Lemma \ref{lemma:naturality}} \\
        &=  (1-p)\cdot \id{X} \tag{Lemma \ref{lemma:initialproperties}.\ref{lemma:1-pf}}
    \end{align*}
    
Similarly, by fixing  $\tilde{p}\defeq  pq$ and $\tilde{q} \defeq \frac{p(1-q)}{1-pq}$, it holds  that
\begin{align}
    \diagptilde{}; (\id{X}\oplus \diagqtilde{}) ; \Iassoc{X}{X}{X}; \pi_1 &= \diagptilde{}; (\id{X}\oplus \diagqtilde{}) ; \Iassoc{X}{X}{X}; ( \id{X \oplus X} \oplus \bang{X}) ; \runit{X\oplus X} \tag{Lemma \ref{lemma:initialproperties}.\ref{lemma:pi1}}\\
     &= \diagptilde{}; (\id{X}\oplus \diagqtilde{}) ; ( \id{X} \oplus (\id{X} \oplus \bang{X})) ; \runit{X} \tag{Symmetric Monoidal Category}\\
 &= \diagptilde{}; (\,\id{X}\oplus ( \diagqtilde{} ;(\id{X} \oplus \bang{X})) \,); \runit{X} \tag{Symmetric Monoidal Category}\\
&= \diagptilde{}; (\,\id{X}\oplus \tilde{q}\cdot \id{X} \,) \tag{Lemma \ref{lemma:initialproperties}.\ref{lemma:pf}}\\
    &=\langle \id{X}, \id{X} \rangle_{\tilde{p},(1-\tilde{p})\tilde{q}} \tag{Lemma \ref{lemma:diagp}}\\
    &= \langle \id{X}, \id{X} \rangle_{pq,p(1-q)} \tag{def of $\tilde{p}$ and $\tilde{q}$}
\end{align} 
    \begin{align}%\marginpar{Da finire qua, mi sembra che si debba usare la coerenza}
    \diagptilde{}; (\id{X}\oplus \diagqtilde{}); \Iassoc{X}{X}{X};\pi_2&= \diagptilde{};( \id{X}\oplus \diagqtilde{}); \Iassoc{X}{X}{X}; (\bang{X\piu X}\piu \id{X});\lunit{X}  \tag{Lemma \ref{lemma:initialproperties}.\ref{lemma:pi2}}\\
    &= \diagptilde{};( \id{X}\oplus \diagqtilde{}); \Iassoc{X}{X}{X}; ((\bang{X}\piu \bang{X})\piu \id{X});\lunit{X}  \tag{Lemma \ref{lemma:coherence}}\\
    &= \diagptilde{}; (\bang{X} \oplus \id{X}); \lunit{X} ; \diagqtilde{X}; (\bang{X}\piu \id{X}) ;\lunit{X}  \tag{Symmetric Monoidal Category}\\
    &= \diagptilde{}; (\bang{X} \oplus \id{X}); \lunit{X} ; (1-\tilde{q})\cdot \id{X}  \tag{Lemma \ref{lemma:initialproperties}.\ref{lemma:1-pf}}\\
    &= \diagptilde{}; (\bang{X} \oplus ( (1-\tilde{q})\cdot \id{X} )) ;  \lunit{X} \tag{Symmetric Monoidal Category}\\
    &= (1-\tilde{p}) \cdot ((1-\tilde{q})\cdot \id{X} )  \tag{Lemma \ref{lemma:initialproperties}.\ref{lemma:1-pf}}\\
    &=  (1-\tilde{p}) (1-\tilde{q}) \cdot \id{X} \tag{Lemma \ref{lemma:initialproperties}.\ref{lemma:pq}}\\
    &= (1-p) \cdot \id{X} \tag{def. $\tilde{p}$ and $\tilde{q}$}
\end{align}
    Hence, $\diagp{} ; (\diagq{} \oplus \id{X}) = \diagptilde{} ; \id{X}\oplus \diagqtilde{}; \Iassoc{X}{X}{X}$.\\

    (PCA2) in Figure~\ref{fig:co-pca axioms} follows from the coherence of the PCA-enrichment (i.e., property \eqref{eq: assioma aggiuntivo}):
  \begin{align*}
    \diagp{X}; \codiag{X} &=   \diagp{X}; (\id{X} \oplus \id{X}) \codiag{X}\\
    &= \id{X}+_p \id{X} \tag{\ref{eq: assioma aggiuntivo}}\\
    &=\id{X} \tag{\ref{eq:pca}}
    \end{align*}
    \\

    (PCA3) in Figure~\ref{fig:co-pca axioms} follows from the universal property of convex products. Indeed, observe that
    \begin{align*}
        \diagp{X};\symm{X}{X};\pi_1 &= \diagp{X};\symm{X}{X};(\id{X}\piu \bang{X});\runit{X} \tag{Lemma \ref{lemma:initialproperties}.\ref{lemma:pi1}}\\
        &= \diagp{X};(\bang{X} \piu \id{X});\lunit{X} \tag{Symmetric Monoidal Categories}\\
        &= (1-p)\cdot \id{X} \tag{Lemma \ref{lemma:initialproperties}.\ref{lemma:1-pf}}
    \end{align*}
    And similarly for $\pi_2$ we have that $\diagp{X};\symm{X}{X};\pi_2 = p\cdot \id{X}$. Hence, the universal property of convex products implies that $\diagp{X};\symm{X}{X} = \diagpbar{X}$.
 \end{proof}

				
\begin{lemma}
Let $\Cat{C}$ be a convex biproducts category. Then $\Cat{C}$ has $n$-ary convex products.
\end{lemma}
\begin{proof}
By induction on $n$, we show that $\bigoplus_{i=1}^n X_i$ is a convex product of $X_1, \dots, X_n$. For $n=0$, observe that the object $\zero$ is final by Definition \ref{def:convbicat}.
For $n+1$ assume by induction hypothesis that $\bigoplus_{i=1}^n X_i$ is a convex product of $X_1, \dots, X_n$ with projection $\pi_i\colon \bigoplus_{i=1}^n X_i \to X_i$. Since $\Cat{C}$ has binary convex product we can take the convex product $(\bigoplus_{i=1}^n X_i) \oplus X_{n+1}$ with projections $\pi'_1\colon (\bigoplus_{i=1}^n X_i) \oplus X_{n+1} \to \bigoplus_{i=1}^n X_i$ and $\pi'_2\colon (\bigoplus_{i=1}^n X_i) \oplus X_{n+1} \to X_{n+1}$. We claim that $(\bigoplus_{i=1}^n X_i) \oplus X_{n+1}$ with projections $\pi''_i\colon (\bigoplus_{i=1}^n X_i) \oplus X_{n+1} \to X_i$ defined for all $i\in 1\dots n+1$ as 
\[\pi''_i = \begin{cases} \pi_1'; \pi_i & i\in 1,\dots n \\ \pi_2' & i=n+1 \end{cases}\]
To check the universal property, let $\vec{p}=p_1,\dots, p_{n+1}$ such that $\sum_{i=1}^{n+1}p_i\leq 1$ and $f\colon A \to X_i$. Take $\vec{q}=q_1,\dots, q_n$ with $q_i=\frac{p_i}{1-p_{n+1}}$, since 
$\bigoplus_{i=1}^n X_i$ is a $n$-ary convex product by induction hypothesis, there exists an arrow $\langle f_1, \dots ,f_n\rangle_{\vec{q}} \colon A \to \bigoplus_{i=1}^n X_i$ such that $p_i\cdot f_i = \langle f_1, \dots ,f_n\rangle_{\vec{q}} ; \pi_i$. For the $n+1$-ary, we construct the mediatiing morphism $h\colon A \to (\bigoplus_{i=1}^n X_i) \oplus X_{n+1}$ as $\langle \, \langle f_1, \dots ,f_n\rangle_{\vec{q}} \,,\, f_{n+1} \, \rangle_{1-p_{n+1},p_{n+1}}$.
 \end{proof}

\begin{lemma}
Any morphism of convex biproduct category is a monoidal functor preserving monoids and coPCAs.
\end{lemma}
\begin{proof}
INSERT PROOF
\end{proof}




==> sections/oldmaterial.tex <==

\section{OLD MATERIAL}

\begin{lemma}\label{keyLemma}
Let $\t\colon A \to B \oplus C$ be an arrow in $\CatTapeC$. If $\t; (\id{B} \oplus\, \bangp{B}) =\, \diagp{};(\s_1 \oplus\, \bangp{C})$
and $\t; (\,\bangp{A} \oplus \id{C}) =\, \diagp{}; (\,\bangp{B} \oplus \s_2)$ then $h =\, \diagp{}; (\s_1 \oplus \s_2)$.
\end{lemma}

\section{Proof of Lemma \ref{keyLemma}} \marginpar{To be moved in the Appendix}

For all natural numbers $n \in \mathbb{N}$ and $p_1, \dots , p_n \in (0,1)$ such that $\sum_{i=1}^n p_i \leq 1$ one can define $\Br{+_{\vec{p}}}\colon A \to \bigoplus_{i=1}^n  A$ as follows:\\

for $n=0$ take $\Br{{+_{\vec{p}}}}\coloneqq\Br{\star}_A$ ;\\




for $n+1$ take $\Br{{+_{\vec{p}}}}\coloneqq \Br{+_{p_{n+1}}}_A; (\id{A} \oplus \Br{{+_{\frac{\vec{p'}}{1-p_{n+1}}}}})$ where $\vec{p'} = p_1, \dots, p_n$.

\marginpar{per ottenere che la probabilità del primo ingresso sia $p_1$ e così via ed evitare di avere la $\star$ nella definizione si deve riscrivere in questo modo}

For all natural numbers $n \in \mathbb{N}$ and $p_1, \dots , p_n \in (0,1)$ such that $\sum_{i=1}^n p_i \leq 1$ one can define $\diaggen{\vec{p}}{A}\colon A \to \bigoplus_{i=1}^{n+1}  A$ as follows:\\

for $n=0$ take $\id{A}$;\\

for $n=k+1$ take $\diaggen{\vec{p}}{A}\defeq\, \diaggen{p_1}{A}; (\id{A} \oplus\, \diaggen{\frac{\vec{p'}}{1-p_1}}{A})$ where $\vec{p'} = p_2, \dots, p_n$.
 \newline
Similarly, for all natural numbers $n \in \mathbb{N}$ one can define $\codiag{A}^n\coloneqq \bigoplus_{i=1}^n A\to A$ as follows:\\

for $n=0$ take $\codiag{A}^0\coloneqq \cobang{A}$;\\

for $n+1$ take $\codiag{A}^{n+1}\coloneqq (\id{A} \oplus \codiag{A}^n  );\codiag{A}$.





\begin{lemma}[Pre normal form]\label{lemma:prenormalform}\marginpar{Questa poi avra' un analogo nelle matrici}
Every arrow $\t\colon A \to \oplus_{i=1}^n B_i$ in $\CatTapeC$ can be written as $\t_1;\t_2;\t_3;\t_4$ where:
\begin{itemize}
    \item $\t_1$ is obtained through the fragment \begin{tabular}{rc ccccccccccccccccccccc}\setlength{\tabcolsep}{0.0pt}
        $\!\!\! \mid \!\!\!$ & $\diagp{A}$  & $\!\!\! \mid \!\!\!$  & $\id{\zero}$ & $\!\!\! \mid \!\!\!$ &  $\id{A}$ & $\!\!\! \mid \!\!\!$   & $   \t ; \t   $ & $\!\!\! \mid \!\!\!$  & $  \t \piu \t  $ & $\!\!\! \mid \!\!\!$  &  $\sigma_{A,B}^{\piu}$
    \end{tabular}
    \item $\t_2$ is obtained through the fragment \begin{tabular}{rc ccccccccccccccccccccc}\setlength{\tabcolsep}{0.0pt}
           $\!\!\! \mid \!\!\!$  &  $\bangp{A}$& $\!\!\! \mid \!\!\!$&  $\id{\zero}$ & $\!\!\! \mid \!\!\!$ & $\id{A}$    & $\!\!\! \mid \!\!\!$   & $   \t ; \t   $ & $\!\!\! \mid \!\!\!$  & $  \t \piu \t  $ & $\!\!\! \mid \!\!\!$  &  $\sigma_{A,B}^{\piu}$
    \end{tabular}
    \item $\t_3$ is obtained through the fragment \begin{tabular}{rc ccccccccccccccccccccc}\setlength{\tabcolsep}{0.0pt}
        $\!\!\! \mid \!\!\!$ & $\tapeFunct{c}$  & $\!\!\! \mid \!\!\!$  &  $\id{\zero}$ & $\!\!\! \mid \!\!\!$ & $\id{A}$&  $\!\!\! \mid \!\!\!$   & $   \t ; \t   $ & $\!\!\! \mid \!\!\!$  & $  \t \piu \t  $ & $\!\!\! \mid \!\!\!$  &  $\sigma_{A,B}^{\piu}$
    \end{tabular}
    \item $\t_4$ is obtained through the fragment \begin{tabular}{rc ccccccccccccccccccccc}\setlength{\tabcolsep}{0.0pt}
        $\!\!\! \mid \!\!\!$ & $\codiag{A}$ &$\!\!\! \mid \!\!\!$ & $\cobang{A}$ & $\!\!\! \mid \!\!\!$  &  $\id{\zero}$ & $\!\!\! \mid \!\!\!$ & $\id{A}$ & $\!\!\! \mid \!\!\!$   & $   \t ; \t   $ & $\!\!\! \mid \!\!\!$  & $  \t \piu \t  $ & $\!\!\! \mid \!\!\!$  &  $\sigma_{A,B}^{\piu}$
    \end{tabular}
\end{itemize}
\end{lemma}
\begin{proof}
Using the naturality, one can first move all the occurrences of $\diagp{}$ to the left. The all the occurrences of $\cobang{}$ to the left until an occurence of $\diagp{}$ is met (note that since $\cobang{}$ is not the unit of $\diagp{}$, $\cobang{}$ remains at the right of $\diagp{}$). Similarly, one can move all occurrences of $\codiag{}$ and $\cobang{}$ on the right.
\end{proof}


\begin{lemma}\label{lemmaB+Cform}
Let $\t\colon A \to B\oplus C$ be an arrow of $\CatTapeC$. Then one of the following holds:
\begin{itemize}
\item$\t=\star_{A,B\oplus C}$;
\item  there exists $\t_1 \colon A \to B$ such that $\t = \t_1 \oplus \cobang{C}$;
\item  there exists $\t_2 \colon A \to C$ such that $\t =  \cobang{B} \oplus \t_2$;
\item there exist $\t_1 \colon A \to B$ and $\t_2\colon A \to C$  and $p\in (0,1)$ 
such that $\t=\Br{+_p}_{A} ; (\t_1 \oplus \t_2)$.
\end{itemize}
\end{lemma}
\begin{proof}
By the prenormal form
\end{proof}

\begin{lemma}\label{lemmaABform}
Let $\t\colon A \to B$ be an arrow of $\CatTapeC$. Then one of the following holds: 
\begin{itemize}
\item $\t=\star_{A,B}$;
\item there exist  $c \in \Cat{C}[A,B]$ such that $\t=\tapeFunct{c}$;
\item there exist distinct $c_1, \dots, c_n \in \Cat{C}[A,B]$ and $\vec{p}=p_1, \dots, p_{n+1}$ such that
\[\t=\, \diagvecp{A} ; ( (\bigoplus_{i=1}^n  \tapeFunct{c_i}) \oplus\, \bangp{A}  ) ; \codiag{B}^n\text{.}\]
\end{itemize}
\end{lemma}
\begin{proof}
By the prenormal form it should be like BLA BLA

The fact that each of the $c_i$ should be distinct follows easily from AXIOMS IDEMPOTENCY
similarly several  occurences of $\Br{\star}_A$ can be collapsed to one by using naturality of $\Br{\star}_A$ and IDEMPOTENCY.
\end{proof}

\begin{lemma}\label{lemma: frecce distribuzioni su n}
    Arrows in $\CatTapeC$ of the form $f:A\to \oplus_{i=1}^{n+1} A$ is obtained through the fragment:
    \begin{center}
    \begin{tabular}{rc ccccccccccccccccccccc}\setlength{\tabcolsep}{0.0pt}
        $\t$ & \emph{::=} &  $\!\!\! \mid \!\!\!$ & $\diagp{A}$  & $\!\!\! \mid \!\!\!$  &  $\id{A}$ & $\!\!\! \mid \!\!\!$   & $   \t ; \t   $ & $\!\!\! \mid \!\!\!$  & $  \t \piu \t  $ 
    \end{tabular}
    \end{center}
are in bijection with $\mathcal{DL}([n+1])\defeq\{ (p_1\dots p_{n+1}) \vert\ p_i\in(0,1), \sum_{i=1}^{n+1}p_i=1 \}$.
\end{lemma}
\begin{proof}
    Every arrow of the form $f:A\to \oplus_{i=1}^{n+1} A$ obtained through $\t$ can be seen as a binary tree with $n+1$ leaves and $n$ nodes labeled by $p_i$ for $i=1,\dots,n$. To every leave corresponds a probability $\mathcal{DL}(f)$ on the set of leaves which is obtained multiplying the labels of the path from the root to the leave. If one takes the top branch of the node $p_i$ then multiply by $p_i$ and if one takes the bottom branch then multiply by $1-p_i$. This correspondence is well-defined since for two equal arrows (by the application of the associativity law) the associated distribution does not change. Vice versa, to every distribution $p_1,\dots,p_{n+1}$ on $n+1$ elements (hence $p_{n+1}=1-\sum_{i=1}^{n}p_i$ ) one can associate the arrow $\diagvecp{A}$ where $\vec{p}=(p_1,\dots,p_n)$. This correspondece is bijective since every arrow $f$ is equal in one of the form $\diaggen{\vec{q}}{A} $ for some $\vec{q}=(q_1,\dots,q_{n})$, applying iteratively the associativity law. Hence, if $\mathcal{DL}(\diaggen{\vec{q}}{A})=\mathcal{DL}(\diagvecp{A})$ then one obtains 
    \begin{align}
       & p_1=q_1 \tag*{}\\
        &(1-p_1)p_2 = (1-q_1)q_2 \tag*{}\\
        \vdots \tag*{}\\
        &(1-p_1)(1-p_2)\dots(1-p_{n-1})p_n = (1-q_1)(1-q_2)\dots(1-q_{n-1})q_n \tag*{}\\
        &(1-p_1)(1-p_2)\dots(1-p_{n-1})(1-p_n) = (1-q_1)(1-q_2)\dots(1-q_{n-1})(1-q_n) \tag*{}
    \end{align}
    which implies that $p_i=q_i$ for all $i=1,\dots,n$. Thus the two arrows are equal.
\end{proof}

\begin{lemma}\label{lemma: arrows A-B subdistributions}
    Arrows in $\CatTapeC$ of the form $f:A\to B$ are in bijection with $\mathcal{D}_{\le}(\Cat{C}[A,B])$.
\end{lemma}
\begin{proof}
    By Lemma \ref{lemmaABform} every arrow $f:A\to B$ is in one of the following forms:
\begin{itemize}
\item $f=\star_{A,B}$;
\item there exists $c \in \Cat{C}[A,B]$ such that $f=\tapeFunct{c}$;
\item there exist distinct $c_1, \dots, c_n \in \Cat{C}[A,B]$ and $\vec{p}=p_1, \dots, p_{n}$ such that 
\[f=\,\diagvecp{A} ; ( (\bigoplus_{i=1}^n  \tapeFunct{c_i}) \oplus\, \bangp{A}  ) ; \codiag{B}^n\text{.}\]
\end{itemize}
The first two cases correspond respectively to the zero subdistribution and the Dirac distribution on $c$. The third case corresponds to the subdistribution $\vec{p}$ on the set of arrows $\{c_1, \dots, c_n\}$, where $p_i$ is the probability of $c_i$. %and $p_{n+1}=1-\sum_{i=1}^{n}p_i$ is the probability of $\Br{\star}_A$.
 If $f$ and $f'=\, \diaggen{\vec{q}}{A} ; ( (\bigoplus_{j=1}^{n'}  \tapeFunct{c'_i}) \oplus\, \bangp{A}  ) ; \codiag{B}^{n'}$ are sent to the same subdistribution, then one has that $n=n'$, $p_i=q_i$ and $c_i=c'_i$ for all $i=1,\dots,n$. 
\end{proof}

\begin{proof}[Proof of Lemma \ref{keyLemma}]
First observe that $\t\colon A \to B\oplus C$ is in one of the four forms of Lemma \ref{lemmaB+Cform}. The proof for the first three cases is trivial. The interesting one is the fourth case: 
(iv) $\t=\diagpX{p'}{A} ; (\t_1 \oplus \t_2)$. Thus
\begin{align}
\diagpX{p'}{A} ; (\t_1 \oplus \cobang{A}) =& \diagpX{p'}{A} ; (\t_1 \oplus \t_2) ; (\id{B} \oplus \cobang{C}) \tag{naturality} \\
=& \t ; (\id{B} \oplus \cobang{C}) \tag{iv} \\
=& \diagpX{p}{A} ; (\s_1 \oplus  \cobang{A})  \tag{Hypothesis} 
\end{align}
%
Now $\t_1$ and $\_1$ can be in one of the three forms of Lemma \ref{lemmaABform}. Again the only interesting case is the last one:
\begin{equation}\label{eq:t1s1}\t_1=\, \diaggen{\vec{p^1}}{A} ; ( (\bigoplus_{i=1}^n  \tapeFunct{c_i}) \oplus\, \bangp{A}  ) ; \codiag{B}^n \qquad \s_1= \, \diaggen{\vec{q^1}}{A}  ; ( (\bigoplus_{i=1}^{n'}  \tapeFunct{c'_i}) \oplus\, \bangp{A}  ) ; \codiag{B}^n\end{equation}
for $c_1, \dots c_n \in \Cat{C}[A,B]$, $c_1', \dots c_{n'}' \in \Cat{C}[A,B]$ and $\vec{p^1}= p^1_1 \dots p^1_{n}$ and $\vec{q^1} = q^1_1, \dots q_{n'}^1$.
%
A symmetric argument leads to
\[\t_2=\, \diaggen{\vec{p^2}}{A} ; ( (\bigoplus_{i=1}^m  \tapeFunct{d_i}) \oplus\,\bangp{A} ) ; \codiag{B}^m \qquad \s_2= \, \diaggen{\vec{q^2}}{A} ; ( (\bigoplus_{i=1}^m  \tapeFunct{d'_i}) \oplus\,\bangp{A}  ) ; \codiag{B}^{m'}\]
for $d_1, \dots d_m \in \Cat{C}[A,B]$, $d_1', \dots d_{m'}' \in \Cat{C}[A,B]$ and $\vec{p^2}= p^2_1 \dots p^2_{m}$ and $\vec{q^1} = q^2_1, \dots q_{m'}^2$.



By replacing in $\diaggen{p'}{A} ; (\t_1 \oplus\, \bangp{A}) = \, \diagp{A}; (\s_1 \oplus\,  \bangp{A}) $ the characterisation of $\t_1$ and $\s_1$ in \eqref{eq:t1s1}, one has that
\[
\diaggen{p'}{A}; (  (\,\diaggen{\vec{p^1}}{A}; ( (\, \bigoplus_{i=1}^n  \tapeFunct{c_i}) \oplus\, \bangp{A}  ) ; \codiag{B}^n) \oplus\, \bangp{A}) =\, \diagp{A} ; ((\,\diaggen{\vec{q^1}}{A} ; ( (\bigoplus_{i=1}^{n'}  \tapeFunct{c_i}) \oplus\, \bangp{A}  ) ; \codiag{B}^{n'}) \oplus\,  \bangp{A}) 
\]
Lemma \ref{lemma: arrows A-B subdistributions} entails that they correspond to the same subdistributions on $\Cat{C}[A,B]$ and thus $n=n'$, $c_i=c'_i$, $p'p_i^1=pq_i^1$  for all $i=1,\dots,n$ and also
 \begin{equation}\label{eq:a}
    p'p_{n+1}^1 + (1-p')= pq_{n+1}^1 + (1-p)\end{equation}
where $p_{n+1}^1 = 1-\sum_{i=1}^{n}p^1_i$ and $q_{n+1}^1 = 1-\sum_{i=1}^{n}q^1_i$. A symmetric argument leads to $m=m'$, $d_i=d'_i$, $(1-p')p_i^2 = (1-p)q_i^2$  for all $i=1,\dots, m$
and also
\begin{equation}\label{eq:b}
(1-p')p_{m+1}^2 +p' = (1-p)q_{m+1}^2+p
\end{equation}
where $p_{m+1}^2 = 1-\sum_{i=1}^{m}p^2_i$ and $q_{m+1}^2 = 1-\sum_{i=1}^{m}q^2_i$.
Hence, taking the sum of \eqref{eq:a} and \eqref{eq:b} one obtains
\begin{equation}\label{eq:sumintheproof}p'p_{n+1}^1 + (1-p')p_{m+1}^2 = pq_{n+1}^1+  (1-p)q_{m+1}^2\text{.}\end{equation}


Then, by repeatetly applying \eqref{eq:diagp assoc} and idempotency laws \marginpar{Why idempotency}, it follows that  $$\t = \diaggen{\vec{t}}{A} ; ( \bigoplus_{i=1}^n  \tapeFunct{c_i} \oplus \bigoplus_{i=1}^m  \tapeFunct{d_i} \oplus\, \bangp{A}  ) ; \codiag{B}^n \oplus \codiag{C}^m$$ where $\vec{t} = (p'p_1^1, \dots, p'p_n^1,  (1-p')p_1^2, \dots, (1-p')p_m^2)$ 
and $$\s=\diaggen{\vec{s}}{A} ; ( \bigoplus_{i=1}^n  \tapeFunct{c_i} \oplus \bigoplus_{i=1}^m  \tapeFunct{d_i} \oplus\, \bangp{A} ) ; \codiag{B}^n\piu \codiag{C}^m $$ where $\vec{s} = (pq_1^1, \dots, pq_n^1, (1-p)q_1^2, \dots, (1-p)q_m^2)$. 


By $p'p_i^1=pq_i^1$, $(1-p')p_i^2 = (1-p)q_i^2$ and \eqref{eq:sumintheproof}, 
both $\diaggen{\vec{t}}{A}$ and $\diaggen{\vec{s}}{A}$ correspond both to the distribution on $[n+m+1]$ given by $(p'p_1^1, \dots, p'p_n^1,  (1-p')p_1^2, \dots, (1-p')p_m^2, p'p_{n+1}^1 + (1-p')p_{m+1}^2)$. Then by Lemma \ref{lemma: frecce distribuzioni su n} it follows that $\diaggen{\vec{t}}{A}=\diaggen{\vec{s}}{A}$ are equal and hence $\t=\s$.
\end{proof}




==> sections/tapes.tex <==

\section{Tape Diagrams with Uniform Traces}\label{sec:tapes}
In this section we introduce tape diagrams for rig categories with finite biproducts and uniform traces. 
The approach is similar to the one in Section~\ref{sc:tape} and it goes through the following adjunction.

% \begin{proposition}
%     $\CatTrTape$ is a $\sort$-sesquistrict ut-fb rig category.
% \end{proposition}
% \begin{proof}
%     The proof of the analogous result for plain, non-traced, tape diagrams, i.e. Theorem 5.10 in~\cite{bonchi2023deconstructing}, relies on several inductive proofs that must be extended to include the additional inductive case $\trace_{S}\t$ in~\eqref{tracedTapesGrammar}.
% \end{proof}

% \begin{theorem}
%     There is an isomorphism of $\sort$-sesquistrict ut-fb rig categories $\UTr(\CatTape) \cong \CatTrTape$.
% \end{theorem}

\begin{equation}\label{eq:adjunction-utfb}
    \begin{tikzcd}
        \SMC \ar[r,"U_1"] &
        \CAT
        \arrow[r, "F_3"{name=F}, bend left] &
        \FBUTr
        \arrow[l, "U_3"{name=U}, bend left]
        \arrow[phantom, from=F, to=U, "\vdash" rotate=90]
    \end{tikzcd}
\end{equation}

The functors $U_1$ and $U_3$ are the obvious forgetful functors. The functor $F_3$ is the left adjoint to $U_3$ and can be described as follows.


\begin{definition}\label{def:strict ut-fb freely generated by C}
Let $\Cat{C}$ be a category. The  strict ut-fb category freely generated by $\Cat{C}$, hereafter denoted by $F_3(\Cat{C})$, has as objects words of objects of $\Cat{C}$. Arrows are terms inductively generated by the following grammar, where $A,B$ and $c$ range over arbitrary objects and arrows of $\Cat{C}$,
    \begin{equation}
        \begin{array}{rcl}
            f & ::=& \; \id{A} \; \mid \; \id{I} \; \mid \; \tapeFunct{c} \; \mid \; \sigma_{A,B}^{\perG} \; \mid \;   f ; f   \; \mid \;  f \perG f  \; \mid \; \bang{A} \; \mid \; \diag{A} \;  \mid \; \cobang{A}\; \mid \; \codiag{A} \; \mid \; \trace_{A} f\\
            \end{array}
    \end{equation}  
    modulo the axioms in  Tables~\ref{fig:freestricmmoncatax},~\ref{fig:freestrictfbcat},~\ref{tab:trace-axioms} and~\ref{tab:uniformity}. %\marginpar{Modulo the axioms, for uniformity we should be clearer, maybe before}
\end{definition}

Similarly to~\eqref{eq:adjunction}, the unit of the adjunction $\eta \colon Id_{\CAT} \Rightarrow F_3U_3$ is defined for each category $\Cat{C}$ as the identity-on-objects functor $G \colon \Cat{C} \to U_3F_3(\Cat{C})$ that maps each arrow $c$ in $\Cat{C}$ into the arrow $\tapeFunct{c}$ of $U_3 F_3(\Cat{C})$.

\begin{lemma}\label{lemma:tr-adj}
    $F_3 \colon \CAT \to \FBUTr$ is left adjoint to $U_3 \colon \FBUTr \to \CAT$.
\end{lemma}

Recall from Section \ref{sec:monoidal} the category of string diagrams $\CatString$ generated by a monoidal signature $\sign$. Hereafter, we focus on  $F_3U_1(\CatString)$, referred to as $\CatTrTape$.
The set of objects of $\CatTrTape$ is the same of $\CatTape$, i.e., words of words of sorts in $\sort$. For arrows, we extend the two-layer grammar in~\eqref{tapesGrammar} with one production accounting for the trace operation.
\begin{equation}\label{tracedTapesGrammar}
    \begin{tabular}{rc ccccccccccccccccccccc}\setlength{\tabcolsep}{0.0pt}
        $c$  & ::= & $\id{A}$ & $\!\!\! \mid \!\!\!$ & $ \id{\uno} $ & $\!\!\! \mid \!\!\!$ & $ \gen $ & $\!\!\! \mid \!\!\!$ & $ \sigma_{A,B} $ & $\!\!\! \mid \!\!\!$ & $   c ; c   $ & $\!\!\! \mid \!\!\!$ & $  c \per c$ & \multicolumn{8}{c}{\;} \\
        $\t$ & ::= & $\id{U}$ & $\!\!\! \mid \!\!\!$ & $ \id{\zero} $ & $\!\!\! \mid \!\!\!$ & $ \tapeFunct{c} $ & $\!\!\! \mid \!\!\!$ & $ \sigma_{U,V}^{\piu} $ & $\!\!\! \mid \!\!\!$ & $   \t ; \t   $ & $\!\!\! \mid \!\!\!$ & $  \t \piu \t  $ & $\!\!\! \mid \!\!\!$ & $ \bang{U} $ & $\!\!\! \mid \!\!\!$ & $\diag{U}$ & $\!\!\! \mid \!\!\!$ & $\cobang{U}$ & $\!\!\! \mid \!\!\!$ & $\codiag{U}$  &  $\!\!\! \mid \!\!\!$ & $\trace_{U}\t$    
    \end{tabular}
\end{equation}  

The terms of the first row are taken modulo the axioms in Table~\ref{fig:freestricmmoncatax} (after replacing $\perG$ with $\per$).
The terms of the second row are taken modulo the axioms in Tables \ref{fig:freestricmmoncatax},~\ref{fig:freestrictfbcat},~\ref{tab:trace-axioms} and~\ref{tab:uniformity} (after replacing $\perG$ with $\piu$ and $A,B$ with $U,V$).

As for $\CatTape$, the grammar in \eqref{tracedTapesGrammar} can be rendered diagrammatically as follows.
\begin{equation*}\label{tracedTapesDiagGrammar}
    \setlength{\tabcolsep}{2pt}
    \begin{tabular}{rc cccccccccccc}
        $c$  & ::= &  $\wire{A}$ & $\mid$ & $ \tikzfig{empty} $ & $\mid$ & $ \Cgen{\gen}{A}{B}  $ & $\mid$ & $ \Csymm{A}{B} $ & $\mid$ & $ \tikzfig{seq_compC}   $ & $\mid$ & $  \tikzfig{par_compC}$ & \\
        $\t$ & ::= & $\Twire{U}$ & $\mid$ & $ \tikzfig{empty} $ & $\mid$ & $ \Tcirc{c}{U}{V}  $ & $\mid$ & $ \Tsymmp{U}{V} $ & $\mid$ & $ \tikzfig{tapes/seq_comp}  $ & $\mid$ & $  \tikzfig{tapes/par_comp}$ & $\mid$ \\
             &     & \multicolumn{12}{l}{$\Tcounit{U} \; \mid \; \Tcomonoid{U} \; \mid \; \Tunit{U} \; \mid \; \Tmonoid{U} \; \mid \; \TTraceMon{\t}[U][P][Q]$}
    \end{tabular}
\end{equation*} 

%%% COMMENTED VERSION PITH GENERIC PRODUCT
\begin{comment}
\begin{table}
\[\begin{array}{ccc}
\begin{array}{rcl}
 \bang{\unoG} & \defeq & \id{\unoG}  \\ 
 \bang{A \perG P} & \defeq & \bang{A} \perG \bang{P}  \\ 
\end{array}
&
\begin{array}{rcl}
\diag{\unoG} & \defeq &  \id{\unoG}  \\ 
\diag{A \perG P} & \defeq & (\diag{A} \perG \diag{P}) ; (\id{A} \perG \symm{A}{P} \perG \id{P})\\ 
\end{array}
\\ \\
\begin{array}{rcl}
 \cobang{\unoG} & \defeq & \id{\unoG}  \\ 
 \cobang{A \perG P} & \defeq & \cobang{A} \perG \cobang{P}  \\ 
\end{array}
&
\begin{array}{rcl}
\codiag{\unoG} & \defeq &  \id{\unoG}  \\ 
\codiag{A \perG P} & \defeq & (\id{A} \perG \symm{A}{P} \perG \id{P}) ; (\codiag{A} \perG \codiag{P}) \\ 
\end{array}
&
\begin{array}{rcl}
\trace_{\unoG}(\t) & \defeq & \t \\
\trace_{A \perG P}(\t) & \defeq & \trace_{P} \trace_A (\t) 
\end{array}
\end{array}\]
\caption{Inductive definitions of $\bang{P}$, $\diag{P}$, $\cobang{P}$,  $\codiag{P}$ and  $\trace_{P}\t$ for all words $P$}
\end{table}
\end{comment}

\begin{table}
\[\begin{array}{ccc}
\begin{array}{rcl}
 \bang{\zero} & \defeq & \id{\zero}  \\ 
 \bang{U \piu P} & \defeq & \bang{U} \piu \bang{P}  \\ 
\end{array}
&
\begin{array}{rcl}
\diag{\zero} & \defeq &  \id{\zero}  \\ 
\diag{U \piu P} & \defeq & (\diag{U} \piu \diag{P}) ; (\id{U} \piu \symm{U}{P} \piu \id{P})\\ 
\end{array}
\\ \\
\begin{array}{rcl}
 \cobang{\zero} & \defeq & \id{\zero}  \\ 
 \cobang{U \piu P} & \defeq & \cobang{U} \piu \cobang{P}  \\ 
\end{array}
&
\begin{array}{rcl}
\codiag{\zero} & \defeq &  \id{\zero}  \\ 
\codiag{U \piu P} & \defeq & (\id{U} \piu \symm{U}{P} \piu \id{P}) ; (\codiag{U} \piu \codiag{P}) \\ 
\end{array}
&
\begin{array}{rcl}
\trace_{\zero}(\t) & \defeq & \t \\
\trace_{U \piu P}(\t) & \defeq & \trace_{P} \trace_U (\t) 
\end{array}
\end{array}\]
\caption{Inductive definitions of $\bang{P}$, $\diag{P}$, $\cobang{P}$,  $\codiag{P}$ and  $\trace_{P}\t$ for all polynomial $P$}\label{tab:inddefutfb}
\end{table}


\begin{figure}[h!]
    \mylabel{ax:trace:tape:sliding}{sliding}
    \centering
    \[
        \begin{array}{c@{}c@{}c @{\quad} c@{}c@{}c}
            \tikzfig{traceTapeAx/tight/lhs} &\stackrel{\text{(tightening)}}{=}& \tikzfig{traceTapeAx/tight/rhs}
            &
            \tikzfig{traceTapeAx/strength/lhs} &\stackrel{\text{(strength)}}{=}& \tikzfig{traceTapeAx/strength/rhs}
            \\[20pt]
            \tikzfig{traceTapeAx/join/lhs} &\stackrel{\text{(joining)}}{=}& \tikzfig{traceTapeAx/join/rhs}
            &
            \tikzfig{traceTapeAx/vanish/lhs} &\stackrel{\text{(vanishing)}}{=}& \tikzfig{traceTapeAx/vanish/rhs}
            \\[40pt]
            \tikzfig{traceTapeAx/slide/lhs} &\stackrel{\text{(sliding)}}{=}& \tikzfig{traceTapeAx/slide/rhs}
            &
            \tikzfig{traceTapeAx/yank/lhs} &\stackrel{\text{(yanking)}}{=}& \tikzfig{traceTapeAx/yank/rhs}
            \\[20pt]
            \multicolumn{6}{c}{
                \tikzfig{traceTapeAx/uniformity/lhs} = \tikzfig{traceTapeAx/uniformity/rhs} \stackrel{(\text{uniformity})}{\implies} \tikzfig{traceTapeAx/uniformity/TR_lhs} = \tikzfig{traceTapeAx/uniformity/TR_rhs}
            }
          \end{array}
    \]
    \caption{Uniform trace axioms in tape diagrams.}
    \label{fig:trace-axiom-tapes}
\end{figure}

%\marginpar{Alessandro puoi fare una versione grafica tape degli assiomi delle tracce?}

%\ale{DIRE COME SI FA $\trace_{S} \t$ ?}

Observe that (co)monoids and traces are defined for arbitrary monomials $U$, but not for all polynomials $P$. They can easily be defined inductively by means of the coherence axioms for (co)monoids and joining and vanishing for traces: see  
Table \ref{tab:inddefutfb}.


%\ale{AGGIUSTARE E FINIRE QUESTI DUE}
%\begin{lemma}\label{lemma:ut-fb-iso}
%    $\CatTrTape$ and $\UTr(\CatTape)$ are isomorphic as ut-fb categories.
%\end{lemma}
In the same way in which $\CatTape$ is the free $\sort$-sesquistrict fb rig category, $\CatTrTape$ is the free uniformly traced one.
\begin{theorem}\label{thm:freeut-fb}
$\CatTrTape$ is the free sesquistrict ut-fb rig category generated by the monoidal signature $(\sort, \sign)$.
\end{theorem}
One can prove the above theorem by extending the inductive definitions of whiskerings for tapes in Table \ref{tab:producttape} with the cases for traces given in Table \ref{tab:wisktraces} and then extends the proof of \Cref{thm:Tapes is free sesquistrict generated by sigma} by considering this additional inductive case. Hereafter we illustrate a more modular proof that allows to reuse Theorem \ref{thm:Tapes is free sesquistrict generated by sigma} and the free uniform state construction discussed in Section \ref{sec:traced}.

\begin{table}
    \begin{center}
    % \tiny{
        \hfill
  \[ \begin{array}{rcl|rcl}
    \LW U {\trace_V \t } &\defeq& \trace_{UV}{ \LW{U}{\t}} & \RW U {\trace_V \t} &\defeq& \trace_{VU}{\RW{U}\t} \\
    \end{array} 
     \]
      \hfill
      \caption{Extension of the definition of left and right whiskerings in Table \ref{tab:producttape} with the case of trace}\label{tab:wisktraces}
    %    }
    \end{center}
\end{table}


\subsection{Proof of Theorem \ref{thm:freeut-fb}}


The adjunction in \eqref{eq:adjunction-utfb} can be decomposed in the following two adjunctions, where the leftmost is the one in~\eqref{eq:adjunction} and the rightmost is the one given by Corollary \ref{cor:free-uniform-trace-fb}.

\begin{equation}
    \begin{tikzcd}
        \SMC \ar[r,"U_1"] &
        \CAT
        \arrow[r, "F_2"{name=F}, bend left] &
        \FBC
        \arrow[r, "\UTr"{name=H}, bend left] 
        \arrow[l, "U_2"{name=U}, bend left]
        \arrow[phantom, from=F, to=U, "\vdash" rotate=90]&
        \FBUTr
        \arrow[l, "U"{name=G}, bend left]
        \arrow[phantom, from=H, to=G, "\vdash" rotate=90]
    \end{tikzcd}
\end{equation}

\begin{proposition}\label{prop:iso}
For all categories $\Cat{C}$, $\UTr F_2 (\Cat{C})$ and $F_3 (\Cat{C})$ are isomorphic as ut-fb-categories.
\end{proposition}
\begin{proof}
Observe that $U U_2 = U_3$. Since adjoints compose, then $\UTr F_2$ is left-adjoint to $U_3$. By uniqueness of adjoints, $\UTr F_2 (\Cat{C})$ is isomorphic to $F_3 (\Cat{C})$.
\end{proof}
\begin{corollary}
 $\CatTrTape$ and $\UTr(\CatTape)$ are isomorphic as ut-fb categories.
\end{corollary}

The above result suggests that to prove that $\CatTrTape$ is the free sesquistrict ut-fb rig category, one could rather prove that $\UTr(\CatTape)$ is the free one. This can be easily achieved by relying on Theorem \ref{thm:Tapes is free sesquistrict generated by sigma} and Proposition \ref{prop:free-uniform-trace-fb-rig}.

\begin{proposition}\label{prop:tracedtacesutfb}
$\UTr(\CatTape)$ is a $\sort$-sesquistrict ut-fb rig category.
\end{proposition}
\begin{proof}
By Proposition \ref{prop:free-uniform-trace-fb-rig}, $\UTr(\CatTape)$ is a ut-fb rig category. One only needs to show that the inclusion  functor $\sort \to \UTr(\CatTape)$ makes $\UTr(\CatTape)$ a $\sort$-sesquistrict rig category according to Definition \ref{def:sesquistrict rig category}. This means that we have to show that for all $A\in \sort$, $\dl{A}{Q}{R}=  \id{(A\per Q)\piu (A\per R)}$. The latter equivalence holds in $\CatTape$ (see e.g. the end of the proof of Theorem 5.10 in \cite{bonchi2023deconstructing}) and thus it also holds in $\UTr(\CatTape)$. %\marginpar{maybe we should have said before what is $\dl{P}{Q}{R}$ in $\UTr(-)$.}
%    It follows from sesquistrictness of $\CatTape$ and the fact that the left distributor in $\UTr(\CatTape)$ is essentially $\delta^l$ in $\CatTape$.
\end{proof}

\begin{theorem}\label{thm:uniformfree}
    $\UTr(\CatTape)$ is the free sesquistrict ut-fb rig category generated by the monoidal signature $(\sort, \sign)$.
\end{theorem}
\begin{proof}
The obvious interpretation of  $(\sign, \sort)$ into $\UTr(\CatTape)$ is $(\id{\sort}, \tape{\cdot} ; \eta)$ where $\eta$ is the unit of the adjunction provided by Proposition \ref{prop:free-uniform-trace-fb-rig} mapping any tape $\t$ in $\CatTape$ into $\St{\t}{\zero}$.

Now, suppose that $M \to D$ is a $\sort$-sesquistrict ut-fb rig category with an interpretation $(\alpha_\sort, \alpha_\sign)$. 

Since $D$ is, in particular, a fb rig category then by Theorem \ref{thm:Tapes is free sesquistrict generated by sigma}, there exists an $\sort$-sesqustrict fb rig functor $(\alpha,\beta)$ with $\alpha\colon \sort \to M$ and $\beta \colon \CatTape \to D$ such that
\begin{equation}\label{eq:one}
\id{\sort}; \alpha = \alpha_\sort \qquad \text{ and } \qquad \tape{\cdot} ; \beta = \alpha_\sign\text{.}
\end{equation}
Since $D$ is a ut-fb rig category, by the adjunction in Proposition \ref{prop:free-uniform-trace-fb-rig}, there exists a unique ut-fb rig functor $\beta^\sharp \colon \UTr(\CatTape) \to D$ such that 
\begin{equation}\label{eq:two}
\eta ; \beta^\sharp = \beta
\end{equation}
From \eqref{eq:one} and \eqref{eq:two}, it immediately follows that $\tape{\cdot}; \eta ; \beta^\sharp = \tape{\cdot}; \beta = \alpha_\sign$. In summary, we have a sesquistrict ut-fb rig functor
$(\alpha\colon \sort \to M, \beta^\sharp \colon \UTr(\CatTape) \to D)$ such that 
\begin{equation}%\label{eq:one}
\id{\sort}; \alpha = \alpha_\sort \qquad \text{ and } \qquad \tape{\cdot} ; \eta ; \beta^\sharp = \alpha_\sign\text{.}
\end{equation}
\end{proof}

%To conclude the proof of Theorem \ref{thm:freeut-fb} one has just to show that 

Thanks to the isomorphism in Proposition \ref{prop:iso}, $\CatTrTape$ inherits the rig structures from $\UTr(\CatTape)$.
Let $H \colon \UTr(\CatTape) \to \CatTrTape$ and $K \colon \CatTrTape \to \UTr(\CatTape)$  be the functors witnessing the isomorphism. Then, one can define $\per$, distributors and symmetries on $\CatTrTape$ as follows:
\begin{equation}\label{eq:rigstruct}
        \t_1 \per \t_2 \defeq H(K(\t_1) \per K(\t_2)) \qquad \dl{P}{Q}{R} \defeq H(\dl{K(P)}{K(Q)}{K(R)} \mid \zero ) \qquad \symmt{P}{Q} \defeq H(\symmt{K(P)}{K(Q)}\mid \zero )
\end{equation}
The above definitions make $\CatTrTape$ and $\UTr(\CatTape)$ isomorphic as ut-fb rig categories. By Theorem \ref{thm:uniformfree}, it follows that  $\CatTrTape$ is the free sesquistrict ut-fb rig category.

\begin{remark}
Observe that the rig structure of $\CatTrTape$ in \eqref{eq:rigstruct} is defined differently than using the whiskerings in Tables \ref{tab:producttape} and \ref{tab:wisktraces} and symmetries and distributors in Table \ref{table:def dl symmt}. 
Since the definition in \eqref{eq:rigstruct} passes through the isomorphism, it is a bit unhandy. The reader can safely use those in Tables \ref{table:def dl symmt}, \ref{tab:producttape} and \ref{tab:wisktraces}, since the two constructions coincide: see Appendix \ref{app:rigtrTape} for a detailed proof.
\end{remark}

